Asymptotic behavior of the Arrow-Hurwicz differential system with Tikhonov regularization

In a real Hilbert space setting, we investigate the asymptotic behavior of the solutions of the classical Arrow-Hurwicz differential system combined with Tikhonov regularizing terms. Under some newly proposed conditions on the Tikhonov terms involved, we show that the solutions of the regularized Arrow-Hurwicz differential system strongly converge toward the element of least norm within its set of zeros. Moreover, we provide fast asymptotic decay rate estimates for the so-called primal-dual gap function and the norm of the solutions' velocity. If, in addition, the Tikhonov regularizing terms are decreasing, we provide some refined estimates in the sense of an exponentially weighted moving average. Under the additional assumption that the governing operator of the Arrow-Hurwicz differential system satisfies a reverse Lipschitz condition, we further provide a fast rate of strong convergence of the solutions toward the unique zero. We conclude our study by deriving the corresponding decay rate estimates with respect to the so-called viscosity curve. Numerical experiments illustrate our theoretical findings.

==> matlab/fig1b.tex <==
0.0100000000000000	5000.50000000000
0.0112590384703905	3944.67129960162
0.0125180769407810	3191.08370892326
0.0137771154111715	2634.49174398318
0.0150361538815620	2211.76972076691
0.0162951923519525	1883.19133852943
0.0175542308223430	1622.74329021931
0.0188132692927335	1412.81366939855
0.0200723077631240	1241.13441178635
0.0218134441469326	1050.90860027320
0.0235545805307411	901.286118552186
0.0252957169145497	781.482842522265
0.0270368532983583	684.070941440933
0.0295181432065920	573.898856602652
0.0319994331148256	488.347379828950
0.0344807230230593	420.591706430668
0.0369620129312930	366.017796657854
0.0405572013330861	304.002722184417
0.0441523897348793	256.510414158142
0.0477475781366724	219.336412891831
0.0513427665384656	189.694569774501
0.0566747420772888	155.680538303391
0.0620067176161121	130.057663207265
0.0673386931549353	110.276777229123
0.0726706686937585	94.6880381991360
0.0809070434834143	76.3907485298986
0.0891434182730702	62.9266865079043
0.0973797930627260	52.7321816306234
0.105616167852382	44.8283361969769
0.119428450217403	35.0588634835721
0.133240732582423	28.1669230970328
0.147053014947444	23.1241389615996
0.160865297312465	19.3236293824326
0.178019219732123	15.7790061137003
0.195173142151780	13.1272370110059
0.212327064571438	11.0918177204053
0.229480986991096	9.49554754519011
0.248483981448880	8.09872473567395
0.267486975906665	6.98888917064432
0.286489970364450	6.09248668972354
0.305492964822234	5.35810233332159
0.326939596021466	4.67819574915091
0.348386227220698	4.11994559451596
0.369832858419931	3.65596850654274
0.391279489619163	3.26617359612990
0.415086736184634	2.90225602817173
0.438893982750104	2.59593721312693
0.462701229315575	2.33567347119673
0.486508475881046	2.11267458720915
0.512579838010910	1.90322614675942
0.538651200140773	1.72344796220965
0.564722562270636	1.56798952274095
0.590793924400500	1.43265423918248
0.619005972967117	1.30503979644808
0.647218021533734	1.19374684271380
0.675430070100351	1.09610624626740
0.703642118666968	1.00997302670642
0.733851831073851	0.928531561857662
0.764061543480734	0.856557961432387
0.794271255887618	0.792639560067382
0.824480968294501	0.735617683795511
0.856524960901709	0.681605972637692
0.888568953508918	0.633331615496479
0.920612946116126	0.590009874773471
0.952656938723335	0.550985744244171
0.986351384409508	0.513984612517022
1.02004583009568	0.480589266520974
1.05374027578186	0.450345965421178
1.08743472146803	0.422870162546683
1.12257805195627	0.396807927588805
1.15772138244452	0.373082884049988
1.19286471293276	0.351423704694005
1.22800804342100	0.331597321422794
1.26438736782175	0.312790199200549
1.30076669222249	0.295538875231913
1.33714601662323	0.279676364676525
1.37352534102397	0.265057493447149
1.41092618586320	0.251191445458729
1.44832703070242	0.238385676020219
1.48572787554165	0.226534781627445
1.52312872038087	0.215546129166005
1.56134640367475	0.205123254104381
1.59956408696864	0.195438506751284
1.63778177026252	0.186423805915212
1.67599945355640	0.178018731006762
1.71484969660907	0.170043999057718
1.75369993966175	0.162593376057454
1.79255018271442	0.155621927662851
1.83140042576709	0.149089421037840
1.87072709840390	0.142886947187631
1.91005377104070	0.137063631289076
1.94938044367751	0.131589193932421
1.98870711631432	0.126436305691307
2.02838611226531	0.121538025234845
2.06806510821629	0.116918976276025
2.10774410416728	0.112558337727808
2.14742310011826	0.108437180201156
2.18736258820969	0.104513375203680
2.22730207630111	0.100798756335599
2.26724156439253	0.0972787202323677
2.30718105248396	0.0939399029100804
2.34731915635702	0.0907547045969493
2.38745726023007	0.0877288033286546
2.42759536410313	0.0848517570805401
2.46773346797619	0.0821139531196186
2.50803462769329	0.0794962014669401
2.54833578741038	0.0770016638575658
2.58863694712748	0.0746227326755267
2.62893810684458	0.0723523666994642
2.66938915757544	0.0701761681170566
2.70984020830630	0.0680966975199682
2.75029125903716	0.0661083112894891
2.79074230976801	0.0642057603850334
2.83134895097666	0.0623773097021016
2.87195559218530	0.0606258686444591
2.91256223339394	0.0589471772772617
2.95316887460259	0.0573372558180424
2.99395288397237	0.0557857802611892
3.03473689334216	0.0542964361929200
3.07552090271194	0.0528659541819755
3.11630491208173	0.0514912673440794
3.15730225154799	0.0501627244361778
3.19829959101425	0.0488849446444502
3.23929693048051	0.0476553783873200
3.28029426994677	0.0464716250716069
3.32155413519608	0.0453242643087710
3.36281400044539	0.0442188778756102
3.40407386569470	0.0431534468020178
3.44533373094400	0.0421260635279355
3.48691858677239	0.0411272638189555
3.52850344260078	0.0401635708486607
3.57008829842917	0.0392333619028823
3.61167315425756	0.0383350989000004
3.65365985811192	0.0374590882406033
3.69564656196628	0.0366127664701681
3.73763326582065	0.0357948102839874
3.77961996967501	0.0350039616534579
3.82210221583512	0.0342301523480318
3.86458446199523	0.0334817226973272
3.90706670815534	0.0327575779212236
3.94954895431544	0.0320566743404758
3.99264150344042	0.0313684304436280
4.03573405256539	0.0307021167046636
4.07882660169036	0.0300568141448049
4.12191915081533	0.0294316443863163
4.16576473103018	0.0288153527010108
4.20961031124503	0.0282182190830774
4.25345589145988	0.0276394604223484
4.29730147167473	0.0270783263602683
4.34208205652409	0.0265226770404210
4.38686264137346	0.0259839581760051
4.43164322622282	0.0254614915811740
4.47642381107218	0.0249546259190175
4.52237971564009	0.0244500274612472
4.56833562020800	0.0239605820606174
4.61429152477591	0.0234856916706753
4.66024742934382	0.0230247806554096
4.70771174380114	0.0225628346685444
4.75517605825846	0.0221146540635183
4.80264037271578	0.0216796999639957
4.85010468717310	0.0212574526082887
4.89744976257724	0.0208484322505051
4.94479483798138	0.0204511058233951
4.99213991338552	0.0200650340075284
5.03948498878966	0.0196897918459209
5.08636308744273	0.0193285226918726
5.13324118609581	0.0189771071895596
5.18011928474888	0.0186351920472175
5.22699738340195	0.0183024345737893
5.27357838501376	0.0179805330910367
5.32015938662558	0.0176670509878311
5.36674038823739	0.0173616986915081
5.41332138984921	0.0170641946327835
5.45976847819635	0.0167750922004807
5.50621556654349	0.0164932759998159
5.55266265489063	0.0162185044766378
5.59910974323777	0.0159505422468360
5.64558241876024	0.0156890215302838
5.69205509428270	0.0154338811477820
5.73852776980517	0.0151849162779898
5.78500044532764	0.0149419269498079
5.83166690899266	0.0147037440710079
5.87833337265768	0.0144712121700113
5.92499983632269	0.0142441547799440
5.97166629998771	0.0140223993201189
6.01871655904510	0.0138040194695585
6.06576681810250	0.0135907024836508
6.11281707715989	0.0133822938226716
6.15986733621728	0.0131786421225272
6.20753009502752	0.0129770407303492
6.25519285383776	0.0127800310649353
6.30285561264800	0.0125874753868802
6.35051837145825	0.0123992386082641
6.39908671418941	0.0122117338752193
6.44765505692057	0.0120284513097140
6.49622339965174	0.0118492656519953
6.54479174238290	0.0116740539129958
6.59477427942936	0.0114977651575498
6.64475681647582	0.0113254405551117
6.69473935352228	0.0111569626145700
6.74472189056874	0.0109922158700003
6.79435030314736	0.0108322188195215
6.84397871572597	0.0106756905865938
6.89360712830458	0.0105225319759092
6.94323554088320	0.0103726453776574
6.99213297011201	0.0102280755277955
7.04103039934083	0.0100865078918935
7.08992782856965	0.00994786017782335
7.13882525779847	0.00981205130428236
7.18736732322589	0.00967996064645946
7.23590938865331	0.00955052010217954
7.28445145408073	0.00942365944597599
7.33299351950815	0.00929930940766764
7.38150321897300	0.00917748397805744
7.43001291843784	0.00905803750812302
7.47852261790269	0.00894090860088767
7.52703231736754	0.00882603663371484
7.57580331165659	0.00871276234397578
7.62457430594563	0.00860165536974536
7.67334530023468	0.00849266087071591
7.72211629452373	0.00838572464918611
7.77144705621219	0.00827960179360087
7.82077781790065	0.00817548133074495
7.87010857958912	0.00807331326014013
7.91943934127758	0.00797304812727367
7.96966620873211	0.00787286771627314
8.01989307618664	0.00777456421805121
8.07011994364117	0.00767809105941703
8.12034681109570	0.00758340214427102
8.17188862971250	0.00748804284769212
8.22343044832929	0.00739447159680262
8.27497226694608	0.00730264394222595
8.32651408556287	0.00721251586892815
8.37995066555843	0.00712082398115802
8.43338724555398	0.00703087023407302
8.48682382554954	0.00694261088181654
8.54026040554509	0.00685600260280151
8.59264630622872	0.00677266017567578
8.64503220691234	0.00669082882803582
8.69741810759597	0.00661047217167699
8.74980400827959	0.00653155410963610
8.80130195951982	0.00645534261246743
8.85279991076004	0.00638045775491364
8.90429786200027	0.00630686885553397
8.95579581324049	0.00623454542854631
9.00691883967619	0.00616397153073661
9.05804186611189	0.00609458966788920
9.10916489254759	0.00602637307694607
9.16028791898329	0.00595929512932457
9.21145411122912	0.00589327517218494
9.26262030347494	0.00582834670353802
9.31378649572077	0.00576448572044342
9.36495268796660	0.00570166831408650
9.41654794015576	0.00563935771555308
9.46814319234492	0.00557806343102158
9.51973844453408	0.00551776338970860
9.57133369672324	0.00545843558958134
9.62392663286122	0.00539893947314953
9.67651956899920	0.00534041127378819
9.72911250513718	0.00528282999358563
9.78170544127516	0.00522617469483339
9.83584912150179	0.00516879518731581
9.88999280172842	0.00511235598034882
9.94413648195504	0.00505683647771413
9.99828016218167	0.00500221615441692
10.0540781056737	0.00494684724740743
10.1098760491657	0.00489239311905115
10.1656739926577	0.00483883350623003
10.2214719361497	0.00478614824348075
10.2756340627963	0.00473582587474865
10.3297961894429	0.00468629343416545
10.3839583160894	0.00463753430379017
10.4381204427360	0.00458953190961384
10.4913006965245	0.00454312089914273
10.5444809503131	0.00449741070717235
10.5976612041017	0.00445238714666398
10.6508414578903	0.00440803605096147
10.7036286794831	0.00436466457263176
10.7564159010759	0.00432193041070450
10.8092031226688	0.00427982099711247
10.8619903442616	0.00423832377815176
10.9148514055899	0.00419737011335063
10.9677124669181	0.00415700750394536
11.0205735282463	0.00411722448139399
11.0734345895746	0.00407800959709565
11.1268048985060	0.00403898232059946
11.1801752074375	0.00400051294620677
11.2335455163689	0.00396259072253743
11.2869158253004	0.00392520493480531
11.3412675119695	0.00388767260137683
11.3956191986386	0.00385067636184257
11.4499708853078	0.00381420585272167
11.5043225719769	0.00377825077847651
11.5602445818107	0.00374178472598975
11.6161665916445	0.00370584443740147
11.6720886014783	0.00367041959285272
11.7280106113121	0.00363549999673406
11.7854922362233	0.00360012314334022
11.8429738611344	0.00356526056445296
11.9004554860456	0.00353090201070694
11.9579371109568	0.00349703742851589
12.0138246466191	0.00346457684575092
12.0697121822814	0.00343256646669423
12.1255997179437	0.00340099773466423
12.1814872536060	0.00336986224602603
12.2364081740881	0.00333967985246996
12.2913290945701	0.00330990143164693
12.3462500150521	0.00328051956665588
12.4011709355341	0.00325152697700822
12.4557093948871	0.00322311488964809
12.5102478542401	0.00319507384364924
12.5647863135931	0.00316739717597629
12.6193247729461	0.00314007836100562
12.6739738559100	0.00311305705365928
12.7286229388739	0.00308638329203290
12.7832720218378	0.00306005090541425
12.8379211048018	0.00303405387471339
12.8932201372012	0.00300808338171137
12.9485191696007	0.00298244516861913
13.0038182020002	0.00295713333242350
13.0591172343996	0.00293214215209627
13.1157877654014	0.00290685838091852
13.1724582964031	0.00288190050953283
13.2291288274048	0.00285726265261608
13.2857993584066	0.00283293916556613
13.3446243075368	0.00280801804768573
13.4034492566669	0.00278342464518251
13.4622742057971	0.00275915283851063
13.5210991549273	0.00273519685404774
13.5783218161257	0.00271219157657594
13.6355444773240	0.00268947558193735
13.6927671385223	0.00266704371492453
13.7499897997207	0.00264489109562575
13.8061231584122	0.00262342732154392
13.8622565171036	0.00260222398843622
13.9183898757951	0.00258127661871558
13.9745232344866	0.00256058096938392
14.0302633175361	0.00254027566908896
14.0860034005856	0.00252021115081618
14.1417434836351	0.00250038335886549
14.1974835666846	0.00248078845913921
14.2533926250767	0.00246136468272806
14.3093016834687	0.00244216833922648
14.3652107418608	0.00242319562690246
14.4211198002529	0.00240444297151072
14.4777370024593	0.00238567381362149
14.5343542046657	0.00236712377377729
14.5909714068721	0.00234878917107433
14.6475886090785	0.00233066657663627
14.7055282387007	0.00231233704066705
14.7634678683228	0.00229422310571979
14.8214074979450	0.00227632107885571
14.8793471275672	0.00225862756977020
14.9394338470089	0.00224049549797298
14.9995205664506	0.00222258114919483
15.0596072858923	0.00220488064559174
15.1196940053340	0.00218739051024291
15.1785299451618	0.00217046548456104
15.2373658849896	0.00215373635569794
15.2962018248174	0.00213719976875737
15.3550377646452	0.00212085270107372
15.4126282162481	0.00210503277020975
15.4702186678511	0.00208938937492245
15.5278091194541	0.00207391960859593
15.5853995710570	0.00205862083865421
15.6425138397232	0.00204361524360155
15.6996281083894	0.00202877329154948
15.7567423770555	0.00201409234428224
15.8138566457217	0.00199957001525543
15.8711953652715	0.00198514812839595
15.9285340848213	0.00197088187592250
15.9858728043710	0.00195676875821734
16.0432115239208	0.00194280653153804
16.1014495158645	0.00192877784021031
16.1596875078082	0.00191490072574281
16.2179254997519	0.00190117272094001
16.2761634916956	0.00188759164477035
16.3359700634670	0.00187379579075004
16.3957766352384	0.00186015082334553
16.4555832070098	0.00184665420944554
16.5153897787812	0.00183330376483042
16.5772595565287	0.00181964469175188
16.6391293342762	0.00180613792250176
16.7009991120237	0.00179278078294422
16.7628688897712	0.00177957104740598
16.8226291025295	0.00176695005188239
16.8823893152878	0.00175446302381149
16.9421495280461	0.00174210774876124
17.0019097408044	0.00172988235151102
17.0604737135166	0.00171802624886592
17.1190376862287	0.00170629177070457
17.1776016589408	0.00169467698024360
17.2361656316529	0.00168318022834525
17.2943437987857	0.00167187479139787
17.3525219659184	0.00166068301898313
17.4107001330511	0.00164960312997289
17.4688783001839	0.00163863361532706
17.5273181214793	0.00162772467872064
17.5857579427747	0.00161692445791303
17.6441977640701	0.00160623124669227
17.7026375853655	0.00159564362002050
17.7619748377587	0.00158500028655658
17.8213120901519	0.00157446323559969
17.8806493425450	0.00156403076622485
17.9399865949382	0.00155370149312118
18.0009772089185	0.00154319084457824
18.0619678228989	0.00153278665324453
18.1229584368792	0.00152248714300556
18.1839490508595	0.00151229092520448
18.2467391781493	0.00150190070970775
18.3095293054391	0.00149161738645866
18.3723194327289	0.00148143908504637
18.4351095600186	0.00147136441374252
18.4958890311180	0.00146171015749405
18.5566685022173	0.00145215075545967
18.6174479733167	0.00144268464325990
18.6782274444160	0.00143331063233978
18.7378730347315	0.00142420022971582
18.7975186250471	0.00141517654109450
18.8571642153626	0.00140623818547500
18.9168098056781	0.00139738410826793
18.9761161336685	0.00138866321124121
19.0354224616590	0.00138002381894025
19.0947287896494	0.00137146464908488
19.1540351176398	0.00136298473155938
19.2137174724110	0.00135453036360346
19.2733998271821	0.00134615453302826
19.3330821819533	0.00133785599301243
19.3927645367245	0.00132963382230173
19.4536313109237	0.00132132648148484
19.5144980851229	0.00131309687932571
19.5753648593222	0.00130494373902435
19.6362316335214	0.00129686615663319
19.6991702047529	0.00128859246158543
19.7621087759845	0.00128039783567625
19.8250473472160	0.00127228089649191
19.8879859184476	0.00126424073052055
19.9504675490644	0.00125633434270046
20.0129491796813	0.00124850202611410
20.0754308102981	0.00124074250421898
20.1379124409149	0.00123305494096837
20.1988318485020	0.00122562840529288
20.2597512560891	0.00121826887567039
20.3206706636762	0.00121097525313789
20.3815900712632	0.00120374680272417
20.4418628007192	0.00119665878758685
20.5021355301751	0.00118963329731805
20.5624082596310	0.00118266932818341
20.6226809890869	0.00117576620968585
20.6830648171870	0.00116891098022667
20.7434486452870	0.00116211563161384
20.8038324733871	0.00115537920001263
20.8642163014871	0.00114870105451071
20.9254176891409	0.00114199158795507
20.9866190767946	0.00113534083964053
21.0478204644484	0.00112874783956715
21.1090218521021	0.00112221197810324
21.1718545315804	0.00111556099995620
21.2346872110587	0.00110896909070858
21.2975198905370	0.00110243522052311
21.3603525700153	0.00109595878532005
21.4250495998080	0.00108934989366922
21.4897466296008	0.00108280073267420
21.5544436593936	0.00107631019267686
21.6191406891863	0.00106987767584195
21.6817036315996	0.00106371229999566
21.7442665740128	0.00105760017133412
21.8068295164261	0.00105154036883367
21.8693924588393	0.00104553237018345
21.9308388102019	0.00103968179683206
21.9922851615645	0.00103388028850535
22.0537315129272	0.00102812702787199
22.1151778642898	0.00102242154345408
22.1764705511298	0.00101677770582534
22.2377632379697	0.00101118056134205
22.2990559248097	0.00100562933575260
22.3603486116497	0.00100012358908801
22.4223000336916	0.000994604683326297
22.4842514557336	0.000989131426079884
22.5462028777755	0.000983703041751766
22.6081542998175	0.000978319108954857
22.6715496881498	0.000972855528761830
22.7349450764822	0.000967437690177262
22.7983404648145	0.000962064773275330
22.8617358531469	0.000956736366751893
22.9276086030674	0.000951246753905730
22.9934813529880	0.000945804372331043
23.0593541029086	0.000940408292861415
23.1252268528292	0.000935058108977685
23.1892682653520	0.000929900603091203
23.2533096778747	0.000924785750276794
23.3173510903975	0.000919712762480886
23.3813925029203	0.000914681276599845
23.4439303515084	0.000909807894290839
23.5064682000966	0.000904973441746689
23.5690060486847	0.000900177235926576
23.6315438972729	0.000895418950308774
23.6935838954000	0.000890735928440508
23.7556238935271	0.000886089628532988
23.8176638916543	0.000881479415689211
23.8797038897814	0.000876904988570883
23.9420528805491	0.000872343755304665
24.0044018713168	0.000867818096915628
24.0667508620844	0.000863327388440118
24.1290998528521	0.000858871346183561
24.1925523682960	0.000854371970551264
24.2560048837398	0.000849907942908798
24.3194573991837	0.000845478612238247
24.3829099146275	0.000841083707878391
24.4484444382408	0.000836580714806188
24.5139789618541	0.000832113883289980
24.5795134854674	0.000827682486975911
24.6450480090807	0.000823286267213712
24.7108250011305	0.000818909187739493
24.7766019931802	0.000814567017127825
24.8423789852300	0.000810259042423520
24.9081559772797	0.000805985024687565
24.9720195866552	0.000801867870737873
25.0358831960306	0.000797782262404817
25.0997468054060	0.000793727598150138
25.1636104147814	0.000789703661074997
25.2265955481551	0.000785765193085592
25.2895806815287	0.000781856186509219
25.3525658149024	0.000777976095428061
25.4155509482761	0.000774124720718393
25.4785556713374	0.000770300895918936
25.5415603943987	0.000766505402638980
25.6045651174600	0.000762737712165868
25.6675698405213	0.000758997639588374
25.7315234913094	0.000755229512392781
25.7954771420975	0.000751489449304588
25.8594307928856	0.000747776902378413
25.9233844436737	0.000744091699263842
25.9892426850350	0.000740325387739086
26.0551009263963	0.000736587681381064
26.1209591677576	0.000732877971864014
26.1868174091189	0.000729196101611164
26.2535502444464	0.000725493844555062
26.3202830797740	0.000721819796592374
26.3870159151016	0.000718173330816295
26.4537487504291	0.000714554305431342
26.5184351348136	0.000711072580470677
26.5831215191980	0.000707616311573103
26.6478079035824	0.000704184975422583
26.7124942879669	0.000700778438021178
26.7762428831831	0.000697445639240068
26.8399914783994	0.000694136623072812
26.9037400736156	0.000690850916412762
26.9674886688319	0.000687588394610841
27.0312432274322	0.000684348836212230
27.0949977860326	0.000681132180559880
27.1587523446329	0.000677937968983940
27.2225069032333	0.000674766086454609
27.2871135974660	0.000671574677133371
27.3517202916987	0.000668405920235466
27.4163269859314	0.000665259342076746
27.4809336801641	0.000662134838490750
27.5473600151609	0.000658945467555700
27.6137863501576	0.000655779157364608
27.6802126851544	0.000652635382528856
27.7466390201512	0.000649514054315037
27.8144911660441	0.000646349068617502
27.8823433119370	0.000643207238817722
27.9501954578299	0.000640087999265664
28.0180476037228	0.000636991277971274
28.0836710412897	0.000634017877522497
28.1492944788567	0.000631065312196802
28.2149179164237	0.000628133116557111
28.2805413539907	0.000625221215371340
28.3451053878376	0.000622376265752736
28.4096694216846	0.000619550747911334
28.4742334555315	0.000616744244564291
28.5387974893785	0.000613956683636463
28.6034183056205	0.000611185761179683
28.6680391218626	0.000608433611740842
28.7326599381047	0.000605699828172090
28.7972807543468	0.000602984345322166
28.8628316080457	0.000600248609904222
28.9283824617446	0.000597531509693122
28.9939333154435	0.000594832619982389
29.0594841691424	0.000592151886139045
29.1269556326181	0.000589411732017357
29.1944270960939	0.000586690620876591
29.2618985595696	0.000583988075395679
29.3293700230453	0.000581304058672497
29.3979909106086	0.000578593532637468
29.4666117981718	0.000575901991740587
29.5352326857351	0.000573228929922569
29.6038535732983	0.000570574325618663
29.6701727865302	0.000568026517773277
29.7364919997621	0.000565495795391825
29.8028112129939	0.000562981744165128
29.8691304262258	0.000560484332382406
29.9343704267019	0.000558043964255457
29.9996104271780	0.000555619551904440
30.0648504276541	0.000553210723672015
30.1300904281302	0.000550817447269064
30.1952858095128	0.000548441495338566
30.2604811908953	0.000546080934081557
30.3256765722779	0.000543735402332542
30.3908719536605	0.000541404872701999
30.4569332436822	0.000539058850461172
30.5229945337039	0.000536728096888010
30.5890558237256	0.000534412235185993
30.6551171137473	0.000532111247997053
30.7230813828530	0.000529759689722905
30.7910456519586	0.000527423745024012
30.8590099210643	0.000525102988304724
30.9269741901699	0.000522797421004504
30.9964305818134	0.000520457166794698
31.0658869734568	0.000518132656206546
31.1353433651002	0.000515823423935157
31.2047997567437	0.000513529490059502
31.2718985486150	0.000511328195825238
31.3389973404864	0.000509141078357352
31.4060961323577	0.000506967758128000
31.4731949242290	0.000504808239267319
31.5391489416833	0.000502699209175436
31.6051029591375	0.000500603415733565
31.6710569765918	0.000498520519732985
31.7370109940461	0.000496450521231144
31.8029038201020	0.000494395499659854
31.8687966461580	0.000492353257548664
31.9346894722139	0.000490323464936474
32.0005822982699	0.000488306125202958
32.0674470725521	0.000486271942194086
32.1343118468343	0.000484250491978463
32.2011766211165	0.000482241426420602
32.2680413953987	0.000480244759406572
32.3369742812759	0.000478199532148552
32.4059071671532	0.000476167397135738
32.4748400530305	0.000474147954778965
32.5437729389077	0.000472141240324257
32.6132976261725	0.000470130449120420
32.6828223134373	0.000468132532142808
32.7523470007020	0.000466147080603460
32.8218716879668	0.000464174138938346
32.8892575400122	0.000462274080637386
32.9566433920577	0.000460385711665481
33.0240292441032	0.000458508693523791
33.0914150961486	0.000456643053607610
33.1579074063846	0.000454813509739481
33.2243997166205	0.000452994981501292
33.2908920268565	0.000451187160423800
33.3573843370924	0.000449390069378383
33.4240362992290	0.000447599623446614
33.4906882613656	0.000445819898438528
33.5573402235022	0.000444050588772848
33.6239921856388	0.000442291720814841
33.6917838285149	0.000440513690837555
33.7595754713910	0.000438746405782654
33.8273671142671	0.000436989538468289
33.8951587571432	0.000435243126676616
33.9652790260747	0.000433447965722754
34.0353992950061	0.000431663940148847
34.1055195639376	0.000429890666061197
34.1756398328691	0.000428128206029611
34.2453776041807	0.000426386361139817
34.3151153754923	0.000424655174192226
34.3848531468039	0.000422934280581266
34.4545909181155	0.000421223740547098
34.5223782426370	0.000419571213227932
34.5901655671585	0.000417928433407219
34.6579528916800	0.000416295094976037
34.7257402162014	0.000414671241183744
34.7928996323729	0.000413071992069267
34.8600590485443	0.000411482015863410
34.9272184647158	0.000409901027474434
34.9943778808873	0.000408329066461466
35.0619929504487	0.000406755762377858
35.1296080200101	0.000405191573361116
35.1972230895715	0.000403636209734988
35.2648381591328	0.000402089716283918
35.3339326818891	0.000400518768438680
35.4030272046454	0.000398957052326706
35.4721217274016	0.000397404248627885
35.5412162501579	0.000395860416961835
35.6131113972494	0.000394263802904929
35.6850065443410	0.000392676880569369
35.7569016914325	0.000391099260589677
35.8287968385241	0.000389531035079393
35.8985499225384	0.000388018808789592
35.9683030065528	0.000386515414918328
36.0380560905672	0.000385020530342471
36.1078091745816	0.000383534223937991
36.1758899819743	0.000382092063772421
36.2439707893671	0.000380658060040931
36.3120515967598	0.000379231935234221
36.3801324041526	0.000377813743564221
36.4478115126495	0.000376411993425935
36.5154906211464	0.000375018065538626
36.5831697296433	0.000373631696167736
36.6508488381403	0.000372252937287520
36.7191711629321	0.000370869002982110
36.7874934877239	0.000369492808561095
36.8558158125157	0.000368124081227964
36.9241381373075	0.000366762879677273
36.9942096873564	0.000365374876875228
37.0642812374052	0.000363994779165348
37.1343527874540	0.000362622278436603
37.2044243375029	0.000361257451394766
37.2770714990837	0.000359850842848341
37.3497186606646	0.000358452481406887
37.4223658222454	0.000357061996954503
37.4950129838262	0.000355679497378992
37.5648860036314	0.000354357622613040
37.6347590234365	0.000353043141572372
37.7046320432417	0.000351735761697695
37.7745050630469	0.000350435559607160
37.8429849056960	0.000349168483528598
37.9114647483452	0.000347908300955260
37.9799445909944	0.000346654754793026
38.0484244336436	0.000345407909203789
38.1167683734507	0.000344170432889092
38.1851123132578	0.000342939627619368
38.2534562530649	0.000341715243439246
38.3218001928720	0.000340497344086485
38.3911454818990	0.000339268447536238
38.4604907709259	0.000338046226398862
38.5298360599529	0.000336830414233034
38.5991813489799	0.000335621084646421
38.6707549934430	0.000334379944209140
38.7423286379060	0.000333145715465202
38.8139022823690	0.000331918085740245
38.8854759268321	0.000330697152689576
38.9573395690528	0.000329478297998173
39.0292032112736	0.000328266209108103
39.1010668534944	0.000327060571664625
39.1729304957152	0.000325861487013733
39.2426006365928	0.000324705527004285
39.3122707774704	0.000323555740241388
39.3819409183480	0.000322411867216365
39.4516110592256	0.000321273986019730
39.5204531079888	0.000320155741247069
39.5892951567520	0.000319043355247820
39.6581372055153	0.000317936589460545
39.7269792542785	0.000316835514525082
39.7961453702529	0.000315735203012438
39.8653114862273	0.000314640644036738
39.9344776022017	0.000313551596788400
40.0036437181761	0.000312468135037028
40.0742469817186	0.000311368151483725
40.1448502452611	0.000310273999577850
40.2154535088036	0.000309185413471133
40.2860567723460	0.000308102480951617
40.3595268224031	0.000306981854942171
40.4329968724601	0.000305867371874325
40.5064669225171	0.000304758704175307
40.5799369725741	0.000303655972624438
40.6513675007179	0.000302589842624593
40.7227980288617	0.000301529351622859
40.7942285570055	0.000300474225261634
40.8656590851494	0.000299424559860985
40.9354139422374	0.000298405036304985
41.0051687993254	0.000297390740661241
41.0749236564134	0.000296381437089289
41.1446785135014	0.000295377204926631
41.2141846577893	0.000294381817586622
41.2836908020773	0.000293391481851544
41.3531969463653	0.000292405970331659
41.4227030906532	0.000291425360026894
41.4930789169469	0.000290437695152979
41.5634547432405	0.000289455072564948
41.6338305695342	0.000288477252114057
41.7042063958279	0.000287504318861614
41.7766738644670	0.000286507825639414
41.8491413331062	0.000285516538257547
41.9216088017454	0.000284530177366390
41.9940762703846	0.000283548849849011
42.0676270896293	0.000282558287332805
42.1411779088741	0.000281572942461145
42.2147287281188	0.000280592515848266
42.2882795473636	0.000279617126900581
42.3592970394703	0.000278680392252061
42.4303145315771	0.000277748386416420
42.5013320236838	0.000276820868222256
42.5723495157906	0.000275897928640824
42.6423081717146	0.000274993456183925
42.7122668276387	0.000274093450938950
42.7822254835628	0.000273197694840212
42.8521841394869	0.000272306268693436
42.9223311803881	0.000271417005209905
42.9924782212893	0.000270532117359883
43.0626252621906	0.000269651386902585
43.1327723030918	0.000268774896294626
43.2042637505405	0.000267886196862802
43.2757551979892	0.000267001926678525
43.3472466454379	0.000266121845908312
43.4187380928867	0.000265246049845737
43.4930174384355	0.000264340908367917
43.5672967839843	0.000263440426478901
43.6415761295332	0.000262544309543165
43.7158554750820	0.000261652684113746
43.7886851215017	0.000260783115288542
43.8615147679214	0.000259917904559293
43.9343444143411	0.000259056792743077
44.0071740607608	0.000258199888872058
44.0780890043289	0.000257369808740222
44.1490039478970	0.000256543751141776
44.2199188914650	0.000255721496879656
44.2908338350331	0.000254903135059339
44.3612464402611	0.000254094641821020
44.4316590454890	0.000253290013668837
44.5020716507170	0.000252489043097818
44.5724842559449	0.000251691814378756
44.6436666325296	0.000250889891906378
44.7148490091142	0.000250091821447461
44.7860313856988	0.000249297385151224
44.8572137622834	0.000248506674184367
44.9304409819765	0.000247697379295255
45.0036682016695	0.000246892060329528
45.0768954213625	0.000246090464316396
45.1501226410556	0.000245292703101863
45.2247367648061	0.000244484059114463
45.2993508885565	0.000243679438561799
45.3739650123070	0.000242878563431053
45.4485791360575	0.000242081561146936
45.5206102726895	0.000241316098908206
45.5926414093215	0.000240554287183404
45.6646725459534	0.000239795902525341
45.7367036825854	0.000239041043164477
45.8076682830009	0.000238301036330600
45.8786328834164	0.000237564483830479
45.9495974838319	0.000236831183548902
46.0205620842474	0.000236101223125137
46.0917592672627	0.000235372441391436
46.1629564502780	0.000234647052122669
46.2341536332932	0.000233924852205376
46.3053508163085	0.000233205930933057
46.3779951965189	0.000232476002686868
46.4506395767293	0.000231749521477839
46.5232839569396	0.000231026262252607
46.5959283371500	0.000230306327698194
46.6715633469138	0.000229560557804317
46.7471983566776	0.000228818435113175
46.8228333664415	0.000228079679052745
46.8984683762053	0.000227344425450286
46.9719520694971	0.000226633728756251
47.0454357627890	0.000225926385410162
47.1189194560809	0.000225222161613473
47.1924031493727	0.000224521167346541
47.2641650684056	0.000223839955919092
47.3359269874386	0.000223161862707134
47.4076889064715	0.000222486686823271
47.4794508255044	0.000221814520525371
47.5510064906415	0.000221147498648485
47.6225621557785	0.000220483502925956
47.6941178209155	0.000219822338453892
47.7656734860526	0.000219164095053630
47.8382453721548	0.000218499706224480
47.9108172582570	0.000217838357133729
47.9833891443591	0.000217179839012549
48.0559610304613	0.000216524250560976
48.1309236142279	0.000215850390981633
48.2058861979945	0.000215179699169863
48.2808487817611	0.000214511926221073
48.3558113655277	0.000213847195271869
48.4308882648717	0.000213184779488308
48.5059651642157	0.000212525463455778
48.5810420635598	0.000211868999353958
48.6561189629038	0.000211215510786076
48.7288161374927	0.000210585828985196
48.8015133120816	0.000209958981051773
48.8742104866705	0.000209334764329391
48.9469076612594	0.000208713276893237
49.0187802551314	0.000208101740451555
49.0906528490033	0.000207492908417728
49.1625254428753	0.000206886593545423
49.2343980367472	0.000206282885844630
49.3067524167097	0.000205677975658748
49.3791067966722	0.000205075743325118
49.4514611766346	0.000204475996526334
49.5238155565971	0.000203878829089518
49.5979508123623	0.000203269867323244
49.6720860681275	0.000202663653156787
49.7462213238926	0.000202059967579256
49.8203565796578	0.000201458921089739
49.8652674347434	0.000201096201189791
49.9101782898289	0.000200734461781855
49.9550891449145	0.000200373690077649
50	0.000200013887136681

==> matlab/fig1c.tex <==
0.0100000000000000	0.500000000000000
0.0112590384703905	0.399958067249561
0.0125180769407810	0.335433026283611
0.0137771154111715	0.291422595874460
0.0150361538815620	0.260032080918151
0.0162951923519525	0.236875778320918
0.0175542308223430	0.219291980919333
0.0188132692927335	0.205612713551879
0.0200723077631240	0.194750472523118
0.0218134441469326	0.183058695519149
0.0235545805307411	0.174118976141966
0.0252957169145497	0.167122317757229
0.0270368532983583	0.161537329769423
0.0295181432065920	0.155334688168502
0.0319994331148256	0.150603129830555
0.0344807230230593	0.146907560681741
0.0369620129312930	0.143962980782199
0.0405572013330861	0.140652432001178
0.0441523897348793	0.138143516844971
0.0477475781366724	0.136194888331962
0.0513427665384656	0.134649680059735
0.0566747420772888	0.132886163951466
0.0620067176161121	0.131564613101567
0.0673386931549353	0.130547530745588
0.0726706686937585	0.129746916427669
0.0809070434834143	0.128807562722101
0.0891434182730702	0.128115667166674
0.0973797930627260	0.127589723733012
0.105616167852382	0.127179045029631
0.119428450217403	0.126665062123420
0.133240732582423	0.126294405068012
0.147053014947444	0.126014332052334
0.160865297312465	0.125793930384443
0.178019219732123	0.125575842461396
0.195173142151780	0.125398617610553
0.212327064571438	0.125248206773314
0.229480986991096	0.125115710752883
0.248483981448880	0.124982910107148
0.267486975906665	0.124859527166203
0.286489970364450	0.124741836527765
0.305492964822234	0.124627293004690
0.326939596021466	0.124499582126279
0.348386227220698	0.124371671241385
0.369832858419931	0.124242177146785
0.391279489619163	0.124110131398983
0.415086736184634	0.123959714970025
0.438893982750104	0.123804506045505
0.462701229315575	0.123643933424758
0.486508475881046	0.123477600061887
0.512579838010910	0.123288497295322
0.538651200140773	0.123091803049805
0.564722562270636	0.122887276091664
0.590793924400500	0.122674758971312
0.619005972967117	0.122435664804292
0.647218021533734	0.122186956667066
0.675430070100351	0.121928551437607
0.703642118666968	0.121660409635297
0.733851831073851	0.121362468011959
0.764061543480734	0.121053327449028
0.794271255887618	0.120732996515058
0.824480968294501	0.120401506546546
0.856524960901709	0.120037742228320
0.888568953508918	0.119661531733813
0.920612946116126	0.119272948838548
0.952656938723335	0.118872077628678
0.986351384409508	0.118437405446723
1.02004583009568	0.117989368067829
1.05374027578186	0.117528093931781
1.08743472146803	0.117053713571929
1.12257805195627	0.116545116705180
1.15772138244452	0.116022583793331
1.19286471293276	0.115486293485011
1.22800804342100	0.114936420800402
1.26438736782175	0.114353091332945
1.30076669222249	0.113755622794312
1.33714601662323	0.113144241248415
1.37352534102397	0.112519165094817
1.41092618586320	0.111862492023474
1.44832703070242	0.111191848456391
1.48572787554165	0.110507504733500
1.52312872038087	0.109809720736531
1.56134640367475	0.109083085002208
1.59956408696864	0.108343000873699
1.63778177026252	0.107589778747049
1.67599945355640	0.106823716703753
1.71484969660907	0.106032122663172
1.75369993966175	0.105227917552233
1.79255018271442	0.104411446513926
1.83140042576709	0.103583041211209
1.87072709840390	0.102732661610873
1.91005377104070	0.101870771608842
1.94938044367751	0.100997745056586
1.98870711631432	0.100113941641292
2.02838611226531	0.0992116633863419
2.06806510821629	0.0982991816580730
2.10774410416728	0.0973768927145468
2.14742310011826	0.0964451782740644
2.18736258820969	0.0954982138569415
2.22730207630111	0.0945425041020111
2.26724156439253	0.0935784615144548
2.30718105248396	0.0926064838599207
2.34731915635702	0.0916220778983495
2.38745726023007	0.0906304876040405
2.42759536410313	0.0896321359865822
2.46773346797619	0.0886274311962917
2.50803462769329	0.0876126616570160
2.54833578741038	0.0865923321092935
2.58863694712748	0.0855668708807509
2.62893810684458	0.0845366913356786
2.66938915757544	0.0834983484965413
2.70984020830630	0.0824561026990973
2.75029125903716	0.0814103829939275
2.79074230976801	0.0803616033390522
2.83134895097666	0.0793061248438132
2.87195559218530	0.0782484106481601
2.91256223339394	0.0771888864891665
2.95316887460259	0.0761279628321945
2.99395288397237	0.0750614052930834
3.03473689334216	0.0739942738087083
3.07552090271194	0.0729269872551116
3.11630491208173	0.0718599489926900
3.15730225154799	0.0707879811118297
3.19829959101425	0.0697170853902542
3.23929693048051	0.0686476706980985
3.28029426994677	0.0675801300715207
3.32155413519608	0.0665080366866869
3.36281400044539	0.0654386403153389
3.40407386569470	0.0643723369878456
3.44533373094400	0.0633095065000468
3.48691858677239	0.0622421963159917
3.52850344260078	0.0611791850047946
3.57008829842917	0.0601208531416170
3.61167315425756	0.0590675645756446
3.65365985811192	0.0580095764107358
3.69564656196628	0.0569574677701541
3.73763326582065	0.0559116012826576
3.77961996967501	0.0548723222568141
3.82210221583512	0.0538278254376651
3.86458446199523	0.0527907730106266
3.90706670815534	0.0517615071905874
3.94954895431544	0.0507403521576415
3.99264150344042	0.0497131361327146
4.03573405256539	0.0486949233127225
4.07882660169036	0.0476860329386311
4.12191915081533	0.0466867653547505
4.16576473103018	0.0456802111214139
4.20961031124503	0.0446842284036504
4.25345589145988	0.0436991106668686
4.29730147167473	0.0427251314290146
4.34208205652409	0.0417421513480032
4.38686264137346	0.0407713449772500
4.43164322622282	0.0398129767505382
4.47642381107218	0.0388672898479680
4.52237971564009	0.0379102084387530
4.56833562020800	0.0369669759875982
4.61429152477591	0.0360378238468818
4.66024742934382	0.0351229604429875
4.70771174380114	0.0341932741165792
4.75517605825846	0.0332792514673109
4.80264037271578	0.0323810853174461
4.85010468717310	0.0314989433281222
4.89744976257724	0.0306351324759484
4.94479483798138	0.0297875667737457
4.99213991338552	0.0289563752539130
5.03948498878966	0.0281416634127323
5.08636308744273	0.0273513128268351
5.13324118609581	0.0265772931961094
5.18011928474888	0.0258196711397163
5.22699738340195	0.0250784921417940
5.27357838501376	0.0243583288892842
5.32015938662558	0.0236544607310425
5.36674038823739	0.0229668984020359
5.41332138984921	0.0222956335630819
5.45976847819635	0.0216425049209432
5.50621556654349	0.0210055354910394
5.55266265489063	0.0203846851424162
5.59910974323777	0.0197798964788885
5.64558241876024	0.0191907805935783
5.69205509428270	0.0186176027964710
5.73852776980517	0.0180602758739234
5.78500044532764	0.0175186969750181
5.83166690899266	0.0169905921886023
5.87833337265768	0.0164781348237720
5.92499983632269	0.0159811932653557
5.97166629998771	0.0154996217562366
6.01871655904510	0.0150294923390531
6.06576681810250	0.0145746670914034
6.11281707715989	0.0141349715241509
6.15986733621728	0.0137102184057247
6.20753009502752	0.0132949710511210
6.25519285383776	0.0128946511371280
6.30285561264800	0.0125090414254138
6.35051837145825	0.0121379132721020
6.39908671418941	0.0117743864215929
6.44765505692057	0.0114254001560393
6.49622339965174	0.0110906926565331
6.54479174238290	0.0107699920103251
6.59477427942936	0.0104542847732612
6.64475681647582	0.0101528134253741
6.69473935352228	0.00986526460613566
6.74472189056874	0.00959131612657001
6.79435030314736	0.00933244213867433
6.84397871572597	0.00908633423473104
6.89360712830458	0.00885266559781256
6.94323554088320	0.00863110325438423
6.99213297011201	0.00842431792339925
7.04103039934083	0.00822863914745205
7.08992782856965	0.00804374260759559
7.13882525779847	0.00786930033253498
7.18736732322589	0.00770614203958404
7.23590938865331	0.00755264301051480
7.28445145408073	0.00740848130983532
7.33299351950815	0.00727333337752758
7.38150321897300	0.00714695794621002
7.43001291843784	0.00702894284236557
7.47852261790269	0.00691896840096408
7.52703231736754	0.00681671508912448
7.57580331165659	0.00672137416469423
7.62457430594563	0.00663319866820305
7.67334530023468	0.00655187124655919
7.72211629452373	0.00647707629842812
7.77144705621219	0.00640774964923798
7.82077781790065	0.00634446947838954
7.87010857958912	0.00628692072898425
7.91943934127758	0.00623479168080361
7.96966620873211	0.00618696693463602
8.01989307618664	0.00614412547551327
8.07011994364117	0.00610595427871060
8.12034681109570	0.00607214530836476
8.17188862971250	0.00604167006236206
8.22343044832929	0.00601515331001335
8.27497226694608	0.00599228326998868
8.32651408556287	0.00597275500333410
8.37995066555843	0.00595572014304225
8.43338724555398	0.00594163808501379
8.48682382554954	0.00593019641970143
8.54026040554509	0.00592109186188101
8.59264630622872	0.00591415262975756
8.64503220691234	0.00590891250546918
8.69741810759597	0.00590511408489814
8.74980400827959	0.00590250911834514
8.80130195951982	0.00590088088295181
8.85279991076004	0.00589995966717911
8.90429786200027	0.00589953735489988
8.95579581324049	0.00589941474434025
9.00691883967619	0.00589940252701651
9.05804186611189	0.00589932322901635
9.10916489254759	0.00589900923619577
9.16028791898329	0.00589830168197197
9.21145411122912	0.00589704980987832
9.26262030347494	0.00589511371764767
9.31378649572077	0.00589236116012895
9.36495268796660	0.00588866852072592
9.41654794015576	0.00588387682132904
9.46814319234492	0.00587790505664975
9.51973844453408	0.00587065341741166
9.57133369672324	0.00586203063934836
9.62392663286122	0.00585174484433554
9.67651956899920	0.00583987155415151
9.72911250513718	0.00582634141955570
9.78170544127516	0.00581109369616648
9.83584912150179	0.00579354763010959
9.88999280172842	0.00577408005658038
9.94413648195504	0.00575265273277493
9.99828016218167	0.00572923616541723
10.0540781056737	0.00570300142657754
10.1098760491657	0.00567462037297895
10.1656739926577	0.00564408882542688
10.2214719361497	0.00561141120965141
10.2756340627963	0.00557765176043228
10.3297961894429	0.00554190315390047
10.3839583160894	0.00550419153583327
10.4381204427360	0.00546454935501329
10.4913006965245	0.00542378533112647
10.5444809503131	0.00538124110934542
10.5976612041017	0.00533696424241717
10.6508414578903	0.00529100688236043
10.7036286794831	0.00524378365446422
10.7564159010759	0.00519502170449093
10.8092031226688	0.00514478475156097
10.8619903442616	0.00509313976761336
10.9148514055899	0.00504008236863766
10.9677124669181	0.00498575841420944
11.0205735282463	0.00493024434925670
11.0734345895746	0.00487361870380368
11.1268048985060	0.00481540231861914
11.1801752074375	0.00475622144456330
11.2335455163689	0.00469616283914379
11.2869158253004	0.00463531425274915
11.3412675119695	0.00457262708766750
11.3956191986386	0.00450930889513126
11.4499708853078	0.00444545505269732
11.5043225719769	0.00438116083313286
11.5602445818107	0.00431465016179208
11.6161665916445	0.00424787921636086
11.6720886014783	0.00418095096301114
11.7280106113121	0.00411396706784462
11.7854922362233	0.00404516318659771
11.8429738611344	0.00397651592990380
11.9004554860456	0.00390813096993885
11.9579371109568	0.00384011138101312
12.0138246466191	0.00377442453959254
12.0697121822814	0.00370926977266613
12.1255997179437	0.00364473453052909
12.1814872536060	0.00358090306924821
12.2364081740881	0.00351894036924949
12.2913290945701	0.00345781123739718
12.3462500150521	0.00339758674457160
12.4011709355341	0.00333833440461662
12.4557093948871	0.00328052042125381
12.5102478542401	0.00322378902424455
12.5647863135931	0.00316819625616756
12.6193247729461	0.00311379434986083
12.6739738559100	0.00306052573055919
12.7286229388739	0.00300854799079601
12.7832720218378	0.00295790265747937
12.8379211048018	0.00290862726108279
12.8932201372012	0.00286019509795907
12.9485191696007	0.00281323224319295
13.0038182020002	0.00276776567381372
13.0591172343996	0.00272381820984227
13.1157877654014	0.00268037692036508
13.1724582964031	0.00263856787574269
13.2291288274048	0.00259840270537122
13.2857993584066	0.00255988869893892
13.3446243075368	0.00252166074074602
13.4034492566669	0.00248521513487811
13.4622742057971	0.00245054587495477
13.5210991549273	0.00241764243656795
13.5783218161257	0.00238731588334336
13.6355444773240	0.00235862948641530
13.6927671385223	0.00233156178103123
13.7499897997207	0.00230608780054454
13.8061231584122	0.00228262028207533
13.8622565171036	0.00226063002224059
13.9183898757951	0.00224008416102049
13.9745232344866	0.00222094720072398
14.0302633175361	0.00220330122516828
14.0860034005856	0.00218696794659763
14.1417434836351	0.00217190536695112
14.1974835666846	0.00215806958090306
14.2533926250767	0.00214537853034626
14.3093016834687	0.00213382828214145
14.3652107418608	0.00212336912974343
14.4211198002529	0.00211395014183764
14.4777370024593	0.00210541881169056
14.5343542046657	0.00209784586439440
14.5909714068721	0.00209117480606641
14.6475886090785	0.00208534861373756
14.7055282387007	0.00208020127503369
14.7634678683228	0.00207581663449300
14.8214074979450	0.00207213187946709
14.8793471275672	0.00206908444365773
14.9394338470089	0.00206653087911167
14.9995205664506	0.00206452665176742
15.0596072858923	0.00206300248865607
15.1196940053340	0.00206189032898483
15.1785299451618	0.00206113640442154
15.2373658849896	0.00206065150801147
15.2962018248174	0.00206037443404085
15.3550377646452	0.00206024575390196
15.4126282162481	0.00206020819166686
15.4702186678511	0.00206020479069900
15.5278091194541	0.00206018402012779
15.5853995710570	0.00206009645949334
15.6425138397232	0.00205989714186616
15.6996281083894	0.00205954109499928
15.7567423770555	0.00205898544649155
15.8138566457217	0.00205818971645633
15.8711953652715	0.00205711104751533
15.9285340848213	0.00205571540468703
15.9858728043710	0.00205396813688339
16.0432115239208	0.00205183726453591
16.1014495158645	0.00204925016068012
16.1596875078082	0.00204620856197382
16.2179254997519	0.00204268621023898
16.2761634916956	0.00203865982398122
16.3359700634670	0.00203397907991942
16.3957766352384	0.00202872579345162
16.4555832070098	0.00202288296056305
16.5153897787812	0.00201643689985413
16.5772595565287	0.00200912258341518
16.6391293342762	0.00200114271218169
16.7009991120237	0.00199249122043041
16.7628688897712	0.00198316570218403
16.8226291025295	0.00197351924485866
16.8823893152878	0.00196324811372651
16.9421495280461	0.00195235771879090
17.0019097408044	0.00194085629414575
17.0604737135166	0.00192900285267431
17.1190376862287	0.00191658520921612
17.1776016589408	0.00190361719501316
17.2361656316529	0.00189011485173405
17.2943437987857	0.00187619035935646
17.3525219659184	0.00186177573967489
17.4107001330511	0.00184689153719855
17.4688783001839	0.00183156002407354
17.5273181214793	0.00181573336396669
17.5857579427747	0.00179950484599586
17.6441977640701	0.00178290067472618
17.7026375853655	0.00176594835448599
17.7619748377587	0.00174840906230128
17.8213120901519	0.00173057125545123
17.8806493425450	0.00171246612933813
17.9399865949382	0.00169412576413488
18.0009772089185	0.00167506381770848
18.0619678228989	0.00165582405800485
18.1229584368792	0.00163644233491014
18.1839490508595	0.00161695494617804
18.2467391781493	0.00159682088861716
18.3095293054391	0.00157665334073429
18.3723194327289	0.00155649120381791
18.4351095600186	0.00153637330722591
18.4958890311180	0.00151697822460509
18.5566685022173	0.00149769497697947
18.6174479733167	0.00147855665942057
18.6782274444160	0.00145959578947609
18.7378730347315	0.00144119200338962
18.7975186250471	0.00142301880255943
18.8571642153626	0.00140510381088899
18.9168098056781	0.00138747374817005
18.9761161336685	0.00137025201954105
19.0354224616590	0.00135336145234022
19.0947287896494	0.00133682440860689
19.1540351176398	0.00132066211077281
19.2137174724110	0.00130479598475784
19.2733998271821	0.00128934852333238
19.3330821819533	0.00127433672034437
19.3927645367245	0.00125977624440378
19.4536313109237	0.00124540654403539
19.5144980851229	0.00123153446793050
19.5753648593222	0.00121817122804174
19.6362316335214	0.00120532655094678
19.6991702047529	0.00119259877020402
19.7621087759845	0.00118044108620222
19.8250473472160	0.00116885794572339
19.8879859184476	0.00115785217668995
19.9504675490644	0.00114749861041428
20.0129491796813	0.00113771410246489
20.0754308102981	0.00112849537678408
20.1379124409149	0.00111983772300258
20.1988318485020	0.00111193088961215
20.2597512560891	0.00110454389396034
20.3206706636762	0.00109766735110546
20.3815900712632	0.00109129076792510
20.4418628007192	0.00108546253767360
20.5021355301751	0.00108009946923767
20.5624082596310	0.00107518729334617
20.6226809890869	0.00107071093306780
20.6830648171870	0.00106664740862121
20.7434486452870	0.00106298799933474
20.8038324733871	0.00105971424326135
20.8642163014871	0.00105680717526486
20.9254176891409	0.00105421494995649
20.9866190767946	0.00105195795583687
21.0478204644484	0.00105001393531423
21.1090218521021	0.00104836046744989
21.1718545315804	0.00104694146240866
21.2346872110587	0.00104577945769322
21.2975198905370	0.00104484853100815
21.3603525700153	0.00104412301655129
21.4250495998080	0.00104356373585169
21.4897466296008	0.00104316673430068
21.5544436593936	0.00104290339528933
21.6191406891863	0.00104274588062200
21.6817036315996	0.00104266863048588
21.7442665740128	0.00104263999252119
21.8068295164261	0.00104263539813311
21.8693924588393	0.00104263126525997
21.9308388102019	0.00104260568313335
21.9922851615645	0.00104253718995262
22.0537315129272	0.00104240492804620
22.1151778642898	0.00104218920180414
22.1764705511298	0.00104187230812252
22.2377632379697	0.00104143565402667
22.2990559248097	0.00104086186854134
22.3603486116497	0.00104013492556797
22.4223000336916	0.00103922944566735
22.4842514557336	0.00103813765083299
22.5462028777755	0.00103684578757949
22.6081542998175	0.00103534165198905
22.6715496881498	0.00103357145256011
22.7349450764822	0.00103155683129023
22.7983404648145	0.00102928810296175
22.8617358531469	0.00102675737401651
22.9276086030674	0.00102384346639297
22.9934813529880	0.00102063374441086
23.0593541029086	0.00101712338077268
23.1252268528292	0.00101330966730439
23.1892682653520	0.00100931034777970
23.2533096778747	0.00100502341295008
23.3173510903975	0.00100044998485780
23.3813925029203	0.000995592929702122
23.4439303515084	0.000990580398422003
23.5064682000966	0.000985306282032411
23.5690060486847	0.000979776229804944
23.6315438972729	0.000973997286942648
23.6935838954000	0.000968026568895760
23.7556238935271	0.000961827589927573
23.8176638916543	0.000955409628967740
23.8797038897814	0.000948783104337081
23.9420528805491	0.000941924956401549
24.0044018713168	0.000934879562178993
24.0667508620844	0.000927659319069462
24.1290998528521	0.000920277548494334
24.1925523682960	0.000912613837169043
24.2560048837398	0.000904812377680881
24.3194573991837	0.000896888393908811
24.3829099146275	0.000888857834442593
24.4484444382408	0.000880469412717263
24.5139789618541	0.000872002908916598
24.5795134854674	0.000863476286707783
24.6450480090807	0.000854908036790039
24.7108250011305	0.000846285165231965
24.7766019931802	0.000837657766635450
24.8423789852300	0.000829043977939114
24.9081559772797	0.000820462144280014
24.9720195866552	0.000812177915431589
25.0358831960306	0.000803957122118779
25.0997468054060	0.000795815268053546
25.1636104147814	0.000787767753131444
25.2265955481551	0.000779938111847544
25.2895806815287	0.000772228603914902
25.3525658149024	0.000764652169265311
25.4155509482761	0.000757221440588499
25.4785556713374	0.000749946389142353
25.5415603943987	0.000742840527238832
25.6045651174600	0.000735914175814996
25.6675698405213	0.000729177203402849
25.7315234913094	0.000722542006606915
25.7954771420975	0.000716120039004206
25.8594307928856	0.000709918787598191
25.9233844436737	0.000703945177252733
25.9892426850350	0.000698038167974651
26.0551009263963	0.000692384544590614
26.1209591677576	0.000686988447189350
26.1868174091189	0.000681853377004629
26.2535502444464	0.000676919149450461
26.3202830797740	0.000672256924787732
26.3870159151016	0.000667866657527530
26.4537487504291	0.000663747679198049
26.5184351348136	0.000660012592615949
26.5831215191980	0.000656528270540792
26.6478079035824	0.000653290956654105
26.7124942879669	0.000650296404605653
26.7762428831831	0.000647578051105468
26.8399914783994	0.000645084881357900
26.9037400736156	0.000642810211034529
26.9674886688319	0.000640747011953948
27.0312432274322	0.000638887643554487
27.0949977860326	0.000637223761745681
27.1587523446329	0.000635746161564159
27.2225069032333	0.000634445459893152
27.2871135974660	0.000633297926889853
27.3517202916987	0.000632311118616443
27.4163269859314	0.000631473521467596
27.4809336801641	0.000630773646541942
27.5473600151609	0.000630185460303306
27.6137863501576	0.000629717172911510
27.6802126851544	0.000629355000771527
27.7466390201512	0.000629085458288334
27.8144911660441	0.000628891883305369
27.8823433119370	0.000628766078132354
27.9501954578299	0.000628692996430536
28.0180476037228	0.000628658205038483
28.0836710412897	0.000628647777347522
28.1492944788567	0.000628646867249212
28.2149179164237	0.000628642502535975
28.2805413539907	0.000628622419269560
28.3451053878376	0.000628575935914625
28.4096694216846	0.000628491513740020
28.4742334555315	0.000628358125673092
28.5387974893785	0.000628165553361755
28.6034183056205	0.000627903967568590
28.6680391218626	0.000627563898273090
28.7326599381047	0.000627136201719669
28.7972807543468	0.000626612668555136
28.8628316080457	0.000625976052073790
28.9283824617446	0.000625225513208831
28.9939333154435	0.000624353982441864
29.0594841691424	0.000623355476835403
29.1269556326181	0.000622189754079976
29.1944270960939	0.000620878785829164
29.2618985595696	0.000619417933094194
29.3293700230453	0.000617803846015844
29.3979909106086	0.000616002726859367
29.4666117981718	0.000614038531806248
29.5352326857351	0.000611909825091975
29.6038535732983	0.000609616545933486
29.6701727865302	0.000607244773489487
29.7364919997621	0.000604721320223162
29.8028112129939	0.000602047932171553
29.8691304262258	0.000599227444908637
29.9343704267019	0.000596312926762019
29.9996104271780	0.000593263302963712
30.0648504276541	0.000590082753399074
30.1300904281302	0.000586776355760988
30.1952858095128	0.000583352282334004
30.2604811908953	0.000579814148266395
30.3256765722779	0.000576168176175510
30.3908719536605	0.000572421346513434
30.4569332436822	0.000568529621631063
30.5229945337039	0.000564549909191461
30.5890558237256	0.000560490259643490
30.6551171137473	0.000556359366994405
30.7230813828530	0.000552044768463666
30.7910456519586	0.000547674171504731
30.8590099210643	0.000543257369985014
30.9269741901699	0.000538804704326671
30.9964305818134	0.000534228327422234
31.0658869734568	0.000529636518374666
31.1353433651002	0.000525040031046546
31.2047997567437	0.000520450014562916
31.2718985486150	0.000516032545887749
31.3389973404864	0.000511641164707402
31.4060961323577	0.000507285147267988
31.4731949242290	0.000502973900801327
31.5391489416833	0.000498788901120810
31.6051029591375	0.000494664363529823
31.6710569765918	0.000490608083689912
31.7370109940461	0.000486627826089606
31.8029038201020	0.000482734740783855
31.8687966461580	0.000478931864334975
31.9346894722139	0.000475225465642367
32.0005822982699	0.000471621675601757
32.0674470725521	0.000468075621286587
32.1343118468343	0.000464646435095398
32.2011766211165	0.000461338690322317
32.2680413953987	0.000458156751471987
32.3369742812759	0.000455012326680493
32.4059071671532	0.000452009139297119
32.4748400530305	0.000449149709709532
32.5437729389077	0.000446436314477393
32.6132976261725	0.000443849416489379
32.6828223134373	0.000441413611160250
32.7523470007020	0.000439128804153013
32.8218716879668	0.000436994669827000
32.8892575400122	0.000435069268780923
32.9566433920577	0.000433282907622876
33.0240292441032	0.000431633205626557
33.0914150961486	0.000430117602960827
33.1579074063846	0.000428750717276518
33.2243997166205	0.000427507860700947
33.2908920268565	0.000426384821185400
33.3573843370924	0.000425377288588606
33.4240362992290	0.000424478692109393
33.4906882613656	0.000423686173477765
33.5573402235022	0.000422993913611621
33.6239921856388	0.000422396104424923
33.6917838285149	0.000421878833648738
33.7595754713910	0.000421446110333836
33.8273671142671	0.000421090606047885
33.8951587571432	0.000420805153537207
33.9652790260747	0.000420575973901064
34.0353992950061	0.000420405406295165
34.1055195639376	0.000420284577583319
34.1756398328691	0.000420205001342834
34.2453776041807	0.000420158543521354
34.3151153754923	0.000420135854187165
34.3848531468039	0.000420128130619981
34.4545909181155	0.000420127104452158
34.5223782426370	0.000420124976524570
34.5901655671585	0.000420113936748412
34.6579528916800	0.000420086424374987
34.7257402162014	0.000420035458525641
34.7928996323729	0.000419955366828366
34.8600590485443	0.000419839149883119
34.9272184647158	0.000419680417012725
34.9943778808873	0.000419473428742519
35.0619929504487	0.000419210966049398
35.1296080200101	0.000418888762096858
35.1972230895715	0.000418501652773869
35.2648381591328	0.000418045223420195
35.3339326818891	0.000417503198570281
35.4030272046454	0.000416880605413555
35.4721217274016	0.000416173690466881
35.5412162501579	0.000415379584042611
35.6131113972494	0.000414458373735352
35.6850065443410	0.000413437875030786
35.7569016914325	0.000412316070694103
35.8287968385241	0.000411092033473382
35.8985499225384	0.000409806634387303
35.9683030065528	0.000408424671178120
36.0380560905672	0.000406946427479934
36.1078091745816	0.000405373088864471
36.1758899819743	0.000403747538495783
36.2439707893671	0.000402034819121631
36.3120515967598	0.000400236982562610
36.3801324041526	0.000398356816822241
36.4478115126495	0.000396409436301217
36.5154906211464	0.000394387176788986
36.5831697296433	0.000392293527875721
36.6508488381403	0.000390132608616638
36.7191711629321	0.000387887567229014
36.7874934877239	0.000385583178271808
36.8558158125157	0.000383224197119521
36.9241381373075	0.000380815932700748
36.9942096873564	0.000378300765354240
37.0642812374052	0.000375745585705188
37.1343527874540	0.000373156337973314
37.2044243375029	0.000370539467075879
37.2770714990837	0.000367804439433511
37.3497186606646	0.000365053991960273
37.4223658222454	0.000362295096878559
37.4950129838262	0.000359535179714751
37.5648860036314	0.000356886772147300
37.6347590234365	0.000354250615316399
37.7046320432417	0.000351632757541070
37.7745050630469	0.000349039468387394
37.8429849056960	0.000346527786252178
37.9114647483452	0.000344051063083812
37.9799445909944	0.000341614393925055
38.0484244336436	0.000339222960085727
38.1167683734507	0.000336886453686536
38.1851123132578	0.000334604504075963
38.2534562530649	0.000332381215666842
38.3218001928720	0.000330220697423357
38.3911454818990	0.000328096742015805
38.4604907709259	0.000326044871241479
38.5298360599529	0.000324068066566929
38.5991813489799	0.000322169267565133
38.6707549934430	0.000320294151022715
38.7423286379060	0.000318507149351164
38.8139022823690	0.000316809855334762
38.8854759268321	0.000315203810499643
38.9573395690528	0.000313684357799807
39.0292032112736	0.000312258505844692
39.1010668534944	0.000310926070285790
39.1729304957152	0.000309686823071640
39.2426006365928	0.000308573913238754
39.3122707774704	0.000307546812860188
39.3819409183480	0.000306603816125414
39.4516110592256	0.000305743189116164
39.5204531079888	0.000304971812854846
39.5892951567520	0.000304276360108678
39.6581372055153	0.000303653889109289
39.7269792542785	0.000303101480062135
39.7961453702529	0.000302613953803803
39.8653114862273	0.000302190295423293
39.9344776022017	0.000301826459606479
40.0036437181761	0.000301518504037041
40.0742469817186	0.000301257637797958
40.1448502452611	0.000301045935370324
40.2154535088036	0.000300878290337787
40.2860567723460	0.000300749822982709
40.3595268224031	0.000300652543353051
40.4329968724601	0.000300586353727106
40.5064669225171	0.000300545016775229
40.5799369725741	0.000300522725940829
40.6513675007179	0.000300513975828541
40.7227980288617	0.000300512184823628
40.7942285570055	0.000300511680447178
40.8656590851494	0.000300507258813128
40.9354139422374	0.000300494429745816
41.0051687993254	0.000300468172141862
41.0749236564134	0.000300423646187068
41.1446785135014	0.000300356505791479
41.2141846577893	0.000300263111037204
41.2836908020773	0.000300139022638109
41.3531969463653	0.000299980197891715
41.4227030906532	0.000299783145118563
41.4930789169469	0.000299541497261165
41.5634547432405	0.000299254050087203
41.6338305695342	0.000298917639906967
41.7042063958279	0.000298529739916363
41.7766738644670	0.000298074318393805
41.8491413331062	0.000297559672591341
41.9216088017454	0.000296983685087197
41.9940762703846	0.000296345006107974
42.0676270896293	0.000295631845418928
42.1411779088741	0.000294852241002741
42.2147287281188	0.000294005517717725
42.2882795473636	0.000293091822934759
42.3592970394703	0.000292146710582434
42.4303145315771	0.000291140269622541
42.5013320236838	0.000290073279244158
42.5723495157906	0.000288947171606403
42.6423081717146	0.000287781882283892
42.7122668276387	0.000286562694400147
42.7822254835628	0.000285291502770377
42.8521841394869	0.000283970753722861
42.9223311803881	0.000282599522978789
42.9924782212893	0.000281183962652443
43.0626252621906	0.000279726915319273
43.1327723030918	0.000278231712674873
43.2042637505405	0.000276672368276743
43.2757551979892	0.000275080780110029
43.3472466454379	0.000273460655034000
43.4187380928867	0.000271816152440049
43.4930174384355	0.000270086441366165
43.5672967839843	0.000268339743617756
43.6415761295332	0.000266580617320429
43.7158554750820	0.000264814068237433
43.7886851215017	0.000263079806327975
43.8615147679214	0.000261347787081364
43.9343444143411	0.000259622336358319
44.0071740607608	0.000257908072173170
44.0780890043289	0.000256254096776987
44.1490039478970	0.000254618981467011
44.2199188914650	0.000253006404855636
44.2908338350331	0.000251420206406338
44.3612464402611	0.000249875119717434
44.4316590454890	0.000248363011877386
44.5020716507170	0.000246886882999129
44.5724842559449	0.000245449819887283
44.6436666325296	0.000244039830176310
44.7148490091142	0.000242675352469957
44.7860313856988	0.000241358622120928
44.8572137622834	0.000240091923346065
44.9304409819765	0.000238843329194388
45.0036682016695	0.000237651616173624
45.0768954213625	0.000236518072759571
45.1501226410556	0.000235444033268365
45.2247367648061	0.000234412084516798
45.2993508885565	0.000233443564455855
45.3739650123070	0.000232538513062913
45.4485791360575	0.000231697031559651
45.5206102726895	0.000230944932614768
45.5926414093215	0.000230251196659974
45.6646725459534	0.000229614727377792
45.7367036825854	0.000229034476609081
45.8076682830009	0.000228516653924894
45.8786328834164	0.000228050485629937
45.9495974838319	0.000227633964172226
46.0205620842474	0.000227265156784950
46.0917592672627	0.000226941067507429
46.1629564502780	0.000226660356615966
46.2341536332932	0.000226420204124846
46.3053508163085	0.000226217923000020
46.3779951965189	0.000226047755652188
46.4506395767293	0.000225910743414691
46.5232839569396	0.000225803282213125
46.5959283371500	0.000225721998351277
46.6715633469138	0.000225661615689444
46.7471983566776	0.000225621669705833
46.8228333664415	0.000225597713500406
46.8984683762053	0.000225585700126170
46.9719520694971	0.000225581779820573
47.0454357627890	0.000225581370664144
47.1189194560809	0.000225580431252421
47.1924031493727	0.000225575334572234
47.2641650684056	0.000225563077637307
47.3359269874386	0.000225540050226805
47.4076889064715	0.000225502812519440
47.4794508255044	0.000225448349429257
47.5510064906415	0.000225374146957110
47.6225621557785	0.000225277062611283
47.6941178209155	0.000225154237427940
47.7656734860526	0.000225003280451534
47.8382453721548	0.000224819304434286
47.9108172582570	0.000224601837231627
47.9833891443591	0.000224348665660491
48.0559610304613	0.000224058117270313
48.1309236142279	0.000223717365786348
48.2058861979945	0.000223333665936266
48.2808487817611	0.000222905582734844
48.3558113655277	0.000222432341244534
48.4308882648717	0.000221912773529709
48.5059651642157	0.000221346972945570
48.5810420635598	0.000220734613820222
48.6561189629038	0.000220076028190214
48.7288161374927	0.000219394975515060
48.8015133120816	0.000218671742012448
48.8742104866705	0.000217907024819453
48.9469076612594	0.000217102048792391
49.0187802551314	0.000216268159516183
49.0906528490033	0.000215397761688691
49.1625254428753	0.000214492349084174
49.2343980367472	0.000213553869944122
49.3067524167097	0.000212577961246332
49.3791067966722	0.000211572858457045
49.4514611766346	0.000210540741246505
49.5238155565971	0.000209484203671048
49.5979508123623	0.000208379299472304
49.6720860681275	0.000207254488682722
49.7462213238926	0.000206112585097032
49.8203565796578	0.000204956803528029
49.8652674347434	0.000204251331169154
49.9101782898289	0.000203542656252663
49.9550891449145	0.000202831484875709
50	0.000202118539041625

==> matlab/fig1d.tex <==
0.0100000000000000	0.500000000000000
0.0112590384703905	0.499999979190838
0.0125180769407810	0.499999824394511
0.0137771154111715	0.499999481006660
0.0150361538815620	0.499998939208842
0.0162951923519525	0.499998188198835
0.0175542308223430	0.499997228308649
0.0188132692927335	0.499996065515069
0.0200723077631240	0.499994707985618
0.0218134441469326	0.499992520664016
0.0235545805307411	0.499989984667584
0.0252957169145497	0.499987114187258
0.0270368532983583	0.499983922902389
0.0295181432065920	0.499978838738723
0.0319994331148256	0.499973140421541
0.0344807230230593	0.499966846214706
0.0369620129312930	0.499959972873322
0.0405572013330861	0.499949008254249
0.0441523897348793	0.499936870447251
0.0477475781366724	0.499923578651703
0.0513427665384656	0.499909151175744
0.0566747420772888	0.499885687072651
0.0620067176161121	0.499859767805855
0.0673386931549353	0.499831411278519
0.0726706686937585	0.499800637664007
0.0809070434834143	0.499748380794534
0.0891434182730702	0.499690398473521
0.0973797930627260	0.499626705218350
0.105616167852382	0.499557327847377
0.119428450217403	0.499428282242787
0.133240732582423	0.499283303060038
0.147053014947444	0.499122396926086
0.160865297312465	0.498945624688858
0.178019219732123	0.498704071142014
0.195173142151780	0.498438111014455
0.212327064571438	0.498147762962314
0.229480986991096	0.497833092365406
0.248483981448880	0.497456184388493
0.267486975906665	0.497049535113517
0.286489970364450	0.496613194790486
0.305492964822234	0.496147241600547
0.326939596021466	0.495585904371754
0.348386227220698	0.494987041407172
0.369832858419931	0.494350756930365
0.391279489619163	0.493677176649049
0.415086736184634	0.492885937549418
0.438893982750104	0.492049074195636
0.462701229315575	0.491166772941564
0.486508475881046	0.490239237137531
0.512579838010910	0.489171850676139
0.538651200140773	0.488050758204161
0.564722562270636	0.486876263136887
0.590793924400500	0.485648682830890
0.619005972967117	0.484260886474456
0.647218021533734	0.482811757094926
0.675430070100351	0.481301755348974
0.703642118666968	0.479731353842377
0.733851831073851	0.477983341214249
0.764061543480734	0.476167271409270
0.794271255887618	0.474283805168414
0.824480968294501	0.472333613929761
0.856524960901709	0.470192854855022
0.888568953508918	0.467978677340326
0.920612946116126	0.465691983643348
0.952656938723335	0.463333685835216
0.986351384409508	0.460777715280993
1.02004583009568	0.458144760915119
1.05374027578186	0.455436001412015
1.08743472146803	0.452652624324053
1.12257805195627	0.449671370171072
1.15772138244452	0.446611714279599
1.19286471293276	0.443475134811654
1.22800804342100	0.440263117392764
1.26438736782175	0.436860279199822
1.30076669222249	0.433379983084461
1.33714601662323	0.429824013729040
1.37352534102397	0.426194161017408
1.41092618586320	0.422387268765131
1.44832703070242	0.418506262881170
1.48572787554165	0.414553223663749
1.52312872038087	0.410530233258123
1.56134640367475	0.406349311462824
1.59956408696864	0.402099878913312
1.63778177026252	0.397784283691344
1.67599945355640	0.393404871196386
1.71484969660907	0.388889999510233
1.75369993966175	0.384314187725056
1.79255018271442	0.379680010491199
1.83140042576709	0.374990034148872
1.87072709840390	0.370188352201567
1.91005377104070	0.365334885684152
1.94938044367751	0.360432386139043
1.98870711631432	0.355483590265815
2.02838611226531	0.350446327059236
2.06806510821629	0.345367606774500
2.10774410416728	0.340250304649977
2.14742310011826	0.335097273895846
2.18736258820969	0.329877218852453
2.22730207630111	0.324626813489042
2.26724156439253	0.319349004003982
2.30718105248396	0.314046706986199
2.34731915635702	0.308696305198080
2.38745726023007	0.303327097240896
2.42759536410313	0.297942050621252
2.46773346797619	0.292544095484054
2.50803462769329	0.287114158229040
2.54833578741038	0.281677117440993
2.58863694712748	0.276235916715433
2.62893810684458	0.270793454538971
2.66938915757544	0.265332373074505
2.70984020830630	0.259875832575362
2.75029125903716	0.254426712322102
2.79074230976801	0.248987838868765
2.83134895097666	0.243541162263452
2.87195559218530	0.238110451217106
2.91256223339394	0.232698484866921
2.95316887460259	0.227307982214043
2.99395288397237	0.221918235434882
3.03473689334216	0.216555542313415
3.07552090271194	0.211222550000898
3.11630491208173	0.205921838351724
3.15730225154799	0.200628487125334
3.19829959101425	0.195372860446719
3.23929693048051	0.190157444863736
3.28029426994677	0.184984652726131
3.32155413519608	0.179824151397678
3.36281400044539	0.174711575772009
3.40407386569470	0.169649225564347
3.44533373094400	0.164639319637502
3.48691858677239	0.159645201601362
3.52850344260078	0.154708710707752
3.57008829842917	0.149831935115843
3.61167315425756	0.145016875692884
3.65365985811192	0.140219862367879
3.69564656196628	0.135489666998394
3.73763326582065	0.130828142022753
3.77961996967501	0.126237046312149
3.82210221583512	0.121665161389235
3.86458446199523	0.117168781583221
3.90706670815534	0.112749498927007
3.94954895431544	0.108408805704698
3.99264150344042	0.104087488107253
4.03573405256539	0.0998498855520649
4.07882660169036	0.0956973031253411
4.12191915081533	0.0916309399789255
4.16576473103018	0.0875831528613275
4.20961031124503	0.0836268647754047
4.25345589145988	0.0797630636365614
4.29730147167473	0.0759926250989728
4.34208205652409	0.0722389597092996
4.38686264137346	0.0685842396286740
4.43164322622282	0.0650290989430008
4.47642381107218	0.0615740528052985
4.52237971564009	0.0581328240280220
4.56833562020800	0.0547977992570428
4.61429152477591	0.0515692110849837
4.66024742934382	0.0484471658328141
4.70771174380114	0.0453344848479237
4.75517605825846	0.0423353449176920
4.80264037271578	0.0394495100589793
4.85010468717310	0.0366766094552062
4.89744976257724	0.0340226965365272
4.94479483798138	0.0314800832270152
4.99213991338552	0.0290480677452916
5.03948498878966	0.0267258263278955
5.08636308744273	0.0245337304915213
5.13324118609581	0.0224473510538007
5.18011928474888	0.0204655932888452
5.22699738340195	0.0185872579448107
5.27357838501376	0.0168219913459082
5.32015938662558	0.0151562219623024
5.36674038823739	0.0135885170284544
5.41332138984921	0.0121173554180626
5.45976847819635	0.0107449596210557
5.50621556654349	0.00946531169543501
5.55266265489063	0.00827668534228270
5.59910974323777	0.00717728117188491
5.64558241876024	0.00616470149055704
5.69205509428270	0.00523765457063995
5.73852776980517	0.00439415730672249
5.78500044532764	0.00363216824608160
5.83166690899266	0.00294691194827105
5.87833337265768	0.00233957234336518
5.92499983632269	0.00180793930167294
5.97166629998771	0.00134975888314725
6.01871655904510	0.000959845309452317
6.06576681810250	0.000639887065793006
6.11281707715989	0.000387469731357943
6.15986733621728	0.000200149753034725
6.20753009502752	7.42386126463829e-05
6.25519285383776	1.00133060203185e-05
6.30285561264800	4.86975731201015e-06
6.35051837145825	5.61900371990813e-05
6.39908671418941	0.000163848935662432
6.44765505692057	0.000324622715010478
6.49622339965174	0.000535721708409588
6.54479174238290	0.000794358980135647
6.59477427942936	0.00110723083497263
6.64475681647582	0.00146448321329711
6.69473935352228	0.00186310991554417
6.74472189056874	0.00230012679926818
6.79435030314736	0.00276910982431250
6.84397871572597	0.00327015117492331
6.89360712830458	0.00380041073936069
6.94323554088320	0.00435708666634373
6.99213297011201	0.00492871087101188
7.04103039934083	0.00552069265035728
7.08992782856965	0.00613047153089555
7.13882525779847	0.00675553677655835
7.18736732322589	0.00738875179947022
7.23590938865331	0.00803224689692907
7.28445145408073	0.00868371680803624
7.33299351950815	0.00934091564994124
7.38150321897300	0.0100012156818193
7.43001291843784	0.0106629274348964
7.47852261790269	0.0113239890780497
7.52703231736754	0.0119824067989896
7.57580331165659	0.0126397603753181
7.62457430594563	0.0132906017340543
7.67334530023468	0.0139331110563830
7.72211629452373	0.0145655446793819
7.77144705621219	0.0151932835025974
7.82077781790065	0.0158073542893674
7.87010857958912	0.0164061856310244
7.91943934127758	0.0169882903229518
7.96966620873211	0.0175623324903556
8.01989307618664	0.0181161798397216
8.07011994364117	0.0186485234856869
8.12034681109570	0.0191581471580822
8.17188862971250	0.0196563130013266
8.22343044832929	0.0201282461126096
8.27497226694608	0.0205729242144225
8.32651408556287	0.0209894270518160
8.37995066555843	0.0213906169098194
8.43338724555398	0.0217598323715064
8.48682382554954	0.0220963780710338
8.54026040554509	0.0223996721761354
8.59264630622872	0.0226642701130890
8.64503220691234	0.0228961104067512
8.69741810759597	0.0230949438798123
8.74980400827959	0.0232606188179701
8.80130195951982	0.0233911094569718
8.85279991076004	0.0234895310259032
8.90429786200027	0.0235559971240717
8.95579581324049	0.0235907032339219
9.00691883967619	0.0235940137303679
9.05804186611189	0.0235666388434273
9.10916489254759	0.0235089924686888
9.16028791898329	0.0234215574598938
9.21145411122912	0.0233047727623540
9.26262030347494	0.0231593153648556
9.31378649572077	0.0229858606132627
9.36495268796660	0.0227851411036724
9.41654794015576	0.0225559300351791
9.46814319234492	0.0223006597503190
9.51973844453408	0.0220202424246834
9.57133369672324	0.0217156360527727
9.62392663286122	0.0213812827390821
9.67651956899920	0.0210239452914078
9.72911250513718	0.0206447695006716
9.78170544127516	0.0202449354275693
9.83584912150179	0.0198130108205442
9.88999280172842	0.0193618373852605
9.94413648195504	0.0188928003459987
9.99828016218167	0.0184073058816421
10.0540781056737	0.0178912661238592
10.1098760491657	0.0173608466022909
10.1656739926577	0.0168176402569416
10.2214719361497	0.0162632439386539
10.2756340627963	0.0157159140332828
10.3297961894429	0.0151610172037013
10.3839583160894	0.0146000132503546
10.4381204427360	0.0140343492235453
10.4913006965245	0.0134757933375665
10.5444809503131	0.0129154766315033
10.5976612041017	0.0123547261393145
10.6508414578903	0.0117948439131854
10.7036286794831	0.0112412190302220
10.7564159010759	0.0106909376893260
10.8092031226688	0.0101451966793438
10.8619903442616	0.00960515778222234
10.9148514055899	0.00907120853371209
10.9677124669181	0.00854521035113570
11.0205735282463	0.00802822354817919
11.0734345895746	0.00752126453140778
11.1268048985060	0.00702058614105250
11.1801752074375	0.00653208468182312
11.2335455163689	0.00605667181635514
11.2869158253004	0.00559520685055584
11.3412675119695	0.00514042768604258
11.3956191986386	0.00470175725247777
11.4499708853078	0.00427994031354278
11.5043225719769	0.00387566068043712
11.5602445818107	0.00347866381529110
11.6161665916445	0.00310151438244401
11.6720886014783	0.00274476303885497
11.7280106113121	0.00240888998399806
11.7854922362233	0.00208584329315195
11.8429738611344	0.00178566982292621
11.9004554860456	0.00150867003971748
11.9579371109568	0.00125506692382225
12.0138246466191	0.00103107145677939
12.0697121822814	0.000829408007600832
12.1255997179437	0.000650083757054309
12.1814872536060	0.000493040791053862
12.2364081740881	0.000360304761035184
12.2913290945701	0.000248800998994392
12.3462500150521	0.000158303588302397
12.4011709355341	8.85320215153207e-05
12.4557093948871	3.94281613422407e-05
12.5102478542401	1.00607675504935e-05
12.5647863135931	7.96367530831945e-09
12.6193247729461	8.80249922878278e-06
12.6739738559100	3.60075003991267e-05
12.7286229388739	8.10690238945558e-05
12.7832720218378	0.000143392440649027
12.8379211048018	0.000222346554517559
12.8932201372012	0.000318487976421114
12.9485191696007	0.000430251949327777
13.0038182020002	0.000556882766108850
13.0591172343996	0.000697597102274361
13.1157877654014	0.000855566787127159
13.1724582964031	0.00102657930296695
13.2291288274048	0.00120971422500207
13.2857993584066	0.00140403333376274
13.3446243075368	0.00161654764617371
13.4034492566669	0.00183899858259600
13.4622742057971	0.00207028934682023
13.5210991549273	0.00230931773232611
13.5783218161257	0.00254820800596014
13.6355444773240	0.00279235043517346
13.6927671385223	0.00304072565253949
13.7499897997207	0.00329232236081575
13.8061231584122	0.00354129178837925
13.8622565171036	0.00379145687916780
13.9183898757951	0.00404189226872445
13.9745232344866	0.00429169069304728
14.0302633175361	0.00453823113864786
14.0860034005856	0.00478241264356101
14.1417434836351	0.00502340390830483
14.1974835666846	0.00526040006380112
14.2533926250767	0.00549331848328291
14.3093016834687	0.00572067292917480
14.3652107418608	0.00594173306408911
14.4211198002529	0.00615580254401707
14.4777370024593	0.00636478116954139
14.5343542046657	0.00656525537931022
14.5909714068721	0.00675660800413524
14.6475886090785	0.00693826327560794
14.7055282387007	0.00711356360022757
14.7634678683228	0.00727761530887776
14.8214074979450	0.00742993270974484
14.8793471275672	0.00757007938666474
14.9394338470089	0.00770214907106162
14.9995205664506	0.00782032962482401
15.0596072858923	0.00792429539232954
15.1196940053340	0.00801377930087042
15.1785299451618	0.00808716491312598
15.2373658849896	0.00814631502888466
15.2962018248174	0.00819113295656341
15.3550377646452	0.00822157429203760
15.4126282162481	0.00823745349043779
15.4702186678511	0.00823961371229897
15.5278091194541	0.00822814917123288
15.5853995710570	0.00820319839916828
15.6425138397232	0.00816531292397064
15.6996281083894	0.00811455754152070
15.7567423770555	0.00805118654598606
15.8138566457217	0.00797549178295271
15.8711953652715	0.00788743336343271
15.9285340848213	0.00778765119934665
15.9858728043710	0.00767654432463357
16.0432115239208	0.00755454303914483
16.1014495158645	0.00741994992946804
16.1596875078082	0.00727510503758053
16.2179254997519	0.00712054702779190
16.2761634916956	0.00695683925740867
16.3359700634670	0.00677981570409568
16.3957766352384	0.00659442163118128
16.4555832070098	0.00640133613918397
16.5153897787812	0.00620125520354872
16.5772595565287	0.00598766781483790
16.6391293342762	0.00576816021259414
16.7009991120237	0.00554354644749326
16.7628688897712	0.00531464705737134
16.8226291025295	0.00509025889152332
16.8823893152878	0.00486339189483089
16.9421495280461	0.00463479220951427
17.0019097408044	0.00440520077447387
17.0604737135166	0.00417995168498361
17.1190376862287	0.00395514335538352
17.1776016589408	0.00373145117495590
17.2361656316529	0.00350953680810138
17.2943437987857	0.00329148479800277
17.3525219659184	0.00307644897731698
17.4107001330511	0.00286503265611789
17.4688783001839	0.00265781833895644
17.5273181214793	0.00245446906635180
17.5857579427747	0.00225647625258622
17.6441977640701	0.00206436366141218
17.7026375853655	0.00187862776855622
17.7619748377587	0.00169704690706014
17.8213120901519	0.00152298885873524
17.8806493425450	0.00135688558430270
17.9399865949382	0.00119913530894111
18.0009772089185	0.00104607888046402
18.0619678228989	0.000902595032307250
18.1229584368792	0.000769005444430165
18.1839490508595	0.000645591030847390
18.2467391781493	0.000529419528732254
18.3095293054391	0.000424509099163750
18.3723194327289	0.000331034049922403
18.4351095600186	0.000249122089295090
18.4958890311180	0.000180925047940775
18.5566685022173	0.000123676233795957
18.6174479733167	7.73716588229483e-05
18.6782274444160	4.19681373382985e-05
18.7378730347315	1.77449779985669e-05
18.7975186250471	3.83112749676800e-06
18.8571642153626	8.13891405611216e-08
18.9168098056781	6.31767125729454e-06
18.9761161336685	2.22120089169681e-05
19.0354224616590	4.75352919115174e-05
19.0947287896494	8.20219742146603e-05
19.1540351176398	0.000125379250453994
19.2137174724110	0.000177643943586271
19.2733998271821	0.000238217770076263
19.3330821819533	0.000306725462458219
19.3927645367245	0.000382770077506428
19.4536313109237	0.000467653640657870
19.5144980851229	0.000559476944071878
19.5753648593222	0.000657756576354503
19.6362316335214	0.000761993543002775
19.6991702047529	0.000875497219723428
19.7621087759845	0.000994236777143445
19.8250473472160	0.00111761586280424
19.8879859184476	0.00124503018062636
19.9504675490644	0.00137490756928462
20.0129491796813	0.00150755312716821
20.0754308102981	0.00164235912997332
20.1379124409149	0.00177871978258894
20.1988318485020	0.00191259166986368
20.2597512560891	0.00204680936949318
20.3206706636762	0.00218082131360839
20.3815900712632	0.00231408571579948
20.4418628007192	0.00244467815187435
20.5021355301751	0.00257351104120323
20.5624082596310	0.00270009079320729
20.6226809890869	0.00282393992897104
20.6830648171870	0.00294481610278800
20.7434486452870	0.00306203863808756
20.8038324733871	0.00317517730999936
20.8642163014871	0.00328382373519010
20.9254176891409	0.00338896073159888
20.9866190767946	0.00348870319878985
21.0478204644484	0.00358269416916764
21.1090218521021	0.00367060419673394
21.1718545315804	0.00375421378513931
21.2346872110587	0.00383079478796695
21.2975198905370	0.00390007869021972
21.3603525700153	0.00396183070105212
21.4250495998080	0.00401733154712714
21.4897466296008	0.00406444565050059
21.5544436593936	0.00410302348632777
21.6191406891863	0.00413295465326189
21.6817036315996	0.00415360621850416
21.7442665740128	0.00416606906581896
21.8068295164261	0.00417034095960778
21.8693924588393	0.00416645264739864
21.9308388102019	0.00415475095269878
21.9922851615645	0.00413532477263334
22.0537315129272	0.00410828905802951
22.1151778642898	0.00407378665402039
22.1764705511298	0.00403210059137631
22.2377632379697	0.00398334696457830
22.2990559248097	0.00392774294632317
22.3603486116497	0.00386552917749304
22.4223000336916	0.00379619833580898
22.4842514557336	0.00372067696999160
22.5462028777755	0.00363927839565362
22.6081542998175	0.00355233489287051
22.6715496881498	0.00345798999598936
22.7349450764822	0.00335859877508579
22.7983404648145	0.00325456974164121
22.8617358531469	0.00314632509988144
22.9276086030674	0.00302985125185769
22.9934813529880	0.00290979660353410
23.0593541029086	0.00278667116565227
23.1252268528292	0.00266099176944021
23.1892682653520	0.00253685437569444
23.2533096778747	0.00241128182593862
23.3173510903975	0.00228475859397634
23.3813925029203	0.00215776700267289
23.4439303515084	0.00203376420420616
23.5064682000966	0.00191021602607235
23.5690060486847	0.00178755910802888
23.6315438972729	0.00166622130045340
23.6935838954000	0.00154756560348163
23.7556238935271	0.00143102048759145
23.8176638916543	0.00131697324573785
23.8797038897814	0.00120579694230537
23.9420528805491	0.00109732144516096
24.0044018713168	0.000992458005263366
24.0667508620844	0.000891538521258237
24.1290998528521	0.000794875662174811
24.1925523682960	0.000701175428161160
24.2560048837398	0.000612477683745421
24.3194573991837	0.000529048705286335
24.3829099146275	0.000451130483136225
24.4484444382408	0.000376671833023983
24.5139789618541	0.000308538314061087
24.5795134854674	0.000246914568974455
24.6450480090807	0.000191955263780800
24.7108250011305	0.000143620357123028
24.7766019931802	0.000102223478601583
24.8423789852300	6.78314590789841e-05
24.9081559772797	4.04804144266289e-05
24.9720195866552	2.06679164087709e-05
25.0358831960306	7.47816361927060e-06
25.0997468054060	8.63971152041073e-07
25.1636104147814	7.52399657476186e-07
25.2265955481551	6.91611166489243e-06
25.2895806815287	1.91923265499378e-05
25.3525658149024	3.74410820070658e-05
25.4155509482761	6.15009414444917e-05
25.4785556713374	9.11998662516242e-05
25.5415603943987	0.000126328325385388
25.6045651174600	0.000166664428190197
25.6675698405213	0.000211968876442475
25.7315234913094	0.000262773662874622
25.7954771420975	0.000318148339923106
25.8594307928856	0.000377792339986204
25.9233844436737	0.000441391996390877
25.9892426850350	0.000510675571559289
26.0551009263963	0.000583437711310669
26.1209591677576	0.000659297631733344
26.1868174091189	0.000737866763965041
26.2535502444464	0.000819837227595154
26.3202830797740	0.000903762780680433
26.3870159151016	0.000989219821682344
26.4537487504291	0.00107578429202729
26.5184351348136	0.00116035037819940
26.5831215191980	0.00124517080577385
26.6478079035824	0.00132986166480626
26.7124942879669	0.00141404512779120
26.7762428831831	0.00149614980214480
26.8399914783994	0.00157704950187053
26.9037400736156	0.00165640212245079
26.9674886688319	0.00173387672935924
27.0312432274322	0.00180916033693894
27.0949977860326	0.00188193523441047
27.1587523446329	0.00195190486688279
27.2225069032333	0.00201878840081684
27.2871135974660	0.00208314569660091
27.3517202916987	0.00214379955347672
27.4163269859314	0.00220050674029096
27.4809336801641	0.00225304426458882
27.5473600151609	0.00230250020944031
27.6137863501576	0.00234713227910851
27.6802126851544	0.00238676291573743
27.7466390201512	0.00242123978961606
27.8144911660441	0.00245100287405744
27.8823433119370	0.00247514278991528
27.9501954578299	0.00249357443313469
28.0180476037228	0.00250624110331632
28.0836710412897	0.00251297971209242
28.1492944788567	0.00251429369348689
28.2149179164237	0.00251020216409858
28.2805413539907	0.00250074808510779
28.3451053878376	0.00248627698346499
28.4096694216846	0.00246676127634132
28.4742334555315	0.00244230374236520
28.5387974893785	0.00241302721154424
28.6034183056205	0.00237904173219338
28.6680391218626	0.00234053108408394
28.7326599381047	0.00229767256140913
28.7972807543468	0.00225066013813607
28.8628316080457	0.00219894244787718
28.9283824617446	0.00214340059530636
28.9939333154435	0.00208428275017935
29.0594841691424	0.00202185009103675
29.1269556326181	0.00195441451060638
29.1944270960939	0.00188406693834174
29.2618985595696	0.00181112745910605
29.3293700230453	0.00173592466137269
29.3979909106086	0.00165746603003339
29.4666117981718	0.00157737487806125
29.5352326857351	0.00149601559753215
29.6038535732983	0.00141375461409972
29.6701727865302	0.00133374151943906
29.7364919997621	0.00125356220020455
29.8028112129939	0.00117354628223029
29.8691304262258	0.00109401916602719
29.9343704267019	0.00101657445798675
29.9996104271780	0.000940214023029990
30.0648504276541	0.000865230849098870
30.1300904281302	0.000791908982099039
30.1952858095128	0.000720571459290953
30.2604811908953	0.000651432836244728
30.3256765722779	0.000584746277078411
30.3908719536605	0.000520751875307341
30.4569332436822	0.000458886100033383
30.5229945337039	0.000400240248561049
30.5890558237256	0.000345020624405868
30.6551171137473	0.000293416425576712
30.7230813828530	0.000244280233328575
30.7910456519586	0.000199322232948594
30.8590099210643	0.000158690525494187
30.9269741901699	0.000122511708927828
30.9964305818134	9.02488884020880e-05
31.0658869734568	6.28369060616311e-05
31.1353433651002	4.03415641608978e-05
31.2047997567437	2.28044102908276e-05
31.2718985486150	1.05881481044102e-05
31.3389973404864	3.01146724117201e-06
31.4060961323577	4.89862403104732e-08
31.4731949242290	1.65508551266223e-06
31.5391489416833	7.62294923451253e-06
31.6051029591375	1.78614503213298e-05
31.6710569765918	3.22725187469540e-05
31.7370109940461	5.07412936478765e-05
31.8029038201020	7.31141264404550e-05
31.8687966461580	9.92593310014805e-05
31.9346894722139	0.000129015141546933
32.0005822982699	0.000162206220410228
32.0674470725521	0.000199204971311091
32.1343118468343	0.000239336248671605
32.2011766211165	0.000282377474971177
32.2680413953987	0.000328095955300432
32.3369742812759	0.000377774895270849
32.4059071671532	0.000429764930136515
32.4748400530305	0.000483781327359351
32.5437729389077	0.000539533564899303
32.6132976261725	0.000597222114913425
32.6828223134373	0.000656065424614892
32.7523470007020	0.000715751315056065
32.8218716879668	0.000775967819466980
32.8892575400122	0.000834543894371046
32.9566433920577	0.000893041365613280
33.0240292441032	0.000951179311142222
33.0914150961486	0.00100868217945436
33.1579074063846	0.00106453634519309
33.2243997166205	0.00111925348024908
33.2908920268565	0.00117258571354210
33.3573843370924	0.00122429460656946
33.4240362992290	0.00127426827231334
33.4906882613656	0.00132215777093705
33.5573402235022	0.00136775194146282
33.6239921856388	0.00141085276370224
33.6917838285149	0.00145194188103680
33.7595754713910	0.00149007735488008
33.8273671142671	0.00152509194664922
33.8951587571432	0.00155683534289191
33.9652790260747	0.00158608508057613
34.0353992950061	0.00161156035591692
34.1055195639376	0.00163314964312231
34.1756398328691	0.00165076270505739
34.2453776041807	0.00166426678487380
34.3151153754923	0.00167371837658175
34.3848531468039	0.00167908738372357
34.4545909181155	0.00168036475697828
34.5223782426370	0.00167769516746670
34.5901655671585	0.00167119674985160
34.6579528916800	0.00166091375336657
34.7257402162014	0.00164690801162849
34.7928996323729	0.00162943802400676
34.8600590485443	0.00160848237816599
34.9272184647158	0.00158414731686014
34.9943778808873	0.00155655377494471
35.0619929504487	0.00152561782909840
35.1296080200101	0.00149166643986107
35.1972230895715	0.00145486267985107
35.2648381591328	0.00141538145931711
35.3339326818891	0.00137246394415236
35.4030272046454	0.00132715412154144
35.4721217274016	0.00127967072041056
35.5412162501579	0.00123024099132400
35.6131113972494	0.00117699431590611
35.6850065443410	0.00112216747097970
35.7569016914325	0.00106603848503721
35.8287968385241	0.00100888951260248
35.8985499225384	0.000952738544916286
35.9683030065528	0.000896159222536792
36.0380560905672	0.000839414037096303
36.1078091745816	0.000782763791340560
36.1758899819743	0.000727810696265685
36.2439707893671	0.000673432600096437
36.3120515967598	0.000619862671390516
36.3801324041526	0.000567328122315155
36.4478115126495	0.000516348420126241
36.5154906211464	0.000466821267642206
36.5831697296433	0.000418948908700830
36.6508488381403	0.000372924085573392
36.7191711629321	0.000328522146929191
36.7874934877239	0.000286368231669975
36.8558158125157	0.000246628668473807
36.9241381373075	0.000209456924494912
36.9942096873564	0.000174148041355005
37.0642812374052	0.000141825971037546
37.1343527874540	0.000112612579330734
37.2044243375029	8.66133019719521e-05
37.2770714990837	6.31470831783374e-05
37.3497186606646	4.33126804060483e-05
37.4223658222454	2.71713181630219e-05
37.4950129838262	1.47642102024739e-05
37.5648860036314	6.37432514592025e-06
37.6347590234365	1.46140727015060e-06
37.7046320432417	1.07233791657274e-08
37.7745050630469	1.99094816333787e-06
37.8429849056960	7.21499247786767e-06
37.9114647483452	1.56292346787560e-05
37.9799445909944	2.71595467592457e-05
38.0484244336436	4.17181262355851e-05
38.1167683734507	5.91663941724641e-05
38.1851123132578	7.94165669134402e-05
38.2534562530649	0.000102342907495393
38.3218001928720	0.000127808684599156
38.3911454818990	0.000156091752822891
38.4604907709259	0.000186672218901022
38.5298360599529	0.000219375291187106
38.5991813489799	0.000254018081829829
38.6707549934430	0.000291606232081716
38.7423286379060	0.000330838953636369
38.8139022823690	0.000371491215896842
38.8854759268321	0.000413333571166821
38.9573395690528	0.000456307488027148
39.0292032112736	0.000500004300019191
39.1010668534944	0.000544181272508875
39.1729304957152	0.000588596336596021
39.2426006365928	0.000631654962638324
39.3122707774704	0.000674490455645108
39.3819409183480	0.000716885971307226
39.4516110592256	0.000758629548355752
39.5204531079888	0.000799033927366155
39.5892951567520	0.000838403321075004
39.6581372055153	0.000876548328367249
39.7269792542785	0.000913287793656035
39.7961453702529	0.000948610131555409
39.8653114862273	0.000982170455911092
39.9344776022017	0.00101381033788980
40.0036437181761	0.00104338272142323
40.0742469817186	0.00107129598530291
40.1448502452611	0.00109677914199716
40.2154535088036	0.00111971150923204
40.2860567723460	0.00113998705218703
40.3595268224031	0.00115816629174566
40.4329968724601	0.00117328022192860
40.5064669225171	0.00118525736421473
40.5799369725741	0.00119404482437138
40.6513675007179	0.00119949671652695
40.7227980288617	0.00120188241892541
40.7942285570055	0.00120120009443803
40.8656590851494	0.00119746429874799
40.9354139422374	0.00119089804669221
41.0051687993254	0.00118148974962606
41.0749236564134	0.00116929413902950
41.1446785135014	0.00115437954367655
41.2141846577893	0.00113689432387084
41.2836908020773	0.00111688209169040
41.3531969463653	0.00109444630092404
41.4227030906532	0.00106970160462412
41.4930789169469	0.00104242294558812
41.5634547432405	0.00101304552916764
41.6338305695342	0.000981718485968884
41.7042063958279	0.000948599595690529
41.7766738644670	0.000912798805791972
41.8491413331062	0.000875462757872969
41.9216088017454	0.000836786693671461
41.9940762703846	0.000796971361921976
42.0676270896293	0.000755607096667213
42.1411779088741	0.000713500207697214
42.2147287281188	0.000670871871168916
42.2882795473636	0.000627944191777149
42.3592970394703	0.000586419709718469
42.4303145315771	0.000545023603166456
42.5013320236838	0.000503953463764149
42.5723495157906	0.000463403526563343
42.6423081717146	0.000424152205289090
42.7122668276387	0.000385769052728121
42.7822254835628	0.000348426650397737
42.8521841394869	0.000312290977232231
42.9223311803881	0.000277429607569482
42.9924782212893	0.000244095163380155
43.0626252621906	0.000212432351119702
43.1327723030918	0.000182576369849382
43.2042637505405	0.000154137366856335
43.2757551979892	0.000127828491697756
43.3472466454379	0.000103760582369532
43.4187380928867	8.20320283535511e-05
43.4930174384355	6.20263159128580e-05
43.5672967839843	4.47212765868133e-05
43.6415761295332	3.01836753651449e-05
43.7158554750820	1.84644264352557e-05
43.7886851215017	9.74447091937231e-06
43.8615147679214	3.78683877919346e-06
43.9343444143411	5.95495049437501e-07
44.0071740607608	1.59801736325847e-07
44.0780890043289	2.35988331704058e-06
44.1490039478970	7.11313189152356e-06
44.2199188914650	1.43710144159396e-05
44.2908338350331	2.40729980465492e-05
44.3612464402611	3.60532140153230e-05
44.4316590454890	5.02897393416858e-05
44.5020716507170	6.66899347236716e-05
44.5724842559449	8.51514842014451e-05
44.6436666325296	0.000105796204914926
44.7148490091142	0.000128308154000826
44.7860313856988	0.000152553628841745
44.8572137622834	0.000178391667835111
44.9304409819765	0.000206477937700902
45.0036682016695	0.000235923881142557
45.0768954213625	0.000266554552255958
45.1501226410556	0.000298190749972931
45.2247367648061	0.000331270768462530
45.2993508885565	0.000365005760061014
45.3739650123070	0.000399195103943214
45.4485791360575	0.000433638178133971
45.5206102726895	0.000466941537690881
45.5926414093215	0.000500113294708045
45.6646725459534	0.000532974647272329
45.7367036825854	0.000565350604877537
45.8076682830009	0.000596605869157495
45.8786328834164	0.000627062741473017
45.9495974838319	0.000656565650679349
46.0205620842474	0.000684965785353398
46.0917592672627	0.000712207721337980
46.1629564502780	0.000738058548041565
46.2341536332932	0.000762388625318950
46.3053508163085	0.000785077781598916
46.3779951965189	0.000806421707150620
46.4506395767293	0.000825832588381862
46.5232839569396	0.000843212428111619
46.5959283371500	0.000858475522779732
46.6715633469138	0.000872038280273119
46.7471983566776	0.000883155260246035
46.8228333664415	0.000891769979231701
46.8984683762053	0.000897841648820833
46.9719520694971	0.000901280396423195
47.0454357627890	0.000902282622032325
47.1189194560809	0.000900850146299859
47.1924031493727	0.000896998575643840
47.2641650684056	0.000890929895493642
47.3359269874386	0.000882619074463724
47.4076889064715	0.000872115079448774
47.4794508255044	0.000859478240565930
47.5510064906415	0.000844824728514138
47.6225621557785	0.000828201370539247
47.6941178209155	0.000809697772886109
47.7656734860526	0.000789412800040115
47.8382453721548	0.000767130585757135
47.9108172582570	0.000743247033278516
47.9833891443591	0.000717889998737932
48.0559610304613	0.000691194328302784
48.1309236142279	0.000662363654268570
48.2058861979945	0.000632417389660703
48.2808487817611	0.000601522401835483
48.3558113655277	0.000569849691632159
48.4308882648717	0.000537524158958286
48.5059651642157	0.000504771716474207
48.5810420635598	0.000471771380387797
48.6561189629038	0.000438702154598141
48.7288161374927	0.000406783814913140
48.8015133120816	0.000375129473599769
48.8742104866705	0.000343897574649959
48.9469076612594	0.000313243051913823
49.0187802551314	0.000283651871583173
49.0906528490033	0.000254915041608649
49.1625254428753	0.000227169181469717
49.2343980367472	0.000200544670033902
49.3067524167097	0.000174999864182918
49.3791067966722	0.000150837097524635
49.4514611766346	0.000128168026974465
49.5238155565971	0.000107095553946277
49.5979508123623	8.72588278019895e-05
49.6720860681275	6.92887759865877e-05
49.7462213238926	5.32660228186335e-05
49.8203565796578	3.92598044657972e-05
49.8652674347434	3.17807267326992e-05
49.9101782898289	2.50741182106876e-05
49.9550891449145	1.91492387868441e-05
50	1.40137315581462e-05

==> matlab/fig1e.tex <==
0.0100000000000000	4.99950004999500e-05
0.0112590384703905	5.06946369125919e-05
0.0125180769407810	5.25548745748989e-05
0.0137771154111715	5.53041077838840e-05
0.0150361538815620	5.87763046718870e-05
0.0162951923519525	6.28817084487805e-05
0.0175542308223430	6.75542306413198e-05
0.0188132692927335	7.27486305026897e-05
0.0200723077631240	7.84328856698847e-05
0.0218134441469326	8.70627233727772e-05
0.0235545805307411	9.65508199106277e-05
0.0252957169145497	0.000106868725557701
0.0270368532983583	0.000117996150524946
0.0295181432065920	0.000135228513987979
0.0319994331148256	0.000154054394904032
0.0344807230230593	0.000174453963418465
0.0369620129312930	0.000196412505411070
0.0405572013330861	0.000230977366269177
0.0441523897348793	0.000268777638074762
0.0477475781366724	0.000309795077650829
0.0513427665384656	0.000354014075651807
0.0566747420772888	0.000425467253369446
0.0620067176161121	0.000503906533485747
0.0673386931549353	0.000589295564899599
0.0726706686937585	0.000681597317329117
0.0809070434834143	0.000837684384820471
0.0891434182730702	0.00101005100968771
0.0973797930627260	0.00119854531236784
0.105616167852382	0.00140300343330702
0.119428450217403	0.00178123731542793
0.133240732582423	0.00220300612351374
0.147053014947444	0.00266732828612823
0.160865297312465	0.00317313721777986
0.178019219732123	0.00385736122950472
0.195173142151780	0.00460147196477539
0.212327064571438	0.00540295729773204
0.229480986991096	0.00625916667600736
0.248483981448880	0.00726821044010858
0.267486975906665	0.00833709629809806
0.286489970364450	0.00946178362193282
0.305492964822234	0.0106381456444387
0.326939596021466	0.0120226075154305
0.348386227220698	0.0134614965627589
0.369832858419931	0.0149487546599601
0.391279489619163	0.0164783819805396
0.415086736184634	0.0182188360607799
0.438893982750104	0.0199963500153695
0.462701229315575	0.0218033069510864
0.486508475881046	0.0236324081152934
0.512579838010910	0.0256526548043541
0.538651200140773	0.0276825335193833
0.564722562270636	0.0297140272787277
0.590793924400500	0.0317397312141832
0.619005972967117	0.0339174010230794
0.647218021533734	0.0360725601054664
0.675430070100351	0.0381982482441573
0.703642118666968	0.0402883178955811
0.733851831073851	0.0424808103703247
0.764061543480734	0.0446206411575571
0.794271255887618	0.0467030423535940
0.824480968294501	0.0487240818090250
0.856524960901709	0.0507972494893348
0.888568953508918	0.0527948827061021
0.920612946116126	0.0547148278524400
0.952656938723335	0.0565556241098258
0.986351384409508	0.0584049341655754
1.02004583009568	0.0601654307074348
1.05374027578186	0.0618373033897568
1.08743472146803	0.0634212058739749
1.12257805195627	0.0649806217318801
1.15772138244452	0.0664470371521632
1.19286471293276	0.0678223190843161
1.22800804342100	0.0691085704294824
1.26438736782175	0.0703487148598548
1.30076669222249	0.0714986105875643
1.33714601662323	0.0725610683310222
1.37352534102397	0.0735389593500346
1.41092618586320	0.0744592028508398
1.44832703070242	0.0752963128673469
1.48572787554165	0.0760534479880439
1.52312872038087	0.0767337175825406
1.56134640367475	0.0773526170435341
1.59956408696864	0.0778976458245695
1.63778177026252	0.0783719182472791
1.67599945355640	0.0787784446742946
1.71484969660907	0.0791252615640312
1.75369993966175	0.0794080523735300
1.79255018271442	0.0796296772017941
1.83140042576709	0.0797928743490791
1.87072709840390	0.0799012526416879
1.91005377104070	0.0799550920952567
1.94938044367751	0.0799569168848527
1.98870711631432	0.0799091322034610
2.02838611226531	0.0798129794655552
2.06806510821629	0.0796709517087540
2.10774410416728	0.0794852311270076
2.14742310011826	0.0792578931216193
2.18736258820969	0.0789890420480202
2.22730207630111	0.0786819951310638
2.26724156439253	0.0783386236199267
2.30718105248396	0.0779607069145785
2.34731915635702	0.0775478254126118
2.38745726023007	0.0771034525876376
2.42759536410313	0.0766291931361888
2.46773346797619	0.0761265742733031
2.50803462769329	0.0755948557447856
2.54833578741038	0.0750374674857805
2.58863694712748	0.0744557927590689
2.62893810684458	0.0738511497728682
2.66938915757544	0.0732224361780519
2.70984020830630	0.0725731121047732
2.75029125903716	0.0719043795736884
2.79074230976801	0.0712173857024580
2.83134895097666	0.0705104945613702
2.87195559218530	0.0697874115319542
2.91256223339394	0.0690491908484557
2.95316887460259	0.0682968398537598
2.99395288397237	0.0675279589372686
3.03473689334216	0.0667467743187072
3.07552090271194	0.0659542192244683
3.11630491208173	0.0651511861669485
3.15730225154799	0.0643342627388724
3.19829959101425	0.0635084881279726
3.23929693048051	0.0626746954713880
3.28029426994677	0.0618336818670081
3.32155413519608	0.0609807721667854
3.36281400044539	0.0601221074633028
3.40407386569470	0.0592584368772988
3.44533373094400	0.0583904769593722
3.48691858677239	0.0575120433746286
3.52850344260078	0.0566306605271629
3.57008829842917	0.0557470057064251
3.61167315425756	0.0548617261378783
3.65365985811192	0.0539668803942733
3.69564656196628	0.0530716558388156
3.73763326582065	0.0521766670340902
3.77961996967501	0.0512825002085858
3.82210221583512	0.0503791952080727
3.86458446199523	0.0494778938307382
3.90706670815534	0.0485791545710398
3.94954895431544	0.0476835086782485
3.99264150344042	0.0467786818613785
4.03573405256539	0.0458780954860838
4.07882660169036	0.0449822566621644
4.12191915081533	0.0440916457909403
4.16576473103018	0.0431913140337046
4.20961031124503	0.0422973548128532
4.25345589145988	0.0414102268797537
4.29730147167473	0.0405303623059905
4.34208205652409	0.0396396616067175
4.38686264137346	0.0387574045776937
4.43164322622282	0.0378840031484609
4.47642381107218	0.0370198420848525
4.52237971564009	0.0361429907977961
4.56833562020800	0.0352766467961551
4.61429152477591	0.0344211752272438
4.66024742934382	0.0335769130086773
4.70771174380114	0.0327170431178665
4.75517605825846	0.0318698124014899
4.80264037271578	0.0310355374988734
4.85010468717310	0.0302145049955243
4.89744976257724	0.0294089921880558
4.94479483798138	0.0286171777333416
4.99213991338552	0.0278392941083298
5.03948498878966	0.0270755462956785
5.08636308744273	0.0263334414498558
5.13324118609581	0.0256055515951506
5.18011928474888	0.0248920283652932
5.22699738340195	0.0241929991176183
5.27357838501376	0.0235128656089180
5.32015938662558	0.0228472540930186
5.36674038823739	0.0221962463108428
5.41332138984921	0.0215599023757027
5.45976847819635	0.0209400330958751
5.50621556654349	0.0203348266146495
5.55266265489063	0.0197443029772761
5.59910974323777	0.0191684628409677
5.64558241876024	0.0186069880095084
5.69205509428270	0.0180601810475281
5.73852776980517	0.0175280064141015
5.78500044532764	0.0170104111283348
5.83166690899266	0.0165052623299374
5.87833337265768	0.0160146774756186
5.92499983632269	0.0155385698756801
5.97166629998771	0.0150768371352419
6.01871655904510	0.0146257445103661
6.06576681810250	0.0141890278506921
6.11281707715989	0.0137665522128573
6.15986733621728	0.0133581685259920
6.20753009502752	0.0129586741223888
6.25519285383776	0.0125733086369358
6.30285561264800	0.0122018901008837
6.35051837145825	0.0118442238839312
6.39908671418941	0.0114936984462285
6.44765505692057	0.0111570234877301
6.49622339965174	0.0108339691179521
6.54479174238290	0.0105242941830980
6.59477427942936	0.0102193097548923
6.64475681647582	0.00992795882132723
6.69473935352228	0.00964995765019126
6.74472189056874	0.00938501254680044
6.79435030314736	0.00913456661449680
6.84397871572597	0.00889640267636693
6.89360712830458	0.00867021848975726
6.94323554088320	0.00845570469954777
6.99213297011201	0.00825545981865244
7.04103039934083	0.00806594100209426
7.08992782856965	0.00788684381135434
7.13882525779847	0.00771785937119775
7.18736732322589	0.00755979949724314
7.23590938865331	0.00741109743982903
7.28445145408073	0.00727144767532004
7.33299351950815	0.00714054239039594
7.38150321897300	0.00701815280652465
7.43001291843784	0.00690388401590998
7.47852261790269	0.00679743010920857
7.52703231736754	0.00669848472958357
7.57580331165659	0.00660626794190316
7.62457430594563	0.00652102658935830
7.67334530023468	0.00644245497586653
7.72211629452373	0.00637024864021452
7.77144705621219	0.00630338106851331
7.82077781790065	0.00624241021988271
7.87010857958912	0.00618703099796813
7.91943934127758	0.00613694117231444
7.96966620873211	0.00609106813027532
8.01989307618664	0.00605006164860232
8.07011994364117	0.00601361726915664
8.12034681109570	0.00598143508464980
8.17188862971250	0.00595253327985142
8.22343044832929	0.00592750055795986
8.27497226694608	0.00590603254741576
8.32651408556287	0.00588783130167434
8.37995066555843	0.00587210007346363
8.43338724555398	0.00585925495085721
8.48682382554954	0.00584898997388074
8.54026040554509	0.00584100789690716
8.59264630622872	0.00583512188744807
8.64503220691234	0.00583089323973964
8.69741810759597	0.00582806916628147
8.74980400827959	0.00582640571606872
8.80130195951982	0.00582567489813708
8.85279991076004	0.00582562671926446
8.90429786200027	0.00582605631070480
8.95579581324049	0.00582676747072389
9.00691883967619	0.00582756773619888
9.05804186611189	0.00582828823081163
9.10916489254759	0.00582876360570575
9.16028791898329	0.00582883706158340
9.21145411122912	0.00582836036441408
9.26262030347494	0.00582719463662676
9.31378649572077	0.00582520915775199
9.36495268796660	0.00582228167459296
9.41654794015576	0.00581826082275468
9.46814319234492	0.00581306025150221
9.51973844453408	0.00580658109540693
9.57133369672324	0.00579873290150737
9.62392663286122	0.00578923953452077
9.67651956899920	0.00577816214808547
9.72911250513718	0.00576543186921169
9.78170544127516	0.00575098831935462
9.83584912150179	0.00573427491872838
9.88999280172842	0.00571564502305044
9.94413648195504	0.00569506046408658
9.99828016218167	0.00567249173153561
10.0540781056737	0.00564713592125901
10.1098760491657	0.00561963885267715
10.1656739926577	0.00558999606481523
10.2214719361497	0.00555821163040788
10.2756340627963	0.00552532300424437
10.3297961894429	0.00549044854046511
10.3839583160894	0.00545361390108298
10.4381204427360	0.00541485101257674
10.4913006965245	0.00537495204787171
10.5444809503131	0.00533327400700310
10.5976612041017	0.00528986386011110
10.6508414578903	0.00524477315909666
10.7036286794831	0.00519840951310834
10.7564159010759	0.00515050585014911
10.8092031226688	0.00510112526417944
10.8619903442616	0.00505033409904617
10.9148514055899	0.00499812852412143
10.9677124669181	0.00494465256087197
11.0205735282463	0.00488998202246299
11.0734345895746	0.00483419481520308
11.1268048985060	0.00477681915332893
11.1801752074375	0.00471847255211504
11.2335455163689	0.00465924115600580
11.2869158253004	0.00459921211926662
11.3412675119695	0.00453735109877520
11.3956191986386	0.00447484989943362
11.4499708853078	0.00441180332400811
11.5043225719769	0.00434830609520448
11.5602445818107	0.00428260415731530
11.6161665916445	0.00421662995001886
11.6720886014783	0.00415048592012889
11.7280106113121	0.00408427324664312
11.7854922362233	0.00401624806142306
11.8429738611344	0.00394836480649046
11.9004554860456	0.00388072872669942
11.9579371109568	0.00381344250740591
12.0138246466191	0.00374845348717148
12.0697121822814	0.00368398124280896
12.1255997179437	0.00362011296475656
12.1814872536060	0.00355693268389650
12.2364081740881	0.00349559433512766
12.2913290945701	0.00343507396321202
12.3462500150521	0.00337544251467545
12.4011709355341	0.00331676741000076
12.4557093948871	0.00325951093137577
12.5102478542401	0.00320332134138926
12.5647863135931	0.00314825467261343
12.6193247729461	0.00309436317549350
12.6739738559100	0.00304159030364040
12.7286229388739	0.00299009266127281
12.7832720218378	0.00293991186682319
12.8379211048018	0.00289108556668280
12.8932201372012	0.00284309226092468
12.9485191696007	0.00279655275164055
13.0038182020002	0.00275149420255060
13.0591172343996	0.00270793964164416
13.1157877654014	0.00266488555128076
13.1724582964031	0.00262344832629037
13.2291288274048	0.00258363987981186
13.2857993584066	0.00254546780345518
13.3446243075368	0.00250757946505102
13.4034492566669	0.00247145824916914
13.4622742057971	0.00243709853992686
13.5210991549273	0.00240449021794485
13.5783218161257	0.00237443728767065
13.6355444773240	0.00234601164124028
13.6927671385223	0.00231919221964161
13.7499897997207	0.00229395446964530
13.8061231584122	0.00227070737691281
13.8622565171036	0.00224892674623650
13.9183898757951	0.00222858012434112
13.9745232344866	0.00220963242281988
14.0302633175361	0.00219216490835207
14.0860034005856	0.00217600105567635
14.1417434836351	0.00216109927132931
14.1974835666846	0.00214741605304092
14.2533926250767	0.00213487016963351
14.3093016834687	0.00212345761449165
14.3652107418608	0.00211312908100655
14.4211198002529	0.00210383403268188
14.4777370024593	0.00209542180248293
14.5343542046657	0.00208796190186304
14.5909714068721	0.00208139823034791
14.6475886090785	0.00207567414982644
14.7055282387007	0.00207062623818454
14.7634678683228	0.00206633628743907
14.8214074979450	0.00206274187089971
14.8793471275672	0.00205978079603077
14.9394338470089	0.00205731297711459
14.9995205664506	0.00205539099668843
15.0596072858923	0.00205394596095923
15.1196940053340	0.00205291017171228
15.1785299451618	0.00205222868906184
15.2373658849896	0.00205181423551923
15.2962018248174	0.00205160590529680
15.3550377646452	0.00205154455342082
15.4126282162481	0.00205157178047110
15.4702186678511	0.00205163230785443
15.5278091194541	0.00205167483125720
15.5853995710570	0.00205165014160690
15.6425138397232	0.00205151295079394
15.6996281083894	0.00205121898794690
15.7567423770555	0.00205072554870035
15.8138566457217	0.00204999230685405
15.8711953652715	0.00204897679286379
15.9285340848213	0.00204764485684203
15.9858728043710	0.00204596196610231
16.0432115239208	0.00204389624568785
16.1014495158645	0.00204137620260095
16.1596875078082	0.00203840264267162
16.2179254997519	0.00203494938105338
16.2761634916956	0.00203099319615206
16.3359700634670	0.00202638575008331
16.3957766352384	0.00202120702323662
16.4555832070098	0.00201544004101265
16.5153897787812	0.00200907113824486
16.5772595565287	0.00200183802116826
16.6391293342762	0.00199394074640420
16.7009991120237	0.00198537323235069
16.7628688897712	0.00197613304441232
16.8226291025295	0.00196657025422921
16.8823893152878	0.00195638397149569
16.9421495280461	0.00194557955633931
17.0019097408044	0.00193416518446283
17.0604737135166	0.00192239803032329
17.1190376862287	0.00191006757420913
17.1776016589408	0.00189718757633167
17.2361656316529	0.00188377400171017
17.2943437987857	0.00186993835727625
17.3525219659184	0.00185561316437057
17.4107001330511	0.00184081888247083
17.4688783001839	0.00182557769522629
17.5273181214793	0.00180984208288680
17.5857579427747	0.00179370483526950
17.6441977640701	0.00177719206266034
17.7026375853655	0.00176033117342302
17.7619748377587	0.00174288464923460
17.8213120901519	0.00172513944191354
17.8806493425450	0.00170712664682241
17.9399865949382	0.00168887824401042
18.0009772089185	0.00166991033304490
18.0619678228989	0.00165076400737168
18.1229584368792	0.00163147501377303
18.1839490508595	0.00161207954838291
18.2467391781493	0.00159203917873691
18.3095293054391	0.00157196425356319
18.3723194327289	0.00155189357443677
18.4351095600186	0.00153186587406541
18.4958890311180	0.00151255680968024
18.5566685022173	0.00149335823103595
18.6174479733167	0.00147430315882159
18.6782274444160	0.00145542403995163
18.7378730347315	0.00143709896241769
18.7975186250471	0.00141900290858717
18.8571642153626	0.00140116344969129
18.9168098056781	0.00138360725687764
18.9761161336685	0.00136645728499321
19.0354224616590	0.00134963674757030
19.0947287896494	0.00133316797338733
19.1540351176398	0.00131707215573144
19.2137174724110	0.00130127109950499
19.2733998271821	0.00128588684991448
19.3330821819533	0.00127093638602100
19.3927645367245	0.00125643536573531
19.4536313109237	0.00124212435405462
19.5144980851229	0.00122830899900419
19.5753648593222	0.00121500051651404
19.6362316335214	0.00120220864110962
19.6991702047529	0.00118953341517921
19.7621087759845	0.00117742622630958
19.8250473472160	0.00116589154589890
19.8879859184476	0.00115493223019453
19.9504675490644	0.00114462282652460
20.0129491796813	0.00113488057141445
20.0754308102981	0.00112570222987404
20.1379124409149	0.00111708313533470
20.1988318485020	0.00110921218437396
20.2597512560891	0.00110185942755082
20.3206706636762	0.00109501553011461
20.3815900712632	0.00108867005077555
20.4418628007192	0.00108287112942479
20.5021355301751	0.00107753596774041
20.5624082596310	0.00107265035317846
20.6226809890869	0.00106819926625148
20.6830648171870	0.00106415982851734
20.7434486452870	0.00106052333201468
20.8038324733871	0.00105727137650793
20.8642163014871	0.00105438505841987
20.9254176891409	0.00105181285482506
20.9866190767946	0.00104957493143426
21.0478204644484	0.00104764909630064
21.1090218521021	0.00104601299307490
21.1718545315804	0.00104461102843004
21.2346872110587	0.00104346533548726
21.2975198905370	0.00104255006093765
21.3603525700153	0.00104183960586266
21.4250495998080	0.00104129528054052
21.4897466296008	0.00104091274559151
21.5544436593936	0.00104066345383302
21.6191406891863	0.00104051963323019
21.6817036315996	0.00104045534905777
21.7442665740128	0.00104043946254628
21.8068295164261	0.00104044745969786
21.8693924588393	0.00104045580976530
21.9308388102019	0.00104044242886900
21.9922851615645	0.00104038612346259
22.0537315129272	0.00104026607832816
22.1151778642898	0.00104006263699908
22.1764705511298	0.00103975810136458
22.2377632379697	0.00103933394346360
22.2990559248097	0.00103877282435531
22.3603486116497	0.00103805874657853
22.4223000336916	0.00103716649823782
22.4842514557336	0.00103608818890215
22.5462028777755	0.00103481008731829
22.6081542998175	0.00103332000826633
22.6715496881498	0.00103156451444782
22.7349450764822	0.00102956493865563
22.7983404648145	0.00102731160793757
22.8617358531469	0.00102479663727704
22.9276086030674	0.00102189949144235
22.9934813529880	0.00101870693038694
23.0593541029086	0.00101521412823691
23.1252268528292	0.00101141837421543
23.1892682653520	0.00100743689064623
23.2533096778747	0.00100316815548956
23.3173510903975	0.000998613281947466
23.3813925029203	0.000993775124354837
23.4439303515084	0.000988781364188271
23.5064682000966	0.000983526318021777
23.5690060486847	0.000978015619436893
23.6315438972729	0.000972256295757469
23.6935838954000	0.000966305283674630
23.7556238935271	0.000960126232919789
23.8176638916543	0.000953728401830883
23.8797038897814	0.000947122186551128
23.9420528805491	0.000940284606281254
24.0044018713168	0.000933259913451951
24.0667508620844	0.000926060481196915
24.1290998528521	0.000918699605576225
24.1925523682960	0.000911057218360216
24.2560048837398	0.000903277115807189
24.3194573991837	0.000895374494717153
24.3829099146275	0.000887365275943405
24.4484444382408	0.000878998842252046
24.5139789618541	0.000870554243079673
24.5795134854674	0.000862049412802934
24.6450480090807	0.000853502812592538
24.7108250011305	0.000844901498210483
24.7766019931802	0.000836295455683697
24.8423789852300	0.000827702794890022
24.9081559772797	0.000819141834157522
24.9720195866552	0.000810877602232785
25.0358831960306	0.000802676518499492
25.0997468054060	0.000794554065698085
25.1636104147814	0.000786525623363051
25.2265955481551	0.000778714451334605
25.2895806815287	0.000771023057020588
25.3525658149024	0.000763464364855502
25.4155509482761	0.000756050992839244
25.4785556713374	0.000748792903721323
25.5415603943987	0.000741703592514506
25.6045651174600	0.000734793369882296
25.6675698405213	0.000728072094999684
25.7315234913094	0.000721452382579522
25.7954771420975	0.000715045439810624
25.8594307928856	0.000708858748750028
25.9233844436737	0.000702899230281275
25.9892426850350	0.000697006239926110
26.0551009263963	0.000691366134759483
26.1209591677576	0.000685983055831173
26.1868174091189	0.000680860506284934
26.2535502444464	0.000675938460964003
26.3202830797740	0.000671287915995420
26.3870159151016	0.000666908833093656
26.4537487504291	0.000662800551772595
26.5184351348136	0.000659075377462519
26.5831215191980	0.000655600528276682
26.6478079035824	0.000652372259211757
26.7124942879669	0.000649386335730680
26.7762428831831	0.000646676090589036
26.8399914783994	0.000644190650463334
26.9037400736156	0.000641923345345264
26.9674886688319	0.000639867161600936
27.0312432274322	0.000638014474188394
27.0949977860326	0.000636356954456080
27.1587523446329	0.000634885414163241
27.2225069032333	0.000633590486864241
27.2871135974660	0.000632448531321769
27.3517202916987	0.000631467042919607
27.4163269859314	0.000630634526797107
27.4809336801641	0.000629939512430300
27.5473600151609	0.000629356112907712
27.6137863501576	0.000628892418895875
27.6802126851544	0.000628534667377638
27.7466390201512	0.000628269392569428
27.8144911660441	0.000628080038992991
27.8823433119370	0.000627958336830688
27.9501954578299	0.000627889260550496
28.0180476037228	0.000627858396623820
28.0836710412897	0.000627851710885786
28.1492944788567	0.000627854504617494
28.2149179164237	0.000627853822295417
28.2805413539907	0.000627837415474380
28.3451053878376	0.000627794557527854
28.4096694216846	0.000627713782929607
28.4742334555315	0.000627584077778197
28.5387974893785	0.000627395235661839
28.6034183056205	0.000627137441630777
28.6680391218626	0.000626801233187052
28.7326599381047	0.000626377476592351
28.7972807543468	0.000625857971201773
28.8628316080457	0.000625225538005041
28.9283824617446	0.000624479288306675
28.9939333154435	0.000623612159426781
29.0594841691424	0.000622618173851586
29.1269556326181	0.000621457231430749
29.1944270960939	0.000620151177506121
29.2618985595696	0.000618695376498605
29.3293700230453	0.000617086480390666
29.3979909106086	0.000615290784050636
29.4666117981718	0.000613332156787288
29.5352326857351	0.000611209162288392
29.6038535732983	0.000608921737656849
29.6701727865302	0.000606555755474505
29.7364919997621	0.000604038219175931
29.8028112129939	0.000601370870974787
29.8691304262258	0.000598556541462094
29.9343704267019	0.000595648190195746
29.9996104271780	0.000592604836044608
30.0648504276541	0.000589430652765731
30.1300904281302	0.000586130711035952
30.1952858095128	0.000582713170962263
30.2604811908953	0.000579181644479251
30.3256765722779	0.000575542346308873
30.3908719536605	0.000571802248319312
30.4569332436822	0.000567917394139100
30.5229945337039	0.000563944593183287
30.5890558237256	0.000559891886586793
30.6551171137473	0.000555767958516784
30.7230813828530	0.000551460537060815
30.7910456519586	0.000547097118705203
30.8590099210643	0.000542687486814673
30.9269741901699	0.000538241970922014
30.9964305818134	0.000533672868747046
31.0658869734568	0.000529088291104125
31.1353433651002	0.000524498981135715
31.2047997567437	0.000519916077034285
31.2718985486150	0.000515505407397771
31.3389973404864	0.000511120745504130
31.4060961323577	0.000506771359038504
31.4731949242290	0.000502466646689692
31.5391489416833	0.000498287967178452
31.6051029591375	0.000494169641052756
31.6710569765918	0.000490119457401162
31.7370109940461	0.000486145174284813
31.8029038201020	0.000482257930266600
31.8687966461580	0.000478460762280848
31.9346894722139	0.000474759934577952
32.0005822982699	0.000471161573622455
32.0674470725521	0.000467620879230678
32.1343118468343	0.000464196899353763
32.2011766211165	0.000460894204651046
32.2680413953987	0.000457717157244193
32.3369742812759	0.000454577607026264
32.4059071671532	0.000451579122432629
32.4748400530305	0.000448724223515137
32.5437729389077	0.000446015186742555
32.6132976261725	0.000443432510530211
32.6828223134373	0.000441000753615051
32.7523470007020	0.000438719823837520
32.8218716879668	0.000436589397921400
32.8892575400122	0.000434667432669186
32.9566433920577	0.000432884354749600
33.0240292441032	0.000431237787395703
33.0914150961486	0.000429725174842321
33.1579074063846	0.000428361102160100
33.2243997166205	0.000427120926993768
33.2908920268565	0.000426000442598429
33.3573843370924	0.000424995344146548
33.4240362992290	0.000424099071717409
33.4906882613656	0.000423308767201843
33.5573402235022	0.000422618617933343
33.6239921856388	0.000422022822135375
33.6917838285149	0.000421507505988000
33.7595754713910	0.000421076650520706
33.8273671142671	0.000420722934694382
33.8951587571432	0.000420439198394485
33.9652790260747	0.000420211725383272
34.0353992950061	0.000420042802915355
34.1055195639376	0.000419923566190112
34.1756398328691	0.000419845536656143
34.2453776041807	0.000419800579716681
34.3151153754923	0.000419779361885227
34.3848531468039	0.000419773088200352
34.4545909181155	0.000419773497479557
34.5223782426370	0.000419772757478063
34.5901655671585	0.000419763104923887
34.6579528916800	0.000419736985333982
34.7257402162014	0.000419687423517231
34.7928996323729	0.000419608739119899
34.8600590485443	0.000419493950933238
34.9272184647158	0.000419336673236105
34.9943778808873	0.000419131170901631
35.0619929504487	0.000418870239238328
35.1296080200101	0.000418549605452987
35.1972230895715	0.000418164109115522
35.2648381591328	0.000417709338586398
35.3339326818891	0.000417169058826682
35.4030272046454	0.000416548263947615
35.4721217274016	0.000415843202786538
35.5412162501579	0.000415051007238727
35.6131113972494	0.000414131846964890
35.6850065443410	0.000413113462376459
35.7569016914325	0.000411993836993735
35.8287968385241	0.000410772043456278
35.8985499225384	0.000409488882379917
35.9683030065528	0.000408109216838151
36.0380560905672	0.000406633329504979
36.1078091745816	0.000405062404312898
36.1758899819743	0.000403439262497503
36.2439707893671	0.000401729002108329
36.3120515967598	0.000399933672793928
36.3801324041526	0.000398056059860311
36.4478115126495	0.000396111259209746
36.5154906211464	0.000394091618653458
36.5831697296433	0.000392000624690080
36.6508488381403	0.000389842392859030
36.7191711629321	0.000387600093518919
36.7874934877239	0.000385298472094390
36.8558158125157	0.000382942280122192
36.9241381373075	0.000380536822343117
36.9942096873564	0.000378024547025051
37.0642812374052	0.000375472268669640
37.1343527874540	0.000372885927022610
37.2044243375029	0.000370271962232662
37.2770714990837	0.000367539942300169
37.3497186606646	0.000364792492244021
37.4223658222454	0.000362036579363276
37.4950129838262	0.000359279624015415
37.5648860036314	0.000356634041072585
37.6347590234365	0.000354000681040971
37.7046320432417	0.000351385588238846
37.7745050630469	0.000348795028136838
37.8429849056960	0.000346285981884025
37.9114647483452	0.000343811852871495
37.9799445909944	0.000341377733011613
38.0484244336436	0.000338988800470885
38.1167683734507	0.000336654739519798
38.1851123132578	0.000334375181986026
38.2534562530649	0.000332154230003878
38.3218001928720	0.000329995990290421
38.3911454818990	0.000327874285456235
38.4604907709259	0.000325824601810560
38.5298360599529	0.000323849919453296
38.5991813489799	0.000321953176640938
38.6707549934430	0.000320080111788878
38.7423286379060	0.000318295089478148
38.8139022823690	0.000316599702193639
38.8854759268321	0.000314995491203300
38.9573395690528	0.000313477806364452
39.0292032112736	0.000312053649275372
39.1010668534944	0.000310722836475922
39.1729304957152	0.000309485140821393
39.2426006365928	0.000308373668218133
39.3122707774704	0.000307347940674635
39.3819409183480	0.000306406254135021
39.4516110592256	0.000305546876431381
39.5204531079888	0.000304776676630038
39.5892951567520	0.000304082344948654
39.6581372055153	0.000303460942042946
39.7269792542785	0.000302909550496983
39.7961453702529	0.000302422998028779
39.8653114862273	0.000302000267682853
39.9344776022017	0.000301637317137378
40.0036437181761	0.000301330206964324
40.0742469817186	0.000301070165552820
40.1448502452611	0.000300859252835908
40.2154535088036	0.000300692365906804
40.2860567723460	0.000300564628370006
40.3595268224031	0.000300468081650652
40.4329968724601	0.000300402601832592
40.5064669225171	0.000300361955621905
40.5799369725741	0.000300340340178823
40.6513675007179	0.000300332235365966
40.7227980288617	0.000300331082067336
40.7942285570055	0.000300331211278363
40.8656590851494	0.000300327422258662
40.9354139422374	0.000300315212846270
41.0051687993254	0.000300289579708760
41.0749236564134	0.000300245685839197
41.1446785135014	0.000300179187625227
41.2141846577893	0.000300086445046360
41.2836908020773	0.000299963023440047
41.3531969463653	0.000299804882308213
41.4227030906532	0.000299608531824800
41.4930789169469	0.000299367615714572
41.5634547432405	0.000299080922835713
41.6338305695342	0.000298745291081727
41.7042063958279	0.000298358194843647
41.7766738644670	0.000297903628395807
41.8491413331062	0.000297389866579094
41.9216088017454	0.000296814792861140
41.9940762703846	0.000296177057909611
42.0676270896293	0.000295464886415009
42.1411779088741	0.000294686302713384
42.2147287281188	0.000293840631694646
42.2882795473636	0.000292928020300001
42.3592970394703	0.000291983982862347
42.4303145315771	0.000290978644594125
42.5013320236838	0.000289912783957199
42.5723495157906	0.000288787832032154
42.6423081717146	0.000287623705308119
42.7122668276387	0.000286405702798810
42.7822254835628	0.000285135718042959
42.8521841394869	0.000283816195808123
42.9223311803881	0.000282446213447983
42.9924782212893	0.000281031918161892
43.0626252621906	0.000279576150810796
43.1327723030918	0.000278082241134773
43.2042637505405	0.000276524225675031
43.2757551979892	0.000274933975700210
43.3472466454379	0.000273315195984707
43.4187380928867	0.000271672043622243
43.4930174384355	0.000269943738012541
43.5672967839843	0.000268198445938531
43.6415761295332	0.000266440723107282
43.7158554750820	0.000264675572662216
43.7886851215017	0.000262942674815010
43.8615147679214	0.000261212010181242
43.9343444143411	0.000259487902453055
44.0071740607608	0.000257774967354408
44.0780890043289	0.000256122270548197
44.1490039478970	0.000254488416639307
44.2199188914650	0.000252877082505295
44.2908338350331	0.000251292105815564
44.3612464402611	0.000249748209992231
44.4316590454890	0.000248237269425111
44.5020716507170	0.000246762282918834
44.5724842559449	0.000245326335943314
44.6436666325296	0.000243917446596604
44.7148490091142	0.000242554040131133
44.7860313856988	0.000241238351046413
44.8572137622834	0.000239972662693518
44.9304409819765	0.000238725074966677
45.0036682016695	0.000237534334389121
45.0768954213625	0.000236401729117702
45.1501226410556	0.000235328593132339
45.2247367648061	0.000234297529104379
45.2993508885565	0.000233329857676587
45.3739650123070	0.000232425619148208
45.4485791360575	0.000231584915030099
45.5206102726895	0.000230833533241496
45.5926414093215	0.000230140482412737
45.6646725459534	0.000229504667043903
45.7367036825854	0.000228925039761062
45.8076682830009	0.000228407802388374
45.8786328834164	0.000227942191782430
45.9495974838319	0.000227526201588899
46.0205620842474	0.000227157900189355
46.0917592672627	0.000226834294335429
46.1629564502780	0.000226554044052782
46.2341536332932	0.000226314330877979
46.3053508163085	0.000226112469219216
46.3779951965189	0.000225942710892306
46.4506395767293	0.000225806090276732
46.5232839569396	0.000225699005119295
46.5959283371500	0.000225618083416748
46.6715633469138	0.000225558064840735
46.7471983566776	0.000225518471785825
46.8228333664415	0.000225494859481701
46.8984683762053	0.000225483182902238
46.9719520694971	0.000225479584735810
47.0454357627890	0.000225479494622661
47.1189194560809	0.000225478873002034
47.1924031493727	0.000225474094495642
47.2641650684056	0.000225462150102978
47.3359269874386	0.000225439438611523
47.4076889064715	0.000225402521694898
47.4794508255044	0.000225348385555583
47.5510064906415	0.000225274516381772
47.6225621557785	0.000225177773869613
47.6941178209155	0.000225055300230311
47.7656734860526	0.000224904705464033
47.8382453721548	0.000224721108527628
47.9108172582570	0.000224504033147796
47.9833891443591	0.000224251266981608
48.0559610304613	0.000223961138174108
48.1309236142279	0.000223620835437820
48.2058861979945	0.000223237600490253
48.2808487817611	0.000222809998804718
48.3558113655277	0.000222337255613896
48.4308882648717	0.000221818203763537
48.5059651642157	0.000221252935950850
48.5810420635598	0.000220641126477899
48.6561189629038	0.000219983107077338
48.7288161374927	0.000219302618030588
48.8015133120816	0.000218579962917864
48.8742104866705	0.000217815838445449
48.9469076612594	0.000217011468823407
49.0187802551314	0.000216178191762111
49.0906528490033	0.000215308418099648
49.1625254428753	0.000214403640879943
49.2343980367472	0.000213465807434960
49.3067524167097	0.000212490558145641
49.3791067966722	0.000211486123250597
49.4514611766346	0.000210454681446243
49.5238155565971	0.000209398825657349
49.5979508123623	0.000208294625370816
49.6720860681275	0.000207170522741003
49.7462213238926	0.000206029330378755
49.8203565796578	0.000204874261765448
49.8652674347434	0.000204169221563225
49.9101782898289	0.000203460978667970
49.9550891449145	0.000202750238892637
50	0.000202037723952045

==> matlab/fig1f.tex <==
0.0100000000000000	0.999800029996000
0.0112590384703905	0.999746516306114
0.0125180769407810	0.999686669150807
0.0137771154111715	0.999620490236814
0.0150361538815620	0.999547981451222
0.0162951923519525	0.999469144861352
0.0175542308223430	0.999383982714626
0.0188132692927335	0.999292497438424
0.0200723077631240	0.999194691639934
0.0218134441469326	0.999049026110358
0.0235545805307411	0.998891286259290
0.0252957169145497	0.998721480677940
0.0270368532983583	0.998539618611896
0.0295181432065920	0.998259633399819
0.0319994331148256	0.997955213776736
0.0344807230230593	0.997626393361441
0.0369620129312930	0.997273208446303
0.0405572013330861	0.996718326030207
0.0441523897348793	0.996112504272920
0.0477475781366724	0.995455883191139
0.0513427665384656	0.994748614365615
0.0566747420772888	0.993606766536334
0.0620067176161121	0.992354455902971
0.0673386931549353	0.990992315022759
0.0726706686937585	0.989521030262253
0.0809070434834143	0.987035536148638
0.0891434182730702	0.984294357407666
0.0973797930627260	0.981300752709109
0.105616167852382	0.978058261666228
0.119428450217403	0.972072600108685
0.133240732582423	0.965417436444845
0.147053014947444	0.958114307237919
0.160865297312465	0.950186528075755
0.178019219732123	0.939508791910594
0.195173142151780	0.927956988680518
0.212327064571438	0.915584884691808
0.229480986991096	0.902448654957245
0.248483981448880	0.887074576703056
0.267486975906665	0.870914859491846
0.286489970364450	0.854051513784933
0.305492964822234	0.836566917989084
0.326939596021466	0.816190367415294
0.348386227220698	0.795242969254340
0.369832858419931	0.773837810022964
0.391279489619163	0.752083962168042
0.415086736184634	0.727653619372640
0.438893982750104	0.703056211781011
0.462701229315575	0.678416651862803
0.486508475881046	0.653849736045703
0.512579838010910	0.627152904293646
0.538651200140773	0.600790248675836
0.564722562270636	0.574868672403631
0.590793924400500	0.549480115262447
0.619005972967117	0.522696854408856
0.647218021533734	0.496708771687239
0.675430070100351	0.471579045609459
0.703642118666968	0.447355119017616
0.733851831073851	0.422457726571263
0.764061543480734	0.398661947328557
0.794271255887618	0.375978491952792
0.824480968294501	0.354405901017839
0.856524960901709	0.332724409599116
0.888568953508918	0.312255432858699
0.920612946116126	0.292966423685945
0.952656938723335	0.274818365316204
0.986351384409508	0.256918083492195
1.02004583009568	0.240175979524887
1.05374027578186	0.224534654926361
1.08743472146803	0.209935466613354
1.12257805195627	0.195755230471040
1.15772138244452	0.182578635689194
1.19286471293276	0.170341167423247
1.22800804342100	0.158980418295071
1.26438736782175	0.148079835799458
1.30076669222249	0.137991338996170
1.33714601662323	0.128655124159325
1.37352534102397	0.120014923370838
1.41092618586320	0.111802266941041
1.44832703070242	0.104216138049260
1.48572787554165	0.0972069202993722
1.52312872038087	0.0907286555113451
1.56134640367475	0.0846132020520364
1.59956408696864	0.0789660410487695
1.63778177026252	0.0737487720667720
1.67599945355640	0.0689261380039887
1.71484969660907	0.0643948539080454
1.75369993966175	0.0602068615156619
1.79255018271442	0.0563337153255208
1.83140042576709	0.0527494165893606
1.87072709840390	0.0493910600047700
1.91005377104070	0.0462818478564986
1.94938044367751	0.0434012566554292
1.98870711631432	0.0407305614222670
2.02838611226531	0.0382313004868084
2.06806510821629	0.0359123128598012
2.10774410416728	0.0337589962938608
2.14742310011826	0.0317580277843719
2.18736258820969	0.0298854690658981
2.22730207630111	0.0281436251487990
2.26724156439253	0.0265221601532970
2.30718105248396	0.0250116326335888
2.34731915635702	0.0235966527661899
2.38745726023007	0.0222769943848606
2.42759536410313	0.0210453336537748
2.46773346797619	0.0198949680277665
2.50803462769329	0.0188155372335822
2.54833578741038	0.0178061837539287
2.58863694712748	0.0168616900295668
2.62893810684458	0.0159772703409949
2.66938915757544	0.0151455485811026
2.70984020830630	0.0143658443343243
2.75029125903716	0.0136344095968302
2.79074230976801	0.0129477981938799
2.83134895097666	0.0123004350740081
2.87195559218530	0.0116920926792390
2.91256223339394	0.0111200510308097
2.95316887460259	0.0105818029873307
2.99395288397237	0.0100728883051056
3.03473689334216	0.00959356809070423
3.07552090271194	0.00914184576433350
3.11630491208173	0.00871587650177780
3.15730225154799	0.00831191257887327
3.19829959101425	0.00793064541929051
3.23929693048051	0.00757059154945073
3.28029426994677	0.00723037706598500
3.32155413519608	0.00690672625246054
3.36281400044539	0.00660067682277225
3.40407386569470	0.00631111260654373
3.44533373094400	0.00603699762447188
3.48691858677239	0.00577537978218829
3.52850344260078	0.00552756295846933
3.57008829842917	0.00529269650110518
3.61167315425756	0.00506998929117694
3.65365985811192	0.00485671685075451
3.69564656196628	0.00465438397584095
3.73763326582065	0.00446233386640763
3.77961996967501	0.00427995458229172
3.82210221583512	0.00410468269932204
3.86458446199523	0.00393817628213329
3.90706670815534	0.00377992142828142
3.94954895431544	0.00362943856698000
3.99264150344042	0.00348427455759063
4.03573405256539	0.00334621030450382
4.07882660169036	0.00321483817965094
4.12191915081533	0.00308977726156486
4.16576473103018	0.00296864095206452
4.20961031124503	0.00285331889620309
4.25345589145988	0.00274348309590646
4.29730147167473	0.00263882669429644
4.34208205652409	0.00253698625346792
4.38686264137346	0.00243996249726405
4.43164322622282	0.00234748739087765
4.47642381107218	0.00225930996004943
4.52237971564009	0.00217304005569516
4.56833562020800	0.00209081078917671
4.61429152477591	0.00201239928951005
4.66024742934382	0.00193759676013911
4.70771174380114	0.00186391998771022
4.75517605825846	0.00179368225160561
4.80264037271578	0.00172669436277100
4.85010468717310	0.00166277905783612
4.89744976257724	0.00160191991146280
4.94479483798138	0.00154379786133585
4.99213991338552	0.00148826768234638
5.03948498878966	0.00143519298753314
5.08636308744273	0.00138493519009951
5.13324118609581	0.00133684204531058
5.18011928474888	0.00129080345559456
5.22699738340195	0.00124671575255425
5.27357838501376	0.00120474330223726
5.32015938662558	0.00116451033216225
5.36674038823739	0.00112593164128406
5.41332138984921	0.00108892682396971
5.45976847819635	0.00105351996535226
5.50621556654349	0.00101953136994132
5.55266265489063	0.000986893845678065
5.59910974323777	0.000955543861150617
5.64558241876024	0.000925405054453030
5.69205509428270	0.000896438083097867
5.73852776980517	0.000868589023055205
5.78500044532764	0.000841806805661768
5.83166690899266	0.000815937681250535
5.87833337265768	0.000791049100059411
5.92499983632269	0.000767097049499580
5.97166629998771	0.000744039791566998
6.01871655904510	0.000721658575513676
6.06576681810250	0.000700108178604165
6.11281707715989	0.000679352060411373
6.15986733621728	0.000659355531805420
6.20753009502752	0.000639839445085980
6.25519285383776	0.000621036524928478
6.30285561264800	0.000602915880957479
6.35051837145825	0.000585448164788110
6.39908671418941	0.000568291350871186
6.44765505692057	0.000551755505589583
6.49622339965174	0.000535813978986538
6.54479174238290	0.000520441439698623
6.59477427942936	0.000505189984933026
6.64475681647582	0.000490490678371798
6.69473935352228	0.000476319810927856
6.74472189056874	0.000462654847557974
6.79435030314736	0.000449566088971972
6.84397871572597	0.000436935012651472
6.89360712830458	0.000424742627001966
6.94323554088320	0.000412970849681749
6.99213297011201	0.000401767057656047
7.04103039934083	0.000390939154715723
7.08992782856965	0.000380472167885498
7.13882525779847	0.000370351812687730
7.18736732322589	0.000360634417585120
7.23590938865331	0.000351232465762236
7.28445145408073	0.000342133794479331
7.33299351950815	0.000333326782587379
7.38150321897300	0.000324805917271451
7.43001291843784	0.000316554633234581
7.47852261790269	0.000308562796275112
7.52703231736754	0.000300820712313568
7.57580331165659	0.000293279333675156
7.62457430594563	0.000285972009679515
7.67334530023468	0.000278890106416767
7.72211629452373	0.000272025358030685
7.77144705621219	0.000265294645311454
7.82077781790065	0.000258770158925815
7.87010857958912	0.000252444386828802
7.91943934127758	0.000246310133270705
7.96966620873211	0.000240254092990505
8.01989307618664	0.000234382474381106
8.07011994364117	0.000228688599369451
8.12034681109570	0.000223166069455951
8.17188862971250	0.000217670662043238
8.22343044832929	0.000212342883700869
8.27497226694608	0.000207176653416672
8.32651408556287	0.000202166145254421
8.37995066555843	0.000197129892328776
8.43338724555398	0.000192249062576682
8.48682382554954	0.000187517951294176
8.54026040554509	0.000182931095908320
8.59264630622872	0.000178569410725744
8.64503220691234	0.000174336610749125
8.69741810759597	0.000170228164589275
8.74980400827959	0.000166239725158145
8.80130195951982	0.000162431819636575
8.85279991076004	0.000158732050857163
8.90429786200027	0.000155136763783507
8.95579581324049	0.000151642446343808
9.00691883967619	0.000148270107727962
9.05804186611189	0.000144990772335502
9.10916489254759	0.000141801386543626
9.16028791898329	0.000138699012785973
9.21145411122912	0.000135678310935987
9.26262030347494	0.000132739209776584
9.31378649572077	0.000129879084337160
9.36495268796660	0.000127095407412438
9.41654794015576	0.000124363329489995
9.46814319234492	0.000121704110206203
9.51973844453408	0.000119115435438822
9.57133369672324	0.000116595076178148
9.62392663286122	0.000114094067176787
9.67651956899920	0.000111659619307277
9.72911250513718	0.000109289622538451
9.78170544127516	0.000106982044303950
9.83584912150179	0.000104669566324589
9.88999280172842	0.000102419108951879
9.94413648195504	0.000100228690756435
9.99828016218167	9.80964036234503e-05
10.0540781056737	9.59578486017221e-05
10.1098760491657	9.38771427622910e-05
10.1656739926577	9.18524219753692e-05
10.2214719361497	8.98818916844493e-05
10.2756340627963	8.80193247890867e-05
10.3297961894429	8.62046663735933e-05
10.3839583160894	8.44364479703178e-05
10.4381204427360	8.27132532612437e-05
10.4913006965245	8.10637825794401e-05
10.5444809503131	7.94551524261337e-05
10.5976612041017	7.78861574751853e-05
10.6508414578903	7.63556336259979e-05
10.7036286794831	7.48733575112467e-05
10.7564159010759	7.34268153853736e-05
10.8092031226688	7.20149802104353e-05
10.8619903442616	7.06368591641804e-05
10.9148514055899	6.92896329251885e-05
10.9677124669181	6.79743205213791e-05
11.0205735282463	6.66900205178532e-05
11.0734345895746	6.54358609977391e-05
11.1268048985060	6.41993383046882e-05
11.1801752074375	6.29918400265053e-05
11.2335455163689	6.18125537309033e-05
11.2869158253004	6.06606933521617e-05
11.3412675119695	5.95150530310688e-05
11.3956191986386	5.83962903526737e-05
11.4499708853078	5.73036533078684e-05
11.5043225719769	5.62364142838688e-05
11.5602445818107	5.51641081913784e-05
11.6161665916445	5.41172017137522e-05
11.6720886014783	5.30949773377572e-05
11.7280106113121	5.20967410523144e-05
11.7854922362233	5.10949596998459e-05
11.8429738611344	5.01171087075767e-05
11.9004554860456	4.91625063229733e-05
11.9579371109568	4.82304933144274e-05
12.0138246466191	4.73453796506723e-05
12.0697121822814	4.64804500084937e-05
12.1255997179437	4.56351553104482e-05
12.1814872536060	4.48089638034101e-05
12.2364081740881	4.40151733768151e-05
12.2913290945701	4.32388599901035e-05
12.3462500150521	4.24795645130411e-05
12.4011709355341	4.17368418076697e-05
12.4557093948871	4.10152652077994e-05
12.5102478542401	4.03091957610532e-05
12.5647863135931	3.96182357700436e-05
12.6193247729461	3.89419993711297e-05
12.6739738559100	3.82787839227062e-05
12.7286229388739	3.76296103231153e-05
12.7832720218378	3.69941237499495e-05
12.8379211048018	3.63719797846090e-05
12.8932201372012	3.57556764813985e-05
12.9485191696007	3.51523564005589e-05
13.0038182020002	3.45616930936873e-05
13.0591172343996	3.39833696374453e-05
13.1157877654014	3.34031837738702e-05
13.1724582964031	3.28353128337576e-05
13.2291288274048	3.22794448248359e-05
13.2857993584066	3.17352769271889e-05
13.3446243075368	3.11824826243252e-05
13.4034492566669	3.06416592603149e-05
13.4622742057971	3.01124974351850e-05
13.5210991549273	2.95946970283107e-05
13.5783218161257	2.91016251375974e-05
13.6355444773240	2.86187684727323e-05
13.6927671385223	2.81458743891009e-05
13.7499897997207	2.76826974943456e-05
13.8061231584122	2.72375490383623e-05
13.8622565171036	2.68013032548254e-05
13.9183898757951	2.63737475565174e-05
13.9745232344866	2.59546752491484e-05
14.0302633175361	2.55467350231273e-05
14.0860034005856	2.51467701484776e-05
14.1417434836351	2.47545944348601e-05
14.1974835666846	2.43700267384790e-05
14.2533926250767	2.39917586473230e-05
14.3093016834687	2.36207943803365e-05
14.3652107418608	2.32569655192615e-05
14.4211198002529	2.29001081549571e-05
14.4777370024593	2.25456720909221e-05
14.5343542046657	2.21980604016472e-05
14.5909714068721	2.18571161615830e-05
14.6475886090785	2.15226866350967e-05
14.7055282387007	2.11870353670181e-05
14.7634678683228	2.08578959505853e-05
14.8214074979450	2.05351175076335e-05
14.8793471275672	2.02185532190926e-05
14.9394338470089	1.98966689836819e-05
14.9995205664506	1.95811593186717e-05
15.0596072858923	1.92718734643484e-05
15.1196940053340	1.89686648007887e-05
15.1785299451618	1.86775193046113e-05
15.2373658849896	1.83919336007102e-05
15.2962018248174	1.81117808762828e-05
15.3550377646452	1.78369376774373e-05
15.4126282162481	1.75729391078090e-05
15.4702186678511	1.73138026879659e-05
15.5278091194541	1.70594214432800e-05
15.5853995710570	1.68096911327115e-05
15.6425138397232	1.65665190510921e-05
15.6996281083894	1.63277248081596e-05
15.7567423770555	1.60932142414838e-05
15.8138566457217	1.58628955411975e-05
15.8711953652715	1.56357981620069e-05
15.9285340848213	1.54127471007940e-05
15.9858728043710	1.51936562173922e-05
16.0432115239208	1.49784415018467e-05
16.1014495158645	1.47637349888064e-05
16.1596875078082	1.45528589249755e-05
16.2179254997519	1.43457316597049e-05
16.2761634916956	1.41422735641943e-05
16.3359700634670	1.39370727328411e-05
16.3957766352384	1.37355774742640e-05
16.4555832070098	1.35377078367834e-05
16.5153897787812	1.33433858725899e-05
16.5772595565287	1.31460126772768e-05
16.6391293342762	1.29522728168619e-05
16.7009991120237	1.27620863819742e-05
16.7628688897712	1.25753755046937e-05
16.8226291025295	1.23982594557849e-05
16.8823893152878	1.22242485054856e-05
16.9421495280461	1.20532776030123e-05
17.0019097408044	1.18852832808792e-05
17.0604737135166	1.17234798714573e-05
17.1190376862287	1.15644187023642e-05
17.1776016589408	1.14080442290193e-05
17.2361656316529	1.12543022141230e-05
17.2943437987857	1.11041271880801e-05
17.3525219659184	1.09564470647978e-05
17.4107001330511	1.08112123032936e-05
17.4688783001839	1.06683745057349e-05
17.5273181214793	1.05272597847070e-05
17.5857579427747	1.03884691019617e-05
17.6441977640701	1.02519567076898e-05
17.7026375853655	1.01176778986867e-05
17.7619748377587	9.98357741580296e-06
17.8213120901519	9.85168993153076e-06
17.8806493425450	9.72197179314152e-06
17.9399865949382	9.59438034858242e-06
18.0009772089185	9.46540629501178e-06
18.0619678228989	9.33859085968708e-06
18.1229584368792	9.21389085932219e-06
18.1839490508595	9.09126411453984e-06
18.2467391781493	8.96714175233558e-06
18.3095293054391	8.84512922370778e-06
18.3723194327289	8.72518366421197e-06
18.4351095600186	8.60726322137823e-06
18.4958890311180	8.49500917508622e-06
18.5566685022173	8.38457811864804e-06
18.6174479733167	8.27593466132311e-06
18.6782274444160	8.16904421089888e-06
18.7378730347315	8.06581945560330e-06
18.7975186250471	7.96421909690135e-06
18.8571642153626	7.86421257338900e-06
18.9168098056781	7.76576999200483e-06
18.9761161336685	7.66940903473046e-06
19.0354224616590	7.57453724640157e-06
19.0947287896494	7.48112711070012e-06
19.1540351176398	7.38915170234078e-06
19.2137174724110	7.29801487783627e-06
19.2733998271821	7.20827807057747e-06
19.3330821819533	7.11991556534904e-06
19.3927645367245	7.03290219601541e-06
19.4536313109237	6.94552604187368e-06
19.5144980851229	6.85950192107801e-06
19.5753648593222	6.77480481893666e-06
19.6362316335214	6.69141025876434e-06
19.6991702047529	6.60652142675753e-06
19.7621087759845	6.52297380488209e-06
19.8250473472160	6.44074205738656e-06
19.8879859184476	6.35980140485011e-06
19.9504675490644	6.28070154205167e-06
20.0129491796813	6.20282701101218e-06
20.0754308102981	6.12615511546000e-06
20.1379124409149	6.05066364783153e-06
20.1988318485020	5.97817546174609e-06
20.2597512560891	5.90676903820746e-06
20.3206706636762	5.83642507203719e-06
20.3815900712632	5.76712465861332e-06
20.4418628007192	5.69956872904156e-06
20.5021355301751	5.63299862906346e-06
20.5624082596310	5.56739715382818e-06
20.6226809890869	5.50274744761018e-06
20.6830648171870	5.43891640661694e-06
20.7434486452870	5.37600780027809e-06
20.8038324733871	5.31400568570707e-06
20.8642163014871	5.25289444042027e-06
20.9254176891409	5.19184913929215e-06
20.9866190767946	5.13168764923555e-06
21.0478204644484	5.07239466654569e-06
21.1090218521021	5.01395519564787e-06
21.1718545315804	4.95483056927826e-06
21.2346872110587	4.89657449537289e-06
21.2975198905370	4.83917171444907e-06
21.3603525700153	4.78260727874815e-06
21.4250495998080	4.72522505841612e-06
21.4897466296008	4.66870049157121e-06
21.5544436593936	4.61301824812006e-06
21.6191406891863	4.55816331657015e-06
21.6817036315996	4.50589082017088e-06
21.7442665740128	4.45436518554543e-06
21.8068295164261	4.40357364927646e-06
21.8693924588393	4.35350370159015e-06
21.9308388102019	4.30501789653683e-06
21.9922851615645	4.25720493462579e-06
22.0537315129272	4.21005364690504e-06
22.1151778642898	4.16355308003833e-06
22.1764705511298	4.11780638990729e-06
22.2377632379697	4.07268602356423e-06
22.2990559248097	4.02818172313161e-06
22.3603486116497	3.98428342612332e-06
22.4223000336916	3.94051907923671e-06
22.4842514557336	3.89735374842832e-06
22.5462028777755	3.85477762570847e-06
22.6081542998175	3.81278108986086e-06
22.6715496881498	3.77039585901742e-06
22.7349450764822	3.72859774488066e-06
22.7983404648145	3.68737701891900e-06
22.8617358531469	3.64672414008005e-06
22.9276086030674	3.60507415577163e-06
22.9934813529880	3.56401687117818e-06
23.0593541029086	3.52354219752311e-06
23.1252268528292	3.48364024573825e-06
23.1892682653520	3.44538746483111e-06
23.2533096778747	3.40765810595932e-06
23.3173510903975	3.37044360119329e-06
23.3813925029203	3.33373554572240e-06
23.4439303515084	3.29837017929504e-06
23.5064682000966	3.26347236301511e-06
23.5690060486847	3.22903470156898e-06
23.6315438972729	3.19504993570378e-06
23.6935838954000	3.16177619437902e-06
23.7556238935271	3.12893432294698e-06
23.8176638916543	3.09651761474101e-06
23.8797038897814	3.06451948424699e-06
23.9420528805491	3.03277716991011e-06
24.0044018713168	3.00144463611097e-06
24.0667508620844	2.97051555325716e-06
24.1290998528521	2.93998370548792e-06
24.1925523682960	2.90931300914099e-06
24.2560048837398	2.87904109331102e-06
24.3194573991837	2.84916175429530e-06
24.3829099146275	2.81966890065602e-06
24.4484444382408	2.78960769419846e-06
24.5139789618541	2.75994590290083e-06
24.5795134854674	2.73067717743407e-06
24.6450480090807	2.70179528587391e-06
24.7108250011305	2.67318936035037e-06
24.7766019931802	2.64496090305367e-06
24.8423789852300	2.61710395460667e-06
24.9081559772797	2.58961266507497e-06
24.9720195866552	2.56326548448295e-06
25.0358831960306	2.53725242353806e-06
25.0997468054060	2.51156841217733e-06
25.1636104147814	2.48620846984071e-06
25.2265955481551	2.46151000864433e-06
25.2895806815287	2.43711739113728e-06
25.3525658149024	2.41302608520162e-06
25.4155509482761	2.38923163685414e-06
25.4785556713374	2.36572240415943e-06
25.5415603943987	2.34250152734639e-06
25.6045651174600	2.31956477384609e-06
25.6675698405213	2.29690798337211e-06
25.7315234913094	2.27419207075527e-06
25.7954771420975	2.25175620073990e-06
25.8594307928856	2.22959624189923e-06
25.9233844436737	2.20770813371968e-06
25.9892426850350	2.18544808347273e-06
26.0551009263963	2.16346780222820e-06
26.1209591677576	2.14176308236283e-06
26.1868174091189	2.12032978987526e-06
26.2535502444464	2.09888456130333e-06
26.3202830797740	2.07770969499818e-06
26.3870159151016	2.05680111223460e-06
26.4537487504291	2.03615480587451e-06
26.5184351348136	2.01638826121962e-06
26.5831215191980	1.99686092986883e-06
26.6478079035824	1.97756934725426e-06
26.7124942879669	1.95851010719163e-06
26.7762428831831	1.93995123154915e-06
26.8399914783994	1.92161160588096e-06
26.9037400736156	1.90348813017133e-06
26.9674886688319	1.88557775540728e-06
27.0312432274322	1.86787583657957e-06
27.0949977860326	1.85038110835888e-06
27.1587523446329	1.83309066827384e-06
27.2225069032333	1.81600166116630e-06
27.2871135974660	1.79888685604729e-06
27.3517202916987	1.78197314522212e-06
27.4163269859314	1.76525770072621e-06
27.4809336801641	1.74873774087178e-06
27.5473600151609	1.73195343955196e-06
27.6137863501576	1.71536997226147e-06
27.6802126851544	1.69898446291851e-06
27.7466390201512	1.68279408336648e-06
27.8144911660441	1.66645475041049e-06
27.8823433119370	1.65031319782416e-06
27.9501954578299	1.63436656042648e-06
28.0180476037228	1.61861202133228e-06
28.0836710412897	1.60355509557069e-06
28.1492944788567	1.58867280091302e-06
28.2149179164237	1.57396271313453e-06
28.2805413539907	1.55942244717188e-06
28.3451053878376	1.54528036829045e-06
28.4096694216846	1.53129820167255e-06
28.4742334555315	1.51747378288877e-06
28.5387974893785	1.50380498160277e-06
28.6034183056205	1.49027788157977e-06
28.6680391218626	1.47690250294698e-06
28.7326599381047	1.46367680870027e-06
28.7972807543468	1.45059879366346e-06
28.8628316080457	1.43748141322474e-06
28.9283824617446	1.42451193428719e-06
28.9939333154435	1.41168836067962e-06
29.0594841691424	1.39900872758469e-06
29.1269556326181	1.38610587612457e-06
29.1944270960939	1.37335139906845e-06
29.2618985595696	1.36074325414023e-06
29.3293700230453	1.34827943177684e-06
29.3979909106086	1.33574927120537e-06
29.4666117981718	1.32336430026132e-06
29.5352326857351	1.31112250526233e-06
29.6038535732983	1.29902190502664e-06
29.6701727865302	1.28745952024588e-06
29.7364919997621	1.27602546450154e-06
29.8028112129939	1.26471803279910e-06
29.8691304262258	1.25353554650800e-06
29.9343704267019	1.24265534098763e-06
29.9996104271780	1.23189289872115e-06
30.0648504276541	1.22124669379976e-06
30.1300904281302	1.21071522332704e-06
30.1952858095128	1.20030409390536e-06
30.2604811908953	1.19000460871993e-06
30.3256765722779	1.17981533449034e-06
30.3908719536605	1.16973485935277e-06
30.4569332436822	1.15963004928084e-06
30.5229945337039	1.14963409432424e-06
30.5890558237256	1.13974559062464e-06
30.6551171137473	1.12996315539635e-06
30.7230813828530	1.12000818538464e-06
30.7910456519586	1.11016258043851e-06
30.8590099210643	1.10042490224253e-06
30.9269741901699	1.09079373449706e-06
30.9964305818134	1.08105971148002e-06
31.0658869734568	1.07143400489861e-06
31.1353433651002	1.06191517189832e-06
31.2047997567437	1.05250179199359e-06
31.2718985486150	1.04350676746519e-06
31.3389973404864	1.03460761158032e-06
31.4060961323577	1.02580310107761e-06
31.4731949242290	1.01709203086336e-06
31.5391489416833	1.00861949255878e-06
31.6051029591375	1.00023497528656e-06
31.6710569765918	9.91937384201796e-07
31.7370109940461	9.83725640311428e-07
31.8029038201020	9.75606181345666e-07
31.8687966461580	9.67570303756947e-07
31.9346894722139	9.59616977408627e-07
32.0005822982699	9.51745186943266e-07
32.0674470725521	9.43839604838848e-07
32.1343118468343	9.36015920498156e-07
32.2011766211165	9.28273118119738e-07
32.2680413953987	9.20610196568155e-07
32.3369742812759	9.12792844256195e-07
32.4059071671532	9.05058276619220e-07
32.4748400530305	8.97405444065912e-07
32.5437729389077	8.89833312494492e-07
32.6132976261725	8.82276881046601e-07
32.6828223134373	8.74800475859963e-07
32.7523470007020	8.67403082253280e-07
32.8218716879668	8.60083700520576e-07
32.8892575400122	8.53063008332425e-07
32.9566433920577	8.46113792740088e-07
33.0240292441032	8.39235182447047e-07
33.0914150961486	8.32426318520641e-07
33.1579074063846	8.25775279540234e-07
33.2243997166205	8.19190522911902e-07
33.2908920268565	8.12671257694000e-07
33.3573843370924	8.06216703932329e-07
33.4240362992290	7.99810824594199e-07
33.4906882613656	7.93468431040377e-07
33.5573402235022	7.87188769883455e-07
33.6239921856388	7.80971098144143e-07
33.6917838285149	7.74709943082446e-07
33.7595754713910	7.68511397226853e-07
33.8273671142671	7.62374710925609e-07
33.8951587571432	7.56299144976240e-07
33.9652790260747	7.50078414867506e-07
34.0353992950061	7.43921501116697e-07
34.1055195639376	7.37827619862810e-07
34.1756398328691	7.31795998452895e-07
34.2453776041807	7.25858276103271e-07
34.3151153754923	7.19980644268460e-07
34.3848531468039	7.14162374797263e-07
34.4545909181155	7.08402749809994e-07
34.5223782426370	7.02859746773858e-07
34.5901655671585	6.97370843916181e-07
34.6579528916800	6.91935408949954e-07
34.7257402162014	6.86552818191357e-07
34.7928996323729	6.81271593322483e-07
34.8600590485443	6.76041044126199e-07
34.9272184647158	6.70860588309262e-07
34.9943778808873	6.65729651368280e-07
35.0619929504487	6.60613352868588e-07
35.1296080200101	6.55546102206402e-07
35.1972230895715	6.50527336310839e-07
35.2648381591328	6.45556499636822e-07
35.3339326818891	6.40525841874365e-07
35.4030272046454	6.35544084322180e-07
35.4721217274016	6.30610657779647e-07
35.5412162501579	6.25725000759731e-07
35.6131113972494	6.20691429525638e-07
35.6850065443410	6.15708363733126e-07
35.7569016914325	6.10775196586166e-07
35.8287968385241	6.05891329775797e-07
35.8985499225384	6.01199534794437e-07
35.9683030065528	5.96553059429750e-07
36.0380560905672	5.91951379466601e-07
36.1078091745816	5.87393977749400e-07
36.1758899819743	5.82988046792740e-07
36.2439707893671	5.78623342304687e-07
36.3120515967598	5.74299402310818e-07
36.3801324041526	5.70015770864121e-07
36.4478115126495	5.65796921568387e-07
36.5154906211464	5.61617025475100e-07
36.5831697296433	5.57475651852013e-07
36.6508488381403	5.53372375512551e-07
36.7191711629321	5.49268317049230e-07
36.7874934877239	5.45202229489171e-07
36.8558158125157	5.41173692103138e-07
36.9241381373075	5.37182289589849e-07
36.9942096873564	5.33126840756426e-07
37.0642812374052	5.29109584944620e-07
37.1343527874540	5.25130091399688e-07
37.2044243375029	5.21187935023347e-07
37.2770714990837	5.17139849953700e-07
37.3497186606646	5.13130985113410e-07
37.4223658222454	5.09160885463027e-07
37.4950129838262	5.05229102109689e-07
37.5648860036314	5.01483196804138e-07
37.6347590234365	4.97771938817562e-07
37.7046320432417	4.94094944354430e-07
37.7745050630469	4.90451834569326e-07
37.8429849056960	4.86913881175569e-07
37.9114647483452	4.83407767916403e-07
37.9799445909944	4.79933151599423e-07
38.0484244336436	4.76489693339551e-07
38.1167683734507	4.73083800793937e-07
38.1851123132578	4.69708280948780e-07
38.2534562530649	4.66362809401862e-07
38.3218001928720	4.63047065785555e-07
38.3911454818990	4.59712800686826e-07
38.4604907709259	4.56408488928947e-07
38.5298360599529	4.53133808231816e-07
38.5991813489799	4.49888440353015e-07
38.6707549934430	4.46569192970794e-07
38.7423286379060	4.43280496642028e-07
38.8139022823690	4.40022014593503e-07
38.8854759268321	4.36793414374564e-07
38.9573395690528	4.33581465763403e-07
39.0292032112736	4.30398982825703e-07
39.1010668534944	4.27245641824404e-07
39.1729304957152	4.24121123164006e-07
39.2426006365928	4.21119192474313e-07
39.3122707774704	4.18143771030879e-07
39.3819409183480	4.15194578449903e-07
39.4516110592256	4.12271337800880e-07
39.5204531079888	4.09408065947369e-07
39.5892951567520	4.06569605031441e-07
39.6581372055153	4.03755697540949e-07
39.7269792542785	4.00966089076129e-07
39.7961453702529	3.98187566173838e-07
39.8653114862273	3.95433066087508e-07
39.9344776022017	3.92702340040132e-07
40.0036437181761	3.89995142254832e-07
40.0742469817186	3.87255708261929e-07
40.1448502452611	3.84540282301251e-07
40.2154535088036	3.81848612361968e-07
40.2860567723460	3.79180449513714e-07
40.3595268224031	3.76428641767790e-07
40.4329968724601	3.73701748960449e-07
40.5064669225171	3.70999500917375e-07
40.5799369725741	3.68321630875697e-07
40.6513675007179	3.65741220341540e-07
40.7227980288617	3.63183365074634e-07
40.7942285570055	3.60647828930633e-07
40.8656590851494	3.58134378644208e-07
40.9354139422374	3.55700984881438e-07
41.0051687993254	3.53288221154340e-07
41.0749236564134	3.50895877964130e-07
41.1446785135014	3.48523748289584e-07
41.2141846577893	3.46179978798405e-07
41.2836908020773	3.43855875798658e-07
41.3531969463653	3.41551241620216e-07
41.4227030906532	3.39265880906743e-07
41.4930789169469	3.36971364246718e-07
41.5634547432405	3.34696210390191e-07
41.6338305695342	3.32440223613218e-07
41.7042063958279	3.30203210495867e-07
41.7766738644670	3.27919337235653e-07
41.8491413331062	3.25655173345699e-07
41.9216088017454	3.23410515095388e-07
41.9940762703846	3.21185161206492e-07
42.0676270896293	3.18946074503981e-07
42.1411779088741	3.16726463414312e-07
42.2147287281188	3.14526125034272e-07
42.2882795473636	3.12344858922326e-07
42.3592970394703	3.10256635094121e-07
42.4303145315771	3.08185831587117e-07
42.5013320236838	3.06132274323123e-07
42.5723495157906	3.04095791249805e-07
42.6423081717146	3.02106199932852e-07
42.7122668276387	3.00132851752969e-07
42.7822254835628	2.98175587855073e-07
42.8521841394869	2.96234251193438e-07
42.9223311803881	2.94303522492987e-07
42.9924782212893	2.92388496087579e-07
43.0626252621906	2.90489018997617e-07
43.1327723030918	2.88604939979303e-07
43.2042637505405	2.86700440289504e-07
43.2757551979892	2.84811622754372e-07
43.3472466454379	2.82938332687958e-07
43.4187380928867	2.81080417181297e-07
43.4930174384355	2.79166173343745e-07
43.5672967839843	2.77268195825939e-07
43.6415761295332	2.75386319058721e-07
43.7158554750820	2.73520379435547e-07
43.7886851215017	2.71706174742057e-07
43.8615147679214	2.69906985144827e-07
43.9343444143411	2.68122661780492e-07
44.0071740607608	2.66353057504518e-07
44.0780890043289	2.64643981578920e-07
44.1490039478970	2.62948590322329e-07
44.2199188914650	2.61266752469710e-07
44.2908338350331	2.59598338222496e-07
44.3612464402611	2.57954897094519e-07
44.4316590454890	2.56324439279952e-07
44.5020716507170	2.54706841902365e-07
44.5724842559449	2.53101983439799e-07
44.6436666325296	2.51492406162042e-07
44.7148490091142	2.49895602231095e-07
44.7860313856988	2.48311450211174e-07
44.8572137622834	2.46739830011129e-07
44.9304409819765	2.45136014047971e-07
45.0036682016695	2.43545206718710e-07
45.0768954213625	2.41967281624440e-07
45.1501226410556	2.40402113796653e-07
45.2247367648061	2.38820296205654e-07
45.2993508885565	2.37251466196695e-07
45.3739650123070	2.35695496029871e-07
45.4485791360575	2.34152259428523e-07
45.5206102726895	2.32674409406888e-07
45.5926414093215	2.31208199192922e-07
45.6646725459534	2.29753518957587e-07
45.7367036825854	2.28310260078857e-07
45.8076682830009	2.26899435356565e-07
45.8786328834164	2.25499490385564e-07
45.9495974838319	2.24110324649764e-07
46.0205620842474	2.22731838714730e-07
46.0917592672627	2.21359468271906e-07
46.1629564502780	2.19997650469196e-07
46.2341536332932	2.18646288093665e-07
46.3053508163085	2.17305284975480e-07
46.3779951965189	2.15947602344518e-07
46.4506395767293	2.14600505377355e-07
46.5232839569396	2.13263895195404e-07
46.5959283371500	2.11937673995841e-07
46.6715633469138	2.10567789950144e-07
46.7471983566776	2.09208955042864e-07
46.8228333664415	2.07861062512537e-07
46.8984683762053	2.06524006799154e-07
46.9719520694971	2.05235261313359e-07
47.0454357627890	2.03956551753985e-07
47.1189194560809	2.02687784491266e-07
47.1924031493727	2.01428866912863e-07
47.2641650684056	2.00208865135105e-07
47.3359269874386	1.98998085106142e-07
47.4076889064715	1.97796443313264e-07
47.4794508255044	1.96603857124699e-07
47.5510064906415	1.95423633866541e-07
47.6225621557785	1.94252252733586e-07
47.6941178209155	1.93089634358483e-07
47.7656734860526	1.91935700203708e-07
47.8382453721548	1.90774168419003e-07
47.9108172582570	1.89621409106003e-07
47.9833891443591	1.88477342886592e-07
48.0559610304613	1.87341891219288e-07
48.1309236142279	1.86177997379229e-07
48.2058861979945	1.85023127358195e-07
48.2808487817611	1.83877197337979e-07
48.3558113655277	1.82740124407201e-07
48.4308882648717	1.81610112591057e-07
48.5059651642157	1.80488821130436e-07
48.5810420635598	1.79376169402151e-07
48.6561189629038	1.78272077651230e-07
48.7288161374927	1.77211065366311e-07
48.8015133120816	1.76157934152590e-07
48.8742104866705	1.75112613872584e-07
48.9469076612594	1.74075035115887e-07
49.0187802551314	1.73056768314589e-07
49.0906528490033	1.72045935570974e-07
49.1625254428753	1.71042471856828e-07
49.2343980367472	1.70046312806543e-07
49.3067524167097	1.69050789949157e-07
49.3791067966722	1.68062541110164e-07
49.4514611766346	1.67081502608689e-07
49.5238155565971	1.66107611413275e-07
49.5979508123623	1.65117097708834e-07
49.6720860681275	1.64133955561211e-07
49.7462213238926	1.63158119241248e-07
49.8203565796578	1.62189523702477e-07
49.8652674347434	1.61606246859411e-07
49.9101782898289	1.61025589474927e-07
49.9550891449145	1.60447537446239e-07
50	1.59872076759060e-07

==> matlab/fig2a1.tex <==
0	0
3.12051768709077e-05	-0.00787369034618651
0.000123247465088009	-0.0155924420689221
0.000274005133664098	-0.0231813962061601
0.000481673961753604	-0.0306552801671605
0.000713809851289472	-0.0372349021090394
0.000988976029187675	-0.0437342343434616
0.00130618789204285	-0.0501572914483143
0.00166451462634225	-0.0565074104917646
0.00243385236027419	-0.0680858434496856
0.00333597610348449	-0.0794379328825616
0.00436597171693060	-0.0905755632731874
0.00551922806815863	-0.101508563598473
0.00733998937814040	-0.116542699016257
0.00938434984725876	-0.131207802260801
0.0116417072040053	-0.145520139329038
0.0141020773089440	-0.159493638412595
0.0172942634167791	-0.175758910209280
0.0207476229924763	-0.191575601579473
0.0244478573750041	-0.206959611232289
0.0283814231447567	-0.221925091992885
0.0329098810009214	-0.237742498667264
0.0376835688455081	-0.253094551427718
0.0426876065701292	-0.267994866714143
0.0479078260235549	-0.282455971022869
0.0536637706346826	-0.297321803343721
0.0596322932645951	-0.311719825265615
0.0657988024143176	-0.325662195831298
0.0721493642726288	-0.339160364492348
0.0790017435244982	-0.352868646298847
0.0860277500802081	-0.366111010451447
0.0932133615917448	-0.378898919019640
0.100545172944069	-0.391243339446521
0.108349462365756	-0.403681124505208
0.116285507730586	-0.415657730061584
0.124340001913400	-0.427184421698671
0.132500227059220	-0.438272094143760
0.141103808356606	-0.449371327389898
0.149795958527738	-0.460016920638366
0.158564196005470	-0.470220263974952
0.167396609436811	-0.479992446552837
0.176643281236958	-0.489714975612939
0.185935013374690	-0.498994348561773
0.195260249208426	-0.507842286786822
0.204607989266652	-0.516270246138424
0.214341658417795	-0.524601346049518
0.224077256040916	-0.532502817343790
0.233804246722608	-0.539986845603444
0.243512643060277	-0.547065362295353
0.253580321126100	-0.554009978991295
0.263607682805197	-0.560541564065375
0.273585310907601	-0.566672851493217
0.283504329398816	-0.572416314539925
0.293758587305755	-0.577996325540420
0.303931536078036	-0.583182936229540
0.314014977621736	-0.587989481450428
0.324001249221005	-0.592429014007431
0.334302284718985	-0.596680888598321
0.344482503147906	-0.600561952119905
0.354535034362703	-0.604086173803064
0.364453537882937	-0.607267206268444
0.374553712470261	-0.610207376467431
0.384498852607222	-0.612809964153202
0.394283715405760	-0.615089102193237
0.403903558196811	-0.617058576006395
0.413494046299083	-0.618754669181169
0.422906312483438	-0.620159424891930
0.432136959497020	-0.621286283054011
0.441183025213705	-0.622148327409760
0.450181820734142	-0.622766063691032
0.458985350242058	-0.623136680989569
0.467591878020051	-0.623272879125080
0.476000042519059	-0.623186991957430
0.484347786293253	-0.622884170721470
0.492488703277420	-0.622376266741879
0.500422551100256	-0.621675190982462
0.508149403635962	-0.620792478984096
0.515807057042190	-0.619718252818347
0.523251188222687	-0.618478646230402
0.530482893274383	-0.617084735365003
0.537503528882789	-0.615547212596802
0.544449588643934	-0.613841494760972
0.551179746616456	-0.612007658543525
0.557696294153305	-0.610055901935625
0.564001729142368	-0.607996032461849
0.570229939847373	-0.605789186986648
0.576243694696754	-0.603488965422995
0.582046346939117	-0.601104646681415
0.587641403327728	-0.598645114550587
0.593158834868531	-0.596057783672577
0.598466641172062	-0.593409237322959
0.603569112166792	-0.590707796470646
0.608470638750951	-0.587961384669341
0.613296041363941	-0.585104380895665
0.617919634287328	-0.582215691438526
0.622346525544856	-0.579302642033779
0.626581871581072	-0.576372161374280
0.630744247654027	-0.573346386488354
0.634715248764273	-0.570315786366286
0.638500687769630	-0.567286655076740
0.642106372857134	-0.564264893013774
0.645643725004701	-0.561161263128090
0.649002418843319	-0.558076970787711
0.652188863008609	-0.555017241781482
0.655209407235979	-0.551986914991056
0.658167639174698	-0.548886277366687
0.660961898690652	-0.545826425211555
0.663599084396704	-0.542811477689438
0.666085979909190	-0.539845177756108
0.668517943797476	-0.536818204775424
0.670802300061668	-0.533850746920634
0.672946333960613	-0.530945774217656
0.674957156824238	-0.528105895865540
0.676921863142475	-0.525212933927134
0.678756737791764	-0.522395514389185
0.680469351223292	-0.519655407434457
0.682067036795956	-0.516994043599629
0.683629081026640	-0.514284874534000
0.685080239700040	-0.511664619324301
0.686428268615922	-0.509133782307230
0.687680616910855	-0.506692556924529
0.688891870904779	-0.504243238006622
0.690014795859564	-0.501890636307524
0.691056888151193	-0.499633941288786
0.692025281526204	-0.497472085848432
0.692937854452756	-0.495377988186023
0.693788564215487	-0.493378126548481
0.694583811660399	-0.491470619390487
0.695329634463790	-0.489653415379890
0.696045329830712	-0.487890669421661
0.696721255807206	-0.486216971451180
0.697362776690983	-0.484629614588330
0.697974897179011	-0.483125798290382
0.698577619329954	-0.481665816666177
0.699158983707719	-0.480287542710204
0.699723348047649	-0.478987638744473
0.700274718461943	-0.477762743479973
0.700834760922506	-0.476572121326990
0.701388560475248	-0.475454163680766
0.701939482261074	-0.474405066522421
0.702490552622479	-0.473421069180345
0.703067254203565	-0.472461920450682
0.703649755739521	-0.471565066797106
0.704240432352264	-0.470726383970516
0.704841338802667	-0.469941857358246
0.705485175408266	-0.469172146834222
0.706143908073897	-0.468453356531852
0.706818912697524	-0.467781177124534
0.707511270210209	-0.467151477127189
0.708266149166122	-0.466525048828461
0.709042121453002	-0.465937426490674
0.709839536320458	-0.465384245174452
0.710658482883692	-0.464861391598016
0.711565464637960	-0.464327141212529
0.712496799257281	-0.463819026819704
0.713451743957126	-0.463332755786841
0.714429345218982	-0.462864373555630
0.715535532136977	-0.462362810088026
0.716666201458323	-0.461874137597853
0.717819350971900	-0.461394264358656
0.718992844785210	-0.460919553501515
0.720241795410708	-0.460424187301318
0.721507870915324	-0.459927695972196
0.722788302534645	-0.459427274966535
0.724080325154259	-0.458920560273665
0.725472789352691	-0.458369080888382
0.726872011547926	-0.457806236622320
0.728274740744887	-0.457230557060405
0.729677868315828	-0.456640982150349
0.731268098283012	-0.455953713118186
0.732850907897937	-0.455247234143299
0.734422513454072	-0.454521599806223
0.735979476017224	-0.453777253660029
0.737465706889067	-0.453041698484468
0.738932921338985	-0.452290526887086
0.740378961037137	-0.451524991240065
0.741801959202250	-0.450746471547819
0.743194344966198	-0.449959918161590
0.744561092723116	-0.449163635273524
0.745901237484033	-0.448359296627400
0.747214040488376	-0.447548561860486
0.748502446726867	-0.446730870212520
0.749762632273027	-0.445910116465350
0.750994570127976	-0.445087932718204
0.752198379559422	-0.444265855625591
0.753330663600170	-0.443476123965782
0.754437599591687	-0.442689099394415
0.755519729873056	-0.441905937041884
0.756577655472051	-0.441127684360230
0.757606131295044	-0.440359747163587
0.758612144270288	-0.439598463384949
0.759596524578137	-0.438844586692794
0.760560105938490	-0.438098766555242
0.761515936838575	-0.437351992434416
0.762452270248424	-0.436614544942685
0.763370068435514	-0.435886814554871
0.764270256003738	-0.435169100066500
0.765176310703108	-0.434443509330118
0.766065811606280	-0.433728828835676
0.766939738307582	-0.433025121144918
0.767799000710289	-0.432332376919020
0.768674460101283	-0.431626330735688
0.769536086079726	-0.430931806467583
0.770384782847162	-0.430248585454896
0.771221361255847	-0.429576402796260
0.772082372261614	-0.428886289953800
0.772931831809769	-0.428207462086380
0.773770493993552	-0.427539483647402
0.774599005166439	-0.426881902588472
0.775457822995102	-0.426202764357080
0.776306737111994	-0.425533987210968
0.777146298970615	-0.424875004717401
0.777976948961939	-0.424225264512620
0.778840016647353	-0.423552330968552
0.779694067787362	-0.422888374789970
0.780539432271672	-0.422232804966946
0.781376338179502	-0.421585070276837
0.782242002874248	-0.420916031616434
0.783098805665467	-0.420254434500545
0.783946883880915	-0.419599774094597
0.784786293605195	-0.418951598638452
0.785644406767029	-0.418288344245289
0.786493335659281	-0.417631192727988
0.787333102869361	-0.416979804117828
0.788163675040151	-0.416333887426881
0.788999893186735	-0.415681560795607
0.789826535665276	-0.415034454907196
0.790643605749667	-0.414392405646283
0.791451071020054	-0.413755280163408
0.792254167773819	-0.413118792712962
0.793047546103857	-0.412487139266165
0.793831257029532	-0.411860281343842
0.794605325392591	-0.411238190840230
0.795371240238916	-0.410619674923275
0.796127622658505	-0.410005952061392
0.796874592432985	-0.409397040932415
0.797612243240185	-0.408792954616168
0.798342852570023	-0.408191910881600
0.799064364325372	-0.407595770208039
0.799776955975384	-0.407004555056583
0.800480773781207	-0.406418273470579
0.801180821862164	-0.405832855564252
0.801872338667825	-0.405252455420926
0.802555535372080	-0.404677069517009
0.803230585301359	-0.404106677138661
0.803905407341604	-0.403534665562665
0.804572294749456	-0.402967711339469
0.805231467466230	-0.402405775003696
0.805883101671824	-0.401848801201550
0.806537412021962	-0.401288101157816
0.807184341009261	-0.400732397025955
0.807824097371962	-0.400181617132258
0.808456842086428	-0.399635677346793
0.809094155898806	-0.399084587612010
0.809724553679863	-0.398538342483234
0.810348220674661	-0.397996849765676
0.810965292691405	-0.397460008664160
0.811587712716467	-0.396917396449805
0.812203579353459	-0.396379420365167
0.812813050430931	-0.395845982100768
0.813416234775771	-0.395316977685541
0.814024536830916	-0.394782350398890
0.814626557909489	-0.394252133246376
0.815222431692769	-0.393726234330798
0.815812244699868	-0.393204557332645
0.816406244492628	-0.392677976414233
0.816994176422611	-0.392155595734288
0.817576157643555	-0.391637337247555
0.818152260443732	-0.391123117947056
0.818731363923492	-0.390604955678456
0.819304588890872	-0.390090818718068
0.819872044329288	-0.389580644290670
0.820433796269848	-0.389074362883575
0.820997532891838	-0.388565000236669
0.821555583382115	-0.388059525259508
0.822108054697673	-0.387557887252204
0.822655011919717	-0.387060026589334
0.823203355239834	-0.386559628405016
0.823746219303157	-0.386063008104387
0.824283711727283	-0.385570121929680
0.824815898487728	-0.385080915301182
0.825349309938496	-0.384589357881667
0.825877461236941	-0.384101482832473
0.826400460345724	-0.383617248733933
0.826918373268194	-0.383136602092060
0.827437647497787	-0.382653533219136
0.827951883185341	-0.382174054106539
0.828461186685365	-0.381698122960234
0.828965621899011	-0.381225685301185
0.829471665349604	-0.380750646538646
0.829972883710296	-0.380279101745476
0.830469379555492	-0.379811008111317
0.830961212629195	-0.379346309947150
0.831454858219281	-0.378878855764179
0.831943876709167	-0.378414795776630
0.832428365459208	-0.377954086980107
0.832908378881010	-0.377496673426265
0.833390285409676	-0.377036448732138
0.833867744981865	-0.376579517097786
0.834340849389384	-0.376125836717530
0.834809647609883	-0.375675352674917
0.835280287574260	-0.375222116527208
0.835746644730420	-0.374772074598248
0.836208805849183	-0.374325187468447
0.836666815174358	-0.373881402231127
0.837126525779779	-0.373435005682419
0.837582105821449	-0.372991709603400
0.838033638038072	-0.372551477521737
0.838481162956024	-0.372114258906833
0.838930221619609	-0.371674598406321
0.839375294197911	-0.371237950792703
0.839816460351504	-0.370804282451864
0.840253757778935	-0.370373545035994
0.840692445896586	-0.369940516525213
0.841127287342795	-0.369510418991445
0.841558359323062	-0.369083221188740
0.841985697233973	-0.368658876461010
0.842414331598085	-0.368232348203418
0.842839254518672	-0.367808673378057
0.843260540982899	-0.367387822540662
0.843678224243849	-0.366969750227214
0.844097155342278	-0.366549559212384
0.844512505598950	-0.366132147141142
0.844924347755962	-0.365717485963996
0.845332712861552	-0.365305531084821
0.845742303297063	-0.364891496284171
0.846148437969747	-0.364480168184214
0.846551187269719	-0.364071519962065
0.846950579939439	-0.363665507780034
0.847351179771264	-0.363257448623679
0.847748442763210	-0.362852025947032
0.848142436908734	-0.362449214171325
0.848533188626896	-0.362048970254725
0.848925119569114	-0.361646720483162
0.849313826389373	-0.361247039151078
0.849699374757010	-0.360849902014646
0.850081788867052	-0.360455266907768
0.850465341118659	-0.360058679340861
0.850845776226151	-0.359664594603482
0.851223157700927	-0.359272989851454
0.851597507693813	-0.358883823836249
0.851972946327984	-0.358492767095757
0.852345369750051	-0.358104150132287
0.852714839511892	-0.357717951493441
0.853081375917306	-0.357334130822920
0.853448950647582	-0.356948482278879
0.853813607685613	-0.356565212956116
0.854175406798465	-0.356184302721312
0.854534366607579	-0.355805712033723
0.854894319473175	-0.355425351498470
0.855251448170207	-0.355047311932425
0.855605810806197	-0.354671574421088
0.855957424434760	-0.354298100146891
0.856309992914664	-0.353922906909505
0.856659826952992	-0.353549978468726
0.857006983079050	-0.353179297038215
0.857351476853889	-0.352810824445682
0.857696892995997	-0.352440677724827
0.858039660708980	-0.352072741530297
0.858379835003349	-0.351706999141541
0.858717430006579	-0.351343412979939
0.859055917834383	-0.350978194188402
0.859391839606561	-0.350615133449639
0.859725248873519	-0.350254215072826
0.860056158390859	-0.349895402042515
0.860387931803771	-0.349534996958408
0.860717218027311	-0.349176699195947
0.861044069219812	-0.348820494070875
0.861368496836464	-0.348466345108762
0.861693759096444	-0.348110644808787
0.862016609715883	-0.347757002802385
0.862337099536828	-0.347405405388212
0.862655238791756	-0.347055816608388
0.862974183442876	-0.346704717084966
0.863290788897624	-0.346355628479077
0.863605104757795	-0.346008538041740
0.863917140109325	-0.345663410301008
0.864229952485504	-0.345316811402736
0.864540495202002	-0.344972177628712
0.864848816689868	-0.344629497146003
0.865154924957253	-0.344288734933976
0.865461783447568	-0.343946539386657
0.865766439069687	-0.343606264674153
0.866068939144398	-0.343267899842339
0.866369290661996	-0.342931410287692
0.866670367352497	-0.342593523222079
0.866969305351433	-0.342257514129646
0.867266150922376	-0.341923372901194
0.867560910091014	-0.341591065319705
0.867856370882413	-0.341257394292792
0.868149754657363	-0.340925559739462
0.868441106671025	-0.340595552366377
0.868730432034212	-0.340267338316626
0.869020436572163	-0.339937793547815
0.869308423377414	-0.339610045059618
0.869594436743720	-0.339284084349248
0.869878480915259	-0.338959877896435
0.870163182626450	-0.338634372432120
0.870445923609818	-0.338310624312702
0.870726747243615	-0.337988625802408
0.871005656952484	-0.337668343695410
0.871285203288042	-0.337346793374515
0.871562843734408	-0.337026962672312
0.871838620798553	-0.336708844596930
0.872112537130793	-0.336392406235100
0.872387069946760	-0.336074729498489
0.872659749653552	-0.335758735815961
0.872930617928519	-0.335444418916587
0.873199676690202	-0.335131746158101
0.873469332634244	-0.334817863823116
0.873737186289682	-0.334505629091737
0.874003278542969	-0.334195036391678
0.874267610620517	-0.333886053330907
0.874532521437013	-0.333575888426252
0.874795678916584	-0.333267336743416
0.875057123190788	-0.332960393387664
0.875316854830984	-0.332655026197646
0.875577147574967	-0.332348503880740
0.875835734148810	-0.332043561430100
0.876092653962987	-0.331740194608888
0.876347906968814	-0.331438371468156
0.876603704171773	-0.331135418989182
0.876857840666165	-0.330834014007640
0.877110355173431	-0.330534152926193
0.877361247058181	-0.330235803991102
0.877612666892867	-0.329936350656102
0.877862469851806	-0.329638413399155
0.878110693997897	-0.329341989244982
0.878357338140843	-0.329047046618692
0.878604494605559	-0.328751023726899
0.878850076471777	-0.328456486407561
0.879094121172785	-0.328163432290764
0.879336626993628	-0.327871829964774
0.879579630108045	-0.327579170725157
0.879821099415049	-0.327287967431843
0.880061071745653	-0.326998218304267
0.880299544888922	-0.326709892078817
0.880538500883335	-0.326420531524150
0.880775962440630	-0.326132598136134
0.881011965815341	-0.325846090708265
0.881246508327713	-0.325560978110705
0.881481519813571	-0.325274853023648
0.881715074873396	-0.324990127138684
0.881947209209594	-0.324706799808840
0.882177919699368	-0.324424840024396
0.882409085821202	-0.324141888877553
0.882638832227123	-0.323860309753491
0.882867194090464	-0.323580102550971
0.883094167869903	-0.323301236367405
0.883321584445810	-0.323021399270855
0.883547616770294	-0.322742907774604
0.883772299509482	-0.322465762310035
0.883995628726888	-0.322189932069305
0.884219388384190	-0.321913150718526
0.884441798061588	-0.321637689275267
0.884662891938751	-0.321363548691022
0.884882665706293	-0.321090698240860
0.885102858014386	-0.320816915862556
0.885321733471186	-0.320544428402720
0.885539325789578	-0.320273237321018
0.885755630308494	-0.320003311964105
0.885972341907038	-0.319732473261887
0.886187768687516	-0.319462905167942
0.886401943914687	-0.319194609638710
0.886614862596025	-0.318927556081600
0.886828177316451	-0.318659607184062
0.887040238201764	-0.318392905239664
0.887251078086287	-0.318127452690747
0.887460691665322	-0.317863218995123
0.887670690644853	-0.317598107407768
0.887879465764795	-0.317334219750735
0.888087049445830	-0.317071558941890
0.888293436089499	-0.316810094479553
0.888500197878696	-0.316547769039874
0.888705764817161	-0.316286645118241
0.888910168927880	-0.316026726098164
0.889113404336227	-0.315767981508989
0.889317005001385	-0.315508392343474
0.889519438896796	-0.315249982873438
0.889720737662911	-0.314992756938593
0.889920895165751	-0.314736684090240
0.890121408386989	-0.314479782572485
0.890320782028545	-0.314224039497380
0.890519047362733	-0.313969459151827
0.890716198012310	-0.313716011100387
0.890913695177420	-0.313461749810401
0.891110079097169	-0.313208626260834
0.891305380689430	-0.312956645177168
0.891499593349089	-0.312705776128890
0.891694143642981	-0.312454108813972
0.891887606203602	-0.312203559069488
0.892080011607398	-0.311954132051276
0.892271353036132	-0.311705797325761
0.892463023525872	-0.311456678863206
0.892653631004131	-0.311208658315746
0.892843205718311	-0.310961741261727
0.893031740651176	-0.310715897256843
0.893220596367024	-0.310469283618198
0.893408413033322	-0.310223748737078
0.893595220580212	-0.309979298606835
0.893781011805010	-0.309735902765081
0.893967115817621	-0.309491750981970
0.894152204011797	-0.309248659280381
0.894336306011636	-0.309006634061512
0.894519414442003	-0.308765644837825
0.894702827936305	-0.308523912968859
0.894885248140184	-0.308283222971427
0.895066704382368	-0.308043581647730
0.895247189127756	-0.307804958478296
0.895427971473525	-0.307565605577219
0.895607782380225	-0.307327276788769
0.895786650891388	-0.307089979309611
0.895964569323933	-0.306853682581820
0.896142778143165	-0.306616668666908
0.896320036723280	-0.306380661542450
0.896496373832305	-0.306145668793326
0.896671781650702	-0.305911659816891
0.896847472881974	-0.305676945841530
0.897022234446806	-0.305443221757396
0.897196094846945	-0.305210495531615
0.897369046137491	-0.304978736510796
0.897542274097533	-0.304746284335094
0.897714592359587	-0.304514805561084
0.897886029167920	-0.304284308532441
0.898056576462936	-0.304054762539226
0.898227393905436	-0.303824534902780
0.898397321036209	-0.303595264575445
0.898566385850429	-0.303366960271997
0.898734580184085	-0.303139591220363
0.898903038355972	-0.302911551715990
0.899070625041273	-0.302684453812844
0.899237367994066	-0.302458306591597
0.899403258955834	-0.302233079212668
0.899569407651151	-0.302007192261068
0.899734703144060	-0.301782231575716
0.899899172955169	-0.301558206598212
0.900062808741007	-0.301335086416287
0.900226696352501	-0.301111317241602
0.900389748524088	-0.300888459359746
0.900551992550175	-0.300666522568499
0.900713420011562	-0.300445475877911
0.900875093580008	-0.300223790484270
0.901035948967825	-0.300003001760670
0.901196013250166	-0.299783119856548
0.901355277941001	-0.299564113699451
0.901514783202544	-0.299344478848203
0.901673487057193	-0.299125726384327
0.901831416367466	-0.298907866804586
0.901988562589111	-0.298690868949385
0.902145944020522	-0.298473252137301
0.902302540350158	-0.298256503759906
0.902458378234224	-0.298040634657162
0.902613449078563	-0.297825613577846
0.902768749940696	-0.297609983015970
0.902923281553780	-0.297395207256325
0.903077070373733	-0.297181297478133
0.903230107764550	-0.296968222334215
0.903383370143986	-0.296754546927488
0.903535878690247	-0.296541713001351
0.903687659664723	-0.296329732070533
0.903838704397355	-0.296118572687714
0.903989969246337	-0.295906822015300
0.904140495256070	-0.295695899803585
0.904290308498913	-0.295485817899226
0.904439400278307	-0.295276544750719
0.904588707453015	-0.295066689047065
0.904737290374745	-0.294857649077230
0.904885174932069	-0.294649437016382
0.905032352409254	-0.294442021204926
0.905179740706601	-0.294234031341381
0.905326418943293	-0.294026844769349
0.905472412829126	-0.293820473989264
0.905617713636300	-0.293614887229655
0.905763220829202	-0.293408734696776
0.905908031772978	-0.293203373289546
0.906052172003435	-0.292998815830571
0.906195632787603	-0.292795030432846
0.906339295658868	-0.292590687323274
0.906482275724370	-0.292387123442083
0.906624598350490	-0.292184351931104
0.906766254805799	-0.291982340784255
0.906908109180671	-0.291779779776168
0.907049293837099	-0.291577986360210
0.907189833976398	-0.291376973994644
0.907329720875200	-0.291176710550873
0.907469801652606	-0.290975904892022
0.907609225454482	-0.290775855442754
0.907748017321244	-0.290576575975103
0.907886168543925	-0.290378034234631
0.908024509726527	-0.290178957726859
0.908162206343293	-0.289980626292770
0.908299283277715	-0.289783054015642
0.908435731841403	-0.289586208511970
0.908572366564495	-0.289388835496239
0.908708368808970	-0.289192196658110
0.908843763305189	-0.288996306389720
0.908978541391364	-0.288801132175363
0.909113501950605	-0.288605437517330
0.909247841806298	-0.288410466374056
0.909381585539302	-0.288216233444266
0.909514724520295	-0.288022706077011
0.909648042398440	-0.287828665152996
0.909780751045891	-0.287635337307763
0.909912874897457	-0.287442737544482
0.910044405362014	-0.287250833074010
0.910176111254595	-0.287058421757466
0.910307219096664	-0.286866713304442
0.910437753180282	-0.286675723020527
0.910567704958116	-0.286485417975513
0.910697828798173	-0.286294612623894
0.910827365484412	-0.286104500135300
0.910956339169298	-0.285915096115827
0.911084741354755	-0.285726367491412
0.911213312336593	-0.285537144933532
0.911341306786657	-0.285348605447197
0.911468748720821	-0.285160764937209
0.911595629695612	-0.284973590182933
0.911722676297765	-0.284785927706586
0.911849156724042	-0.284598938713757
0.911975094856590	-0.284412639406261
0.912100482311774	-0.284226996414250
0.912226032319023	-0.284040871754365
0.912351026248333	-0.283855411188044
0.912475487850858	-0.283670631212525
0.912599408807922	-0.283486498306172
0.912723489332564	-0.283301889633242
0.912847023627123	-0.283117935856790
0.912970035314364	-0.282934653767989
0.913092516145598	-0.282752009690906
0.913215153647902	-0.282568895599832
0.913337254525489	-0.282386427395977
0.913458842275218	-0.282204622163064
0.913579908723312	-0.282023446068415
0.913701129031277	-0.281841805567621
0.913821822084711	-0.281660802127744
0.913942011256933	-0.281480453123759
0.914061688453917	-0.281300724563859
0.914181516782251	-0.281120537064841
0.914300826998110	-0.280940977978672
0.914419642353518	-0.280762064970379
0.914537954838952	-0.280583763886696
0.914656415807422	-0.280405009193823
0.914774367584125	-0.280226874439393
0.914891833301936	-0.280049377577379
0.915008805040506	-0.279872484290779
0.915125922691637	-0.279695142591375
0.915242539856909	-0.279518412525246
0.915358679552081	-0.279342312334292
0.915474333950580	-0.279166807535548
0.915590131766698	-0.278990859390335
0.915705437594371	-0.278815514738182
0.915820274334184	-0.278640792107978
0.915934634257859	-0.278466656848620
0.916049135177531	-0.278292083182438
0.916163152403769	-0.278118105029897
0.916276708723813	-0.277944741206027
0.916389796512148	-0.277771956889456
0.916503022946107	-0.277598738982182
0.916615773785101	-0.277426108765900
0.916728071704776	-0.277254085341019
0.916839909186774	-0.277082633713809
0.916951883033196	-0.276910753191662
0.917063389192248	-0.276739452690733
0.917174450229632	-0.276568751596117
0.917285058738490	-0.276398614739687
0.917395801397831	-0.276228053566681
0.917506084091985	-0.276058064894207
0.917615929278273	-0.275888668391445
0.917725329665628	-0.275719828713862
0.917834862054889	-0.275550569183584
0.917943942021007	-0.275381874778576
0.918052591914405	-0.275213765451575
0.918160804564042	-0.275046205679673
0.918269147130611	-0.274878230407206
0.918377044641032	-0.274710813026619
0.918484519340231	-0.274543973773750
0.918591564181382	-0.274377676945385
0.918698736916330	-0.274210968859583
0.918805471791992	-0.274044811570693
0.918911790949117	-0.273879225597277
0.919017687469243	-0.273714175053916
0.919123709920227	-0.273548717389809
0.919229301543402	-0.273383803562723
0.919334484376580	-0.273219454373643
0.919439251633779	-0.273055633753073
0.919544142917502	-0.272891410044504
0.919648610244091	-0.272727723344900
0.919752675549593	-0.272564594737436
0.919856332184577	-0.272401987966702
0.919960110998827	-0.272238982039185
0.920063472570246	-0.272076506421264
0.920166438734212	-0.271914582478142
0.920269002981891	-0.271753173766687
0.920371687617177	-0.271591369730464
0.920473961571842	-0.271430089430099
0.920575846581627	-0.271269354512734
0.920677336282302	-0.271109128345728
0.920778944633135	-0.270948510588979
0.920880148717603	-0.270788410117017
0.920980970172766	-0.270628848858901
0.921081402782991	-0.270469789990721
0.921181952358733	-0.270310343173057
0.921282103938410	-0.270151407308894
0.921381879061294	-0.269993004609259
0.921481271664314	-0.269835098057236
0.921580779599764	-0.269676807103234
0.921679895669357	-0.269519020888442
0.921778641315409	-0.269361761905967
0.921877010631353	-0.269204992944171
0.921975493696907	-0.269047843037209
0.922073590890458	-0.268891191769444
0.922171323558134	-0.268735061916246
0.922268685953801	-0.268579416069560
0.922366160565344	-0.268423392645733
0.922463255166000	-0.268267861872731
0.922559991006414	-0.268112846808441
0.922656362504802	-0.267958309846707
0.922752844733258	-0.267803398588941
0.922848952682700	-0.267648974102711
0.922944707508938	-0.267495059728733
0.923040103798442	-0.267341617661093
0.923135609379041	-0.267187804493386
0.923230746286640	-0.267034472324522
0.923325535582805	-0.266881644778425
0.923419972026149	-0.266729283847777
0.923514516367363	-0.266576554929655
0.923608697519004	-0.266424301341861
0.923702536448925	-0.266272546991975
0.923796028091776	-0.266121253669638
0.923889626284002	-0.265969595390712
0.923982866650662	-0.265818406875427
0.924075770066375	-0.265667712315531
0.924168331645713	-0.265517473296004
0.924260998469717	-0.265366872270609
0.924353312715810	-0.265216735541716
0.924445295165797	-0.265067087585815
0.924536941118060	-0.264917889781617
0.924628691053093	-0.264768332843713
0.924720093544481	-0.264619234832498
0.924811169281589	-0.264470620509846
0.924901913750497	-0.264322451046602
0.924992760982205	-0.264173925244714
0.925083265794021	-0.264025853094876
0.925173448783187	-0.263878259645048
0.925263305627373	-0.263731105856615
0.925353264055464	-0.263583598448922
0.925442884979685	-0.263436539511712
0.925532188905418	-0.263289954379802
0.925621171705829	-0.263143803803534
0.925710254951507	-0.262997302253063
0.925799005504296	-0.262851244082546
0.925887443777941	-0.262705654914488
0.925975565845009	-0.262560495286607
0.926063787258164	-0.262414987256595
0.926151680686983	-0.262269917605056
0.926239266453736	-0.262125312243084
0.926326540834321	-0.261981131494205
0.926413913500521	-0.261836604843527
0.926500962791037	-0.261692511656967
0.926587708936781	-0.261548878135170
0.926674148420919	-0.261405664385893
0.926760685168177	-0.261262107164652
0.926846903050947	-0.261118978578421
0.926932822208855	-0.260976305118420
0.927018439336293	-0.260834046675076
0.927104152741676	-0.260691447120208
0.927189551698683	-0.260549271454662
0.927274656255678	-0.260407546461330
0.927359463322259	-0.260266231811739
0.927444365718256	-0.260124578342805
0.927528957989208	-0.259983344099152
0.927613260092187	-0.259842556156503
0.927697269155999	-0.259702173965914
0.927781372636727	-0.259561455180964
0.927865170225184	-0.259421151037171
0.927948681787079	-0.259281288904313
0.928031904674451	-0.259141828011411
0.928115221101688	-0.259002032682915
0.928198235781029	-0.258862647489691
0.928280968486701	-0.258723700096859
0.928363416798036	-0.258585149509837
0.928445957807041	-0.258446266580786
0.928528201126218	-0.258307789357720
0.928610166438149	-0.258169745802465
0.928691851553547	-0.258032094695255
0.928773628558777	-0.257894113275238
0.928855111847971	-0.257756533206925
0.928936321011853	-0.257619382750275
0.929017254096638	-0.257482620458760
0.929098278297266	-0.257345529820196
0.929179012673339	-0.257208836252512
0.929259476723465	-0.257072568315296
0.929339668733519	-0.256936684333669
0.929419951118786	-0.256800473908138
0.929499947490571	-0.256664656344609
0.929579677255066	-0.256529260503866
0.929659138942005	-0.256394244481085
0.929738690296421	-0.256258903855737
0.929817959369870	-0.256123951953991
0.929896965475781	-0.255989417939460
0.929975707391986	-0.255855259675776
0.930054538300472	-0.255720778589676
0.930133090583742	-0.255586682157821
0.930211383462064	-0.255452999848369
0.930289415965658	-0.255319689291788
0.930367536818416	-0.255186057632560
0.930445382626678	-0.255052806625875
0.930522972517116	-0.254919966046211
0.930600305776671	-0.254787493289254
0.930677726774002	-0.254654701089654
0.930754876234214	-0.254522285607190
0.930831773189897	-0.254390276924517
0.930908417189098	-0.254258632200900
0.930985148346106	-0.254126669635436
0.931061611401662	-0.253995079916673
0.931137825293742	-0.253863893437378
0.931213789835940	-0.253733067118742
0.931289840987054	-0.253601924500448
0.931365627402256	-0.253471150922109
0.931441167924332	-0.253340777088608
0.931516462636921	-0.253210759681400
0.931591843440325	-0.253080427458635
0.931666962804766	-0.252950460531511
0.931741839477219	-0.252820889919117
0.931816473815924	-0.252691672061484
0.931891193757887	-0.252562140814751
0.931965655490737	-0.252432971180557
0.932039877664966	-0.252304194494361
0.932113860918039	-0.252175766953077
0.932187929317106	-0.252047027391960
0.932261742671254	-0.251918645820304
0.932335319533773	-0.251790653892186
0.932408660826047	-0.251663007559681
0.932482086837139	-0.251535050519796
0.932555260903251	-0.251407447905157
0.932628201479707	-0.251280231690794
0.932700909776570	-0.251153357582200
0.932773702394999	-0.251026174022174
0.932846246105491	-0.250899341380916
0.932918559264588	-0.250772891956823
0.932990643375871	-0.250646781207048
0.933062811441196	-0.250520362205644
0.933134733574049	-0.250394290673165
0.933206428031325	-0.250268599233882
0.933277896615038	-0.250143243094821
0.933349448814892	-0.250017579848002
0.933420757997433	-0.249892260675830
0.933491842319001	-0.249767318531044
0.933562703885041	-0.249642708368735
0.933633648758848	-0.249517792186786
0.933704353471438	-0.249393216739728
0.933774836077629	-0.249269015311456
0.933845098991385	-0.249145142603288
0.933915444933957	-0.249020964908054
0.933985553513543	-0.248897124661460
0.934055442682424	-0.248773655481339
0.934125115168259	-0.248650511813370
0.934194870433365	-0.248527064135420
0.934264391077014	-0.248403950672375
0.934333694947879	-0.248281205378883
0.934402785092592	-0.248158782443093
0.934471957796375	-0.248036056419044
0.934540898564656	-0.247913661427717
0.934609625141378	-0.247791631763552
0.934678140897515	-0.247669921355242
0.934746739021906	-0.247547908724993
0.934815107842266	-0.247426223995891
0.934883264996630	-0.247304901805256
0.934951214185797	-0.247183895820362
0.935019245581808	-0.247062588424427
0.935087050251831	-0.246941605847762
0.935154645726763	-0.246820983073752
0.935222036042813	-0.246700673506261
0.935289508433772	-0.246580063283110
0.935356756624384	-0.246459774846156
0.935423798037118	-0.246339843528148
0.935490637049295	-0.246220222467508
0.935557558034011	-0.246100301450939
0.935624257292612	-0.245980699235429
0.935690752137784	-0.245861451506506
0.935757047293790	-0.245742511135078
0.935823424349674	-0.245623271451565
0.935889582103223	-0.245504347631067
0.935955537755930	-0.245385775715414
0.936021296384951	-0.245267508305894
0.936087136871023	-0.245148942172059
0.936152760429014	-0.245030689009462
0.936218184147754	-0.244912785219888
0.936283413463376	-0.244795183132846
0.936348724623291	-0.244677282852784
0.936413821180755	-0.244559692697652
0.936478720110395	-0.244442449432960
0.936543427213546	-0.244325505114244
0.936608216178492	-0.244208263077015
0.936672792818858	-0.244091328363094
0.936737173993465	-0.243974738105622
0.936801365875219	-0.243858444083914
0.936865639666831	-0.243741852760903
0.936929703364815	-0.243625566003506
0.936993573710510	-0.243509621316535
0.937057257254918	-0.243393970200785
0.937121022788076	-0.243278022143192
0.937184580412445	-0.243162375936711
0.937247946750143	-0.243047069462000
0.937311128736945	-0.242932053938986
0.937374392822578	-0.242816741775225
0.937437451138928	-0.242701728790545
0.937500320187078	-0.242587053245773
0.937563007294429	-0.242472666077565
0.937625776642259	-0.242357982510682
0.937688342315735	-0.242243595492620
0.937750720693011	-0.242129543668853
0.937812919500140	-0.242015777690298
0.937875200721393	-0.241901715495379
0.937937280319365	-0.241787947260118
0.937999174547315	-0.241674512019259
0.938060891537157	-0.241561360135463
0.938122691147226	-0.241447912157045
0.938184291141932	-0.241334755589554
0.938245707647585	-0.241221929861801
0.938306949209365	-0.241109385045600
0.938368273630469	-0.240996544195016
0.938429400401641	-0.240883992246424
0.938490345520106	-0.240771769027660
0.938551117951920	-0.240659824317039
0.938611973515690	-0.240547583569822
0.938672633353115	-0.240435629254831
0.938733113330112	-0.240324001604068
0.938793422841436	-0.240212650099625
0.938853815791546	-0.240101002492746
0.938914014897672	-0.239989638886895
0.938974035892109	-0.239878599923563
0.939033888606352	-0.239767834785818
0.939093825101061	-0.239656773415031
0.939153569593509	-0.239545993652054
0.939213137679960	-0.239435536553385
0.939272539636932	-0.239325351000192
0.939332025751651	-0.239214869017239
0.939391321665760	-0.239104666286292
0.939450442836981	-0.238994784284576
0.939509399995384	-0.238885171588396
0.939568441725210	-0.238775262198223
0.939627295016541	-0.238665629741116
0.939685975185941	-0.238556316120954
0.939744493425829	-0.238447269606137
0.939803096688100	-0.238337926063983
0.939861513234966	-0.238228857172286
0.939919758239112	-0.238120105267731
0.939977843364367	-0.238011618307677
0.940036014001190	-0.237902833916153
0.940093999607157	-0.237794321928294
0.940151815208236	-0.237686125119976
0.940209472949024	-0.237578191134282
0.940267216729823	-0.237469959240339
0.940324777126232	-0.237361997538591
0.940382169014542	-0.237254349250728
0.940439405029784	-0.237146961702228
0.940496727653838	-0.237039275694076
0.940553868502312	-0.236931857701489
0.940610842298743	-0.236824751398857
0.940667662178575	-0.236717903790610
0.940724569277581	-0.236610757094518
0.940781296172566	-0.236503876271744
0.940837857431096	-0.236397305456523
0.940894266699359	-0.236290991328691
0.940950763840027	-0.236184377405658
0.941007082311356	-0.236078027247629
0.941063236521591	-0.235971985456126
0.941119240638345	-0.235866198382718
0.941175327743895	-0.235760121302440
0.941231237718168	-0.235654305853081
0.941286984801501	-0.235548797084095
0.941342583677900	-0.235443541048912
0.941398161182540	-0.235338193829971
0.941453563812115	-0.235233105033432
0.941508805544840	-0.235128319646413
0.941563901280755	-0.235023784059691
0.941619002924262	-0.234919107062855
0.941673931774812	-0.234814685750270
0.941728701638660	-0.234710565141156
0.941783327702074	-0.234606691707323
0.941837952421967	-0.234502692187206
0.941892406476241	-0.234398945465919
0.941946703437355	-0.234295496546115
0.942000858712733	-0.234192292085668
0.942055020288895	-0.234088948339475
0.942109013176435	-0.233985854660430
0.942162850740135	-0.233883056098407
0.942216548671044	-0.233780499445985
0.942270247232511	-0.233677815788084
0.942323779118491	-0.233575379451716
0.942377157484446	-0.233473235487226
0.942430398268612	-0.233371330848710
0.942483643149113	-0.233269293993654
0.942536723304625	-0.233167501780760
0.942589651680778	-0.233065999277830
0.942642444471540	-0.232964733587101
0.942695241167139	-0.232863337443007
0.942747875050916	-0.232762183296935
0.942800358859483	-0.232661316233194
0.942852709042636	-0.232560683506907
0.942905063467331	-0.232459921071264
0.942957256960174	-0.232359398032645
0.943009302051292	-0.232259159489942
0.943061215444514	-0.232159152849181
0.943113133565838	-0.232059016942111
0.943164892600519	-0.231959117869745
0.943216504872260	-0.231859500745274
0.943267987337290	-0.231760113126116
0.943319475078226	-0.231660596547832
0.943370805541235	-0.231561314282678
0.943421990844873	-0.231462311459176
0.943473048198127	-0.231363535785347
0.943524111167781	-0.231264631848409
0.943575018635734	-0.231165959740880
0.943625782516467	-0.231067564605690
0.943676420270355	-0.230969394301569
0.943727064122372	-0.230871096143628
0.943777554215712	-0.230773027369428
0.943827902261694	-0.230675233136394
0.943878125971376	-0.230577661453579
0.943928356216064	-0.230479962399833
0.943978434412784	-0.230382490321167
0.944028372070632	-0.230285290389445
0.944078187150662	-0.230188310763885
0.944128009195788	-0.230091204250923
0.944177680872268	-0.229994322340667
0.944227213487935	-0.229897710219254
0.944276625253044	-0.229801316195865
0.944326044418904	-0.229704795745342
0.944375314864683	-0.229608497560682
0.944424447697841	-0.229512466842194
0.944473461377076	-0.229416652048849
0.944522482891153	-0.229320711279396
0.944571357303606	-0.229224990473823
0.944620095522398	-0.229129534846529
0.944668716253967	-0.229034293006107
0.944717345248870	-0.228938925639630
0.944765828731222	-0.228843775969175
0.944814177410350	-0.228748889223125
0.944862410239699	-0.228654214159546
0.944910651761465	-0.228559414007091
0.944958749330996	-0.228464829316263
0.945006713459817	-0.228370505329337
0.945054563347674	-0.228276390953721
0.945102422354583	-0.228182151919730
0.945150138941454	-0.228088126145765
0.945197723422817	-0.227994358887909
0.945245195244032	-0.227900799202788
0.945292676609078	-0.227807115282201
0.945340017058782	-0.227713642452185
0.945387226711475	-0.227620425982548
0.945434325257441	-0.227527415079025
0.945481433770436	-0.227434280355045
0.945528402845887	-0.227341354583699
0.945575242406690	-0.227248683048435
0.945621972387386	-0.227156215104006
0.945668712756709	-0.227063623746495
0.945715315139969	-0.226971239234579
0.945761789265379	-0.226879106865272
0.945808155311074	-0.226787176142262
0.945854532165330	-0.226695122406263
0.945900772459258	-0.226603273439117
0.945946885727117	-0.226511674551329
0.945992892389987	-0.226420275395458
0.946038910279900	-0.226328753619203
0.946084793010029	-0.226237434564768
0.946130549921387	-0.226146363556083
0.946176201677363	-0.226055490394517
0.946221865077334	-0.225964494998058
0.946267394693412	-0.225873700305523
0.946312799674055	-0.225783151654200
0.946358100924334	-0.225692798994223
0.946403414234166	-0.225602324477666
0.946448595111874	-0.225512048675710
0.946493652514025	-0.225422016938942
0.946538607586760	-0.225332179366233
0.946583575133166	-0.225242220308373
0.946628411575600	-0.225152458003824
0.946673125679396	-0.225062937816407
0.946717738831159	-0.224973609993711
0.946762364869483	-0.224884161050184
0.946806861108875	-0.224794906926173
0.946851236124065	-0.224705892998679
0.946895511541530	-0.224617069663999
0.946939800257056	-0.224528125566226
0.946983960456060	-0.224439374381147
0.947028000523285	-0.224350861498891
0.947071942324499	-0.224262537464468
0.947115897834119	-0.224174093017821
0.947159726087472	-0.224085839603511
0.947203435279912	-0.223997822624744
0.947247047515926	-0.223909992775261
0.947290673869462	-0.223822042857890
0.947334174205296	-0.223734282118466
0.947377556529966	-0.223646755973228
0.947420843186124	-0.223559415264669
0.947464144367778	-0.223471954826038
0.947507320749047	-0.223384681736445
0.947550380148225	-0.223297641425116
0.947593345145574	-0.223210784883339
0.947636325075315	-0.223123808942827
0.947679181401188	-0.223037018547448
0.947721921753780	-0.222950459139380
0.947764568950429	-0.222864081858748
0.947807231485255	-0.222777585504494
0.947849771592351	-0.222691272916011
0.947892196715129	-0.222605189548386
0.947934529907475	-0.222519286690646
0.947976878842817	-0.222433265078036
0.948019106506607	-0.222347425475924
0.948061220155594	-0.222261813352273
0.948103243079697	-0.222176380145077
0.948145282150619	-0.222090828495645
0.948187201086612	-0.222005457125078
0.948229006958259	-0.221920311514189
0.948270723291006	-0.221835343250019
0.948312456173453	-0.221750256850174
0.948354070038437	-0.221665349020776
0.948395571770855	-0.221580665255452
0.948436985131186	-0.221496157290385
0.948478415443250	-0.221411531490098
0.948519727836548	-0.221327082574626
0.948560929010752	-0.221242856050387
0.948602042960890	-0.221158803802804
0.948643174263896	-0.221074634014627
0.948684188728435	-0.220990639448005
0.948725092869409	-0.220906865622124
0.948765910915919	-0.220823264571759
0.948806746715621	-0.220739546269558
0.948847466739130	-0.220656001547621
0.948888077317009	-0.220572675937881
0.948928602911974	-0.220489521624583
0.948969146659708	-0.220406250342358
0.949009575675858	-0.220323151020676
0.949049896107064	-0.220240269204200
0.949090132649202	-0.220157557226780
0.949130387742928	-0.220074728557681
0.949170529132355	-0.219992070250587
0.949210562780614	-0.219909627862878
0.949250513616296	-0.219827353878146
0.949290483401712	-0.219744963473275
0.949330340493143	-0.219662741852677
0.949370090670591	-0.219580734586435
0.949409759094935	-0.219498894308036
0.949449446866482	-0.219416937875493
0.949489022937712	-0.219335148669926
0.949528492905879	-0.219253572274110
0.949567882163725	-0.219172161471586
0.949607291165633	-0.219090634775369
0.949646589444573	-0.219009273768901
0.949685782415412	-0.218928124047644
0.949724895702348	-0.218847138545362
0.949764029129614	-0.218766037404385
0.949803052795263	-0.218685100435646
0.949841971932118	-0.218604373247292
0.949880812395434	-0.218523808923486
0.949919673394817	-0.218443129210547
0.949958425578241	-0.218362612171704
0.949997073996823	-0.218282303427787
0.950035644736481	-0.218202156213549
0.950074236407414	-0.218121893854431
0.950112720192659	-0.218041792690296
0.950151100961943	-0.217961898354659
0.950189405031471	-0.217882164233058
0.950227730426996	-0.217802315205566
0.950265948852008	-0.217722625912641
0.950304064995154	-0.217643142000484
0.950342105402557	-0.217563817005630
0.950380167530289	-0.217484377338526
0.950418123587881	-0.217405095963945
0.950455978083189	-0.217326018540782
0.950493757791895	-0.217247098756780
0.950531559614805	-0.217168064529099
0.950569256253423	-0.217089187169947
0.950606852035096	-0.217010512350925
0.950644373964716	-0.216931993911209
0.950681918402068	-0.216853361251201
0.950719358526727	-0.216774884053471
0.950756698485799	-0.216696608002333
0.950793965513047	-0.216618487088632
0.950831255441261	-0.216540252172853
0.950868441914403	-0.216462171330533
0.950905528899588	-0.216384290258720
0.950942543859122	-0.216306563100168
0.950979582112468	-0.216228722152901
0.951016517754644	-0.216151033907411
0.951053354573016	-0.216073544073492
0.951090120258117	-0.215996206946064
0.951126909629711	-0.215918756238074
0.951163597220574	-0.215841456877025
0.951200186638551	-0.215764354585475
0.951236705802098	-0.215687403810769
0.951273249044535	-0.215610339658811
0.951309691323470	-0.215533425515510
0.951346036067443	-0.215456707116217
0.951382311422531	-0.215380139060967
0.951418611248749	-0.215303457826783
0.951454810915725	-0.215226925279251
0.951490913672897	-0.215150587166534
0.951526947893681	-0.215074398241641
0.951563006977634	-0.214998096331335
0.951598966693878	-0.214921941801673
0.951634830112940	-0.214845980413663
0.951670625835295	-0.214770167073573
0.951706446812778	-0.214694240936652
0.951742169201590	-0.214618460890100
0.951777795893523	-0.214542872707797
0.951813355715850	-0.214467431449568
0.951848941185137	-0.214391877578357
0.951884428832525	-0.214316468522705
0.951919821371237	-0.214241250069399
0.951955147855086	-0.214166177432126
0.951990500377709	-0.214090992360865
0.952025755833159	-0.214015950845561
0.952060916756247	-0.213941098685944
0.952096012427080	-0.213866391249877
0.952131134528442	-0.213791571554149
0.952166160305531	-0.213716894169732
0.952201092114886	-0.213642404909335
0.952235959462676	-0.213568059295321
0.952270853632802	-0.213493601591174
0.952305652209941	-0.213419284968398
0.952340357372491	-0.213345155252723
0.952374998852458	-0.213271168121343
0.952409667546603	-0.213197069064692
0.952444241367644	-0.213123109873933
0.952478722315952	-0.213049336387864
0.952513140349159	-0.212975704438849
0.952547585988464	-0.212901960724771
0.952581937463343	-0.212828355675332
0.952616196596251	-0.212754935142441
0.952650393570240	-0.212681655113985
0.952684618542382	-0.212608263475995
0.952718750047772	-0.212535009315383
0.952752789731045	-0.212461938497217
0.952786768000480	-0.212389007165265
0.952820774660261	-0.212315964374715
0.952854688540158	-0.212243057888040
0.952888511107063	-0.212170333583525
0.952922272994304	-0.212097747761182
0.952956063664285	-0.212025050626552
0.952989762230628	-0.211952488635831
0.953023369982559	-0.211880107680574
0.953056917778280	-0.211807864217415
0.953090494749334	-0.211735509583746
0.953123980282566	-0.211663288947336
0.953157375489591	-0.211591248213069
0.953190711453325	-0.211519343994586
0.953224076985306	-0.211447328742667
0.953257351735028	-0.211375446354457
0.953290536636544	-0.211303742748232
0.953323662997336	-0.211232174695032
0.953356819319502	-0.211160495741096
0.953389885504897	-0.211088948530208
0.953422862310051	-0.211017578994097
0.953455781266871	-0.210946344061606
0.953488730578593	-0.210874998356383
0.953521590389132	-0.210803783286228
0.953554361277519	-0.210732744796391
0.953587074999959	-0.210661839973930
0.953619819471133	-0.210590824502347
0.953652475066982	-0.210519938570329
0.953685042189052	-0.210449228136716
0.953717552817728	-0.210378650447201
0.953750094589435	-0.210307962227513
0.953782548102111	-0.210237402464164
0.953814913579820	-0.210167017129658
0.953847223227019	-0.210096763628754
0.953879564411943	-0.210026399712207
0.953911817944728	-0.209956163180853
0.953943983871946	-0.209886100020938
0.953976094622033	-0.209816167796725
0.954008237305032	-0.209746125266848
0.954040292933543	-0.209676209062908
0.954072261376622	-0.209606465184971
0.954104175286602	-0.209536851357253
0.954136121525186	-0.209467127329367
0.954167981297844	-0.209397528579861
0.954199754296088	-0.209328101122705
0.954231473396071	-0.209258802842524
0.954263225220924	-0.209189394463116
0.954294891159478	-0.209120110326048
0.954326470725658	-0.209050996459278
0.954357997019375	-0.208982010908308
0.954389556434772	-0.208912915354640
0.954421030534713	-0.208843943018605
0.954452418655477	-0.208775139942239
0.954483754120685	-0.208706464332395
0.954515123105072	-0.208637678811747
0.954546407336201	-0.208569015495178
0.954577605972647	-0.208500520438901
0.954608752561695	-0.208432152011601
0.954639933068011	-0.208363673761046
0.954671029374771	-0.208295316711999
0.954702040462762	-0.208227126934939
0.954733000102913	-0.208159062960885
0.954763994059215	-0.208090889246406
0.954794904361303	-0.208022835741675
0.954825729812091	-0.207954948531536
0.954856504406130	-0.207887186309844
0.954887313715851	-0.207819314426249
0.954918039908479	-0.207751561771279
0.954948681608950	-0.207683974444251
0.954979273035437	-0.207616511302367
0.955009899578021	-0.207548938572347
0.955040443532540	-0.207481484100307
0.955070903345846	-0.207414194000141
0.955101313459739	-0.207347027292923
0.955131759090866	-0.207279751067016
0.955162122654999	-0.207212592138753
0.955192402420782	-0.207145596636721
0.955222633053658	-0.207078723746396
0.955252899605888	-0.207011741402009
0.955283084604362	-0.206944875405088
0.955313186139381	-0.206878171899021
0.955343239100066	-0.206811590234235
0.955373328383025	-0.206744899175671
0.955403336617762	-0.206678323524390
0.955433261716086	-0.206611909438703
0.955463138790839	-0.206545616434536
0.955493052591828	-0.206479214092080
0.955522885842541	-0.206412926226569
0.955552636276142	-0.206346799011358
0.955582339229248	-0.206280792128437
0.955612079313442	-0.206214675958328
0.955641739337843	-0.206148673344517
0.955671316856800	-0.206082830475530
0.955700847430770	-0.206017107199994
0.955730415541861	-0.205951274683406
0.955759904076294	-0.205885554812019
0.955789310409420	-0.205819993789654
0.955818670325620	-0.205754551632163
0.955848068185876	-0.205689000275495
0.955877386945375	-0.205623560662325
0.955906623800279	-0.205558279011909
0.955935814758985	-0.205493115507915
0.955965044070003	-0.205427842841485
0.955994194749043	-0.205362681026109
0.956023263812874	-0.205297676296618
0.956052287494014	-0.205232789005096
0.956081349936724	-0.205167792583545
0.956110334209224	-0.205102906129719
0.956139237148671	-0.205038175894163
0.956168095211826	-0.204973562397999
0.956196992447203	-0.204908839799057
0.956225811967231	-0.204844226293491
0.956254550429232	-0.204779768147711
0.956283244514335	-0.204715426052498
0.956311978183373	-0.204650974877439
0.956340634585124	-0.204586631930247
0.956369210196832	-0.204522443493349
0.956397741924143	-0.204458370427824
0.956426313648639	-0.204394188300049
0.956454808547212	-0.204330113543346
0.956483222916777	-0.204266192456313
0.956511593887655	-0.204202386070975
0.956540005270115	-0.204138470636607
0.956568340261420	-0.204074661725092
0.956596594977891	-0.204011005651363
0.956624806774693	-0.203947463619047
0.956653059399114	-0.203883812545505
0.956681236060647	-0.203820267155050
0.956709332694745	-0.203756873779116
0.956737386881603	-0.203693593793606
0.956765482313389	-0.203630204770153
0.956793502204153	-0.203566920598345
0.956821442308187	-0.203503787626285
0.956849340430919	-0.203440767402837
0.956877280217579	-0.203377638139331
0.956905144878772	-0.203314612904229
0.956932929987330	-0.203251738062484
0.956960673574128	-0.203188975336610
0.956988459245239	-0.203126103563932
0.957016170200223	-0.203063335004496
0.957043801830138	-0.203000716040281
0.957071392391530	-0.202938208568160
0.957099025459518	-0.202875592036759
0.957126584214589	-0.202813077911397
0.957154063865702	-0.202750712591274
0.957181502895318	-0.202688458148335
0.957208984855149	-0.202626094629266
0.957236392899235	-0.202563832716874
0.957263722054095	-0.202501718827764
0.957291011028364	-0.202439715209689
0.957318343358591	-0.202377602492520
0.957345602164289	-0.202315590590394
0.957372782289188	-0.202253725937525
0.957399922668369	-0.202191970958212
0.957427106830673	-0.202130106852409
0.957454217853798	-0.202068342777624
0.957481250398317	-0.202006725185878
0.957508243626040	-0.201945216678777
0.957535281066322	-0.201883599011482
0.957562245746985	-0.201822080598684
0.957589132145067	-0.201760707910426
0.957615979649418	-0.201699443726383
0.957642871797232	-0.201638070344044
0.957669691559281	-0.201576795447066
0.957696433228677	-0.201515665523726
0.957723136421621	-0.201454643532555
0.957749884691428	-0.201393512298300
0.957776560943693	-0.201332478787557
0.957803159287197	-0.201271589507066
0.957829719565835	-0.201210807594999
0.957856325356227	-0.201149916390749
0.957882859491752	-0.201089122155332
0.957909315896439	-0.201028471414170
0.957935734642221	-0.200967927485899
0.957962199337396	-0.200907274209206
0.957988592734898	-0.200846717153747
0.958014908573572	-0.200786302863869
0.958041187153767	-0.200725994839478
0.958067512122444	-0.200665577406362
0.958093766145241	-0.200605255453838
0.958119942775373	-0.200545075545414
0.958146082541978	-0.200485001363116
0.958172269139285	-0.200424817703901
0.958198385137169	-0.200364728791516
0.958224423902754	-0.200304781208885
0.958250426194381	-0.200244938820991
0.958276475760226	-0.200184986884422
0.958302455067847	-0.200125128967674
0.958328357297800	-0.200065411673336
0.958354223438037	-0.200005799050227
0.958380137299631	-0.199946076797790
0.958405981238997	-0.199886447844854
0.958431748249639	-0.199826958813943
0.958457479549571	-0.199767573938577
0.958483259019021	-0.199708079350443
0.958508968897121	-0.199648677348042
0.958534601989812	-0.199589414574094
0.958560199745609	-0.199530255447735
0.958585846123369	-0.199470986514863
0.958611423235586	-0.199411809460461
0.958636923700120	-0.199352770947737
0.958662389196485	-0.199293835582326
0.958687903767837	-0.199234790315064
0.958713349394462	-0.199175836225363
0.958738718505602	-0.199117019997192
0.958764053012233	-0.199058306423641
0.958789437052072	-0.198999482840602
0.958814752463050	-0.198940749740547
0.958839991485245	-0.198882153828519
0.958865196261643	-0.198823660085970
0.958890451029265	-0.198765056226682
0.958915637479029	-0.198706542161961
0.958940747661275	-0.198648164618203
0.958965823951493	-0.198589888766225
0.958990950697484	-0.198531502674952
0.959016009431784	-0.198473205696000
0.959040992014422	-0.198415044577460
0.959065941053991	-0.198356984680433
0.959090941012410	-0.198298814425081
0.959115873260565	-0.198240732605764
0.959140729467561	-0.198182785992551
0.959165552475611	-0.198124940137893
0.959190426874163	-0.198066983785908
0.959215233859143	-0.198009115199699
0.959239964908137	-0.197951381171692
0.959264663097643	-0.197893747446605
0.959289413145593	-0.197836003094149
0.959314096072045	-0.197778345842960
0.959338703162410	-0.197720822508104
0.959363277727998	-0.197663399027708
0.959387904631871	-0.197605864762218
0.959412464701677	-0.197548416939398
0.959436949030035	-0.197491102397374
0.959461401163819	-0.197433887268585
0.959485906108264	-0.197376561214972
0.959510344501579	-0.197319320950953
0.959534707242883	-0.197262213337982
0.959559038115129	-0.197205204704061
0.959583422287558	-0.197148084965620
0.959607740187231	-0.197091050369529
0.959631982519130	-0.197034147801058
0.959656193303158	-0.196977343784616
0.959680457863106	-0.196920428517111
0.959704656424303	-0.196863597749962
0.959728779496825	-0.196806898392489
0.959752871338001	-0.196750297166921
0.959777017456669	-0.196693584483287
0.959801097846084	-0.196636955663833
0.959825102820785	-0.196580457642515
0.959849076876554	-0.196524057340100
0.959873105686825	-0.196467545431561
0.959897069033113	-0.196411116755935
0.959920957033563	-0.196354818271967
0.959944814422785	-0.196298617100639
0.959968727084017	-0.196242304079909
0.959992574542059	-0.196186073666738
0.960016346718053	-0.196129972845401
0.960040088586716	-0.196073968937565
0.960063886201570	-0.196017853040895
0.960087618869963	-0.195961819130860
0.960111276315054	-0.195905914217271
0.960134903751832	-0.195850105824580
0.960158587474904	-0.195794185147871
0.960182206503751	-0.195738345843078
0.960205750363014	-0.195682634946544
0.960229264509633	-0.195627020185504
0.960252835406140	-0.195571293028587
0.960276341856799	-0.195515646632560
0.960299773186564	-0.195460128060024
0.960323175094082	-0.195404705243845
0.960346634325835	-0.195349169657056
0.960370029355543	-0.195293714226988
0.960393349308097	-0.195238386043935
0.960416640126204	-0.195183153245479
0.960439988707007	-0.195127807627440
0.960463273325994	-0.195072541564431
0.960486482906501	-0.195017402173635
0.960509663634280	-0.194962357801555
0.960532902754500	-0.194907200105041
0.960556078148360	-0.194852121370042
0.960579178537609	-0.194797168742845
0.960602250354569	-0.194742310776223
0.960625380949881	-0.194687339565488
0.960648448051132	-0.194632446723110
0.960671440176412	-0.194577679422691
0.960694404002163	-0.194523006429969
0.960717427330400	-0.194468219464476
0.960740387391722	-0.194413510284935
0.960763272501220	-0.194358926095894
0.960786129585070	-0.194304435870087
0.960809046452575	-0.194249832007523
0.960831900277787	-0.194195305345007
0.960854679169664	-0.194140903114379
0.960877430298972	-0.194086594506797
0.960900242103993	-0.194032171132579
0.960922991085525	-0.193977824388262
0.960945665148418	-0.193923601539246
0.960968311717464	-0.193869471982677
0.960991019038614	-0.193815228493669
0.961013663753538	-0.193761061053686
0.961036233557807	-0.193707016954482
0.961058776120042	-0.193653065819783
0.961081380634756	-0.193598998881774
0.961103922753575	-0.193545007437401
0.961126389967567	-0.193491138816025
0.961148830205698	-0.193437362842813
0.961171332074502	-0.193383472868189
0.961193771757709	-0.193329657807234
0.961216136532702	-0.193275965012901
0.961238474569058	-0.193222364550387
0.961260876016189	-0.193168646815974
0.961283215479356	-0.193115003459794
0.961305480032595	-0.193061481879192
0.961327718115871	-0.193008052329000
0.961350018512829	-0.192954509193544
0.961372257129592	-0.192901039849337
0.961394420819620	-0.192847691710909
0.961416558255492	-0.192794435297233
0.961438760894326	-0.192741059340235
0.961460901945673	-0.192687756669632
0.961482968064120	-0.192634574756426
0.961505008209630	-0.192581484282472
0.961527110946349	-0.192528281638089
0.961549152293086	-0.192475151670482
0.961571118671886	-0.192422141854206
0.961593059258159	-0.192369223181090
0.961615067472653	-0.192316181159785
0.961637014481161	-0.192263211362560
0.961658886518398	-0.192210361342868
0.961680733077124	-0.192157602197793
0.961702641684042	-0.192104734312504
0.961724489275468	-0.192051937987875
0.961746261831049	-0.191999260753021
0.961768009024545	-0.191946674105546
0.961789827490540	-0.191893957337002
0.961811585118476	-0.191841311772271
0.961833267727301	-0.191788785061978
0.961854925361949	-0.191736348687320
0.961876642869041	-0.191683811010559
0.961898299717155	-0.191631343757920
0.961919881425308	-0.191578994499940
0.961941438153439	-0.191526735301338
0.961963072150967	-0.191474333459285
0.961984645669021	-0.191422001868348
0.962006144124869	-0.191369788302182
0.962027618145836	-0.191317664554624
0.962049146675055	-0.191265454773664
0.962070614876591	-0.191213314223149
0.962092007775344	-0.191161290487577
0.962113375993140	-0.191109356318281
0.962134831962730	-0.191057255990100
0.962156227814388	-0.191005225078378
0.962177548599510	-0.190953311525814
0.962198845573468	-0.190901487284364
0.962220185641867	-0.190849607149378
0.962241465667520	-0.190797794923993
0.962262670115423	-0.190746098154626
0.962283850031140	-0.190694490515485
0.962305136459856	-0.190642672868344
0.962326363169623	-0.190590924016537
0.962347514928397	-0.190539292151158
0.962368643678290	-0.190487749061262
0.962389793211651	-0.190436207027731
0.962410882881931	-0.190384731329895
0.962431896460976	-0.190333369389117
0.962452885383632	-0.190282096263672
0.962474013825834	-0.190230534241530
0.962495083079497	-0.190179040773224
0.962516077809627	-0.190127664421143
0.962537050677301	-0.190076376173085
0.962558004352558	-0.190025189389934
0.962578898080591	-0.189974066917422
0.962599714670788	-0.189923055941646
0.962620506012021	-0.189872133763872
0.962641490661798	-0.189820792681316
0.962662417035545	-0.189769520527074
0.962683270074655	-0.189718366367272
0.962704102981325	-0.189667299208282
0.962724854973804	-0.189616487198001
0.962745546259730	-0.189565736813788
0.962766158162345	-0.189515094992558
0.962786743545046	-0.189464542714544
0.962807592410709	-0.189413401633659
0.962828384951362	-0.189362330598045
0.962849107134940	-0.189311379065222
0.962869811634383	-0.189260512216418
0.962890373376705	-0.189210052878090
0.962910871957838	-0.189159652019370
0.962931286282929	-0.189109356915700
0.962951672319831	-0.189059154042250
0.962972345476649	-0.189008310195804
0.962992966951026	-0.188957537301237
0.963013524997145	-0.188906883724749
0.963034067573366	-0.188856309387787
0.963054542951529	-0.188805949439595
0.963074948556077	-0.188755646676832
0.963095259415727	-0.188705451694574
0.963115542032840	-0.188655356562079
0.963135815209656	-0.188605373736630
0.963156047472383	-0.188555456847909
0.963176230092259	-0.188505646720759
0.963196393666396	-0.188455903615582
0.963217314783991	-0.188404313750670
0.963238147502990	-0.188352792666668
0.963258859395609	-0.188301407914280
0.963279557428989	-0.188250145458595
0.963298779430473	-0.188202709569621
0.963317979245342	-0.188155308235560
0.963337143028024	-0.188107959239591
0.963356260914301	-0.188060655987965
0.963373356617657	-0.188018280388537
0.963390401491027	-0.187975972240838
0.963407398630715	-0.187933764579770
0.963424391337702	-0.187891630202961
0.963441400117716	-0.187849517391492
0.963458391466259	-0.187807442877519
0.963475359781772	-0.187765418510601
0.963492302075086	-0.187723431544667
0.963514172747274	-0.187669213653999
0.963535922598575	-0.187615100910987
0.963557506113152	-0.187561207091416
0.963579129301862	-0.187507471499938
0.963596910593211	-0.187463616429525
0.963614673216386	-0.187419731579007
0.963632376513495	-0.187375815677927
0.963649981374920	-0.187331933355452
0.963665545461216	-0.187293010251700
0.963681069685402	-0.187254181692187
0.963696578046481	-0.187215473545685
0.963712112317434	-0.187176833886499
0.963727679107459	-0.187138199219199
0.963743243748839	-0.187099577131889
0.963758793081793	-0.187060967302462
0.963774305482706	-0.187022373840997
0.963790832852470	-0.186981155232999
0.963807300628044	-0.186940000933861
0.963823709921822	-0.186898947937249
0.963840113570195	-0.186857975417370
0.963856540255906	-0.186817032146535
0.963872959572672	-0.186776126719807
0.963889368378333	-0.186735266188552
0.963905755346729	-0.186694432947648
0.963925806834825	-0.186644421205427
0.963945756062542	-0.186594491016336
0.963965568062313	-0.186544725021655
0.963985391878916	-0.186495095446736
0.964002804876796	-0.186451758284865
0.964020210983562	-0.186408420584699
0.964037587240907	-0.186365082394802
0.964054895737409	-0.186321768967217
0.964070263954730	-0.186283183871347
0.964085585141321	-0.186244674757013
0.964100872833484	-0.186206270831614
0.964116170680307	-0.186167936993653
0.964131494274272	-0.186129619797176
0.964146814628001	-0.186091326275197
0.964162124347042	-0.186053058212864
0.964177407025810	-0.186014809928472
0.964197750642379	-0.185963853702809
0.964217971451554	-0.185912992899877
0.964238022222550	-0.185862333476657
0.964258110466510	-0.185811834630780
0.964274793433130	-0.185770254484886
0.964291475830878	-0.185728642528129
0.964308122188253	-0.185686989068817
0.964324676552891	-0.185645349104714
0.964342556329755	-0.185600185920961
0.964360345339980	-0.185555166365288
0.964378056710777	-0.185510380903533
0.964395849521532	-0.185465712320176
0.964410722813251	-0.185428634820744
0.964425587392771	-0.185391517770779
0.964440405042518	-0.185354359369795
0.964455141396108	-0.185317210764895
0.964472616168968	-0.185273003570199
0.964489994469712	-0.185228929870090
0.964507285465220	-0.185185076408437
0.964524646942410	-0.185141346238674
0.964539340461072	-0.185104610025977
0.964554035471570	-0.185067840514966
0.964568698150174	-0.185031031523479
0.964583288100296	-0.184994224530968
0.964600471180925	-0.184950712466963
0.964617554402838	-0.184907319265141
0.964634540686381	-0.184864127021314
0.964651582317582	-0.184821061412168
0.964666256318090	-0.184784254768988
0.964680939021294	-0.184747423698837
0.964695601835323	-0.184710559076361
0.964710200474551	-0.184673692549579
0.964727443096218	-0.184629986769966
0.964744580551721	-0.184586391424922
0.964761607533919	-0.184542990502608
0.964778683322131	-0.184499721904393
0.964793379595670	-0.184462774481140
0.964808087633967	-0.184425804081772
0.964822780080447	-0.184388799945249
0.964837409029081	-0.184351792018368
0.964854455313400	-0.184308500586682
0.964871396940825	-0.184265317424694
0.964888228171326	-0.184222325427994
0.964905106990709	-0.184179465021325
0.964919677401760	-0.184142758184164
0.964934260710620	-0.184106028783059
0.964948830181140	-0.184069265546501
0.964963337113321	-0.184032497528433
0.964980199177341	-0.183989591507319
0.964996957201537	-0.183946791858131
0.965013605056088	-0.183904180517074
0.965030299594001	-0.183861699930368
0.965044747897688	-0.183825226950384
0.965059209972345	-0.183788731588073
0.965073659557602	-0.183752202159842
0.965088047277108	-0.183715667148650
0.965104726628447	-0.183673143421526
0.965121302726477	-0.183630724551474
0.965137769295081	-0.183588491562305
0.965154282020887	-0.183546388307931
0.965168605600142	-0.183510158436771
0.965182943623641	-0.183473906163898
0.965197270184023	-0.183437619475678
0.965211535372369	-0.183401326524062
0.965228031244247	-0.183359188292330
0.965244424783443	-0.183317153610137
0.965260709748601	-0.183275302567630
0.965277040521030	-0.183233580090953
0.965291238251512	-0.183197598151674
0.965305450987986	-0.183161593730556
0.965319653131054	-0.183125554536298
0.965333794343677	-0.183089508474778
0.965350110693633	-0.183047747551923
0.965366325644738	-0.183006088980227
0.965382433027447	-0.182964611958203
0.965398585965551	-0.182923262322724
0.965412659021045	-0.182887527230035
0.965426747583476	-0.182851769515854
0.965440826322471	-0.182815976634093
0.965454844505530	-0.182780176321347
0.965470983265823	-0.182738789598028
0.965487021584532	-0.182697504116528
0.965502953419857	-0.182656398195619
0.965518930624092	-0.182615418457234
0.965532879682339	-0.182579930202002
0.965546844708557	-0.182544419161714
0.965560800622201	-0.182508872553383
0.965574696328858	-0.182473317977251
0.965590660489560	-0.182432299802658
0.965606525156438	-0.182391381812195
0.965622284429773	-0.182350641468411
0.965638088917552	-0.182310026115991
0.965651915351405	-0.182274782830407
0.965665758193412	-0.182239516581705
0.965679592600621	-0.182204214358327
0.965693367128320	-0.182168903644561
0.965709159442625	-0.182128248950381
0.965724853195736	-0.182087693423599
0.965740442639959	-0.182047313691096
0.965756077164170	-0.182007057777411
0.965769782325233	-0.181972057575126
0.965783504322781	-0.181937034225316
0.965797218544317	-0.181901974492810
0.965810873201469	-0.181866905755073
0.965826496444738	-0.181826609410016
0.965842022037560	-0.181786411245148
0.965857444385939	-0.181746387071896
0.965872911688539	-0.181706485570936
0.965886497030923	-0.181671726240056
0.965900099633209	-0.181636943576754
0.965913695109996	-0.181602124124366
0.965927231330432	-0.181567295154959
0.965942688284378	-0.181527351985301
0.965958048472253	-0.181487506031568
0.965973306450294	-0.181447832310212
0.965988609259339	-0.181408280145555
0.966002076277372	-0.181373759321801
0.966015560978224	-0.181339214983141
0.966029039202297	-0.181304633451684
0.966042458473764	-0.181270041891238
0.966057751855169	-0.181230446851681
0.966072949326483	-0.181190948082410
0.966088045588322	-0.181151619824686
0.966103186556346	-0.181112412041117
0.966116536745018	-0.181078127312457
0.966129905041921	-0.181043818891290
0.966143267513612	-0.181009472877645
0.966156571334767	-0.180975116320674
0.966171703827396	-0.180935864411461
0.966186741235761	-0.180896707842125
0.966201678396737	-0.180857720098328
0.966216660134507	-0.180818851781065
0.966229894992527	-0.180784800684579
0.966243148388903	-0.180750725724401
0.966256396617820	-0.180716612776761
0.966269586498176	-0.180682488767422
0.966284560734641	-0.180643575076976
0.966299440681579	-0.180604755808929
0.966314221302751	-0.180566103712575
0.966329046364818	-0.180527570031007
0.966342167378396	-0.180493750097488
0.966355307366765	-0.180459906136614
0.966368442854035	-0.180426023798515
0.966381520295889	-0.180392129875050
0.966396338858212	-0.180353549578057
0.966411063894052	-0.180315062797075
0.966425690483745	-0.180276741563921
0.966440361370484	-0.180238537770269
0.966453370010370	-0.180204946533798
0.966466398069045	-0.180171331114674
0.966479422303504	-0.180137676934199
0.966492388797869	-0.180104010638388
0.966507054218458	-0.180065758993237
0.966521626843516	-0.180027599967325
0.966536101858954	-0.179989604893587
0.966550621018564	-0.179951726320892
0.966563518737195	-0.179918361327954
0.966576436327194	-0.179884972006072
0.966589350781920	-0.179851543544645
0.966602207804857	-0.179818102430759
0.966616722565459	-0.179780174782576
0.966631145229154	-0.179742338865258
0.966645471075934	-0.179704665331148
0.966659840904165	-0.179667107396629
0.966672629133355	-0.179633966213404
0.966685437695927	-0.179600800564470
0.966698243825539	-0.179567595403983
0.966710992835353	-0.179534377046019
0.966725359368257	-0.179496768824366
0.966739634470397	-0.179459251452544
0.966753813503946	-0.179421894920303
0.966768036345704	-0.179384653123300
0.966780716495884	-0.179351733338754
0.966793417451655	-0.179318788961701
0.966806116691304	-0.179285804707492
0.966818759127455	-0.179252806702214
0.966832979816201	-0.179215513420202
0.966847109707738	-0.179178310113375
0.966861144234199	-0.179141266126623
0.966875222384531	-0.179104336047896
0.966887795844163	-0.179071635276285
0.966900390592481	-0.179038909795729
0.966912984357098	-0.179006144079009
0.966925521639408	-0.178973364048422
0.966939598819952	-0.178936381300759
0.966953585804169	-0.178899487659156
0.966967478081652	-0.178862751841115
0.966981413787066	-0.178826129141038
0.966993881922478	-0.178793645023216
0.967006371841208	-0.178761136090730
0.967018861525245	-0.178728586569847
0.967031295053592	-0.178696022162483
0.967045231015278	-0.178659345624088
0.967059077348774	-0.178622757327328
0.967072829588371	-0.178586325379554
0.967086625047897	-0.178550005796836
0.967098989203266	-0.178517736001080
0.967111375648756	-0.178485441296002
0.967123762626108	-0.178453105657242
0.967136093780346	-0.178420754548973
0.967149890767240	-0.178384379972678
0.967163598661251	-0.178348092777516
0.967177213028371	-0.178311960477701
0.967190870394913	-0.178275939827195
0.967203131892475	-0.178243882049411
0.967215416199745	-0.178211799279039
0.967227701823936	-0.178179675236817
0.967239931964057	-0.178147535131048
0.967253592175943	-0.178111458346179
0.967267163797328	-0.178075468085112
0.967280642412677	-0.178039631285727
0.967294163794014	-0.178003905457088
0.967306323934214	-0.177972057421092
0.967318507417115	-0.177940184320961
0.967330693021438	-0.177908269618097
0.967342823487725	-0.177876338246043
0.967356349081394	-0.177840555156241
0.967369786553907	-0.177804857735345
0.967383131494736	-0.177769312361516
0.967396518954768	-0.177733877317095
0.967408579016623	-0.177702236774320
0.967420662968192	-0.177670571107918
0.967432749866088	-0.177638863515355
0.967444781979480	-0.177607138635747
0.967458175069787	-0.177571645217373
0.967471480475106	-0.177536236614724
0.967484693776220	-0.177500978662679
0.967497949335980	-0.177465830435991
0.967509910577350	-0.177434395165375
0.967521896270104	-0.177402934724025
0.967533885755458	-0.177371432040722
0.967545820817861	-0.177339911439684
0.967559083478913	-0.177304703739876
0.967572258857802	-0.177269580003610
0.967585342512677	-0.177234605538761
0.967598468151445	-0.177199740232603
0.967610331809409	-0.177168508040199
0.967622220495721	-0.177137250642690
0.967634113843267	-0.177105950695244
0.967645953137962	-0.177074632185912
0.967659087404205	-0.177039706320867
0.967672134757570	-0.177004863567466
0.967685090719380	-0.176970168722715
0.967698088375692	-0.176935582507499
0.967709855666898	-0.176904551226098
0.967721648579373	-0.176873494718306
0.967733447045093	-0.176842395360597
0.967745191837149	-0.176811276782728
0.967758199704478	-0.176776628935902
0.967771120994445	-0.176742063348395
0.967783951177089	-0.176707644322354
0.967796822749758	-0.176673333434363
0.967808494870760	-0.176642500923137
0.967820193222589	-0.176611643177695
0.967831898044100	-0.176580742290544
0.967843549580770	-0.176549821510166
0.967856433007461	-0.176515447930925
0.967869230158275	-0.176481155757537
0.967881936437229	-0.176447008813184
0.967894683786181	-0.176412969553263
0.967906261913770	-0.176382333697395
0.967917866899082	-0.176351672613326
0.967929479296021	-0.176320968104153
0.967941038807147	-0.176290243013194
0.967953799715058	-0.176256140014748
0.967966474614238	-0.176222117566826
0.967979058827655	-0.176188239029450
0.967991683775005	-0.176154467760988
0.968003169066620	-0.176124026471061
0.968014681860922	-0.176093559973187
0.968026203035433	-0.176063049775421
0.968037671733945	-0.176032518291090
0.968050312009391	-0.175998682249223
0.968062866508574	-0.175964925899960
0.968075330458074	-0.175931312155883
0.968087834788899	-0.175897805303586
0.968099228382907	-0.175867556515290
0.968110650143397	-0.175837282553959
0.968122081280479	-0.175806964626776
0.968133460362771	-0.175776624691274
0.968145981857485	-0.175743052042862
0.968158417773342	-0.175709558225803
0.968170763224860	-0.175676205720898
0.968183148688025	-0.175642959769345
0.968194451704084	-0.175612901442942
0.968205783570041	-0.175582817993516
0.968217125837998	-0.175552690321339
0.968228416484392	-0.175522539901323
0.968240821016551	-0.175489227142660
0.968253140131760	-0.175455992350016
0.968265368816458	-0.175422897588021
0.968277637125497	-0.175389909080025
0.968288850664892	-0.175360039199864
0.968300093758049	-0.175330144262252
0.968311348308917	-0.175300204854295
0.968322551684118	-0.175270241940387
0.968334841039224	-0.175237185625850
0.968347045103313	-0.175204206407142
0.968359158718343	-0.175171365948311
0.968371311552199	-0.175138631483625
0.968382436698144	-0.175108948057709
0.968393592123034	-0.175079239655958
0.968404760092985	-0.175049486545832
0.968415877346514	-0.175019709152184
0.968428053278238	-0.174986905893010
0.968440144008365	-0.174954178853832
0.968452144217586	-0.174921589313688
0.968464183221284	-0.174889105547811
0.968475221039220	-0.174859606607347
0.968486289883518	-0.174830082789227
0.968497372393274	-0.174800514034536
0.968508404659906	-0.174770920198381
0.968520468891070	-0.174738366661048
0.968532447972960	-0.174705888461424
0.968544336407770	-0.174673546509118
0.968556263193224	-0.174641310151712
0.968567214731150	-0.174611993750558
0.968578198066049	-0.174582652587032
0.968589196221333	-0.174553266268861
0.968600144621590	-0.174523854049954
0.968612098844903	-0.174491546955210
0.968623967933514	-0.174459314308595
0.968635746193442	-0.174427216665897
0.968647562340006	-0.174395224479842
0.968658428628714	-0.174366088694161
0.968669327509220	-0.174336928279075
0.968680242401132	-0.174307722501697
0.968691108041690	-0.174278489981963
0.968702953920668	-0.174246426103362
0.968714714641051	-0.174214435775150
0.968726384294506	-0.174182579214949
0.968738091349673	-0.174150828014914
0.968748873403059	-0.174121870942606
0.968759688868360	-0.174092889392155
0.968770521573840	-0.174063862282517
0.968781305548035	-0.174034807565480
0.968793044717762	-0.174002983728328
0.968804698665750	-0.173971232534762
0.968816261250607	-0.173939613879961
0.968827860730552	-0.173908100531371
0.968838559545870	-0.173879320291618
0.968849292619656	-0.173850515743935
0.968860044201905	-0.173821665451263
0.968870747590199	-0.173792786661587
0.968882381658192	-0.173761199741620
0.968893930401180	-0.173729684548436
0.968905387425444	-0.173698300670583
0.968916880815631	-0.173667022088331
0.968927497373743	-0.173638416821124
0.968938149064530	-0.173609787435847
0.968948820573445	-0.173581112131242
0.968959444443912	-0.173552407414245
0.968970974990811	-0.173521054336760
0.968982420068373	-0.173489772058270
0.968993773010661	-0.173458619876619
0.969005161766271	-0.173427573024216
0.969015697031836	-0.173399140889990
0.969026268333240	-0.173370684847951
0.969036860805811	-0.173342182724093
0.969047406214591	-0.173313650245386
0.969058834795028	-0.173282527983918
0.969070177719685	-0.173251475581639
0.969081428029856	-0.173220552061761
0.969092713576345	-0.173189733950039
0.969103168498111	-0.173161473129021
0.969113660389223	-0.173133188631640
0.969124174850051	-0.173104857902220
0.969134642841925	-0.173076495847031
0.969145970985234	-0.173045601422446
0.969157213243067	-0.173014775904143
0.969168362342680	-0.172984078056931
0.969179546076170	-0.172953485743163
0.969189921587111	-0.172925394435059
0.969200335032743	-0.172897279704096
0.969210772494429	-0.172869118603591
0.969221164103283	-0.172840925176455
0.969232393314224	-0.172810255656033
0.969243536365484	-0.172779654074736
0.969254585648238	-0.172749178955401
0.969265668935877	-0.172718809542400
0.969275965953393	-0.172690885965894
0.969286301904382	-0.172662939243010
0.969296663368007	-0.172634946026281
0.969306979617382	-0.172606919450519
0.969318111376968	-0.172576471946771
0.969329156656787	-0.172546091399524
0.969340107489039	-0.172515836106301
0.969351091669429	-0.172485686741261
0.969359126120693	-0.172463877599030
0.969367185611790	-0.172442054993026
0.969375256741815	-0.172420206647425
0.969383312772285	-0.172398336636892

==> matlab/fig2a2.tex <==
0	0
1.15980193919542e-05	-0.00478865553848715
4.54078190390233e-05	-0.00941408565709344
0.000100192993358230	-0.0139197798701548
0.000175037113046884	-0.0183307019366436
0.000269257772586993	-0.0226591018469411
0.000382240394939396	-0.0269159824204762
0.000513454547862948	-0.0311092254394858
0.000662428828627291	-0.0352449568144938
0.000926371510781328	-0.0415286007620253
0.00123027759398286	-0.0477000014216694
0.00157291033953699	-0.0537700066029077
0.00195315423234964	-0.0597472470648624
0.00260229277864609	-0.0686877915873390
0.00333314161045606	-0.0774482187696411
0.00414280453521921	-0.0860440988664459
0.00502864590288711	-0.0944880066844984
0.00638910302800126	-0.106047926549303
0.00788760095309145	-0.117353457355015
0.00951871129773872	-0.128423131846203
0.0112774390318705	-0.139272214647978
0.0135773024614690	-0.152163688021957
0.0160508973108055	-0.164767363585555
0.0186911947787527	-0.177099212785845
0.0214916291433401	-0.189172778566791
0.0249147684646375	-0.202801106686161
0.0285342622215576	-0.216115846920466
0.0323418330834285	-0.229130197230828
0.0363296570525169	-0.241855610764023
0.0408594264329134	-0.255369550804472
0.0455844131580969	-0.268565226205752
0.0504960862718272	-0.281452659196328
0.0555863002228618	-0.294040750850721
0.0612230236815347	-0.307190341468678
0.0670462613166649	-0.320014912021357
0.0730472944961938	-0.332522427115532
0.0792177397573890	-0.344720106245409
0.0859282591615869	-0.357307434709409
0.0928105633019768	-0.369561834084641
0.0998557890326658	-0.381489973454610
0.107055372901146	-0.393098017366477
0.114781290399057	-0.404962111547402
0.122659388995099	-0.416485068119059
0.130680698575646	-0.427672806676123
0.138836525436676	-0.438530902788040
0.147496418247635	-0.449534151118188
0.156284786376413	-0.460188797575760
0.165192605210758	-0.470500411233925
0.174211112877386	-0.480474327624915
0.183704057017417	-0.490500081774411
0.193298373874680	-0.500171406309539
0.202985053882671	-0.509493818159961
0.212755344101295	-0.518472677807720
0.222964770909743	-0.527425139507910
0.233245769506287	-0.536019685507764
0.243589430032811	-0.544262005633853
0.253987099034980	-0.552157686660356
0.264784756662266	-0.559962179880742
0.275622183023615	-0.567408136398059
0.286490664488448	-0.574501587307244
0.297381748095875	-0.581248496286604
0.308631550058653	-0.587851479352239
0.319887996224227	-0.594098530124993
0.331142674141541	-0.599996143670398
0.342387439575751	-0.605550769326095
0.353949043874076	-0.610919421532467
0.365483495208137	-0.615938191515851
0.376982792623076	-0.620614123265104
0.388439213151444	-0.624954225331667
0.400171234128865	-0.629075622514176
0.411842235662560	-0.632856737702739
0.423444741520864	-0.636305217164510
0.434971564525446	-0.639428672377525
0.446734372158614	-0.642308630669823
0.458402772847212	-0.644861470048254
0.469969929503628	-0.647095465850756
0.481429305629653	-0.649018850857640
0.493087408032027	-0.650680530750295
0.504618682743623	-0.652031761084353
0.516017046515471	-0.653081450741276
0.527276727954172	-0.653838450698607
0.538700760984643	-0.654320802043903
0.549966937119740	-0.654512774402894
0.561070041840226	-0.654423895975356
0.572005182799019	-0.654063614659121
0.583073547007428	-0.653419720756883
0.593954777576051	-0.652508785455811
0.604644644657276	-0.651340926461604
0.615139249293464	-0.649926151965825
0.625739441684574	-0.648221502945267
0.636125272242839	-0.646276272713811
0.646293614769231	-0.644101125779962
0.656241680415696	-0.641706581042613
0.666271369779100	-0.639017273340438
0.676061745764982	-0.636116833135840
0.685610911364513	-0.633016418543908
0.694917310401766	-0.629726998647077
0.704285203245075	-0.626137811817332
0.713391259293042	-0.622369831858724
0.722234948746583	-0.618434649075057
0.730816082270387	-0.614343613021337
0.739281228234001	-0.610030838552524
0.747475098567644	-0.605579665922582
0.755398624727503	-0.601001387976056
0.763053049548637	-0.596307018372117
0.770475878362228	-0.591483282290901
0.777630476579613	-0.586563852650487
0.784519100699251	-0.581559137871867
0.791144269941093	-0.576479246887759
0.797551507999156	-0.571298536114122
0.803697676724153	-0.566061350769390
0.809586198880985	-0.560777161853403
0.815220711804925	-0.555455123801365
0.820651924130286	-0.550056324276670
0.825832761212875	-0.544636817637959
0.830767666482887	-0.539205091345493
0.835461249977026	-0.533769302410414
0.839966113805494	-0.528277483203461
0.844234381811759	-0.522797319542798
0.848271381908357	-0.517336271485269
0.852082560430611	-0.511901458060835
0.855719570955815	-0.506428423439272
0.859136450945896	-0.500996029190065
0.862339283328799	-0.495610666083226
0.865334220679469	-0.490278376734230
0.868169530006166	-0.484923051870398
0.870803497750940	-0.479633988108654
0.873242836931810	-0.474416466519988
0.875494280472123	-0.469275416541638
0.877600637110875	-0.464124112512971
0.879526432925783	-0.459061331500799
0.881278888775135	-0.454091205123368
0.882865194301682	-0.449217513817505
0.884320967564065	-0.444344099737132
0.885618647009175	-0.439578112000875
0.886765840019326	-0.434922492440343
0.887770069762299	-0.430379836497747
0.888658353647118	-0.425845833830945
0.889412416517745	-0.421434799908287
0.890040130093851	-0.417148443957145
0.890549226353065	-0.412988138542111
0.890957028522190	-0.408842740366044
0.891255635308435	-0.404832489492219
0.891453057612517	-0.400957814216174
0.891557107629726	-0.397218821716611
0.891574645121895	-0.393498824472466
0.891508948345778	-0.389922787877751
0.891368036504276	-0.386489800400683
0.891159666344675	-0.383198652117438
0.890879818940817	-0.379928262694511
0.890543471445929	-0.376807285747552
0.890158510705713	-0.373833391435988
0.889732490417610	-0.371003983624553
0.889250525035299	-0.368194414035647
0.888739503636689	-0.365536364326047
0.888207023542708	-0.363025970802790
0.887660267555854	-0.360659148745468
0.887092297820624	-0.358378292617494
0.886523405669982	-0.356238770495454
0.885960090711315	-0.354235506615795
0.885408400648854	-0.352363285833848
0.884871414779060	-0.350608578847918
0.884357155888241	-0.348975172385654
0.883870507092065	-0.347457376353025
0.883415915393903	-0.346049454556955
0.882992283072993	-0.344729505927316
0.882609468956626	-0.343510242137525
0.882270848786561	-0.342385570872507
0.881979380948416	-0.341349438767975
0.881733147543778	-0.340376847201911
0.881541040852614	-0.339483835519157
0.881404985906334	-0.338664089604416
0.881326513528845	-0.337911416278549
0.881307093871185	-0.337200405538567
0.881350757167682	-0.336547458201176
0.881457992143215	-0.335946207548832
0.881628923024696	-0.335390491014391
0.881873786027299	-0.334854860604836
0.882186558615720	-0.334355437952527
0.882566264544112	-0.333885972943059
0.883011602444359	-0.333440508974546
0.883549351986155	-0.332991413339385
0.884155767385476	-0.332556287829589
0.884828313094196	-0.332129181119820
0.885564183138503	-0.331704538850215
0.886420243018015	-0.331245991313202
0.887341517804034	-0.330778381199941
0.888323677422492	-0.330296274308159
0.889362204254431	-0.329794768329421
0.890477544704635	-0.329257316517323
0.891641710878518	-0.328690785201808
0.892849411986309	-0.328091517695601
0.894095322197486	-0.327456398082608
0.895382720925541	-0.326778193866034
0.896697912465056	-0.326058861582562
0.898035458988309	-0.325296735611565
0.899390028873245	-0.324490626430548
0.900796594964557	-0.323614165674974
0.902210064842068	-0.322690007428568
0.903625041929634	-0.321718281905096
0.905036367204851	-0.320699536508994
0.906515440645900	-0.319575213026741
0.907979453244360	-0.318401225631928
0.909423239475656	-0.317179555773634
0.910842020514435	-0.315912532583984
0.912254970688132	-0.314579966794660
0.913633231300909	-0.313206391752876
0.914972980778703	-0.311795215901794
0.916270846954038	-0.310350034850160
0.917489456539344	-0.308916291729764
0.918663395054556	-0.307457641092835
0.919790733844177	-0.305977804060341
0.920869925963413	-0.304480523528377
0.921900876592199	-0.302967931097958
0.922881583493838	-0.301445461913784
0.923811583235935	-0.299916890745439
0.924690740572114	-0.298385896986938
0.925538022977216	-0.296820313308420
0.926332797901650	-0.295259739811946
0.927075920485690	-0.293707800227363
0.927768517725307	-0.292167919604506
0.928440026364036	-0.290574598210208
0.929059764248832	-0.289001514642564
0.929629899508341	-0.287451916693983
0.930152799017227	-0.285928747169404
0.930622439668890	-0.284462445094165
0.931051705630096	-0.283026430769316
0.931443344368415	-0.281622696577960
0.931800171024334	-0.280252936729983
0.932121359247585	-0.278934333365540
0.932414270231138	-0.277651400381538
0.932681797818363	-0.276404993638210
0.932926803657223	-0.275195705086682
0.933153896802758	-0.274014440972721
0.933363903856500	-0.272871370192814
0.933559668463773	-0.271766370413833
0.933743922002835	-0.270699093775881
0.933923582105853	-0.269643735533900
0.934096679716548	-0.268626597019576
0.934265828052241	-0.267646658039586
0.934433456541643	-0.266702721177020
0.934609009121768	-0.265755643196942
0.934787784130555	-0.264844470827786
0.934971971790432	-0.263967330680132
0.935163510021510	-0.263122237085817
0.935377420218096	-0.262255396811482
0.935603427205551	-0.261419858920610
0.935843058658209	-0.260612909153291
0.936097519604811	-0.259831815219592
0.936373667597735	-0.259057888663217
0.936666956029077	-0.258305114556700
0.936977803105567	-0.257570595170079
0.937306328180835	-0.256851530800352
0.937658498341267	-0.256133142434153
0.938028415972001	-0.255425177021670
0.938415445304781	-0.254725023497831
0.938818722349326	-0.254030262277029
0.939258310296645	-0.253304400236992
0.939713193807571	-0.252579610402322
0.940181769511832	-0.251853747778048
0.940662289651624	-0.251124949679031
0.941200190186089	-0.250321306767573
0.941747598550529	-0.249510449814169
0.942301867336887	-0.248690988544441
0.942860336746477	-0.247861927510682
0.943463154771095	-0.246958044211601
0.944064496867729	-0.246041945948100
0.944661232784303	-0.245113705552928
0.945250435658290	-0.244173796953220
0.945845188848288	-0.243196677761564
0.946426393123035	-0.242209405515763
0.946991653013205	-0.241213560199931
0.947538934243770	-0.240210943178327
0.948053267777776	-0.239229437614231
0.948547668070549	-0.238245449999062
0.949021216165340	-0.237261093130191
0.949473322079315	-0.236278475373366
0.949884037091211	-0.235345420115348
0.950275034942336	-0.234417718807141
0.950646572844772	-0.233497146022181
0.950999113409599	-0.232585350105953
0.951339237397413	-0.231667543713121
0.951661267334509	-0.230761976582522
0.951966283105949	-0.229870019201976
0.952255477354978	-0.228992832205734
0.952527238158397	-0.228140672502397
0.952786192969108	-0.227304731090142
0.953033786521225	-0.226485618817351
0.953271461778990	-0.225683735586604
0.953495232541718	-0.224917995404209
0.953712329949654	-0.224168933867842
0.953924101632441	-0.223436451760060
0.954131814062484	-0.222720293184109
0.954338699475951	-0.222013158680635
0.954543879207431	-0.221321751988485
0.954748459137723	-0.220645433364353
0.954953409397079	-0.219983461812195
0.955167451735698	-0.219310628411992
0.955383688537055	-0.218651355981619
0.955602842903554	-0.218004579775515
0.955825461869651	-0.217369201014121
0.956067546346841	-0.216701787352812
0.956314397365164	-0.216044711765639
0.956566189342717	-0.215396609545619
0.956822896266288	-0.214756172321327
0.957106276097850	-0.214069672613873
0.957394817892317	-0.213389195170289
0.957687963478856	-0.212713369106092
0.957984980099627	-0.212040995376287
0.958301473042556	-0.211334473645399
0.958620224146474	-0.210629607999868
0.958940065549511	-0.209925591530829
0.959259775996277	-0.209221856167776
0.959634226205935	-0.208393466722795
0.960004824980658	-0.207564779153032
0.960369737277265	-0.206735949491133
0.960727303833925	-0.205907453504246
0.961043864807642	-0.205157328188002
0.961352278874162	-0.204408854614052
0.961651830894147	-0.203662899532969
0.961942001386783	-0.202920375122536
0.962222456678807	-0.202182235345501
0.962493078580575	-0.201449519778029
0.962753936368982	-0.200723227544428
0.963005257705444	-0.200004257043663
0.963243349373333	-0.199305512895792
0.963473118948442	-0.198615400231597
0.963695197552044	-0.197934555446228
0.963910268953211	-0.197263449522800
0.964110461215757	-0.196629841487921
0.964305637061330	-0.196005733506594
0.964496539549102	-0.195391240271052
0.964683872051774	-0.194786340440305
0.964863893821039	-0.194205152295406
0.965041815362827	-0.193632804305331
0.965218235546831	-0.193069031508865
0.965393665678836	-0.192513485936432
0.965571396977243	-0.191956892324445
0.965749011815283	-0.191407908375717
0.965926870369399	-0.190866025963084
0.966105219801805	-0.190330706893707
0.966292856226689	-0.189776054728475
0.966481350924240	-0.189227375828729
0.966670747739202	-0.188684052442012
0.966860972962320	-0.188145495618967
0.967067084338820	-0.187568787500877
0.967273738812968	-0.186996369350124
0.967480618036259	-0.186427695106125
0.967687313343587	-0.185862309176414
0.967915910970173	-0.185238300284222
0.968143102990060	-0.184617549749809
0.968368267732020	-0.183999852591874
0.968590774914991	-0.183385130906928
0.968832821650506	-0.182709399815830
0.969070223199958	-0.182037626464772
0.969302433965186	-0.181370204470360
0.969529026866454	-0.180707572369891
0.969749228956153	-0.180051647251268
0.969963456331438	-0.179401613827173
0.970171771236700	-0.178758070872067
0.970374342060865	-0.178121495018471
0.970553770008703	-0.177549080885142
0.970729005590694	-0.176983109274109
0.970900429297111	-0.176423824794991
0.971068420721353	-0.175871345311922
0.971222949059910	-0.175360246983420
0.971375191330325	-0.174855172807770
0.971525511432933	-0.174356071273099
0.971674220435921	-0.173862808964779
0.971819775991995	-0.173381205271546
0.971964318537734	-0.172904933370703
0.972108089342742	-0.172433766580366
0.972251254393570	-0.171967437045627
0.972397250547629	-0.171494933751867
0.972542857297732	-0.171026904133834
0.972688143532802	-0.170563049655207
0.972833099486916	-0.170103069263100
0.972984813036701	-0.169624153465595
0.973136031478657	-0.169148906338663
0.973286646070748	-0.168677073982611
0.973436487264461	-0.168208431210355
0.973595030871607	-0.167712500226939
0.973752262380135	-0.167219842212631
0.973907966915331	-0.166730369766331
0.974061908864826	-0.166244029967682
0.974222134924910	-0.165734382265451
0.974379957868865	-0.165228306578622
0.974535229654543	-0.164725928625489
0.974687822965401	-0.164227366233714
0.974838779983302	-0.163728983874031
0.974986938396144	-0.163234822433549
0.975132358799435	-0.162745073132199
0.975275118421015	-0.162259859991875
0.975410644235107	-0.161795364737362
0.975543957782581	-0.161335320362983
0.975675249918517	-0.160879801087099
0.975804690396758	-0.160428802988896
0.975928628614273	-0.159995622133077
0.976051176763053	-0.159566636639327
0.976172517051103	-0.159141784029165
0.976292783440128	-0.158720945859020
0.976411719534543	-0.158305235579810
0.976529826396341	-0.157893254925479
0.976647205689582	-0.157484862534221
0.976763901010247	-0.157079888487107
0.976882571269967	-0.156668984629603
0.977000567781839	-0.156261328798609
0.977117892356474	-0.155856773988032
0.977234494305602	-0.155455167107211
0.977354911019954	-0.155040461886274
0.977474407557952	-0.154628698144714
0.977592914745912	-0.154219794492946
0.977710329812506	-0.153813671477483
0.977831311851859	-0.153393660685596
0.977950916119639	-0.152976608526172
0.978069079390771	-0.152562534483985
0.978185727099363	-0.152151444027622
0.978303173773606	-0.151734866367053
0.978418970598487	-0.151321498894187
0.978533137416231	-0.150911416522938
0.978645688171358	-0.150504649446452
0.978755873096717	-0.150104020745693
0.978864573318796	-0.149706749963903
0.978971885684514	-0.149312877058310
0.979077885285778	-0.148922382873153
0.979181025094404	-0.148541195062342
0.979283072630649	-0.148163243319015
0.979384133574552	-0.147788496969491
0.979484274709867	-0.147416875641080
0.979583284697172	-0.147049230684497
0.979681507908846	-0.146684542661180
0.979779007764643	-0.146322735781658
0.979875802254690	-0.145963702049053
0.979973414102655	-0.145601648838916
0.980070317999728	-0.145242273954984
0.980166522844658	-0.144885502627607
0.980261996778606	-0.144531241293855
0.980359368707722	-0.144169427320233
0.980455899083836	-0.143810140463868
0.980551565669811	-0.143453346923912
0.980646317683343	-0.143098995609672
0.980742687867407	-0.142737285240042
0.980838016730315	-0.142378127730728
0.980932296483840	-0.142021538726503
0.981025501549273	-0.141667503803966
0.981118838451838	-0.141311278040234
0.981211072506975	-0.140957706882644
0.981302240534913	-0.140606821028666
0.981392360793411	-0.140258604981618
0.981481271068024	-0.139913706055821
0.981569216667513	-0.139571467973456
0.981656263163521	-0.139231894464302
0.981742447570848	-0.138894939319827
0.981827444252926	-0.138561903756273
0.981911675568212	-0.138231397280154
0.981995198750283	-0.137903389320942
0.982078034604992	-0.137577807833235
0.982160674021958	-0.137252639008795
0.982242659780538	-0.136929816026503
0.982324019857932	-0.136609296300827
0.982404745595829	-0.136291006091985
0.982486212269820	-0.135969321891136
0.982567006318195	-0.135649849153304
0.982647131623037	-0.135332560773095
0.982726561672217	-0.135017402437525
0.982806972282971	-0.134697479972603
0.982886620104854	-0.134379735264353
0.982965508572661	-0.134064169001309
0.983043618048565	-0.133750749104663
0.983122138739772	-0.133434520221913
0.983199848445303	-0.133120500803739
0.983276771438603	-0.132808706228966
0.983352910595385	-0.132499108992577
0.983428649796280	-0.132190074628459
0.983503634217830	-0.131883250387203
0.983577906679804	-0.131578641864573
0.983651483718210	-0.131276207225964
0.983724418164501	-0.130975683382512
0.983796706438571	-0.130677290798902
0.983868389929781	-0.130381016181991
0.983939478610534	-0.130086802793805
0.984010353437638	-0.129792970681904
0.984080653317446	-0.129501151941623
0.984150403888708	-0.129211325542554
0.984219598942876	-0.128923433426950
0.984289134969713	-0.128633572459619
0.984358094805964	-0.128345634209420
0.984426490665630	-0.128059606454722
0.984494306847889	-0.127775442220229
0.984562645923923	-0.127488325595289
0.984630369505196	-0.127203100415956
0.984697490345367	-0.126919769933595
0.984763997653007	-0.126638298683065
0.984830731232208	-0.126354977649470
0.984896836513370	-0.126073549885294
0.984962337890387	-0.125794025495994
0.985027236818914	-0.125516369647904
0.985091933949881	-0.125238768444973
0.985156044586480	-0.124963038971478
0.985219601610984	-0.124689184805401
0.985282611922709	-0.124417162446010
0.985345316164058	-0.124145838738402
0.985407495350313	-0.123876321073561
0.985469179167543	-0.123608603489404
0.985530368806747	-0.123342635873577
0.985591509463973	-0.123076350124553
0.985652158042835	-0.122811791470213
0.985712334774592	-0.122548952600942
0.985772032147993	-0.122287785490854
0.985831965141613	-0.122024993971806
0.985891400914282	-0.121763876253470
0.985950354436781	-0.121504432483209
0.986008815905792	-0.121246621919409
0.986067540330929	-0.120986948660813
0.986125754185078	-0.120728929212850
0.986183475807354	-0.120472571591574
0.986240700836443	-0.120217839214008
0.986297972640089	-0.119962178688795
0.986354745414792	-0.119708157543915
0.986411044033768	-0.119455784311443
0.986466869985289	-0.119205019618410
0.986522552302278	-0.118954271108093
0.986577771199803	-0.118705124543161
0.986632552988674	-0.118457583288257
0.986686898718422	-0.118211602996122
0.986741139053576	-0.117965559635728
0.986794947279794	-0.117721061972197
0.986848345146195	-0.117478110344272
0.986901328779345	-0.117236659590894
0.986954384003081	-0.116994343419454
0.987007016031656	-0.116753523585559
0.987059242045861	-0.116514203340271
0.987111055237415	-0.116276341185237
0.987163034230626	-0.116037120817138
0.987214586423038	-0.115799368669198
0.987265729267172	-0.115563093293315
0.987316458047089	-0.115328256511036
0.987367274687699	-0.115092389903422
0.987417670123740	-0.114857973499615
0.987467665407150	-0.114625017802324
0.987517259643982	-0.114393483924058
0.987566810007174	-0.114161575049658
0.987615960323772	-0.113931088274672
0.987664733305129	-0.113702031854692
0.987713128731347	-0.113474363969780
0.987761458353915	-0.113246484902173
0.987809410429381	-0.113019986631081
0.987857005441369	-0.112794875386463
0.987904240596579	-0.112571108417796
0.987951501130686	-0.112346712631010
0.987998394537663	-0.112123657904181
0.988044938372570	-0.111901951929666
0.988091127943520	-0.111681553929472
0.988137415277741	-0.111460152732421
0.988183337303502	-0.111240065566678
0.988228911368561	-0.111021303448401
0.988274133914492	-0.110803827596962
0.988319423825156	-0.110585477624620
0.988364354534936	-0.110368421868582
0.988408945335158	-0.110152672864167
0.988453194976038	-0.109938191414978
0.988497434686799	-0.109723235294174
0.988541330084549	-0.109509548145050
0.988584901326494	-0.109297141469268
0.988628147585530	-0.109085974349724
0.988671365202825	-0.108874460529222
0.988714253941339	-0.108664182813764
0.988756832521955	-0.108455151825566
0.988799098653296	-0.108247326249939
0.988841387583455	-0.108038909500874
0.988883355905673	-0.107831697652621
0.988925020646789	-0.107625702570500
0.988966378678703	-0.107420884208286
0.989007800351930	-0.107215257799058
0.989048905350124	-0.107010813079815
0.989089710738567	-0.106807564059978
0.989130214394439	-0.106605471653887
0.989170760404859	-0.106402674211747
0.989210996922072	-0.106201038707577
0.989250942078621	-0.106000579978277
0.989290595103267	-0.105801258370344
0.989330246803207	-0.105601471715699
0.989369600659052	-0.105402823260994
0.989408674912304	-0.105205327330970
0.989447468788962	-0.105008943296011
0.989486258137875	-0.104812131308136
0.989524760126792	-0.104616430273494
0.989562991879875	-0.104421854503375
0.989600951807813	-0.104228363463793
0.989638940290929	-0.104034277801726
0.989676647494525	-0.103841278600981
0.989714089713754	-0.103649381427990
0.989751265339434	-0.103458546566052
0.989788485480798	-0.103267029359024
0.989825429268179	-0.103076578949866
0.989862113267629	-0.102887212241280
0.989898536821108	-0.102698889711248
0.989934984453533	-0.102509996799051
0.989971163348174	-0.102322151490563
0.990007090511117	-0.102135371015791
0.990042765942021	-0.101949615224906
0.990078444642650	-0.101763413884190
0.990113863663029	-0.101578238099491
0.990149039618105	-0.101394105007417
0.990183972290731	-0.101210974064304
0.990218916937545	-0.101027361756978
0.990253608915080	-0.100844752542718
0.990288064053108	-0.100663164136122
0.990322281905629	-0.100482556323783
0.990356530966724	-0.100301365212508
0.990390532270460	-0.100121157754567
0.990424301412535	-0.0999419527757777
0.990457838436486	-0.0997637103911538
0.990491405601313	-0.0995848922544851
0.990524730604675	-0.0994070403672729
0.990557829279293	-0.0992301742712334
0.990590702375504	-0.0990542538053188
0.990623589801333	-0.0988778526630111
0.990656242153273	-0.0987023992911374
0.990688675178840	-0.0985279134069597
0.990720889818084	-0.0983543544178678
0.990753115228176	-0.0981803444026339
0.990785112123239	-0.0980072625935563
0.990816895713819	-0.0978351290673917
0.990848466854533	-0.0976639032465086
0.990880060372253	-0.0974921669553462
0.990911430325523	-0.0973213407225709
0.990942591551214	-0.0971514454522680
0.990973545196874	-0.0969824407811052
0.991004526667322	-0.0968128979230184
0.991035289317691	-0.0966442489003417
0.991065848003344	-0.0964765153854397
0.991096204471413	-0.0963096568882938
0.991126580679423	-0.0961423118239845
0.991156743734558	-0.0959758443390425
0.991186708446158	-0.0958102764842496
0.991216476918426	-0.0956455674160244
0.991246259334496	-0.0954804128274032
0.991275834261127	-0.0953161187610918
0.991305216137934	-0.0951527076302148
0.991334407160587	-0.0949901384742051
0.991363617675374	-0.0948270978815790
0.991392625346458	-0.0946649014060600
0.991421444254351	-0.0945035721298086
0.991450076868373	-0.0943430691726683
0.991478734480619	-0.0941820669602582
0.991507193507745	-0.0940218938876735
0.991535467928668	-0.0938625737507615
0.991563560734490	-0.0937040655626894
0.991591674970061	-0.0935450842012268
0.991619595367219	-0.0933869173128770
0.991647335813982	-0.0932295891644856
0.991674899710292	-0.0930730584782133
0.991702480524207	-0.0929160877902832
0.991729872306360	-0.0927599164794860
0.991757088647199	-0.0926045692306099
0.991784133166324	-0.0924500046081761
0.991811197336386	-0.0922949895702503
0.991838076635503	-0.0921407592237202
0.991864784338407	-0.0919873388619295
0.991891324388468	-0.0918346870326780
0.991917888099221	-0.0916815655580299
0.991944270784907	-0.0915292151034816
0.991970485565618	-0.0913776616175873
0.991996536879739	-0.0912268635113752
0.992022610152102	-0.0910756112389501
0.992048506500261	-0.0909251166400197
0.992074238899323	-0.0907754061672891
0.992099812213760	-0.0906264379724493
0.992125404677819	-0.0904770385528216
0.992150824309481	-0.0903283832844651
0.992176083806898	-0.0901804990917495
0.992201188343840	-0.0900333439599284
0.992226313845565	-0.0898857520065690
0.992251270165870	-0.0897388910599369
0.992276069721598	-0.0895927886396557
0.992300718078577	-0.0894474026467747
0.992325390027934	-0.0893015686937727
0.992349896251726	-0.0891564533328266
0.992374248985959	-0.0890120846989082
0.992398454295706	-0.0888684205148566
0.992422682123689	-0.0887243203511815
0.992446747815176	-0.0885809266028349
0.992470663413609	-0.0884382679233801
0.992494435425080	-0.0882963017910331
0.992518228535257	-0.0881539141059449
0.992541863007981	-0.0880122206462494
0.992565350610470	-0.0878712505830810
0.992588698232022	-0.0877309612256134
0.992612068576166	-0.0875902454391225
0.992635283469691	-0.0874502120849097
0.992658354419462	-0.0873108909333751
0.992681288776087	-0.0871722391559624
0.992704247439011	-0.0870331561545508
0.992727053745337	-0.0868947443122797
0.992749718998758	-0.0867570339919907
0.992772251066487	-0.0866199821496382
0.992794806634283	-0.0864825096267310
0.992817212989858	-0.0863456971415974
0.992839481203007	-0.0862095755920272
0.992861619606243	-0.0860741016992309
0.992883781178110	-0.0859382146811078
0.992905796536063	-0.0858029766882816
0.992927676469980	-0.0856684191777457
0.992949429768615	-0.0855344986939197
0.992971207778997	-0.0854001604660084
0.992992842366179	-0.0852664606497065
0.993014344067754	-0.0851334313090598
0.993035722197635	-0.0850010288023088
0.993057125846043	-0.0848682087244053
0.993078388832289	-0.0847360167907274
0.993099521462210	-0.0846044856495068
0.993120533589085	-0.0844735714180399
0.993141570758982	-0.0843422482089685
0.993162470003651	-0.0842115429882171
0.993183241360019	-0.0840814889659294
0.993203895187191	-0.0839520420330663
0.993224574562353	-0.0838221882515191
0.993245118588149	-0.0836929425104282
0.993265537018285	-0.0835643386171296
0.993285840744849	-0.0834363322663747
0.993306171325699	-0.0833079159281755
0.993326369018336	-0.0831800980347036
0.993346443317235	-0.0830529130079927
0.993366405694294	-0.0829263163138860
0.993386395242476	-0.0827993131315836
0.993406254347311	-0.0826728990084619
0.993425992235459	-0.0825471089592159
0.993445620948983	-0.0824218981985729
0.993465276892209	-0.0822962861584499
0.993484804752052	-0.0821712539239557
0.993504213459692	-0.0820468371099983
0.993523515624151	-0.0819229907062921
0.993542811780595	-0.0817989623891596
0.993561982611991	-0.0816755027875352
0.993581036730821	-0.0815526477435758
0.993599987098423	-0.0814303524637883
0.993618924405853	-0.0813079274449795
0.993637739180448	-0.0811860599757218
0.993656439759077	-0.0810647860219008
0.993675039433645	-0.0809440610620527
0.993693627664149	-0.0808232031475517
0.993712096143677	-0.0807028919453264
0.993730452928872	-0.0805831635118499
0.993748711608166	-0.0804639735572174
0.993766960333817	-0.0803446480023919
0.993785091961768	-0.0802258585641334
0.993803114240457	-0.0801076414088667
0.993821041042532	-0.0799899525071904
0.993838959083768	-0.0798721266796201
0.993856762528947	-0.0797548267137970
0.993874458841432	-0.0796380889105110
0.993892062217803	-0.0795218694971857
0.993909656836451	-0.0794055198195527
0.993927139343495	-0.0792896860024649
0.993944516933503	-0.0791744044443153
0.993961804112725	-0.0790596316048965
0.993979083570201	-0.0789447284299230
0.993996253337812	-0.0788303313311363
0.994013320321822	-0.0787164767977969
0.994030299313020	-0.0786031215299994
0.994047271929989	-0.0784896333169830
0.994064137144852	-0.0783766416752055
0.994080901578808	-0.0782641832096264
0.994097580329073	-0.0781522148687658
0.994114253099846	-0.0780401172304671
0.994130820700225	-0.0779285069157884
0.994147289484999	-0.0778174206312667
0.994163674863215	-0.0777068155569818
0.994180054867701	-0.0775960835507157
0.994196331896770	-0.0774858298219365
0.994212512031735	-0.0773760911612844
0.994228610971309	-0.0772668249776904
0.994244705721688	-0.0771574300515842
0.994260699591297	-0.0770485045884528
0.994276598383062	-0.0769400854776988
0.994292418091712	-0.0768321303658263
0.994308234291923	-0.0767240479078384
0.994323951633209	-0.0766164263387821
0.994339575653387	-0.0765093026460669
0.994355122654333	-0.0764026347050322
0.994370666641457	-0.0762958421553049
0.994386113756841	-0.0761895021153252
0.994401469274067	-0.0760836516542486
0.994416749788183	-0.0759782488696026
0.994432028242118	-0.0758727209277667
0.994447211738573	-0.0757676373156832
0.994462305281183	-0.0756630351894380
0.994477325756063	-0.0755588728745588
0.994492344964460	-0.0754545857410100
0.994507271056894	-0.0753507349733305
0.994522108774677	-0.0752473578185988
0.994536875304890	-0.0751444128267287
0.994551641085331	-0.0750413452765388
0.994566315552857	-0.0749387063148349
0.994580903190483	-0.0748365332681513
0.994595421479045	-0.0747347849040047
0.994609939802905	-0.0746329142968006
0.994624368560927	-0.0745314646785717
0.994638711973879	-0.0744304734550529
0.994652987811303	-0.0743298996142819
0.994667264479414	-0.0742292035906095
0.994681453263367	-0.0741289211486630
0.994695558125665	-0.0740290897777669
0.994709597131384	-0.0739296686853016
0.994723637527804	-0.0738301270854157
0.994737591680939	-0.0737309918349604
0.994751463299486	-0.0736323004995276
0.994765270740807	-0.0735340125002642
0.994779080260771	-0.0734356047103010
0.994792805131867	-0.0733375961998879
0.994806448806931	-0.0732400246084428
0.994820029930399	-0.0731428495719228
0.994833613885602	-0.0730455548509789
0.994847114729654	-0.0729486525114930
0.994860535661667	-0.0728521802699556
0.994873895617299	-0.0727560979768290
0.994887258990696	-0.0726598972383787
0.994900540750160	-0.0725640821450164
0.994913743844951	-0.0724686904857328
0.994926887500542	-0.0723736823212506
0.994940035210430	-0.0722785565385436
0.994953102762733	-0.0721838098141794
0.994966092856092	-0.0720894800067871
0.994979025001391	-0.0719955273874422
0.994991961904507	-0.0719014573741395
0.995004820057394	-0.0718077599872459
0.995017601909437	-0.0717144731570547
0.995030327259306	-0.0716215573648590
0.995043057958977	-0.0715285251458378
0.995055711277393	-0.0714358592696351
0.995068289417793	-0.0713435977351806
0.995080812465860	-0.0712517012308075
0.995093341471559	-0.0711596891011501
0.995105794427917	-0.0710680371688547
0.995118173291975	-0.0709767834989289
0.995130498432960	-0.0708858889864676
0.995142830191404	-0.0707948791698068
0.995155087189714	-0.0707042235456505
0.995167271139833	-0.0706139602462146
0.995179402695867	-0.0705240503731450
0.995191541454339	-0.0704340260037168
0.995203606706455	-0.0703443499576247
0.995215599921501	-0.0702550604320723
0.995227542037786	-0.0701661187328541
0.995239491945267	-0.0700770632656705
0.995251369566156	-0.0699883503801731
0.995263176127371	-0.0699000183365020
0.995274932848756	-0.0698120286442513
0.995286697985410	-0.0697239255643700
0.995298392017612	-0.0696361594529398
0.995310015930954	-0.0695487686335931
0.995321591227566	-0.0694617148193839
0.995333175511177	-0.0693745483293818
0.995344689840188	-0.0692877133186874
0.995356134960792	-0.0692012481726296
0.995367532656619	-0.0691151148058817
0.995378939912874	-0.0690288694101460
0.995390278333046	-0.0689429501222775
0.995401548424357	-0.0688573953877560
0.995412772249898	-0.0687721673225824
0.995424006230690	-0.0686868276388718
0.995435172460496	-0.0686018088093144
0.995446271208612	-0.0685171493397392
0.995457324818015	-0.0684328115470167
0.995468389139101	-0.0683483627829681
0.995479386765022	-0.0682642297329568
0.995490317728669	-0.0681804509616169
0.995501204651958	-0.0680969889852781
0.995512102846561	-0.0680134166081927
0.995522935372916	-0.0679301549137193
0.995533702027996	-0.0678472425241955
0.995544425711126	-0.0677646421552088
0.995555161235767	-0.0676819318087795
0.995565832089250	-0.0675995272217178
0.995576437833676	-0.0675174670740259
0.995587001645979	-0.0674357142800007
0.995597577841137	-0.0673538521043923
0.995608090335671	-0.0672722908690555
0.995618538458017	-0.0671910693103068
0.995628945661636	-0.0671101505400973
0.995639365794683	-0.0670291228920936
0.995649723170983	-0.0669483914657346
0.995660016885819	-0.0668679950529179
0.995670270668074	-0.0667878969631217
0.995680537928578	-0.0667076904229447
0.995690743349533	-0.0666277754853298
0.995700885794091	-0.0665481909975393
0.995710989266558	-0.0664689004659728
0.995721106744799	-0.0663895020322894
0.995731163276515	-0.0663103906777464
0.995741157493675	-0.0662316053038143
0.995751113674863	-0.0661531096130733
0.995761084395759	-0.0660745064677099
0.995770995038595	-0.0659961859710578
0.995780844004700	-0.0659181870783522
0.995790655846184	-0.0658404736882558
0.995800482757269	-0.0657626532708116
0.995810250434867	-0.0656851111633044
0.995819957050639	-0.0656078863743729
0.995829627430008	-0.0655309429981445
0.995839313394379	-0.0654538930941472
0.995848940947704	-0.0653771172493783
0.995858508032714	-0.0653006545249478
0.995868039747024	-0.0652244692099848
0.995877587567767	-0.0651481777702104
0.995887077777343	-0.0650721562251326
0.995896508090136	-0.0649964436880895
0.995905903875477	-0.0649210046430916
0.995915316280403	-0.0648454598965734
0.995924671852616	-0.0647701809646333
0.995933968079023	-0.0646952070123662
0.995943230600244	-0.0646205027180917
0.995952510245999	-0.0645456931708526
0.995961733817089	-0.0644711454393737
0.995970898573542	-0.0643968987398327
0.995980030426265	-0.0643229179446247
0.995989179912364	-0.0642488322676774
0.995998274061230	-0.0641750044875846
0.996007309906624	-0.0641014738714667
0.996016313629441	-0.0640282054856101
0.996025335484295	-0.0639548326312699
0.996034302720043	-0.0638817138326503
0.996043212144934	-0.0638088884072910
0.996052090209208	-0.0637363216149096
0.996060986901321	-0.0636636507510512
0.996069829673550	-0.0635912301770758
0.996078615109127	-0.0635190992605397
0.996087369926873	-0.0634472234545123
0.996096143868579	-0.0633752439291607
0.996104864570903	-0.0633035110019357
0.996113528392702	-0.0632320640902783
0.996122162321101	-0.0631608688403525
0.996130815860104	-0.0630895702646704
0.996139416822685	-0.0630185146670947
0.996147961343934	-0.0629477415144647
0.996156476678521	-0.0628772166457485
0.996165012110954	-0.0628065888012570
0.996173495612397	-0.0627362003847978
0.996181923094638	-0.0626660909124439
0.996190322079379	-0.0625962264159435
0.996198741645576	-0.0625262592859796
0.996207109909311	-0.0624565281025678
0.996215422559684	-0.0623870724308295
0.996223707385070	-0.0623178584950033
0.996232013269045	-0.0622485422878560
0.996240268462949	-0.0621794586121234
0.996248468433680	-0.0621106470816286
0.996256641235534	-0.0620420741129947
0.996264835574439	-0.0619733991870485
0.996272979819505	-0.0619049534424712
0.996281069215902	-0.0618367765417724
0.996289132083544	-0.0617688350938979
0.996297216960320	-0.0617007920228658
0.996305252324215	-0.0616329748465920
0.996313233199216	-0.0615654232760380
0.996321188170325	-0.0614981041122366
0.996329165620224	-0.0614306836468556
0.996337094123200	-0.0613634858512248
0.996344968482457	-0.0612965504846253
0.996352817547515	-0.0612298445402003
0.996360689560306	-0.0611630375876533
0.996368513177397	-0.0610964501403938
0.996376282981697	-0.0610301220060388
0.996384028086988	-0.0609640203697029
0.996391796602567	-0.0608978180428514
0.996399517259719	-0.0608318321155151
0.996407184421503	-0.0607661024434488
0.996414827465333	-0.0607005964036422
0.996422494382469	-0.0606349899545938
0.996430113964493	-0.0605695968567148
0.996437680354985	-0.0605044570139689
0.996445223194670	-0.0604395379952603
0.996452790366716	-0.0603745188523361
0.996460310713634	-0.0603097100684170
0.996467778159998	-0.0602451515956440
0.996475222609465	-0.0601808111946731
0.996482691846824	-0.0601163709560317
0.996490114756086	-0.0600521381387230
0.996497485043161	-0.0599881527430284
0.996504832874103	-0.0599243827214098
0.996512205948728	-0.0598605131158825
0.996519533179440	-0.0597968480476119
0.996526808053887	-0.0597334275651848
0.996534061000329	-0.0596702198128227
0.996541339640644	-0.0596069127521737
0.996548572909108	-0.0595438073967487
0.996555754075493	-0.0594809438433951
0.996562913829744	-0.0594182904280269
0.996570099728088	-0.0593555379511155
0.996577240714503	-0.0592929843982672
0.996584329841191	-0.0592306699147738
0.996591398059500	-0.0591685630283404
0.996598492869347	-0.0591063573243609
0.996605543215551	-0.0590443478131575
0.996612541933150	-0.0589825746885937
0.996619520234616	-0.0589210066700493
0.996626525571462	-0.0588593400842502
0.996633486881680	-0.0587978670082841
0.996640396783434	-0.0587366276846754
0.996647286749843	-0.0586755910245701
0.996654204196231	-0.0586144560134436
0.996661078041764	-0.0585535118768296
0.996667900688071	-0.0584927989062220
0.996674703868820	-0.0584322862045285
0.996681534968945	-0.0583716753906412
0.996688322883434	-0.0583112528621808
0.996695059797712	-0.0582510589596998
0.996701777705536	-0.0581910629778297
0.996708523972517	-0.0581309690934961
0.996715227458423	-0.0580710609507418
0.996721880132735	-0.0580113789395099
0.996728514249113	-0.0579518925462943
0.996735177161913	-0.0578923084589514
0.996741797688050	-0.0578329076137315
0.996748367581414	-0.0577737304502254
0.996754919355359	-0.0577147466466786
0.996761500359802	-0.0576556653634453
0.996768039362108	-0.0575967648658672
0.996774527900815	-0.0575380856434178
0.996780998748565	-0.0574795975662394
0.996787499262125	-0.0574210121879903
0.996793958148188	-0.0573626051814204
0.996800366730246	-0.0573044170863482
0.996806758040256	-0.0572464179647935
0.996813179445966	-0.0571883217495779
0.996819559589627	-0.0571304015331861
0.996825889579963	-0.0570726979059808
0.996832202707792	-0.0570151811218574
0.996838546362862	-0.0569575674127607
0.996844849111863	-0.0569001273700394
0.996851101848972	-0.0568429016351296
0.996857338123861	-0.0567858606539581
0.996863605354203	-0.0567287229265032
0.996869832025641	-0.0566717565725613
0.996876008818135	-0.0566150022849885
0.996882169540003	-0.0565584307015962
0.996888361643528	-0.0565017625484569
0.996894513526525	-0.0564452635142907
0.996900615654917	-0.0563889743437985
0.996906702095383	-0.0563328658669028
0.996912820345108	-0.0562766609618410
0.996918898703989	-0.0562206229592992
0.996924927424213	-0.0561647926564331
0.996930940830988	-0.0561091410751586
0.996936986468529	-0.0560533932464934
0.996942992536877	-0.0559978101404477
0.996948949074705	-0.0559424326069311
0.996954890665230	-0.0558872318599360
0.996960864912106	-0.0558319349857332
0.996966799902893	-0.0557768006905938
0.996972685462964	-0.0557218698779748
0.996978556433869	-0.0556671139540467
0.996984460480693	-0.0556122620631270
0.996990325577004	-0.0555575706429620
0.996996141335180	-0.0555030806509104
0.997001942854714	-0.0554487636851308
0.997007777871067	-0.0553943508797482
0.997013574234414	-0.0553400964711696
0.997019321344262	-0.0552860414713923
0.997025054558092	-0.0552321576708994
0.997030821689175	-0.0551781781443005
0.997036550457286	-0.0551243549747830
0.997042230049408	-0.0550707292296494
0.997047896081170	-0.0550172728913525
0.997053596444960	-0.0549637209785796
0.997059258728599	-0.0549103234156078
0.997064871906667	-0.0548571213255178
0.997070471852411	-0.0548040868830624
0.997076106551890	-0.0547509569299984
0.997081703446306	-0.0546979793525278
0.997087251298116	-0.0546451953306013
0.997092786238982	-0.0545925772310798
0.997098356343984	-0.0545398637819817
0.997103888912721	-0.0544873007653070
0.997109372495769	-0.0544349294181211
0.997114843482287	-0.0543827222993444
0.997120350052867	-0.0543304198773280
0.997125819348131	-0.0542782659759514
0.997131239706887	-0.0542263018907159
0.997136647776744	-0.0541745003729058
0.997142091841509	-0.0541226036754759
0.997147498886070	-0.0540708536172942
0.997152857037887	-0.0540192915526769
0.997158203202463	-0.0539678904246158
0.997163585774976	-0.0539163942001193
0.997168931575118	-0.0538650427625995
0.997174228518956	-0.0538138775262583
0.997179513770076	-0.0537628716266284
0.997184835845738	-0.0537117706629529
0.997190121390564	-0.0536608126642734
0.997195358109738	-0.0536100391057349
0.997200583425710	-0.0535594233143570
0.997205845968695	-0.0535087126202776
0.997211072216600	-0.0534581430959706
0.997216249663710	-0.0534077562778417
0.997221415989920	-0.0533575256852592
0.997226619967213	-0.0533072001126773
0.997231787877552	-0.0532570139446246
0.997236907004666	-0.0532070087808699
0.997242015288519	-0.0531571583324468
0.997247161617383	-0.0531072131271018
0.997252272103686	-0.0530574055862957
0.997257333820912	-0.0530077773726275
0.997262384966121	-0.0529583023886915
0.997267474582186	-0.0529087325191143
0.997272528571030	-0.0528592986024660
0.997277533795781	-0.0528100423670567
0.997282528714262	-0.0527609379078228
0.997287562499441	-0.0527117387417760
0.997292560870403	-0.0526626738427169
0.997297510480790	-0.0526137850040195
0.997302450046378	-0.0525650465108502
0.997307428892091	-0.0525162132811382
0.997312372527590	-0.0524675126570765
0.997317267396378	-0.0524189864995282
0.997322152474193	-0.0523706092868820
0.997327077247611	-0.0523221372847048
0.997331967011409	-0.0522737962553449
0.997336808000263	-0.0522256281281263
0.997341639450848	-0.0521776075703417
0.997346510979400	-0.0521294924966078
0.997351347693362	-0.0520815067816086
0.997356135617775	-0.0520336924229893
0.997360914246328	-0.0519860242814859
0.997365733405517	-0.0519382611448780
0.997370517936457	-0.0518906257857298
0.997375253655610	-0.0518431602748949
0.997379980322925	-0.0517958396618345
0.997384747860264	-0.0517484247721880
0.997389480958162	-0.0517011360915783
0.997394165224577	-0.0516540157592404
0.997398840671901	-0.0516070390162237
0.997403557481380	-0.0515599670519614
0.997408240021828	-0.0515130197635565
0.997412873692171	-0.0514662393689125
0.997417498777155	-0.0514196013003254
0.997422165534520	-0.0513728690452429
0.997426798207014	-0.0513262599445292
0.997431381987027	-0.0512798162850640
0.997435957408531	-0.0512335136852487
0.997440574998668	-0.0511871158537382
0.997445158659144	-0.0511408396846356
0.997449693372158	-0.0510947275475823
0.997454219946220	-0.0510487552586751
0.997458789033911	-0.0510026884105963
0.997463324368878	-0.0509567417558701
0.997467810729265	-0.0509109577372774
0.997472289177676	-0.0508653123473796
0.997476810542876	-0.0508195723092556
0.997481298302248	-0.0507739510025035
0.997485737022695	-0.0507284909513911
0.997490168030704	-0.0506831683557667
0.997494642469907	-0.0506377499362886
0.997499083461803	-0.0505924488413879
0.997503475370800	-0.0505473076811782
0.997507859801505	-0.0505023028209930
0.997512287803077	-0.0504572049196311
0.997516682513899	-0.0504122228965729
0.997521028088462	-0.0503673994311428
0.997525366359113	-0.0503227111028191
0.997529749083555	-0.0502779244314725
0.997534098632660	-0.0502332523044302
0.997538398955849	-0.0501887375138972
0.997542692219784	-0.0501443568025865
0.997547029605889	-0.0500998858434663
0.997551334015816	-0.0500555279878373
0.997555589197027	-0.0500113260690330
0.997559837471395	-0.0499672570324025
0.997564131300771	-0.0499230860965228
0.997568392186860	-0.0498790270021016
0.997572603660130	-0.0498351227388190
0.997576808469823	-0.0497913504442488
0.997581057938018	-0.0497474909936892
0.997585274748550	-0.0497037419620648
0.997589442250306	-0.0496601463398006
0.997593603247123	-0.0496166814067082
0.997597810797123	-0.0495731119286996
0.997601985599085	-0.0495296516388604
0.997606110758257	-0.0494863437305227
0.997610229604041	-0.0494431657747544
0.997614393953151	-0.0493999004878499
0.997618525952238	-0.0493567430616054
0.997622608561024	-0.0493137366668662
0.997626685105410	-0.0492708588618582
0.997630808573839	-0.0492278806817158
0.997634899489862	-0.0491850090260547
0.997638940530256	-0.0491422872640634
0.997642975518035	-0.0490996934623171
0.997647057963646	-0.0490569997097562
0.997651108284714	-0.0490144114637988
0.997655109051803	-0.0489719721560115
0.997659104292894	-0.0489296595499904
0.997663145040243	-0.0488872710758141
0.997667153556741	-0.0488449863416572
0.997671112108704	-0.0488028487795377
0.997675064709705	-0.0487608370090366
0.997679069452666	-0.0487186810821887
0.997683042008354	-0.0486766286474007
0.997686964517327	-0.0486347236050854
0.997690882217229	-0.0485929438966885
0.997694840104798	-0.0485511586556824
0.997698766526321	-0.0485094740862989
0.997702643422279	-0.0484679333982517
0.997706514239115	-0.0484265156965618
0.997710447301702	-0.0483848451508454
0.997714347342854	-0.0483432765899827
0.997718195911866	-0.0483018548291854
0.997722040610979	-0.0482605582283032
0.997725913376078	-0.0482194095614327
0.997729756549712	-0.0481783580805050
0.997733551986574	-0.0481374462139961
0.997737341041368	-0.0480966530082627
0.997741210931265	-0.0480553937615894
0.997745045239598	-0.0480142355045357
0.997748824470203	-0.0479732247399996
0.997752600754700	-0.0479323413876149
0.997756384803041	-0.0478918679680688
0.997760143390438	-0.0478514881019461
0.997763858816711	-0.0478112426222168
0.997767567984585	-0.0477711086444884
0.997771383767656	-0.0477301969169973
0.997775158249272	-0.0476893847817928
0.997778869879813	-0.0476487212603415
0.997782578147040	-0.0476081914064232
0.997786274978339	-0.0475683511676749
0.997789954084069	-0.0475286026384979
0.997793599209443	-0.0474889846310774
0.997797240993179	-0.0474494672155768
0.997800997656261	-0.0474090308131967
0.997804703587589	-0.0473686881027476
0.997808333824736	-0.0473284897226910
0.997811954303091	-0.0472884345076666
0.997815594700654	-0.0472487973217284
0.997819227897386	-0.0472092595502179
0.997822840717508	-0.0471698614185793
0.997826463891861	-0.0471305527308163
0.997830088291402	-0.0470915397908002
0.997833655006032	-0.0470525979463822
0.997837136279535	-0.0470137722720118
0.997840584062508	-0.0469750883682480
0.997844345839551	-0.0469335065840735
0.997848092844858	-0.0468920722474665
0.997851810062275	-0.0468508593060717
0.997855596855507	-0.0468097573248204
0.997858908138231	-0.0467746496142170
0.997862177532294	-0.0467395437409284
0.997865368998703	-0.0467044656581476
0.997868468010177	-0.0466694759262471
0.997871119055076	-0.0466390660865975
0.997873750255544	-0.0466087815738075
0.997876386393502	-0.0465786389029207
0.997879077646241	-0.0465485936874637
0.997881838945092	-0.0465185778804396
0.997884639425119	-0.0464885763411950
0.997887459734726	-0.0464585789839819
0.997890254014287	-0.0464285765461828
0.997893535239149	-0.0463927380004648
0.997896698538206	-0.0463569816475557
0.997899720275835	-0.0463213665540379
0.997902715909052	-0.0462859543993086
0.997905800669076	-0.0462506831604918
0.997908975988195	-0.0462155256331642
0.997912255231446	-0.0461804842783644
0.997915603624979	-0.0461454163716321
0.997918562570202	-0.0461141769192303
0.997921413413653	-0.0460829245760396
0.997924118547269	-0.0460517080992645
0.997926708728616	-0.0460206269044285
0.997929420961376	-0.0459879699626323
0.997932158368219	-0.0459555174550737
0.997934965485228	-0.0459232861329732
0.997937927466426	-0.0458911309689571
0.997940673508189	-0.0458625807425871
0.997943432554135	-0.0458339547672264
0.997946149653875	-0.0458052515414613
0.997948749093910	-0.0457765284674130
0.997951451491283	-0.0457451971715196
0.997954016230385	-0.0457140252868687
0.997956467612287	-0.0456830816087649
0.997958971652750	-0.0456523676213880
0.997961431937254	-0.0456242314696905
0.997964027365817	-0.0455961287770889
0.997966750798618	-0.0455680098402673
0.997969511712241	-0.0455397996050626
0.997972166958387	-0.0455118990169007
0.997974694346442	-0.0454839685314575
0.997977057034283	-0.0454560655880739
0.997979289165989	-0.0454282932493509
0.997981598284909	-0.0453992304466549
0.997983930047043	-0.0453703777416883
0.997986344299055	-0.0453417395001171
0.997988920595095	-0.0453131865099294
0.997991456445923	-0.0452865736196571
0.997994044643377	-0.0452598776129962
0.997996629623144	-0.0452330801591496
0.997999116192911	-0.0452062180024862
0.998001649914736	-0.0451772107589587
0.998004017082360	-0.0451483135889300
0.998006230999004	-0.0451196026474013
0.998008436967151	-0.0450911254204322
0.998010756074155	-0.0450629561514845
0.998013227828649	-0.0450348885874080
0.998015874237163	-0.0450068714289850
0.998018627799594	-0.0449787683637683
0.998021157359617	-0.0449526997332558
0.998023589922326	-0.0449265525658282
0.998025871939180	-0.0449003711726114
0.998027996283415	-0.0448742634069164
0.998030229367973	-0.0448457374816575
0.998032417134621	-0.0448174422027171
0.998034624394104	-0.0447894109259285
0.998036992614521	-0.0447615378323518
0.998039277824536	-0.0447367879664083
0.998041666971737	-0.0447119753855820
0.998044114812446	-0.0446870596415055
0.998046516066919	-0.0446620379737293
0.998047069683689	-0.0446560347273096
0.998047615361599	-0.0446500296186588
0.998048152647502	-0.0446440237265124
0.998048681250173	-0.0446380181619269

==> matlab/fig2a3.tex <==
0	0
1.42172830446005e-06	-0.00167404631372067
5.53234083966090e-06	-0.00327706669288221
1.21363636220212e-05	-0.00482489935074513
2.10868354462101e-05	-0.00632851834729682
3.22754906489584e-05	-0.00779514989077415
4.56122345575181e-05	-0.00923056297725695
6.10225023515531e-05	-0.0106391904995966
7.84434029647620e-05	-0.0120245223720506
0.000119319872689130	-0.0147484165454920
0.000167756771795057	-0.0174053302514175
0.000223473126395607	-0.0200072501805284
0.000286238609368686	-0.0225629388668987
0.000393638851857574	-0.0263374481900342
0.000516071506196174	-0.0300370787119667
0.000653095958104766	-0.0336736747850717
0.000804337165598524	-0.0372560787773600
0.00107816824993246	-0.0429501438274255
0.00138722165718729	-0.0485397095163076
0.00173054014506976	-0.0540400439952915
0.00210728853841057	-0.0594625679765890
0.00266832664592210	-0.0666822938876892
0.00328757741971491	-0.0737911416314600
0.00396367880230257	-0.0808015621630619
0.00469539973358753	-0.0877232611432091
0.00574911681425167	-0.0967736271622129
0.00689633799890073	-0.105695017444368
0.00813498985366746	-0.114498471345482
0.00946315269488977	-0.123192798635962
0.0112791375925875	-0.134105089337944
0.0132338013402324	-0.144863616132059
0.0153240732329870	-0.155477771995721
0.0175470537227754	-0.165955140337372
0.0202323640501528	-0.177709411430730
0.0230819932408337	-0.189301992844953
0.0260923867324757	-0.200738913226990
0.0292601264603394	-0.212025092375776
0.0329175784420498	-0.224254661466058
0.0367568306695430	-0.236311452493108
0.0407738695113247	-0.248199044082884
0.0449647843045321	-0.259920328135904
0.0496958330076994	-0.272431020838870
0.0546217197080050	-0.284751692199209
0.0597378522820875	-0.296884244547790
0.0650397157452530	-0.308830140681587
0.0709170344515675	-0.321414407819352
0.0769968352079042	-0.333786984928490
0.0832738484112976	-0.345948601065594
0.0897428619084648	-0.357899708410921
0.0968079745434831	-0.370345295987953
0.104077192666452	-0.382554452339730
0.111544492351568	-0.394527122837548
0.119203893530522	-0.406263092734074
0.127463555229083	-0.418355116864686
0.135922441789140	-0.430184308124371
0.144573731295565	-0.441750164341979
0.153410638550966	-0.453052112763783
0.162835263470453	-0.464578851898971
0.172447518567288	-0.475816138891109
0.182239780793817	-0.486763330604767
0.192204463514691	-0.497419784935712
0.202728585227716	-0.508179501746136
0.213422138043277	-0.518624350798251
0.224276738895163	-0.528753830777743
0.235284047809494	-0.538567499705749
0.246808854503609	-0.548375283235312
0.258478720739330	-0.557845307419698
0.270284588247213	-0.566977468975246
0.282217455303448	-0.575771771139477
0.294615122300600	-0.584465543454569
0.307128019940830	-0.592802330532719
0.319746538657299	-0.600782650922584
0.332461145053967	-0.608407166737607
0.345580442300474	-0.615852251334893
0.358780612472349	-0.622925696683404
0.372051650057723	-0.629628829019652
0.385383650580044	-0.635963145487404
0.399056185406762	-0.642055106493252
0.412771763732936	-0.647765990722934
0.426520161690261	-0.653098076568634
0.440291285395246	-0.658053831252608
0.454337768336360	-0.662719596994581
0.468387096073912	-0.667000452392746
0.482429016907855	-0.670899730335353
0.496453440905440	-0.674420961350706
0.510689497929541	-0.677618473613037
0.524886910040435	-0.680433004178457
0.539035592924446	-0.682869002376092
0.553125657411070	-0.684931115268846
0.567366893792616	-0.686647864541614
0.581527709063688	-0.687989293431287
0.595598379693731	-0.688960992782267
0.609569411116751	-0.689568743030987
0.623635604290917	-0.689819569208160
0.637580215174380	-0.689708297304834
0.651394068032464	-0.689241652406344
0.665068249349970	-0.688426533338426
0.678786677575856	-0.687251023319194
0.692343763676205	-0.685731928031647
0.705731057640642	-0.683877071994762
0.718940403504025	-0.681694430426523
0.732148395406758	-0.679154165316249
0.745157358064087	-0.676293786444789
0.757959734947028	-0.673122160019764
0.770548293245418	-0.669648273181977
0.783095117509437	-0.665824095738639
0.795407862491101	-0.661707872216605
0.807480022976347	-0.657309433883597
0.819305444383263	-0.652638696816218
0.831053662209424	-0.647628099519108
0.842535857107518	-0.642357751341122
0.853746724453404	-0.636838356445509
0.864681333880751	-0.631080661546228
0.875507721697408	-0.624995342022646
0.886039636837073	-0.618686439875956
0.896273118370104	-0.612165427040421
0.906204599474768	-0.605443769646918
0.916000724284885	-0.598407361579245
0.925477739103969	-0.591187090698079
0.934633167128244	-0.583795080412671
0.943464941239201	-0.576243393671296
0.952137439486576	-0.568389352575852
0.960470263729983	-0.560394452163889
0.968462564008530	-0.552271340838653
0.976113910782961	-0.544032545039282
0.983584481813859	-0.535502141668739
0.990699100164872	-0.526876979960738
0.997458694934292	-0.518170096772902
1.00386462081110	-0.509394337625128
1.01006968797437	-0.500334674571990
1.01590697738748	-0.491229391836450
1.02137937001245	-0.482091767235904
1.02649017098122	-0.472934808232209
1.03138006055735	-0.463496701495977
1.03589492372300	-0.454065298450759
1.04003980502924	-0.444653957130034
1.04382016362056	-0.435275673517824
1.04727561621215	-0.425846284251142
1.05037147175070	-0.416476283797318
1.05311467117170	-0.407177998453085
1.05551251421507	-0.397963328709247
1.05756674862339	-0.388872095598263
1.05929339969078	-0.379886381550618
1.06070078099691	-0.371016756905154
1.06179748334316	-0.362273336756895
1.06259201267512	-0.353670676822634
1.06309427170860	-0.345212978770006
1.06331368160947	-0.336909019393730
1.06325986066652	-0.328767099627823
1.06294168540602	-0.320778307452557
1.06236911731581	-0.312967552059233
1.06155244569948	-0.305341790309520
1.06050207795464	-0.297907490376572
1.05922119014596	-0.290632654382671
1.05772563082158	-0.283562990568721
1.05602634895770	-0.276703618966743
1.05413433305697	-0.270059164544061
1.05204269212272	-0.263581401571437
1.04977773175364	-0.257330096119426
1.04735085261613	-0.251308503547253
1.04477341572132	-0.245519384800131
1.04202539014412	-0.239903772770365
1.03914670901225	-0.234530081943323
1.03614901455479	-0.229399670636618
1.03304382875267	-0.224513411047027
1.02979486354766	-0.219805313998396
1.02645882054014	-0.215348910439552
1.02304737764413	-0.211143625631501
1.01957200950301	-0.207188414955803
1.01597725908333	-0.203414474856750
1.01233963307212	-0.199896440293668
1.00867064007614	-0.196631754957907
1.00498149834158	-0.193617417569498
1.00119471869437	-0.190786827010986
0.997409765352163	-0.188210911663809
0.993637767895554	-0.185885057797558
0.989889471660512	-0.183804241729294
0.986062325537775	-0.181910451687967
0.982282354736325	-0.180264743404170
0.978560085224744	-0.178860315788249
0.974905553276586	-0.177690005753070
0.971193356200057	-0.176714639476045
0.967574676594393	-0.175974665493727
0.964059133055007	-0.175460901951433
0.960655732391582	-0.175163873355797
0.957415312933156	-0.175073697135227
0.954299856411998	-0.175175387575035
0.951316339597779	-0.175459059397420
0.948471144346174	-0.175914670455217
0.945784461579119	-0.176528220094220
0.943245503063520	-0.177291533775264
0.940858870687100	-0.178194321396453
0.938628592090809	-0.179226253796165
0.936553294910319	-0.180379897928541
0.934641552433951	-0.181642382930162
0.932895763182258	-0.183003225159844
0.931317774132567	-0.184452009529811
0.929896199024147	-0.185993374195137
0.928647803377299	-0.187603216546868
0.927572861636698	-0.189271060595152
0.926671123963886	-0.190986603104145
0.925931025390749	-0.192769476018054
0.925367893043934	-0.194580679801455
0.924979889279619	-0.196409949591339
0.924764686440381	-0.198247299437604
0.924720497973436	-0.200128682243160
0.924851353987673	-0.201998155749263
0.925153248775345	-0.203845884638708
0.925621731153127	-0.205662426537205
0.926276834866964	-0.207500045679782
0.927099253455284	-0.209284910097543
0.928082661236621	-0.211007866674614
0.929220347325330	-0.212660285951805
0.930571881813529	-0.214309050950125
0.932076771590633	-0.215862456213765
0.933726039908411	-0.217312355838072
0.935510411870174	-0.218651291917586
0.937384917200848	-0.219851584906428
0.939371151494954	-0.220932486438982
0.941459608959905	-0.221888804235599
0.943640664134639	-0.222715997084018
0.945879775102337	-0.223403398407372
0.948190414230692	-0.223957421211627
0.950563009056319	-0.224375473780647
0.952988013852167	-0.224655566549010
0.955460443762892	-0.224796424933124
0.957966363413454	-0.224796574471487
0.960496325928984	-0.224655746804245
0.963041039704142	-0.224374230440531
0.965624185401298	-0.223946526844782
0.968203734984589	-0.223376762660713
0.970770572567373	-0.222666887262144
0.973315861976618	-0.221819357930876
0.975891706287710	-0.220811612849270
0.978427037089297	-0.219666245505172
0.980913303171759	-0.218387441984773
0.983342364289191	-0.216979837200433
0.985795547783524	-0.215387524377745
0.988170499552576	-0.213668006289544
0.990459521751918	-0.211827874737298
0.992655480025514	-0.209874092027266
0.994772187702307	-0.207792908127982
0.996781007483503	-0.205611182223867
0.998676311405738	-0.203337106199005
1.00045310437796	-0.200979087362403
1.00206990169970	-0.198603225607445
1.00356593268093	-0.196163736894647
1.00493823872099	-0.193668946384945
1.00618443928391	-0.191127223824454
1.00729433742243	-0.188567616951573
1.00827709600240	-0.185978370457975
1.00913201032405	-0.183367708360933
1.00985890442846	-0.180743762832215
1.01046095003910	-0.178100660167154
1.01093481963142	-0.175460357066096
1.01128186975888	-0.172830778045821
1.01150393572303	-0.170219632617852
1.01160397809980	-0.167589639996987
1.01157993940238	-0.164994187973901
1.01143518315368	-0.162440675372866
1.01117349337586	-0.159936163532711
1.01078575699382	-0.157412746819615
1.01028326093887	-0.154955589658559
1.00967144110388	-0.152571291344715
1.00895607904252	-0.150265980027441
1.00811138604993	-0.147964745292659
1.00716912401087	-0.145760386893763
1.00613678935669	-0.143658159510118
1.00502210827760	-0.141662711079831
1.00386797700807	-0.139830401155457
1.00265113842593	-0.138105905703728
1.00137919352303	-0.136491899072786
1.00005979516160	-0.134990504853812
0.998718545535074	-0.133620617784364
0.997346042135271	-0.132363021254633
0.995949715449771	-0.131218252210175
0.994536910918951	-0.130186350832029
0.993112635464610	-0.129265509790232
0.991686347454026	-0.128456538724491
0.990265117237423	-0.127758066765543
0.988855810796771	-0.127168280169722
0.987443586464591	-0.126678228895681
0.986057332471727	-0.126295174855832
0.984703562884936	-0.126015918164145
0.983388470693071	-0.125836876286648
0.982081066861675	-0.125753072431803
0.980826995755198	-0.125766597183245
0.979631945994542	-0.125872389960946
0.978501160101424	-0.126065084887126
0.977390428210170	-0.126354078193134
0.976360595670585	-0.126725423646734
0.975416152830331	-0.127172013625704
0.974560993480937	-0.127686545351512
0.973812636010085	-0.128249594402133
0.973155867994267	-0.128863494975203
0.972592761609884	-0.129520947184922
0.972124833797751	-0.130214633380971
0.971757511741181	-0.130927151208741
0.971484188351306	-0.131660724752234
0.971304823844091	-0.132408371858213
0.971218889169415	-0.133163234280868
0.971225581146977	-0.133921403635679
0.971323926724000	-0.134673353679467
0.971512011303659	-0.135412586796754
0.971787494748275	-0.136132853508999
0.972155510945372	-0.136841484150958
0.972608188710437	-0.137518027733144
0.973141807192767	-0.138156690597102
0.973752293232627	-0.138752050858778
0.974462212283013	-0.139318569154478
0.975244828702020	-0.139827765761410
0.976094540773812	-0.140274853339174
0.977005490885799	-0.140655555111085
0.978001817899688	-0.140974413547421
0.979049756095699	-0.141215145526318
0.980142206314474	-0.141374722931798
0.981271970530972	-0.141450728489620
0.982398864166036	-0.141442774273819
0.983547345889172	-0.141352969831315
0.984710662178609	-0.141180668347911
0.985882134180110	-0.140925746605709
0.987047333397584	-0.140591109023846
0.988207659046186	-0.140176172785852
0.989356869391924	-0.139682247903585
0.990488933434734	-0.139111091733246
0.991612256225741	-0.138456016295182
0.992706157768153	-0.137726644562817
0.993765083309073	-0.136926084912955
0.994783816371880	-0.136057815125950
0.995788580486704	-0.135094065750784
0.996740228758850	-0.134066787427826
0.997634167267426	-0.132980905988296
0.998466278463500	-0.131841619755671
0.999257402164923	-0.130613870471884
0.999975043024491	-0.129341218252185
1.00061622511739	-0.128030155253800
1.00117856338897	-0.126687292779528
1.00164521817648	-0.125366155384768
1.00203543789867	-0.124027776030541
1.00234856637634	-0.122678309752833
1.00258444759242	-0.121323852269685
1.00274211182168	-0.119984874541064
1.00282524897172	-0.118652715190422
1.00283505749966	-0.117333023954676
1.00277315817151	-0.116031257180852
1.00263987073449	-0.114739682214480
1.00243795984146	-0.113477028563656
1.00217029552073	-0.112248273683342
1.00184009191239	-0.111058079545244
1.00143816219547	-0.109876606703998
1.00097782586252	-0.108745147565713
1.00046360943829	-0.107667741592316
0.999900287125203	-0.106647984106885
0.999269655942310	-0.105654830363795
0.998597458922433	-0.104730137036576
0.997889707601459	-0.103876442115475
0.997152513922354	-0.103095724384539
0.996418535162040	-0.102412457302981
0.995668561718865	-0.101799439387688
0.994908248501628	-0.101257052808522
0.994143179688503	-0.100785209899640
0.993386889249420	-0.100387242173314
0.992636625312585	-0.100056882376855
0.991897519224667	-0.0997927904035933
0.991174503217064	-0.0995932344244641
0.990464663432246	-0.0994549308754766
0.989780829440442	-0.0993778996457368
0.989127439450467	-0.0993592509937413
0.988508615641852	-0.0993957834306779
0.987910208869678	-0.0994876502846319
0.987356566439592	-0.0996304093391686
0.986851162408052	-0.0998196405359501
0.986397031634507	-0.100050712355008
0.985980656673160	-0.100331207139274
0.985625457898429	-0.100646289896336
0.985333411964587	-0.100990128636378
0.985105939615066	-0.101356832247681
0.984948263568871	-0.101727490068802
0.984852137780718	-0.102108548671084
0.984817466764695	-0.102494649394902
0.984843698417623	-0.102880542689910
0.984928944405447	-0.103258150151745
0.985071811233463	-0.103625568294291
0.985270547358311	-0.103978063590216
0.985523031740772	-0.104311139100650
0.985832181426489	-0.104625378374154
0.986191354185934	-0.104910898389557
0.986597290599863	-0.105163764409497
0.987046452714952	-0.105380398107724
0.987556184505159	-0.105564045166999
0.988104112576966	-0.105701591890127
0.988685443197548	-0.105790214550630
0.989295223551443	-0.105827579288465
0.989936031541979	-0.105811307438737
0.990595326605710	-0.105739165141975
0.991267643100728	-0.105610189863953
0.991947538145547	-0.105423939407221
0.992611595042994	-0.105187632359272
0.993272729523425	-0.104897557732050
0.993926091646844	-0.104554616466096
0.994567005744284	-0.104160124604836
0.995192134369423	-0.103714902916354
0.995795879360056	-0.103221747820217
0.996374127646925	-0.102683104746232
0.996923064230150	-0.102101739919072
0.997453448791507	-0.101462358316817
0.997945549720248	-0.100784676599695
0.998396217667492	-0.100072612411243
0.998802727574367	-0.0993302956076140
0.999177584020100	-0.0985275383273842
0.999499574012924	-0.0977016562686340
0.999767027367721	-0.0968579130991271
0.999978817906646	-0.0960016222896975
1.00012915055649	-0.0951730689365296
1.00022754115486	-0.0943426591053174
1.00027430706558	-0.0935150924376067
1.00027019437561	-0.0926949465142953
1.00021712597889	-0.0918945916212767
1.00011680085511	-0.0911100994413294
0.999971065891123	-0.0903454878749748
0.999782100507877	-0.0896045281807075
0.999547836265901	-0.0888779800356840
0.999274284910516	-0.0881831104982572
0.998964669864918	-0.0875230874687449
0.998622447003852	-0.0869007153949566
0.998232812566249	-0.0862915540827955
0.997815871596495	-0.0857288801060850
0.997376254223457	-0.0852146693559861
0.996918687096246	-0.0847504015000943
0.996458453681711	-0.0843456355612296
0.995990233298722	-0.0839901433251500
0.995518579682265	-0.0836840260221206
0.995047964245831	-0.0834269461663297
0.994591443735796	-0.0832216395868989
0.994144224231217	-0.0830617478817232
0.993710218394802	-0.0829458405726457
0.993293128085691	-0.0828721473862412
0.992892376142142	-0.0828384314971833
0.992515884869859	-0.0828432235198388
0.992166785646977	-0.0828837781504181
0.991847887054578	-0.0829571067033621
0.991551137381738	-0.0830645986276780
0.991292182306594	-0.0832001657683962
0.991073087883235	-0.0833597824041058
0.990895478213561	-0.0835393023253650
0.990758891253124	-0.0837374511689169
0.990667112601299	-0.0839471667159522
0.990620534511128	-0.0841638948307277
0.990619082536554	-0.0843831389495915
0.990660501039212	-0.0845946669971511
0.990743318355342	-0.0848003443829139
0.990866322352166	-0.0849962856319898
0.991027945668815	-0.0851788028450768
0.991227395994609	-0.0853452022865490
0.991461698352223	-0.0854911430297406
0.991728324026416	-0.0856135296988875
0.992024491572258	-0.0857095788861721
0.992359527147283	-0.0857787045600280
0.992719470648810	-0.0858144012542540
0.993100535699979	-0.0858146179816360
0.993498807778277	-0.0857777351873340
0.993920670038044	-0.0857001689944004
0.994351930749469	-0.0855814701583477
0.994788131058972	-0.0854212190848364
0.995224867548882	-0.0852194740092952
0.995644056936517	-0.0849851306298295
0.996055792881533	-0.0847132077765209
0.996456339091843	-0.0844049067272746
0.996842160171587	-0.0840617827077339
0.997211209880004	-0.0836843067032556
0.997558876041001	-0.0832758746831891
0.997882244454600	-0.0828389841479298
0.998178717263396	-0.0823763769269488
0.998455738230219	-0.0818718062494676
0.998699020643657	-0.0813462556640790
0.998906724040724	-0.0808034585540086
0.999077445895614	-0.0802472603596292
0.999210949441068	-0.0796778338247372
0.999305365348454	-0.0791029369133858
0.999360518075689	-0.0785266739176961
0.999376675564085	-0.0779530755492318
0.999355714756117	-0.0774027043430714
0.999299641206832	-0.0768621174160031
0.999209769349928	-0.0763347055080790
0.999087737341374	-0.0758236505993811
0.998934338330188	-0.0753286269497221
0.998752571438509	-0.0748560559655719
0.998544956167937	-0.0744085089706418
0.998314226762697	-0.0739882386313636
0.998052222009405	-0.0735812117441266
0.997771813115420	-0.0732078325617436
0.997476670717505	-0.0728695781998797
0.997170543205922	-0.0725674903974208
0.996859182756861	-0.0723037212480548
0.996544540731862	-0.0720765537868426
0.996230379100320	-0.0718858367085888
0.995920358727013	-0.0717310131064899
0.995625064630056	-0.0716135874214580
0.995340338838442	-0.0715283002089286
0.995069230695728	-0.0714736506606371
0.994814564812452	-0.0714478471808332
0.994576059985009	-0.0714490085379669
0.994359598452579	-0.0714752470410187
0.994167390104906	-0.0715239447493329
0.994001315170606	-0.0715923035687697
0.993856736806084	-0.0716820304850995
0.993744185510875	-0.0717865742342177
0.993664717459236	-0.0719022349098827
0.993618944579734	-0.0720252800745238
0.993606989800116	-0.0721499790555338
0.993627712975140	-0.0722746027489564
0.993680561488850	-0.0723956398553159
0.993764604143890	-0.0725097209993481
0.993876468689599	-0.0726120234670018
0.994015757869110	-0.0727015222797966
0.994180665570632	-0.0727754824606758
0.994369126475600	-0.0728314274603503
0.994583915990524	-0.0728677011327480
0.994818250479052	-0.0728806492609071
0.995069249268997	-0.0728684645991239
0.995333895097086	-0.0728297046083695
0.995626118151670	-0.0727583056403375
0.995926299965339	-0.0726548366704650
0.996230535627738	-0.0725188375901644
0.996534963503662	-0.0723503272778870
0.996821955475393	-0.0721597702900936
0.997102399901041	-0.0719408068904990
0.997373182126018	-0.0716945242478949
0.997631383639993	-0.0714223382231660
0.997873655642386	-0.0711267855516384
0.998098172400342	-0.0708091546559930
0.998302668285381	-0.0704716650789362
0.998485181768119	-0.0701167418205290
0.998650070984185	-0.0697314513128527
0.998787736844534	-0.0693332289316362
0.998896987432117	-0.0689253352570056
0.998977046735617	-0.0685110917167280
0.999027437138070	-0.0680949221929063
0.999048365893938	-0.0676791668911737
0.999040186721385	-0.0672671468516972
0.999003637481749	-0.0668620598745006
0.998941792673563	-0.0664770442981578
0.998855365517522	-0.0661042633160341
0.998745941357478	-0.0657462589540132
0.998615360784838	-0.0654053313752994
0.998462899261821	-0.0650780591951855
0.998293087310753	-0.0647725662574996
0.998108511950037	-0.0644904990643440
0.997911891260067	-0.0642331611349516
0.997693930980883	-0.0639889430054475
0.997469137109894	-0.0637742927494318
0.997241013709478	-0.0635895852978559
0.997013019973243	-0.0634347481886937
0.996799240322450	-0.0633146788452450
0.996591560595589	-0.0632205100166383
0.996392738421681	-0.0631511972803347
0.996205341635362	-0.0631053950660644
0.996032298209921	-0.0630815298367775
0.995875168942789	-0.0630775621071939
0.995735899239404	-0.0630914280000510
0.995616144951819	-0.0631208833249500
0.995513656974700	-0.0631655434038167
0.995435106141569	-0.0632216244312173
0.995381404371593	-0.0632861523265229
0.995353073868291	-0.0633561156344633
0.995350326546230	-0.0634288545837162
0.995373206953067	-0.0635009216105551
0.995421185154266	-0.0635692991459732
0.995493370550533	-0.0636311117389301
0.995586084585277	-0.0636825340645372
0.995699326839137	-0.0637226582590823
0.995831436459596	-0.0637492682274502
0.995980525347301	-0.0637604022820591
0.996148556570961	-0.0637539795701290
0.996329751005016	-0.0637279353938477
0.996521527258994	-0.0636809867595638
0.996721209989088	-0.0636122027515944
0.996936163145167	-0.0635159363146986
0.997153540333051	-0.0633946432964245
0.997370116830326	-0.0632483908678458
0.997582764250600	-0.0630776654890535
0.997779841085772	-0.0628921168480318
0.997967974744436	-0.0626859908690743
0.998144773516042	-0.0624606286171884
0.998308073041050	-0.0622176347680394
0.998457067132727	-0.0619566801833209
0.998588577092786	-0.0616817823848282
0.998701104440433	-0.0613952200396977
0.998793475217952	-0.0610994015413303
0.998868600646453	-0.0607776007964439
0.998919268687992	-0.0604513291653251
0.998945192265556	-0.0601237536233103
0.998946518298376	-0.0597979900893973
0.998925434287084	-0.0594925000373981
0.998883331903997	-0.0591939990704956
0.998821275550766	-0.0589049232395730
0.998740612036350	-0.0586275095520313
0.998643405612903	-0.0583649292891745
0.998531146750130	-0.0581177820562195
0.998405828606209	-0.0578876588448583
0.998269594623698	-0.0576758568284697
0.998117471409660	-0.0574745227426345
0.997958599686498	-0.0572953442555568
0.997795792133811	-0.0571388390413354
0.997631852560431	-0.0570051339499400
0.997473008478509	-0.0568961515151239
0.997318331952575	-0.0568082736438856
0.997170293775748	-0.0567406793100804
0.997031191536884	-0.0566922464549362
0.996904920857824	-0.0566619096782633
0.996791289841087	-0.0566472718051879
0.996691962352485	-0.0566465719478760
0.996608332710086	-0.0566578808020602
0.996539367382564	-0.0566800919846165
0.996489545042702	-0.0567105357369467
0.996459548741730	-0.0567466714548197
0.996449702334699	-0.0567859363785429
0.996460217973433	-0.0568261842941875
0.996491003151397	-0.0568643510319794
0.996541416389043	-0.0568978784464396
0.996610487074264	-0.0569243660846432
0.996694646468872	-0.0569412799390298
0.996793951543561	-0.0569474048185130
0.996906775433749	-0.0569410065504720
0.997031305763922	-0.0569206113029489
0.997169826249159	-0.0568836488685482
0.997316373273004	-0.0568294169707322
0.997468540375494	-0.0567571394851005
0.997623882117913	-0.0566663897530062
0.997783726023859	-0.0565541689545081
0.997941648198565	-0.0564226525220161
0.998095067671305	-0.0562723856314051
0.998241554259047	-0.0561042589315751
0.998374626007434	-0.0559255945759979
0.998497119147252	-0.0557326404986414
0.998607303505126	-0.0555269485612140
0.998703705785017	-0.0553102615277492
0.998787085253808	-0.0550782575666565
0.998853536731290	-0.0548388922769441
0.998902284158188	-0.0545944866897250
0.998932896628034	-0.0543474031823499
0.998945319426685	-0.0540953365299064
0.998938973257731	-0.0538455091971208
0.998914375007336	-0.0536003839560973
0.998872376501068	-0.0533622771331480
0.998816321684722	-0.0531408366107549
0.998746353264229	-0.0529298238690102
0.998663955531745	-0.0527308755905034
0.998570795469109	-0.0525453793075169
0.998465952649186	-0.0523702690714994
0.998353823436868	-0.0522115436311389
0.998236617170203	-0.0520699153117073
0.998116579498189	-0.0519457638592513
0.997993483566514	-0.0518371419086188
0.997872220425844	-0.0517466012351181
0.997755132092618	-0.0516736118589297
0.997644413932619	-0.0516173209557326
0.997545280734749	-0.0515776823545864
0.997455769989050	-0.0515513617569630
0.997377418192345	-0.0515369051308277
0.997311515990871	-0.0515326852591410
0.997257908534392	-0.0515371442712578
0.997219467434399	-0.0515484668211063
0.997196818273755	-0.0515645142029111
0.997190261290606	-0.0515831202733639
0.997200296440834	-0.0516026293003267
0.997227060620633	-0.0516201763040131
0.997269952996472	-0.0516334865877632
0.997328054069649	-0.0516404433915019
0.997397707072404	-0.0516392765998004
0.997479204234331	-0.0516286561638727
0.997571047524570	-0.0516071424193425
0.997671576480018	-0.0515735507853274
0.997782525809773	-0.0515252247780792
0.997898711636909	-0.0514622298835737
0.998017969894526	-0.0513840738844533
0.998138129071453	-0.0512905991989790
0.998258863460492	-0.0511801399504189
0.998376050713638	-0.0510544622024471
0.998487556411880	-0.0509143039575685
0.998591423209767	-0.0507607011840666
0.998683528447603	-0.0505994364729560
0.998765195678799	-0.0504280495824887
0.998835149887941	-0.0502481160004335
0.998892383771324	-0.0500613502146830
0.998937685477595	-0.0498613910489611
0.998967746005292	-0.0496581752578662
0.998982288285918	-0.0494539173900037
0.998981382867206	-0.0492508036406557
0.998965736726061	-0.0490537453136390
0.998936065042506	-0.0488618971104205
0.998893261294610	-0.0486771379281271
0.998838474141073	-0.0485011533073317
0.998774117800102	-0.0483378309321944
0.998700949036084	-0.0481857557478834
0.998620600886972	-0.0480459675251102
0.998534810854972	-0.0479192322053003
0.998440382443756	-0.0478002088454118
0.998344137499490	-0.0476966275861553
0.998248290873816	-0.0476084940852399
0.998154985096270	-0.0475354639200679
0.998069268504601	-0.0474786918990319
0.997989622995311	-0.0474345663662140
0.997917674724388	-0.0474020339035509
0.997854839607481	-0.0473798269992242
0.997802378726344	-0.0473665079976545
0.997761265642248	-0.0473604515186775
0.997732288548918	-0.0473599501416210
0.997715952653406	-0.0473632294026911
0.997712757784205	-0.0473688860945719
0.997724418694969	-0.0473745113211136
0.997750609983157	-0.0473778686882184
0.997790649699810	-0.0473768515579192
0.997840427103841	-0.0473700733080182
0.997900682745265	-0.0473560370870423
0.997970162546089	-0.0473333642206593
0.998047439035401	-0.0473009121964400
0.998132433712060	-0.0472569179037808
0.998222095720616	-0.0472010884448386
0.998314579292884	-0.0471329393507857
0.998408021632116	-0.0470522914096258
0.998503689321390	-0.0469558474729573
0.998596347499599	-0.0468465110438980
0.998684057049598	-0.0467249528603962
0.998765053852360	-0.0465921372135240
0.998835390713434	-0.0464543682669261
0.998896692167562	-0.0463085156589789
0.998947883704920	-0.0461560177753930
0.998988150533783	-0.0459984349972849
0.999017890050134	-0.0458304670944626
0.999034716160617	-0.0456607353493854
0.999038528537903	-0.0454912189528654
0.999029555868979	-0.0453238452702880
0.999008818236808	-0.0451634634092589
0.998976982692427	-0.0450086408122371
0.998935006686756	-0.0448609289382656
0.998884065554941	-0.0447216728947438
0.998826075639786	-0.0445931483492334
0.998762083655035	-0.0444750087448486
0.998693664649672	-0.0443679648815530
0.998622455210472	-0.0442724525841501
0.998545202481246	-0.0441833779099888
0.998468754952502	-0.0441076273287539
0.998395130119640	-0.0440448348060570
0.998326208759768	-0.0439942990920205
0.998267058451954	-0.0439569717655295
0.998215004632598	-0.0439286621767593
0.998171218200711	-0.0439081709409038
0.998136637894798	-0.0438941491359992
0.998111587123845	-0.0438849881848122
0.998097446562312	-0.0438793733390283
0.998094518635084	-0.0438755963060136
0.998102813264164	-0.0438719563877294
0.998122696330980	-0.0438666201899736
0.998153600424069	-0.0438578980296255
0.998194757845351	-0.0438441429042232
0.998245147776031	-0.0438238955655277
0.998301913122300	-0.0437967269343145
0.998364974043015	-0.0437611588770281
0.998432912936190	-0.0437163828674810
0.998504226453109	-0.0436618504071590
0.998581565728853	-0.0435932459834282
0.998659032920212	-0.0435132694774020
0.998734761031964	-0.0434221064497810
0.998806983621655	-0.0433202630478632
0.998872016035438	-0.0432122043835501
0.998930797819593	-0.0430957721086964
0.998982097921240	-0.0429720750134845
0.999024915241392	-0.0428423909628196
0.999058721013685	-0.0427069176948191
0.999082476573684	-0.0425683497415385
0.999095828517858	-0.0424283055527972
0.999098712060338	-0.0422884063355032
0.999090990820894	-0.0421466839375660
0.999072890410694	-0.0420085132700379
0.999045116215284	-0.0418754880542287
0.999008628056563	-0.0417490185813174
0.998966174542460	-0.0416341631276702
0.998917880235896	-0.0415275616606883
0.998865076562342	-0.0414299746448287
0.998809176999425	-0.0413419101761843
0.998748513278931	-0.0412596892594813
0.998687813090657	-0.0411884539919429
0.998628815559459	-0.0411280077009220
0.998573158216594	-0.0410778469145970
0.998524091524148	-0.0410385151780098
0.998480830704242	-0.0410071678095704
0.998444484319585	-0.0409827542039758
0.998415939683989	-0.0409640691605290
0.998395727259517	-0.0409496691271657
0.998384684690815	-0.0409382963023863
0.998383086380359	-0.0409284442640147
0.998390933274527	-0.0409186123425108
0.998408750946139	-0.0409068868209164
0.998435947185495	-0.0408919982789968
0.998471782647569	-0.0408724672193580
0.998515276135360	-0.0408470041588946
0.998563637918201	-0.0408156142290297
0.998616882308298	-0.0407767464662514
0.998673692164249	-0.0407297564456239
0.998732684292799	-0.0406742534762351
0.998796210647159	-0.0406057298606125
0.998858858602126	-0.0405274460356851
0.998918946560750	-0.0404397385509139
0.998974922329493	-0.0403432472948394
0.999023437747817	-0.0402432658760306
0.999065724334590	-0.0401369826849479
0.999100830595886	-0.0400255219219273
0.999128041606267	-0.0399101364114553
0.999147178903072	-0.0397895558846365
0.999157217894452	-0.0396677998509549
0.999158089244114	-0.0395463982498401
0.999150007642485	-0.0394268346145930
0.999133429052671	-0.0393105136250680
0.999109011532672	-0.0391988148220414
0.999077623992623	-0.0390929519687431
0.999040325284055	-0.0389939316375333
0.998998934593587	-0.0389037830150365
0.998954239981916	-0.0388216998009946
0.998907579784836	-0.0387480758993714
0.998860313214778	-0.0386830473310985
0.998811367047608	-0.0386237513063520
0.998764829249527	-0.0385735573529522
0.998722173618465	-0.0385318738598734
0.998684699563659	-0.0384978479899122
0.998654848595594	-0.0384715816342108
0.998631579609890	-0.0384502501362902
0.998615544079124	-0.0384326844909554
0.998607155711702	-0.0384176403197221
0.998606789595272	-0.0384031608000904
0.998615083064310	-0.0383885103052604
0.998631795203703	-0.0383722028386215
0.998656407453596	-0.0383528580022851
0.998687369546809	-0.0383298120479544
0.998724298078024	-0.0383015742537797
0.998766168861853	-0.0382672391320907
0.998811826988161	-0.0382261278634058
0.998860744824631	-0.0381770071254782
0.998910900971128	-0.0381201170300302
0.998960906198414	-0.0380553951146061
0.999009413751557	-0.0379830460220089
0.999055882539765	-0.0379020985871236
0.999098183230181	-0.0378143599021159
0.999135177886623	-0.0377206859730172
0.999165940889588	-0.0376221191633901
0.999189412894387	-0.0375215615623504
0.999205623396894	-0.0374186436311759
0.999214269345476	-0.0373146495432241
0.999215304310029	-0.0372108700469315
0.999208439705435	-0.0371039438808627
0.999193860015061	-0.0370000778481343
0.999172224240527	-0.0369005867873838
0.999144428049047	-0.0368065963824968
0.999113083550345	-0.0367227414381062
0.999078157210824	-0.0366454723698535
0.999040803837496	-0.0365752761211447
0.999002225205760	-0.0365123993404474
0.998961155103362	-0.0364535130131959
0.998921566846402	-0.0364027949900958
0.998884870197923	-0.0363598080933505
0.998852323019542	-0.0363238424231600
0.998826291782101	-0.0362953806064793
0.998805818603172	-0.0362714798049138
0.998791547288502	-0.0362510954638448
0.998783893416649	-0.0362330996166250
0.998783165783785	-0.0362157159891881
0.998789817586698	-0.0361982836749722
0.998803652873156	-0.0361794868821452
0.998824217518846	-0.0361581039914115
0.998850524666380	-0.0361333198446658
0.998881966466842	-0.0361039259406664
0.998917590620394	-0.0360691070869251
0.998956321069681	-0.0360282708685124
0.998997453868082	-0.0359804725410431
0.999039317361592	-0.0359258969952125
0.999080649700924	-0.0358645500149980
0.999120242435307	-0.0357966913441433
0.999157504849614	-0.0357215963248877
0.999190680036252	-0.0356409423519653
0.999218805445456	-0.0355555846277190
0.999241135118946	-0.0354665391850420
0.999256973909349	-0.0353760363234712
0.999266253932099	-0.0352842083047526
0.999268833110190	-0.0351922574878720
0.999264818632831	-0.0351013639082527
0.999254128160027	-0.0350100437563271
0.999237314138483	-0.0349222447299217
0.999215115445085	-0.0348390240834297
0.999188460325549	-0.0347612365154183
0.999159370164128	-0.0346916332533696
0.999128158023873	-0.0346282294426599
0.999095941272189	-0.0345712821096547
0.999063842025396	-0.0345208105924845
0.999031327645521	-0.0344743908883596
0.999001435009541	-0.0344345591918209
0.998975311405955	-0.0344006808498834
0.998953914248662	-0.0343719008442505
0.998938628499188	-0.0343482791791867
0.998928888656832	-0.0343273858118161
0.998925041569640	-0.0343081692326963
0.998927204490951	-0.0342895508077696
0.998936113940798	-0.0342690116005113
0.998951548949902	-0.0342466025311004
0.998972964941233	-0.0342211069380128
0.998999570990229	-0.0341914851458957
0.999028713841466	-0.0341587946643059
0.999060709835967	-0.0341210011268298
0.999094533010914	-0.0340776871111496
0.999129113943888	-0.0340286663767240
0.999165397655616	-0.0339704955228908
0.999200033207856	-0.0339061470216891
0.999231820066726	-0.0338360782962291
0.999259715584994	-0.0337609935945114
0.999281972176948	-0.0336851865919138
0.999299189359146	-0.0336064942598024
0.999310902091258	-0.0335259142400725
0.999316877067281	-0.0334444985007800
0.999316948487023	-0.0333593436908916
0.999310825896144	-0.0332756969930403
0.999298903091345	-0.0331947335463544
0.999281819709196	-0.0331174835483291
0.999261382073407	-0.0330477885330022
0.999237811681778	-0.0329829780929332
0.999212054037051	-0.0329235365310905
0.999185115840654	-0.0328697239835814
0.999156960632483	-0.0328198034038332
0.999129823141833	-0.0327759344427930
0.999104820509477	-0.0327377874847718
0.999082943058570	-0.0327047966676186
0.999065520895177	-0.0326770191675646
0.999052528276557	-0.0326525924897957
0.999044471600156	-0.0326306125075959
0.999041638703433	-0.0326101052993607
0.999044290385979	-0.0325894233204405
0.999052544824167	-0.0325681136260893
0.999066122975972	-0.0325451021955195
0.999084516682085	-0.0325194269499379
0.999106738969118	-0.0324906348820017
0.999132209267807	-0.0324577143971455
0.999160032974508	-0.0324201318216697
0.999189237604201	-0.0323775751079892
0.999219586962483	-0.0323286092340260
0.999249214571469	-0.0322743246647249
0.999277055009690	-0.0322149831823288
0.999302152402882	-0.0321510769544635
0.999323457604715	-0.0320840408521537
0.999340553067538	-0.0320139678797838
0.999352907189089	-0.0319417457524052
0.999360212583066	-0.0318683399878297
0.999362348949885	-0.0317929900266257
0.999359125222846	-0.0317185484387512
0.999350809941336	-0.0316460649047313
0.999337901879835	-0.0315764754268052
0.999321463042698	-0.0315119262227063
0.999302019180002	-0.0314515998911305
0.999280429999047	-0.0313959919579360
0.999257626580314	-0.0313453796356556
0.999233998694945	-0.0312987727742269
0.999211162597030	-0.0312574398464317
0.999190123352433	-0.0312211041633741
0.999171772264670	-0.0311892669360530
0.999157121472698	-0.0311617560648657
0.999146432097121	-0.0311371948658968
0.999140166226898	-0.0311147411906797
0.999138571692943	-0.0310934863476896
0.999141861134390	-0.0310719122756027
0.999150057744369	-0.0310495893579144
0.999162866370848	-0.0310255456274467
0.999179776184335	-0.0309989252017189
0.999199874569498	-0.0309693472151745
0.999222568911797	-0.0309359273817884
0.999247003696902	-0.0308982348304927
0.999272263425916	-0.0308560575787733
0.999298228805197	-0.0308077644538253
0.999323042222923	-0.0307548025586928
0.999345735805245	-0.0306975199566460
0.999365473633183	-0.0306364810943906
0.999381268278551	-0.0305737557399288
0.999393009964538	-0.0305089029177695
0.999400331165527	-0.0304427904861826
0.999403086387127	-0.0303763302133676
0.999401143557319	-0.0303075767943595
0.999394493269043	-0.0302404822199225
0.999383564707937	-0.0301759994598001
0.999369001921353	-0.0301149245391107
0.999352378590598	-0.0300602020094451
0.999333936674167	-0.0300096478762296
0.999314530263926	-0.0299635360451125
0.999295036127833	-0.0299219247655748
0.999275244545051	-0.0298826036616062
0.999257335339690	-0.0298478863480761
0.999242212994949	-0.0298172593299430
0.999230603283041	-0.0297900048486011
0.999223341481604	-0.0297664963829256
0.999220095130128	-0.0297444537487279
0.999221042341800	-0.0297230299996508
0.999226150677826	-0.0297013763160638
0.999236100599505	-0.0296767871828738
0.999250236727953	-0.0296499836239230
0.999267934533793	-0.0296201068599937
0.999288376693857	-0.0295865070882856
0.999309288675842	-0.0295510638014004
0.999330965590689	-0.0295116657515060
0.999352545633547	-0.0294682480804164
0.999373193340454	-0.0294209576245270
0.999393124760789	-0.0293671666071354
0.999410285184713	-0.0293099356809120
0.999423962581738	-0.0292499551896806
0.999433661832997	-0.0291880632087319
0.999438962228781	-0.0291275385863964
0.999440165536650	-0.0290669618531356
0.999437329367988	-0.0290071945645759
0.999430721389206	-0.0289490395652158
0.999420519709244	-0.0288920187788893
0.999407412624860	-0.0288381388899978
0.999392113991261	-0.0287879472801644
0.999375439404627	-0.0287417798228805
0.999358448833615	-0.0287002365337002
0.999341819046352	-0.0286627874926334
0.999326380704191	-0.0286292596253960
0.999312877700082	-0.0285992790594002
0.999301902732898	-0.0285721867270982
0.999294103736609	-0.0285475169155678
0.999289892252017	-0.0285245363427439
0.999289472283301	-0.0285024444895939
0.999292939933399	-0.0284801181272160
0.999300219940933	-0.0284570016730375
0.999311020119613	-0.0284322932240872
0.999324856263030	-0.0284053072445662
0.999341033849100	-0.0283756172820555
0.999358908960850	-0.0283426591662064
0.999377710586166	-0.0283061488358500
0.999396634328543	-0.0282660136787145
0.999415633268464	-0.0282204310128487
0.999433018320910	-0.0281712908033785
0.999448004148692	-0.0281190469547160
0.999459970339724	-0.0280643399089102
0.999468235832556	-0.0280098340059485
0.999472951313486	-0.0279544895099932
0.999473995063456	-0.0278990968728427
0.999471455565874	-0.0278444357536921
0.999465139222036	-0.0277880941134866
0.999455537910510	-0.0277342301699208
0.999443274753793	-0.0276835333997361
0.999429129589911	-0.0276364791440900
0.999414817304675	-0.0275956188105469
0.999400362312759	-0.0275583828908858
0.999386528248601	-0.0275247149997988
0.999374023371512	-0.0274943627771382
0.999363195710528	-0.0274661345882752
0.999355069348909	-0.0274404508775584
0.999350116044455	-0.0274166452123173
0.999348601334885	-0.0273939591707213
0.999350564793340	-0.0273718700258274
0.999355928654761	-0.0273493206000542
0.999364480100140	-0.0273255733827228
0.999375821190512	-0.0272999859412657
0.999389607923593	-0.0272716482940584
0.999405075174414	-0.0272404116447840
0.999421505752958	-0.0272059754338342
0.999438139516383	-0.0271682481006895
0.999454640789589	-0.0271261621561427
0.999469756058056	-0.0270809193708045
0.999482769192372	-0.0270329219528637
0.999493115818936	-0.0269827488035759
0.999500251505618	-0.0269323072918361
0.999504172937682	-0.0268811536743317
0.999504776121981	-0.0268300279299214
0.999502162590733	-0.0267796570650647
0.999496169650482	-0.0267277869079504
0.999487305564223	-0.0266782910976890
0.999476182270602	-0.0266317883737328
0.999463556661561	-0.0265886806415598
0.999451016096885	-0.0265513131032674
0.999438594072072	-0.0265172146898050
0.999426996143268	-0.0264862772831445
0.999416859432834	-0.0264582061983524
0.999408567182396	-0.0264319820961671
0.999402897146764	-0.0264077545680238
0.999400213023746	-0.0263848708813702
0.999400674542484	-0.0263626118913074
0.999404269762721	-0.0263402340756936
0.999410868694835	-0.0263170205092668
0.999420175163871	-0.0262923044834069
0.999431721874634	-0.0262655385687348
0.999444925169649	-0.0262363074153862
0.999459144276692	-0.0262042835344543
0.999473685985807	-0.0261693078489527
0.999487850412061	-0.0261314234764536
0.999501679710459	-0.0260884375626908
0.999513601917266	-0.0260428069106518
0.999522999845678	-0.0259950694264572
0.999529454383149	-0.0259459162228244
0.999532648982278	-0.0258984588526971
0.999532863705980	-0.0258511084564300
0.999530176659373	-0.0258045532761376
0.999524855667499	-0.0257594198299333
0.999517079121275	-0.0257151221725612
0.999507490746717	-0.0256734074645673
0.999496726557128	-0.0256346375717335
0.999485491115680	-0.0255989657664598
0.999474600774576	-0.0255666549548800
0.999464642106289	-0.0255372296100819
0.999456244077556	-0.0255103948636917
0.999449913472343	-0.0254856894431812
0.999446053078243	-0.0254627482324057
0.999444873501677	-0.0254407342912053
0.999446496234912	-0.0254189992465353
0.999450849550461	-0.0253968956564485
0.999458194117665	-0.0253723852715554
0.999467969211818	-0.0253461044874966
0.999479641088048	-0.0253175054523258
0.999492537445701	-0.0252862372815413
0.999505334520739	-0.0252536794241537
0.999517920050636	-0.0252184839033612
0.999529652147238	-0.0251807729686559
0.999539960593247	-0.0251408480537596
0.999548605189705	-0.0250977587118615
0.999554781997843	-0.0250533236572154
0.999558205745667	-0.0250081837848258
0.999558802328204	-0.0249630277063579
0.999556657206750	-0.0249183451173263
0.999551977284985	-0.0248750019240992
0.999545135700158	-0.0248335830783440
0.999536661701061	-0.0247945232893994
0.999527429439128	-0.0247590208396247
0.999517844827516	-0.0247261994161354
0.999508534111102	-0.0246960721239260
0.999500090471238	-0.0246684652181211
0.999492722293635	-0.0246417981265108
0.999487449474648	-0.0246171096926933
0.999484681315244	-0.0245938197721758
0.999484617594036	-0.0245712525851622
0.999487126755714	-0.0245495779421134
0.999492072160377	-0.0245273065844547
0.999499219900719	-0.0245038683031728
0.999508177780418	-0.0244787953887216
0.999518626145769	-0.0244512762087466
0.999529860554129	-0.0244214225950215
0.999541262909519	-0.0243891085358448
0.999552212306605	-0.0243544040583415
0.999562583216056	-0.0243156633443393
0.999571200778304	-0.0242749083641080
0.999577572476487	-0.0242326505680688
0.999581403027767	-0.0241895296853287
0.999582579456453	-0.0241480865401164
0.999581321060342	-0.0241071006025864
0.999577785262868	-0.0240671602316763
0.999572300966952	-0.0240287691129535
0.999565200589285	-0.0239918079400919
0.999557080089944	-0.0239571944084660
0.999548530912551	-0.0239251182530273
0.999540167766405	-0.0238955703376953
0.999532447303993	-0.0238678913745338
0.999526116624394	-0.0238423873944119
0.999521663727373	-0.0238186438059594
0.999519411828498	-0.0237961124748059
0.999519490528048	-0.0237748515632165
0.999521856170864	-0.0237535846031076
0.999526421304040	-0.0237317490428943
0.999532928739268	-0.0237088418163019
0.999541406157500	-0.0236832777189871
0.999551094257187	-0.0236556841321503
0.999561409888753	-0.0236258106572274
0.999571722643450	-0.0235936131836383
0.999581360829465	-0.0235594212798110
0.999589813677042	-0.0235232775024378
0.999596591850098	-0.0234855442611888
0.999601353704107	-0.0234467202925819
0.999603884641399	-0.0234078362836290
0.999604158966851	-0.0233690144116456
0.999602234725034	-0.0233308262625536
0.999598349390397	-0.0232937888143134
0.999592651874095	-0.0232571357817301
0.999585721955550	-0.0232225860468998
0.999578122419751	-0.0231904013198718
0.999570468067012	-0.0231606358147999
0.999563488016414	-0.0231336646431938
0.999557579370129	-0.0231087167906246
0.999553208342380	-0.0230854594111692
0.999550702241334	-0.0230634258244333
0.999550245168069	-0.0230423539993898
0.999551887793788	-0.0230214200757853
0.999555583284952	-0.0230000884708666
0.999561114085542	-0.0229778702094086
0.999568585258060	-0.0229529519714506
0.999577257302915	-0.0229261723522722
0.999586570150935	-0.0228972685364381
0.999595906774964	-0.0228661882955165
0.999604466961774	-0.0228338432272676
0.999611943551844	-0.0227997403766507
0.999617885570694	-0.0227642176647439
0.999621983407724	-0.0227277428126307
0.999624059554802	-0.0226910569847646
0.999624067938041	-0.0226544963465730
0.999622080277391	-0.0226185976689952
0.999618342741306	-0.0225838391302142
0.999613034417319	-0.0225495574379911
0.999606717036742	-0.0225172641213631
0.999599931777734	-0.0224871714382724
0.999593258747721	-0.0224592871562806
0.999587331851856	-0.0224337970564635
0.999582553128759	-0.0224100754799478
0.999579334630001	-0.0223877666413552
0.999577939360861	-0.0223663942970206
0.999578463750492	-0.0223457925030672
0.999580897136762	-0.0223250783620515
0.999585133144067	-0.0223037590374083
0.999590905982473	-0.0222814067734005
0.999598175191324	-0.0222565905831316
0.999606239572238	-0.0222299760165921
0.999614562719346	-0.0222014043847062
0.999622585103515	-0.0221709168595659
0.999629808946152	-0.0221385782646405
0.999635724108654	-0.0221047912656995
0.999639952956285	-0.0220699595470794
0.999642285827877	-0.0220345947448150
0.999642676729323	-0.0219999605384315
0.999641229747494	-0.0219658505799100
0.999638119441181	-0.0219327424761704
0.999633674781669	-0.0219010215861743
0.999628252345322	-0.0218706306323838
0.999622370238457	-0.0218421499166375
0.999616537502146	-0.0218156471481297
0.999611253845338	-0.0217910042718799
0.999606825422076	-0.0217671267274197
0.999603900098767	-0.0217446201883520
0.999602790448171	-0.0217230224879957
0.999603615346871	-0.0217017833655294
0.999606175810098	-0.0216812771356405
0.999610347110891	-0.0216601232591415
0.999615886068579	-0.0216379103540723
0.999622419971083	-0.0216143369954167
0.999629634330148	-0.0215887639800820
0.999636939863020	-0.0215614830012572
0.999643846333400	-0.0215325236001713
0.999649904599613	-0.0215020880494374
0.999654998765115	-0.0214685093862628
0.999658357920422	-0.0214340798975057
0.999659768256865	-0.0213993305491117
0.999659236681565	-0.0213648390126851
0.999657059794251	-0.0213324320254940
0.999653488975504	-0.0213012085474660
0.999648875946004	-0.0212715214462279
0.999643679233376	-0.0212435692503002
0.999638493991590	-0.0212178938100281
0.999633683538015	-0.0211939175732864
0.999629680967749	-0.0211714874898189
0.999626835836852	-0.0211503031951658
0.999625382567929	-0.0211295578873370
0.999625581139988	-0.0211092669428894
0.999627485517076	-0.0210889574172548
0.999630970063072	-0.0210681655033161
0.999635960556901	-0.0210457388963198
0.999642019658296	-0.0210219838258605
0.999648708375243	-0.0209966381265218
0.999655513677963	-0.0209696256637987
0.999661758962447	-0.0209418153913807
0.999667195092526	-0.0209126556741251
0.999671448845518	-0.0208824176597917
0.999674271555589	-0.0208514929331788
0.999675542698432	-0.0208201342190312
0.999675199318464	-0.0207889911811860
0.999673332858273	-0.0207585140103465
0.999670197596075	-0.0207290877803405
0.999666023472079	-0.0207002223293980
0.999661310718706	-0.0206730162557051
0.999656535141056	-0.0206475736554261
0.999652181182344	-0.0206238033753607
0.999648691976908	-0.0206015401161370
0.999646421766998	-0.0205804154505847
0.999645638451900	-0.0205600428779519
0.999646440432935	-0.0205399549276320
0.999648705119748	-0.0205201912381777
0.999652317418272	-0.0204998372779101
0.999657049112599	-0.0204785336798247
0.999662550567694	-0.0204560289031542
0.999668530014112	-0.0204317061212034
0.999674448630494	-0.0204059297339192
0.999679871226986	-0.0203787657270322
0.999684415654275	-0.0203504427908586
0.999687930361781	-0.0203197405957734
0.999689889284206	-0.0202885551334222
0.999690176228388	-0.0202573726270754
0.999688884483221	-0.0202266936243008
0.999686323535407	-0.0201975520480982
0.999682773897011	-0.0201696756104173
0.999678620301041	-0.0201433166077205
0.999674323361723	-0.0201185531619884
0.999670450939854	-0.0200959580927792
0.999667269500230	-0.0200746761958223
0.999665115237388	-0.0200544685290277
0.999664208780111	-0.0200349796673811
0.999664658142195	-0.0200157290740203
0.999666499136373	-0.0199963887363438
0.999669642085523	-0.0199765618404721
0.999673847280871	-0.0199559110068613
0.999679054491973	-0.0199330299215191
0.999684656264812	-0.0199087592297900
0.999690197917512	-0.0198830284224607
0.999695224042792	-0.0198559609357048
0.999699340235316	-0.0198278305474667
0.999702230750939	-0.0197989411550182
0.999703686110257	-0.0197696904362544
0.999703676742167	-0.0197405360290244
0.999702359017051	-0.0197125059600592
0.999699924692992	-0.0196853653080652
0.999696654412573	-0.0196594176799855
0.999692933236396	-0.0196348307473514
0.999689218642938	-0.0196118884327245
0.999685860153524	-0.0195902842567391
0.999683220119213	-0.0195698720092022
0.999681577694266	-0.0195503681628317
0.999681113755469	-0.0195310145619699
0.999681989414725	-0.0195118485109459
0.999684196937776	-0.0194924650720550
0.999687560613425	-0.0194724873894729
0.999691997133237	-0.0194506688921500
0.999697017532019	-0.0194276129123306
0.999702195427465	-0.0194031823795218
0.999707070839572	-0.0193774351498585
0.999711123506101	-0.0193513337709024
0.999714178842506	-0.0193244250736836
0.999716005706468	-0.0192970404565088
0.999716527350622	-0.0192695855887234
0.999715807168862	-0.0192426229806490
0.999713976386923	-0.0192163619289269
0.999711264538428	-0.0191911160783655
0.999708016763506	-0.0191670805652287
0.999704632662608	-0.0191444014386042
0.999701477044900	-0.0191230039483380
0.999698909332785	-0.0191027788025804
0.999697218913168	-0.0190834721809507
0.999696597529522	-0.0190642143723564
0.999697243369772	-0.0190452026865265
0.999699169831304	-0.0190260398596171
0.999702215440580	-0.0190063468850445
0.999706182368648	-0.0189854273918299
0.999710696501720	-0.0189633973592175
0.999715370374187	-0.0189401253003299
0.999719781857237	-0.0189156596623576
0.999723493677425	-0.0188906009831210
0.999726279218278	-0.0188647958225670
0.999727919789792	-0.0188385578432580
0.999728347057450	-0.0188122739387771
0.999727627608379	-0.0187864472756644
0.999725892298766	-0.0187613047370920
0.999723367399456	-0.0187371381170540
0.999720390128316	-0.0187141202059316
0.999717346430872	-0.0186923833489781
0.999714580130593	-0.0186718254587995
0.999712425710569	-0.0186523237593151
0.999711141955229	-0.0186336174119277
0.999710895507746	-0.0186149236589689
0.999711827971164	-0.0185963587846903
0.999713920546863	-0.0185775506394150
0.999716988046140	-0.0185581577129185
0.999720879477082	-0.0185372090689027
0.999725160581649	-0.0185151537290774
0.999729439654309	-0.0184919065062860
0.999733308806534	-0.0184675698778306
0.999736366312422	-0.0184428791530623
0.999738439546583	-0.0184176317601837
0.999739366299656	-0.0183921615017330
0.999739146437876	-0.0183668527853221
0.999737921483131	-0.0183422564551384
0.999735875195830	-0.0183184780930222
0.999733275179049	-0.0182957509111148
0.999730476176457	-0.0182741702226763
0.999727875143745	-0.0182539548281480
0.999725756859678	-0.0182347432960147
0.999724400715873	-0.0182163529647584
0.999723986099948	-0.0181984873468812
0.999724596938154	-0.0181806039073657
0.999726249365060	-0.0181625757217255
0.999728844563009	-0.0181440814405483
0.999732144186026	-0.0181248632080028
0.999736020801972	-0.0181037644038846
0.999739967978942	-0.0180815888763997
0.999743609855092	-0.0180583532982755
0.999746601175146	-0.0180342530567051
0.999748713420127	-0.0180091851042334
0.999749712339154	-0.0179838774689874
0.999749536601658	-0.0179587114976289
0.999748316970250	-0.0179340728407513
0.999746362126375	-0.0179107845473713
0.999743928567939	-0.0178885206440761
0.999741348552334	-0.0178674041764998
0.999738991464850	-0.0178473886446929
0.999737221491537	-0.0178287211988566
0.999736229905323	-0.0178107424723108
0.999736193169834	-0.0177931814955346
0.999737149817404	-0.0177757008040143
0.999739011348884	-0.0177580502294411
0.999741650311666	-0.0177398711252182
0.999744854543486	-0.0177209354336442
0.999748319438538	-0.0177011256287476
0.999751784346961	-0.0176800114819155
0.999754864940878	-0.0176580398257701
0.999757278518777	-0.0176353670430245
0.999758833543153	-0.0176122718833863
0.999759450623437	-0.0175885387155246
0.999759068346013	-0.0175650425824277
0.999757781451971	-0.0175421082785390
0.999755837582624	-0.0175199915963863
0.999753518673496	-0.0174984897019291
0.999751187416313	-0.0174780699762957
0.999749188511300	-0.0174587010431397
0.999747828777695	-0.0174401768830200
0.999747319346016	-0.0174219901145240
0.999747815098124	-0.0174040409728210
0.999749341949719	-0.0173859828212705
0.999751744977391	-0.0173674738464956
0.999754685143124	-0.0173486802644337
0.999757939420997	-0.0173290387698049
0.999761196846221	-0.0173084765304045
0.999764128366078	-0.0172870773839285
0.999766468730280	-0.0172648934869211
0.999767984917477	-0.0172422937820843
0.999768548660300	-0.0172195706670140
0.999768185133510	-0.0171970607802608
0.999767045647032	-0.0171751817281628
0.999765315108672	-0.0171540580705131
0.999763248341213	-0.0171338625031870
0.999761169516939	-0.0171146282038936
0.999759414724778	-0.0170965091673142
0.999758209751060	-0.0170791168801469
0.999757758508086	-0.0170622470827812
0.999758151813685	-0.0170456068009761
0.999759379456258	-0.0170288071929553
0.999761367411439	-0.0170116572295325
0.999763957103026	-0.0169939195863921
0.999766882274927	-0.0169754474231727
0.999769928534078	-0.0169556109663644
0.999772709788961	-0.0169349737958018
0.999774946404033	-0.0169136558863694
0.999776436011982	-0.0168919114313633
0.999777090321541	-0.0168694252272706
0.999776829625356	-0.0168471362090391
0.999775735751608	-0.0168253571815537
0.999774052770547	-0.0168043365469870
0.999772076898784	-0.0167839811906469
0.999770140851795	-0.0167646046341065
0.999768566893594	-0.0167461610936391
0.999767633293317	-0.0167284281586700
0.999767513676473	-0.0167110892757626
0.999768294895935	-0.0166938500296395
0.999769961636137	-0.0166763940122411
0.999772325161116	-0.0166584278206644
0.999775065305036	-0.0166399748318669
0.999777931730553	-0.0166207202151606
0.999780624331755	-0.0166006505381497
0.999782851684814	-0.0165799116946046
0.999784410755701	-0.0165585229400383
0.999785133989222	-0.0165369662283788
0.999784973990545	-0.0165155420773777
0.999784048966259	-0.0164945575822295
0.999782595178328	-0.0164743809108464
0.999780847456542	-0.0164550350889120
0.999779087821027	-0.0164365955759885
0.999777622264192	-0.0164189786532241
0.999776715216586	-0.0164022945646504
0.999776506143189	-0.0163860154911233
0.999777093381212	-0.0163698901056805
0.999778436668157	-0.0163536277086089
0.999780386830364	-0.0163370058431676
0.999782771051682	-0.0163198020284103
0.999785359229304	-0.0163018900114565
0.999787867576255	-0.0162832690949900
0.999790061732278	-0.0162637441109136
0.999791682441043	-0.0162437480112187
0.999792570248477	-0.0162234980420365
0.999792690160467	-0.0162032823286442
0.999792112848491	-0.0161832727376097
0.999790959778498	-0.0161638150217049
0.999789426872943	-0.0161450924150704
0.999787797252087	-0.0161271696290033
0.999786368629623	-0.0161101366829038
0.999785360485080	-0.0160937521614890
0.999784966751903	-0.0160778501284272
0.999785280914971	-0.0160621682527182
0.999786301382077	-0.0160463105781226
0.999787962642657	-0.0160301516712146
0.999790121943173	-0.0160134812464047
0.999792529983878	-0.0159961754703123
0.999794976131302	-0.0159776800864591
0.999797126987857	-0.0159585348308030
0.999798744967186	-0.0159388696482232
0.999799677179725	-0.0159189393313367
0.999799879589043	-0.0158986694454283
0.999799355212667	-0.0158787050084698
0.999798222165299	-0.0158593000016758
0.999796739558819	-0.0158406243062340
0.999795220285915	-0.0158228181575395
0.999793920886318	-0.0158057714206046
0.999793089867280	-0.0157893810355042
0.999792902871603	-0.0157734027044277
0.999793431716359	-0.0157574237791441
0.999794674199376	-0.0157413014768395
0.999796536938441	-0.0157247852280844
0.999798783561160	-0.0157076881800758
0.999801195253406	-0.0156893648367214
0.999803421792508	-0.0156703422062327
0.999805192969888	-0.0156507153248397
0.999806307130976	-0.0156307378465044
0.999806685027397	-0.0156104421264053
0.999806310241617	-0.0155903977469956
0.999805283769074	-0.0155708799007442
0.999803874549851	-0.0155520859515956
0.999802436078246	-0.0155344136761357
0.999801208365581	-0.0155174913076351
0.999800443229351	-0.0155012179758791
0.999800319082699	-0.0154853403697821
0.999800892559536	-0.0154696251829450
0.999802144415299	-0.0154537449981048
0.999803974060333	-0.0154374588181070
0.999806138402151	-0.0154205939490054
0.999808393423783	-0.0154026905769833
0.999810423091107	-0.0153841404913195
0.999811976343646	-0.0153650523201336
0.999812878839980	-0.0153456845677085
0.999813078329555	-0.0153262169825611
0.999812595210781	-0.0153070463627563
0.999811546362423	-0.0152884210825213
0.999810200763764	-0.0152705026175320
0.999808897561969	-0.0152536841009164
0.999807852550686	-0.0152375401622317
0.999807289681497	-0.0152219548057721
0.999807351419485	-0.0152066766853133
0.999808061448118	-0.0151914860385373
0.999809378461889	-0.0151760793834187
0.999811186457431	-0.0151602430943570
0.999813243545044	-0.0151438402587058
0.999815313920135	-0.0151264806007725
0.999817108550090	-0.0151085475294569
0.999818406258493	-0.0150901658780858
0.999819071703352	-0.0150715915493562
0.999819086521418	-0.0150530152530759
0.999818498325639	-0.0150347804877284
0.999817439076983	-0.0150171041735488
0.999816172444490	-0.0150001082138859
0.999815010820146	-0.0149841057077583
0.999814150847781	-0.0149687006694271
0.999813787807977	-0.0149537634815779
0.999814028310769	-0.0149390470138098
0.999814866055680	-0.0149243222408895
0.999816239075660	-0.0149093345914734
0.999818017235601	-0.0148938977743585
0.999819960980717	-0.0148779100221699
0.999821845270401	-0.0148610363988113
0.999823406877663	-0.0148436631446193
0.999824454264816	-0.0148259301764385
0.999824890363963	-0.0148080901161434
0.999824730299754	-0.0147903377061517
0.999824047218803	-0.0147729693511064
0.999822987387140	-0.0147561707107969
0.999821808932260	-0.0147400245395708
0.999820798148922	-0.0147247731601298
0.999820131445458	-0.0147100402550345
0.999819974767737	-0.0146956828781873
0.999820398163629	-0.0146814585750552
0.999821364813678	-0.0146671352575249
0.999822790998063	-0.0146525028865200
0.999824532543550	-0.0146374039741000
0.999826353156779	-0.0146217735071997
0.999828040525369	-0.0146053290157904
0.999829358733168	-0.0145884639720151
0.999830147681270	-0.0145713332426754
0.999830350520937	-0.0145541849906393
0.999830017447301	-0.0145372096746188
0.999829246982766	-0.0145206608991230
0.999828199571160	-0.0145046910934163
0.999827126629880	-0.0144893417016842
0.999826286423565	-0.0144747851275658
0.999825832898218	-0.0144606612313825
0.999825900074726	-0.0144468136838263
0.999826518555409	-0.0144330061115388
0.999827619309794	-0.0144190051160144
0.999829094937573	-0.0144046486731487
0.999830787048544	-0.0143898114367573
0.999832464441258	-0.0143744688747426
0.999833931373703	-0.0143583849028850
0.999834982223705	-0.0143419703185274
0.999835492244469	-0.0143253951017918
0.999835449215176	-0.0143089007314781
0.999834941591322	-0.0142926607914707
0.999834094284941	-0.0142768905468576
0.999833081996478	-0.0142617047681169
0.999832146904899	-0.0142470986168100
0.999831514495290	-0.0142331702950457
0.999831311836299	-0.0142195748443570
0.999831635695992	-0.0142061424426129
0.999832471355440	-0.0141926458348972
0.999833714397739	-0.0141788487401711
0.999835230282187	-0.0141646494811108
0.999836846180021	-0.0141499613845077
0.999838339752047	-0.0141348076277414
0.999839538922245	-0.0141189864212323
0.999840274561209	-0.0141029459352172
0.999840465154469	-0.0140868714695864
0.999840152000286	-0.0140709930635997
0.999839467566402	-0.0140554443333669
0.999838565955620	-0.0140404085861828
0.999837635939629	-0.0140259536624335
0.999836904505439	-0.0140120181397399
0.999836553670022	-0.0139986106748575
0.999836674345206	-0.0139854073856557
0.999837314993078	-0.0139722255381955
0.999838403719952	-0.0139588543850159
0.999839795759900	-0.0139450423151887
0.999841322605729	-0.0139307839247069
0.999842797692553	-0.0139160449045196
0.999844016954913	-0.0139009108753944
0.999844847181872	-0.0138851783225886
0.999845170001251	-0.0138693839383866
0.999844964459002	-0.0138537271921983
0.999844344505562	-0.0138384139392954
0.999843496455255	-0.0138234769086037
0.999842609660451	-0.0138090888044449
0.999841883910997	-0.0137952491752577
0.999841513569405	-0.0137818171181800
0.999841610656806	-0.0137686574891125
0.999842206147561	-0.0137555061390335
0.999843273900891	-0.0137421729910836
0.999844658245524	-0.0137284869789616
0.999846170472425	-0.0137141078436267
0.999847591014146	-0.0136992622301429
0.999848727526079	-0.0136840028657373
0.999849426787895	-0.0136685129530872
0.999849634862410	-0.0136524061744571
0.999849328989505	-0.0136365188147555
0.999848596944168	-0.0136210515042398
0.999847676036892	-0.0136061349079091
0.999846844312770	-0.0135919052095073
0.999846288863029	-0.0135781602852897
0.999846178982052	-0.0135647784662445
0.999846592521512	-0.0135515095818367
0.999847456186300	-0.0135384787233353
0.999848679450307	-0.0135251481654669
0.999850121141768	-0.0135113894634321
0.999851551253683	-0.0134971719978379
0.999852751748097	-0.0134825441385131
0.999853570685960	-0.0134676465685255
0.999853902001325	-0.0134526387225000
0.999853752516107	-0.0134377490352140
0.999853232907573	-0.0134232492274085
0.999852474937796	-0.0134091939840104
0.999851646441068	-0.0133956639587734
0.999850967814686	-0.0133826182207726
0.999850622675858	-0.0133701256449094
0.999850696698814	-0.0133578342289774
0.999851241940650	-0.0133455780759174
0.999852195880391	-0.0133331569615168
0.999853422145447	-0.0133203456743313
0.999854765638527	-0.0133071299125679
0.999856054547243	-0.0132934793053514
0.999857098991395	-0.0132794789671193
0.999857778173703	-0.0132649373051743
0.999857992968328	-0.0132503670521798
0.999857734158558	-0.0132359532014194
0.999857123881370	-0.0132218820098915
0.999856347863678	-0.0132081379445810
0.999855589580619	-0.0131948955014209
0.999855033549406	-0.0131821344443838
0.999854847356382	-0.0131696973472299
0.999855109410478	-0.0131573724287889
0.999855821640877	-0.0131449759456018
0.999856929645153	-0.0131323348781277
0.999858253019490	-0.0131193136316693
0.999859605951464	-0.0131054812306698
0.999860760193956	-0.0130912403361175
0.999861545001345	-0.0130766847116503
0.999861859097891	-0.0130620350794467
0.999861711476066	-0.0130472733904594
0.999861170889541	-0.0130328505822305
0.999860371571336	-0.0130189181549355
0.999859568288568	-0.0130055200420291
0.999859027564402	-0.0129931729448132
0.999858839786997	-0.0129811299661694
0.999859102007335	-0.0129692448646993
0.999859803885803	-0.0129572992115684
0.999860821706766	-0.0129452811989540
0.999862037380983	-0.0129329117397369
0.999863296404657	-0.0129201265232595
0.999864400290867	-0.0129069682415882
0.999865201199529	-0.0128933390178112
0.999865585210063	-0.0128796014448713
0.999865510906411	-0.0128659250527170
0.999865059331509	-0.0128525051645719
0.999864388172039	-0.0128394189314626
0.999863657137329	-0.0128267950347237
0.999863039176915	-0.0128146450430071
0.999862714038965	-0.0128028508515553
0.999862787545548	-0.0127912810446467
0.999863286750484	-0.0127797160623746
0.999864189345791	-0.0127679899980739
0.999865352069828	-0.0127559512872980
0.999866604040227	-0.0127432623401120
0.999867746760586	-0.0127301760587407
0.999868613510746	-0.0127167497848508
0.999869079365533	-0.0127031631413792
0.999869113614838	-0.0126889901842446
0.999868723850067	-0.0126750726503628
0.999868012462421	-0.0126615789071571
0.999867221861820	-0.0126485941012071
0.999866620562996	-0.0126364381869365
0.999866334572571	-0.0126246293537516
0.999866482528712	-0.0126130331017291
0.999867079308678	-0.0126014176797768
0.999867998234523	-0.0125899393144454
0.999869132633949	-0.0125781312176969
0.999870334921035	-0.0125659200580404
0.999871403515779	-0.0125533380778903
0.999872178685141	-0.0125404049830897
0.999872558060876	-0.0125273568502870
0.999872497023827	-0.0125143561323881
0.999872070933977	-0.0125015954082829
0.999871433616199	-0.0124891780404786
0.999870738318743	-0.0124772015957063
0.999870151341078	-0.0124656778912480
0.999869847236995	-0.0124544915274754
0.999869927360102	-0.0124435063008906
0.999870414949564	-0.0124325166846256
0.999871285618752	-0.0124213630362652
0.999872395931982	-0.0124099009929205
0.999873577969796	-0.0123977940247006
0.999874637361241	-0.0123853083633765
0.999875414736968	-0.0123725060840514
0.999875796079627	-0.0123595695952615
0.999875760471366	-0.0123460581268600
0.999875329348333	-0.0123328215642563
0.999874613206110	-0.0123200175816732
0.999873859760548	-0.0123077126547937
0.999873335305049	-0.0122963260317024
0.999873138955714	-0.0122852370683554
0.999873370524112	-0.0122743071688389
0.999874022076127	-0.0122633140857105
0.999874952674118	-0.0122523950669599
0.999876050703532	-0.0122411395644569
0.999877167759542	-0.0122294929296772
0.999878114156768	-0.0122175079074619
0.999878751748778	-0.0122051714857001
0.999878993768696	-0.0121927709645057
0.999878816127906	-0.0121804679758053
0.999878316393807	-0.0121684404361714
0.999877659475373	-0.0121567232015852
0.999877004952417	-0.0121454377547160
0.999876515659435	-0.0121345724981350
0.999876346337697	-0.0121239877789180
0.999876569437332	-0.0121134659149391
0.999877183295959	-0.0121028688046764
0.999878136494821	-0.0120920437097071
0.999879258734246	-0.0120808728305853
0.999880379026896	-0.0120689410559656
0.999881289598093	-0.0120566618782031
0.999881843799109	-0.0120441319871038
0.999881968733564	-0.0120315672996786
0.999881702732207	-0.0120190832549864
0.999881139235974	-0.0120069427576679
0.999880415511831	-0.0119952605604143
0.999879768405237	-0.0119840377246837
0.999879417529565	-0.0119736781284240
0.999879419866976	-0.0119635114903550
0.999879832810190	-0.0119533927617040
0.999880603284448	-0.0119431295476412
0.999881587061559	-0.0119326592608223
0.999882652203773	-0.0119218378882660
0.999883647528627	-0.0119106450477726
0.999884405493178	-0.0118991709155158
0.999884826134774	-0.0118873033809283
0.999884848374894	-0.0118754633930061
0.999884485028387	-0.0118638122892020
0.999883874276517	-0.0118525009015136
0.999883199515248	-0.0118414281351856
0.999882633714513	-0.0118307714674202
0.999882332808586	-0.0118204772213509
0.999882412733894	-0.0118103620566056
0.999882896446073	-0.0118000442265774
0.999883731208180	-0.0117895265933718
0.999884816227760	-0.0117786730198327
0.999885933869293	-0.0117674224085325
0.999886867734765	-0.0117557898672103
0.999887475507725	-0.0117439173909134
0.999887657562033	-0.0117319464028266
0.999887427372593	-0.0117201029205870
0.999886924438943	-0.0117089348527644
0.999886278506327	-0.0116981554877088
0.999885641156213	-0.0116878132269187
0.999885203791572	-0.0116778356377272
0.999885100945052	-0.0116682526633235
0.999885370421852	-0.0116587336706826
0.999886018385204	-0.0116491297037769
0.999886937624145	-0.0116392836966683
0.999887974744933	-0.0116289587171492
0.999888964716909	-0.0116182753182011
0.999889756049540	-0.0116072642198837
0.999890218319031	-0.0115960715558178
0.999890305421205	-0.0115844551041329
0.999890011858419	-0.0115730178412559
0.999889411193912	-0.0115619126405233
0.999888706440423	-0.0115512335966739
0.999888112868634	-0.0115408089765451
0.999887796585844	-0.0115307247527989
0.999887880983923	-0.0115208604813935
0.999888391600281	-0.0115109803659736
0.999889197478090	-0.0115012906914312
0.999890191472107	-0.0114912837515937
0.999891231570146	-0.0114808939321310
0.999892120271968	-0.0114701639365510
0.999892701548222	-0.0114592901866225
0.999892911140721	-0.0114483479947306
0.999892723525943	-0.0114374905788619
0.999892232073472	-0.0114268911198640
0.999891598564022	-0.0114166154999636
0.999890974773661	-0.0114067429786042
0.999890514794817	-0.0113972599906089
0.999890364385647	-0.0113880285240621
0.999890588099581	-0.0113788089951947
0.999891177933833	-0.0113694966620663
0.999892077926668	-0.0113599474967906
0.999893115540182	-0.0113500560717570
0.999894123456433	-0.0113394221773971
0.999894900118409	-0.0113284696733023
0.999895311265060	-0.0113173032540261
0.999895304789150	-0.0113061438532589
0.999894948492896	-0.0112952940699127
0.999894353225596	-0.0112847934546442
0.999893659290716	-0.0112747327592882
0.999893088507305	-0.0112650855083384
0.999892828301667	-0.0112561278980664
0.999892920283438	-0.0112473021431206
0.999893399695523	-0.0112384644745924
0.999894190454853	-0.0112294395593857
0.999895142922015	-0.0112201099182557
0.999896115672980	-0.0112104320223265
0.999896960672910	-0.0112004090183927
0.999897529764400	-0.0111901562513220
0.999897749929690	-0.0111795548280669
0.999897590750634	-0.0111690514750765
0.999897094130268	-0.0111587994245534
0.999896427295416	-0.0111489197528756
0.999895780390820	-0.0111391934870049
0.999895332061110	-0.0111298406125463
0.999895222293302	-0.0111207720236562
0.999895521182172	-0.0111117716268805
0.999896177545456	-0.0111026833366872
0.999897092443358	-0.0110933112919229
0.999898134819332	-0.0110835583522107
0.999899085529137	-0.0110734305103804
0.999899743485626	-0.0110632923962205
0.999900046707823	-0.0110530329455805
0.999899947917785	-0.0110428007780212
0.999899517506028	-0.0110327839453214
0.999898913554482	-0.0110232058076258
0.999898275234959	-0.0110140167758576
0.999897753258819	-0.0110052213488910
0.999897504427860	-0.0109967027518875
0.999897611526754	-0.0109882756911264
0.999898082873449	-0.0109797995878116
0.999898881314280	-0.0109711300201404
0.999899854132236	-0.0109621465862902
0.999900836686465	-0.0109525366193310
0.999901642285124	-0.0109425962245062
0.999902132518565	-0.0109324077587255
0.999902231546193	-0.0109221697046044
0.999901962544683	-0.0109118179057364
0.999901406953572	-0.0109017834226817
0.999900694297488	-0.0108921788890168
0.999900060430903	-0.0108830067808895
0.999899723074718	-0.0108746059732408
0.999899728159731	-0.0108663686937218
0.999900125387384	-0.0108581532721560
0.999900852392599	-0.0108497729481083
0.999901753941605	-0.0108412025358005
0.999902700566313	-0.0108322896362642
0.999903546504464	-0.0108230270196858
0.999904137582506	-0.0108135185666488
0.999904390452070	-0.0108037084663103
0.999904269059303	-0.0107939677513741
0.999903804497580	-0.0107844480136544
0.999903151066838	-0.0107752777698989
0.999902492648179	-0.0107662983715751
0.999902002354903	-0.0107576919744531
0.999901821494838	-0.0107493817704192
0.999902032326394	-0.0107411654159538
0.999902615365173	-0.0107327087916347
0.999903481710181	-0.0107239834571098
0.999904506268444	-0.0107148806437542
0.999905462005353	-0.0107053910453434
0.999906130793189	-0.0106959136219656
0.999906450828679	-0.0106862968262108
0.999906367580364	-0.0106766877143984
0.999905944530316	-0.0106672805321567
0.999905342024346	-0.0106583675679250
0.999904694903671	-0.0106498365508818
0.999904152230713	-0.0106416962690158
0.999903872877704	-0.0106338354395277
0.999903943677506	-0.0106260787899776
0.999904376306119	-0.0106182809593968
0.999905137718086	-0.0106102980402982
0.999906079530668	-0.0106020070143786
0.999907037439089	-0.0105931269716826
0.999907828952144	-0.0105839151408078
0.999908315744837	-0.0105744493991289
0.999908418291624	-0.0105649237702503
0.999908152447584	-0.0105552283099729
0.999907593907124	-0.0105458418660158
0.999906869794469	-0.0105368800588016
0.999906218111316	-0.0105283502479538
0.999905861688024	-0.0105205677540387
0.999905846382923	-0.0105129500262586
0.999906223456251	-0.0105053555130113
0.999906931389113	-0.0104975955738206
0.999907812035206	-0.0104896592000264
0.999908737606908	-0.0104813801355592
0.999909562844080	-0.0104727509942615
0.999910133708473	-0.0104638757869743
0.999910366611995	-0.0104547275163481
0.999910228079714	-0.0104456478520902
0.999909749564063	-0.0104367871779003
0.999909085038364	-0.0104282728681260
0.999908417148636	-0.0104199569032040
0.999907918749957	-0.0104120090425169
0.999907730017613	-0.0104043519146756
0.999907931685204	-0.0103967834372312
0.999908502864538	-0.0103889770743844
0.999909353856333	-0.0103808985812893
0.999910359065252	-0.0103724404442139
0.999911291564366	-0.0103635955256014
0.999911934432689	-0.0103547584600090
0.999912228854572	-0.0103457849909540
0.999912122246909	-0.0103368218215063
0.999911679851623	-0.0103280615998208
0.999911062697945	-0.0103197789686818
0.999910405578848	-0.0103118755321184
0.999909857075989	-0.0103043581901750
0.999909574272736	-0.0102971142150742
0.999909641918218	-0.0102899562740941
0.999910070620961	-0.0102827503600642
0.999910825351893	-0.0102753527811128
0.999911755387631	-0.0102676423489926
0.999912695059410	-0.0102593530877212
0.999913461651399	-0.0102507327496151
0.999913917824379	-0.0102418617824755
0.999913987263024	-0.0102329370951701
0.999913691249943	-0.0102239197210177
0.999913111420882	-0.0102152133687821
0.999912376332055	-0.0102069295988585
0.999911721213700	-0.0101990709638421
0.999911363808780	-0.0101919015312759
0.999911348866917	-0.0101848885321660
0.999911724926132	-0.0101778900102272
0.999912427564199	-0.0101707193753235
0.999913298819632	-0.0101633464895504
0.999914208986879	-0.0101556284725166
0.999915012569312	-0.0101475602589842
0.999915556974674	-0.0101392488054991
0.999915760735437	-0.0101306842952197
0.999915594106220	-0.0101221937709052
0.999915091341118	-0.0101139269767886
0.999914409020826	-0.0101060086947128
0.999913729969728	-0.0100982925092580
0.999913228383406	-0.0100909401899545
0.999913043320936	-0.0100838710959096
0.999913251677589	-0.0100768803473088
0.999913824996422	-0.0100696799736878
0.999914670318358	-0.0100622004533111
0.999915660163609	-0.0100543376384311
0.999916569205044	-0.0100460895249458
0.999917184972079	-0.0100378372842468
0.999917451208963	-0.0100294540215682
0.999917318356998	-0.0100210864594695
0.999916854316873	-0.0100129246605503
0.999916219880275	-0.0100052133631855
0.999915550771824	-0.00999788026124680
0.999914995620877	-0.00999093003555713
0.999914709876734	-0.00998424796203329
0.999914776202023	-0.00997763525312223
0.999915204207164	-0.00997096764683657
0.999915956684055	-0.00996410118704436
0.999916880202121	-0.00995691621392993
0.999917807406998	-0.00994916060805040
0.999918554729020	-0.00994107334374609
0.999918985267703	-0.00993273753627022
0.999919025421106	-0.00992435325062986
0.999918701782313	-0.00991594339723047
0.999918101045839	-0.00990784685037739
0.999917353228958	-0.00990017196703681
0.999916691340842	-0.00989291746711975
0.999916329245453	-0.00988630216707187
0.999916311434278	-0.00987983755275297
0.999916684624708	-0.00987338106042632
0.999917382400081	-0.00986674732972100
0.999918247144628	-0.00985989020632560
0.999919147393718	-0.00985268489657017
0.999919937085849	-0.00984512766841657
0.999920464071740	-0.00983732743838922
0.999920647709868	-0.00982929148891468
0.999920460565276	-0.00982133188549197
0.999919938444666	-0.00981359831611522
0.999919239384504	-0.00980621449785655
0.999918546326363	-0.00979904135008399
0.999918034779020	-0.00979223050541626
0.999917843679476	-0.00978569960067143
0.999918048464591	-0.00977924226442100
0.999918617590838	-0.00977258639369631
0.999919456801363	-0.00976564696309593
0.999920437536664	-0.00975832068426153
0.999921334533341	-0.00975060736435974
0.999921936285785	-0.00974287680923437
0.999922187462438	-0.00973501538874095
0.999922039274407	-0.00972717000633267
0.999921560153846	-0.00971953018384368
0.999920910622387	-0.00971232659590451
0.999920226829240	-0.00970550100233339
0.999919657766195	-0.00969905780051187
0.999919359005137	-0.00969288217875055
0.999919413499787	-0.00968677150975002
0.999919831712891	-0.00968060457809086
0.999920576381629	-0.00967423656995425
0.999921493479464	-0.00966754711326048
0.999922414189100	-0.00966030113449579
0.999923154839860	-0.00965272005185827
0.999923577754439	-0.00964488700509363
0.999923608479357	-0.00963700272810394
0.999923273009725	-0.00962910726332608
0.999922658244721	-0.00962152387747686
0.999921894313499	-0.00961436165316664
0.999921214647209	-0.00960762050178588
0.999920834809028	-0.00960148962098963
0.999920800621086	-0.00959551117409898
0.999921159979079	-0.00958954194081488
0.999921847328191	-0.00958339514837659
0.999922704753912	-0.00957702048508017
0.999923600638133	-0.00957029458737300
0.999924388185058	-0.00956321253592993
0.999924913644993	-0.00955588253441913
0.999925094290703	-0.00954833218335282
0.999924902346758	-0.00954085340374300
0.999924372274472	-0.00953359646444014
0.999923660614930	-0.00952668691987291
0.999922949797228	-0.00952000392512630
0.999922415826612	-0.00951368538549361
0.999922198998253	-0.00950765069688499
0.999922377860203	-0.00950169527251489
0.999922927077349	-0.00949552554906428
0.999923755042542	-0.00948907313793947
0.999924733869336	-0.00948223098939951
0.999925635464884	-0.00947499460629868
0.999926046385503	-0.00947042050164125
0.999926327416249	-0.00946576913384925
0.999926458876323	-0.00946108035008604
0.999926437719896	-0.00945639921395294

==> matlab/fig2b1.tex <==
0.0100000000000000	5.50000000000000
0.0179621434110699	4.20919748141188
0.0259242868221399	3.56653288082458
0.0338864302332098	3.16213586182982
0.0418485736442798	2.87637111654315
0.0489549209391593	2.68062999996773
0.0560612682340389	2.52182011434379
0.0631676155289185	2.38930704450740
0.0702739628237981	2.27631787632041
0.0834365541784869	2.10418322829194
0.0965991455331757	1.96606545161415
0.109761736887865	1.85157617812902
0.122924328242553	1.75431909303519
0.141422220690948	1.63900330480190
0.159920113139343	1.54209594721224
0.178418005587737	1.45883387404364
0.196915898036132	1.38604475360330
0.219013608897574	1.30978130882642
0.241111319759016	1.24269212648435
0.263209030620457	1.18291006239169
0.285306741481899	1.12907532757127
0.309342274650222	1.07608873624875
0.333377807818544	1.02794246599341
0.357413340986866	0.983873343960361
0.381448874155189	0.943284392502180
0.406933021704955	0.903522472251584
0.432417169254721	0.866684369484525
0.457901316804488	0.832401279201136
0.483385464354254	0.800370574914646
0.510146684095585	0.768884856643038
0.536907903836916	0.739362944685296
0.563669123578246	0.711600386649122
0.590430343319577	0.685423779542160
0.618396556862693	0.659602556456129
0.646362770405808	0.635205926592251
0.674328983948924	0.612108276260884
0.702295197492039	0.590200474666364
0.731440138666079	0.568532575271896
0.760585079840118	0.547958499661165
0.789730021014158	0.528394741306906
0.818874962188198	0.509767409188196
0.849202310632316	0.491307893109781
0.879529659076434	0.473725066679367
0.909857007520552	0.456959806241135
0.940184355964671	0.440959031335030
0.971722764316052	0.425078777567975
1.00326117266743	0.409924818906819
1.03479958101881	0.395453042166773
1.06633798937020	0.381623371799261
1.09914059673297	0.367881307925551
1.13194320409574	0.354756696952370
1.16474581145851	0.342215103591973
1.19754841882128	0.330224935268263
1.23169524674606	0.318297900705334
1.26584207467084	0.306906584952110
1.29998890259562	0.296023007783774
1.33413573052039	0.285621286559211
1.36973897643827	0.275263107443933
1.40534222235615	0.265377299252756
1.44094546827402	0.255940284745894
1.47654871419190	0.246930104283630
1.51333148231955	0.238047920704175
1.55011425044721	0.229578204570971
1.58689701857486	0.221501092408479
1.62367978670251	0.213797966792341
1.66101214689026	0.206344170624311
1.69834450707800	0.199240316004585
1.73567686726574	0.192470126966199
1.77300922745348	0.186018255405710
1.81093729414381	0.179774469739622
1.84886536083414	0.173829813543198
1.88679342752446	0.168170605306819
1.92472149421479	0.162783883204341
1.96329948808217	0.157571685766164
2.00187748194955	0.152616306463997
2.04045547581692	0.147906006023135
2.07903346968430	0.143429624612299
2.11832628074299	0.139099763667190
2.15761909180168	0.134990796296898
2.19691190286036	0.131092483623309
2.23620471391905	0.127395069532872
2.27628788215811	0.123820622918079
2.31637105039716	0.120436069692456
2.35645421863622	0.117232365803445
2.39653738687527	0.114200882025363
2.43749810706159	0.111272363458639
2.47845882724791	0.108506632216615
2.51941954743422	0.105895624059600
2.56038026762054	0.103431641086591
2.60231930174224	0.101053456336798
2.64425833586394	0.0988141091537672
2.68619736998564	0.0967063617207625
2.72813640410734	0.0947233075327080
2.77117099359047	0.0928111528369770
2.81420558307360	0.0910165062514104
2.85724017255673	0.0893328458573555
2.90027476203986	0.0877539555284151
2.94454280820470	0.0862328805807473
2.98881085436955	0.0848102103513265
3.03307890053439	0.0834800587527969
3.07734694669924	0.0822368268145248
3.12301296380697	0.0810397697304898
3.16867898091470	0.0799239469995309
3.21434499802243	0.0788840504260850
3.26001101513015	0.0779150452770853
3.30727473639622	0.0769817023263758
3.35453845766229	0.0761141366034931
3.40180217892835	0.0753075763634403
3.44906590019442	0.0745575134347213
3.49817508767041	0.0738334410396675
3.54728427514641	0.0731612357887815
3.59639346262241	0.0725366336893928
3.64550265009840	0.0719556273412297
3.69677296104368	0.0713914920994657
3.74804327198896	0.0708667340983951
3.79931358293424	0.0703775787943864
3.85058389387952	0.0699205036085543
3.90443140626832	0.0694713967249623
3.95827891865712	0.0690504988683522
4.01212643104593	0.0686545159231696
4.06597394343473	0.0682804031761857
4.12210104024892	0.0679106988206407
4.17822813706310	0.0675587653136036
4.23435523387729	0.0672219112004397
4.29048233069147	0.0668976793716306
4.34732453072746	0.0665798912035757
4.40416673076345	0.0662706408812767
4.46100893079944	0.0659680180970256
4.51785113083543	0.0656703041037828
4.57582743647441	0.0653701118489335
4.63380374211339	0.0650719724175987
4.69178004775237	0.0647746004293369
4.74975635339135	0.0644768673596800
4.80927575174908	0.0641698056946520
4.86879515010681	0.0638604212598250
4.92831454846454	0.0635479430696866
4.98783394682227	0.0632317270548815
5.04934227097890	0.0629004608140687
5.11085059513554	0.0625641924285978
5.17235891929218	0.0622225818440118
5.23386724344882	0.0618753887275341
5.29789405007311	0.0615078931206277
5.36192085669741	0.0611341304121056
5.42594766332170	0.0607541254202819
5.48997446994599	0.0603679767747361
5.55719875822752	0.0599561175265155
5.62442304650904	0.0595379482748674
5.69164733479056	0.0591138047493851
5.75887162307208	0.0586840705458446
5.83023614825156	0.0582222315747967
5.90160067343103	0.0577551461183567
5.97296519861051	0.0572834163927090
6.04432972378998	0.0568076649106683
6.12127947749308	0.0562909115234403
6.19822923119618	0.0557710625177795
6.27517898489927	0.0552489521091002
6.35212873860237	0.0547254029580919
6.43723247735917	0.0541456790025885
6.52233621611597	0.0535662793369482
6.60743995487277	0.0529882533042400
6.69254369362957	0.0524125962562462
6.78171540330365	0.0518129949642556
6.87088711297772	0.0512180715626351
6.96005882265180	0.0506287870406994
7.04923053232588	0.0500460188540591
7.14466391282726	0.0494304534598205
7.24009729332864	0.0488241584844017
7.33553067383002	0.0482279163797953
7.43096405433140	0.0476424016970679
7.53934576535893	0.0469911792912276
7.64772747638647	0.0463552207027819
7.75610918741400	0.0457350574754762
7.86449089844153	0.0451310758263391
7.96911887225926	0.0445635995561623
8.07374684607698	0.0440115392147765
8.17837481989470	0.0434748969641361
8.28300279371242	0.0429535924284454
8.38717830981286	0.0424496211097546
8.49135382591330	0.0419604450068740
8.59552934201374	0.0414857560010373
8.69970485811419	0.0410252052508506
8.80416336793757	0.0405772050843963
8.90862187776095	0.0401425688395809
9.01308038758434	0.0397208164445773
9.11753889740773	0.0393114597857855
9.21807327203068	0.0389287184392134
9.31860764665363	0.0385565158679608
9.41914202127658	0.0381943772103275
9.51967639589953	0.0378418395452741
9.61962880891270	0.0375004078337787
9.71958122192588	0.0371675545398929
9.81953363493905	0.0368428353367688
9.91948604795222	0.0365258283613498
10.0207435189413	0.0362121306169668
10.1220009899305	0.0359055107922410
10.2232584609196	0.0356055713639248
10.3245159319087	0.0353119434154062
10.4283846120172	0.0350169376789248
10.5322532921256	0.0347278422244251
10.6361219722340	0.0344443184871696
10.7399906523424	0.0341660596151866
10.8475748287719	0.0338830971404269
10.9551590052014	0.0336051793697452
11.0627431816309	0.0333320340436580
11.1703273580604	0.0330634211444518
11.2826122346865	0.0327876731567521
11.3948971113127	0.0325163967102611
11.5071819879388	0.0322493878151740
11.6194668645650	0.0319864728294677
11.7372536318931	0.0317149105287759
11.8550403992212	0.0314475233406136
11.9728271665493	0.0311841708972652
12.0906139338774	0.0309247390139748
12.2143018181317	0.0306564252825630
12.3379897023860	0.0303922224389272
12.4616775866403	0.0301320410261429
12.5853654708946	0.0298758118398758
12.7146136383583	0.0296122255248785
12.8438618058221	0.0293528235365110
12.9731099732858	0.0290975467232463
13.1023581407496	0.0288463497396705
13.2358862805105	0.0285910777089016
13.3694144202714	0.0283400619343918
13.5029425600323	0.0280932499916806
13.6364706997933	0.0278505981946050
13.7724345754501	0.0276077509293712
13.9083984511069	0.0273691093826879
14.0443623267637	0.0271346106800006
14.1803262024205	0.0269041983746643
14.3171940356473	0.0266763234383825
14.4540618688741	0.0264524526126162
14.5909297021008	0.0262325076302781
14.7277975353276	0.0260164168609888
14.8649284638827	0.0258037037727586
15.0020593924377	0.0255946960716057
15.1391903209927	0.0253893044007071
15.2763212495477	0.0251874475071437
15.4138654423835	0.0249884526639113
15.5514096352193	0.0247928364486746
15.6889538280551	0.0246005057422698
15.8264980208909	0.0244113771647485
15.9650100243167	0.0242240725032700
16.1035220277425	0.0240398379178516
16.2420340311683	0.0238585830717125
16.3805460345941	0.0236802286122602
16.5206781669815	0.0235026629745634
16.6608102993689	0.0233278997248462
16.8009424317563	0.0231558557812612
16.9410745641437	0.0229864597112519
17.0834062487309	0.0228170471512063
17.2257379333181	0.0226502174676225
17.3680696179053	0.0224858970599302
17.5104013024924	0.0223240240694242
17.6553488510412	0.0221616329365872
17.8002963995899	0.0220016508678665
17.9452439481386	0.0218440139624096
18.0901914966873	0.0216886697004647
18.2379619557187	0.0215326108837828
18.3857324147501	0.0213788239620288
18.5335028737815	0.0212272534251383
18.6812733328129	0.0210778545164137
18.8318594722471	0.0209278012296702
18.9824456116813	0.0207799066510101
19.1330317511155	0.0206341215089130
19.2836178905498	0.0204904065986026
19.4368432212972	0.0203462613190471
19.5900685520447	0.0202041728759550
19.7432938827921	0.0200640960123445
19.8965192135396	0.0199259949651857
20.0521273153262	0.0197877350426975
20.2077354171128	0.0196514322091217
20.3633435188993	0.0195170435566546
20.5189516206859	0.0193845353010993
20.6767074948662	0.0192520859921111
20.8344633690465	0.0191214922452807
20.9922192432268	0.0189927126731413
21.1499751174070	0.0188657148375021
21.3097363309718	0.0187388882110434
21.4694975445366	0.0186138146014961
21.6292587581014	0.0184904540456381
21.7890199716662	0.0183687754815052
21.9507550228406	0.0182472780379325
22.1124900740149	0.0181274332485732
22.2742251251893	0.0180092028869424
22.4359601763636	0.0178925576215572
22.5997219235879	0.0177760386761317
22.7634836708122	0.0176610775591101
22.9272454180365	0.0175476381639504
23.0910071652607	0.0174356932512569
23.2568857402592	0.0173238000354599
23.4227643152578	0.0172133774779570
23.5886428902563	0.0171043918223005
23.7545214652548	0.0169968181011326
23.9225997668194	0.0168892354180600
24.0906780683841	0.0167830443808048
24.2587563699487	0.0166782135809125
24.4268346715134	0.0165747202731661
24.5971602465273	0.0164711872925188
24.7674858215413	0.0163689743011270
24.9378113965552	0.0162680520400976
25.1081369715692	0.0161683997610558
25.2807146345169	0.0160687067242173
25.4532922974645	0.0159702679089135
25.6258699604122	0.0158730559083139
25.7984476233598	0.0157770516716830
25.9732496005806	0.0156810245083505
26.1480515778014	0.0155861902067677
26.3228535550222	0.0154925229186225
26.4976555322430	0.0154000050138804
26.6746407580550	0.0153074871983535
26.8516259838669	0.0152161042377370
27.0286112096789	0.0151258316206796
27.2055964354908	0.0150366529394746
27.3847291106506	0.0149474919505643
27.5638617858103	0.0148594106648245
27.7429944609701	0.0147723857763146
27.9221271361299	0.0146864019876026
28.1033873526667	0.0146004436137968
28.2846475692035	0.0145155125775625
28.4659077857403	0.0144315867149892
28.6471680022771	0.0143486517863202
28.8305524749318	0.0142657413030460
29.0139369475864	0.0141838086929623
29.1973214202411	0.0141028329007587
29.3807058928957	0.0140228007134327
29.5662216026754	0.0139427875266630
29.7517373124551	0.0138637057321068
29.9372530222348	0.0137855353469629
30.1227687320145	0.0137082641468198
30.3104244405387	0.0136310063674082
30.4980801490630	0.0135546364224846
30.6857358575872	0.0134791353474201
30.8733915661115	0.0134044918495243
31.0631915046256	0.0133298586670540
31.2529914431398	0.0132560724838600
31.4427913816539	0.0131831152821844
31.6325913201681	0.0131109766293647
31.8245330634793	0.0130388481166236
32.0164748067905	0.0129675282175764
32.2084165501018	0.0128969997838576
32.4003582934130	0.0128272531676141
32.5944343723426	0.0127575184002655
32.7885104512723	0.0126885560447749
32.9825865302019	0.0126203497500417
33.1766626091316	0.0125528905848006
33.3728638888244	0.0124854453718436
33.5690651685172	0.0124187383438436
33.7652664482099	0.0123527538866725
33.9614677279027	0.0122874837294483
34.1597863981921	0.0122222289418527
34.3581050684815	0.0121576799444694
34.5564237387709	0.0120938218118816
34.7547424090604	0.0120306468885633
34.9551733102377	0.0119674877328050
35.1556042114151	0.0119050037072131
35.3560351125925	0.0118431805350023
35.5564660137699	0.0117820111380321
35.7590062381233	0.0117208571585427
35.9615464624766	0.0116603493025297
36.1640866868299	0.0116004739053845
36.3666269111833	0.0115412244312265
36.5712744813487	0.0114819897779630
36.7759220515142	0.0114233738090529
36.9805696216796	0.0113653634363731
37.1852171918451	0.0113079526316976
37.3919698016115	0.0112505561990636
37.5987224113779	0.0111937524833198
37.8054750211443	0.0111375289373451
38.0122276309107	0.0110818800063122
38.2210820628669	0.0110262452836582
38.4299364948231	0.0109711786816928
38.6387909267793	0.0109166681599761
38.8476453587355	0.0108627086042274
39.0585976322966	0.0108087632983672
39.2695499058576	0.0107553627924562
39.4805021794187	0.0107024955208019
39.6914544529798	0.0106501567793246
39.9045003567214	0.0105978323709845
40.1175462604631	0.0105460306322260
40.3305921642047	0.0104947404431765
40.5436380679464	0.0104439574825581
40.7587736492092	0.0103931888556021
40.9739092304720	0.0103429218847175
41.1890448117348	0.0102931458697649
41.4041803929976	0.0102438568475386
41.6214021542161	0.0101945820425062
41.8386239154346	0.0101457889320560
42.0558456766532	0.0100974672119175
42.2730674378717	0.0100496132542711
42.4923722413425	0.0100017733175546
42.7116770448134	0.00995439610607075
42.9309818482842	0.00990747168915757
43.1502866517551	0.00986099675318322
43.3716714967573	0.00981453562061903
43.5930563417596	0.00976851917880538
43.8144411867618	0.00972293784968653
44.0358260317640	0.00967778861383193
44.2592878797955	0.00963265298142886
44.4827497278270	0.00958794488506475
44.7062115758585	0.00954365507948251
44.9296734238900	0.00949978082064899
45.1552091541436	0.00945591998934625
45.3807448843971	0.00941247036693634
45.6062806146507	0.00936942302241311
45.8318163449043	0.00932677546958137
46.0594228148368	0.00928414117775516
46.2870292847694	0.00924190254670501
46.5146357547020	0.00920005094242354
46.7422422246345	0.00915858412025354
46.9719163573238	0.00911713038487860
47.2015904900131	0.00907605749651383
47.4312646227023	0.00903535710213331
47.6609387553916	0.00899502718350017
47.8926775894859	0.00895471016219705
48.1244164235803	0.00891475986726407
48.3561552576747	0.00887516821174218
48.5878940917691	0.00883593338974699
48.8216947775496	0.00879671126329461
49.0554954633302	0.00875784239729779
49.2892961491107	0.00871931895691359
49.5230968348912	0.00868113933546187
49.6423226261684	0.00866180208905524
49.7615484174456	0.00864255256829799
49.8807742087228	0.00862339009106573
50	0.00860431413996236

==> matlab/fig2b2.tex <==
0.0100000000000000	50.5000000000000
0.0148893961920471	34.0417010682050
0.0197787923840941	25.7126620785033
0.0246681885761412	20.6803898552010
0.0295575847681883	17.3095033384267
0.0344469809602354	14.8929612780769
0.0393363771522824	13.0751504632823
0.0442257733443295	11.6576669981654
0.0491151695363766	10.5210794069913
0.0566647429666537	9.14930735097196
0.0642143163969308	8.09809786741507
0.0717638898272080	7.26644791302980
0.0793134632574851	6.59178288604967
0.0908118553010885	5.77771558980006
0.102310247344692	5.14463570108425
0.113808639388295	4.63785236597986
0.125307031431899	4.22272223229550
0.141369341375589	3.75404014459130
0.157431651319280	3.37924374600277
0.173493961262971	3.07239797127158
0.189556271206662	2.81633756332145
0.209054765188173	2.55701133190537
0.228553259169684	2.34067659553905
0.248051753151195	2.15728726450073
0.267550247132706	1.99971421989122
0.290054092995263	1.84321905718143
0.312557938857820	1.70836533139467
0.335061784720377	1.59085339583646
0.357565630582934	1.48745950095603
0.382022894637376	1.38823835564004
0.406480158691819	1.30035005192157
0.430937422746262	1.22190371415659
0.455394686800704	1.15141122180441
0.481569771421338	1.08343739202783
0.507744856041972	1.02204812588953
0.533919940662606	0.966301340167471
0.560095025283240	0.915429082644672
0.587815541450838	0.866166645991008
0.615536057618436	0.821041615635355
0.643256573786034	0.779538071274957
0.670977089953632	0.741224140234018
0.700118255075150	0.703986881786985
0.729259420196668	0.669513898760849
0.758400585318186	0.637500854958395
0.787541750439704	0.607687671361789
0.818002822213866	0.578633414964923
0.848463893988028	0.551518345318279
0.878924965762190	0.526152024767152
0.909386037536352	0.502368989544706
0.941083529314273	0.479146287242974
0.972781021092195	0.457339091522966
1.00447851287012	0.436822366217893
1.03617600464804	0.417485982086585
1.06904120797423	0.398579605577637
1.10190641130043	0.380741200866412
1.13477161462662	0.363885298168576
1.16763681795282	0.347935750964894
1.20161504757622	0.332326633261515
1.23559327719962	0.317546125811156
1.26957150682302	0.303533743068867
1.30354973644643	0.290235066684988
1.33860026934466	0.277212579144352
1.37365080224289	0.264848544639132
1.40870133514113	0.253098826305177
1.44375186803936	0.241923374172552
1.47984820246859	0.230976254789684
1.51594453689782	0.220563242664777
1.55204087132705	0.210651224810293
1.58813720575629	0.201209926910916
1.62526753796055	0.191960100938811
1.66239787016482	0.183151249536905
1.69952820236909	0.174757885314282
1.73665853457335	0.166756548289620
1.77482648733532	0.158917462788714
1.81299444009729	0.151448016508124
1.85116239285926	0.144328113560212
1.88933034562123	0.137539144116302
1.92855606837490	0.130888689742406
1.96778179112857	0.124552089512718
2.00700751388225	0.118513131708328
2.04623323663592	0.112756721190249
2.08655507259207	0.107119143339169
2.12687690854821	0.101750938066578
2.16719874450436	0.0966387370965328
2.20752058046051	0.0917700317474066
2.24899759325488	0.0870035533159829
2.29047460604925	0.0824703212334536
2.33195161884362	0.0781590768359268
2.37342863163800	0.0740592396075613
2.41614443981355	0.0700474117676047
2.45886024798911	0.0662389754709356
2.50157605616466	0.0626242537907351
2.54429186434021	0.0591941185096956
2.58836050906038	0.0558396636153239
2.63242915378054	0.0526635213571432
2.67649779850070	0.0496572090133460
2.72056644322086	0.0468126998915835
2.76614153781910	0.0440330564512991
2.81171663241733	0.0414103365729231
2.85729172701556	0.0389369605552689
2.90286682161380	0.0366057388393621
2.94925709579494	0.0343717541949533
2.99564736997608	0.0322711139865063
3.04203764415721	0.0302972930080314
3.08842791833835	0.0284440858689558
3.13504806192754	0.0266972428381312
3.18166820551672	0.0250605113110763
3.22828834910590	0.0235284281541775
3.27490849269509	0.0220957852697385
3.32184817451336	0.0207487528471091
3.36878785633164	0.0194926287833066
3.41572753814992	0.0183227728043189
3.46266721996820	0.0172347543439906
3.51002497981212	0.0162156738494471
3.55738273965604	0.0152714128834341
3.60474049949997	0.0143979848815343
3.65209825934389	0.0135915806624432
3.69997786202684	0.0128407081028451
3.74785746470979	0.0121510073863393
3.79573706739275	0.0115190249660274
3.84361667007570	0.0109414611862064
3.89212998835124	0.0104085236841844
3.94064330662678	0.00992506630666681
3.98915662490232	0.00948808092754737
4.03766994317786	0.00909469595365566
4.08694045495193	0.00873697454359658
4.13621096672600	0.00841864125663777
4.18548147850007	0.00813706893314975
4.23475199027414	0.00788975393202778
4.28491921268052	0.00767066782168317
4.33508643508690	0.00748221143861659
4.38525365749328	0.00732209070147199
4.43542087989966	0.00718812516459663
4.48664627573137	0.00707616767950493
4.53787167156309	0.00698721312036013
4.58909706739480	0.00691926475663036
4.64032246322651	0.00687043190650939
4.69279768899344	0.00683835633910370
4.74527291476036	0.00682263266774106
4.79774814052728	0.00682153498939496
4.85022336629421	0.00683343757499742
4.90418235407362	0.00685762160201547
4.95814134185303	0.00689235992987801
5.01210032963244	0.00693617822987155
5.06605931741185	0.00698769777542029
5.12179691896912	0.00704763388197611
5.17753452052639	0.00711308181785641
5.23327212208366	0.00718280571205038
5.28900972364093	0.00725566174436460
5.34691229243864	0.00733353080206277
5.40481486123634	0.00741254225437547
5.46271743003406	0.00749169133708842
5.52061999883177	0.00757006262522564
5.58121953325118	0.00765034735763796
5.64181906767059	0.00772800421257310
5.70241860209001	0.00780225856736394
5.76301813650942	0.00787242318550355
5.82511460237858	0.00793944521034904
5.88721106824774	0.00800096527358718
5.94930753411689	0.00805649150613210
6.01140399998605	0.00810560828308978
6.07380159490291	0.00814815928429811
6.13619918981976	0.00818360604635238
6.19859678473662	0.00821172723338620
6.26099437965347	0.00823236091066139
6.32419436949673	0.00824551824154204
6.38739435933999	0.00825082673658510
6.45059434918325	0.00824827747234270
6.51379433902651	0.00823790713968965
6.57830719489551	0.00821933716724523
6.64282005076451	0.00819282620236398
6.70733290663351	0.00815853733029633
6.77184576250251	0.00811666718609719
6.83824117080171	0.00806589908706778
6.90463657910091	0.00800762207503300
6.97103198740010	0.00794214211603316
7.03742739569930	0.00786978742322476
7.10642156558373	0.00778769138261173
7.17541573546816	0.00769896155650582
7.24440990535259	0.00760402579092524
7.31340407523702	0.00750332278981692
7.38600948734619	0.00739161359109379
7.45861489945535	0.00727454808838119
7.53122031156452	0.00715266260239337
7.60382572367369	0.00702649174345890
7.68169060479945	0.00688702469563145
7.75955548592521	0.00674389650737305
7.83742036705097	0.00659774953718449
7.91528524817673	0.00644920857850112
7.99490567291899	0.00629547636757717
8.07452609766125	0.00614051112484699
8.15414652240351	0.00598492054084117
8.23376694714577	0.00582928206803483
8.31391886159019	0.00567311212180417
8.39407077603461	0.00551798457424892
8.47422269047904	0.00536439919572318
8.55437460492346	0.00521281904885734
8.63687721049298	0.00505933965500611
8.71937981606250	0.00490887259266528
8.80188242163202	0.00476180999620975
8.88438502720155	0.00461850164278836
8.97139686058978	0.00447177023652781
9.05840869397802	0.00432988074719675
9.14542052736626	0.00419310537893547
9.23243236075449	0.00406166776910105
9.32093858739016	0.00393363332894604
9.40944481402583	0.00381145141700154
9.49795104066150	0.00369522142291302
9.58645726729716	0.00358499939996793
9.67248667547180	0.00348363579181844
9.75851608364644	0.00338794546360420
9.84454549182108	0.00329787810301678
9.93057489999572	0.00321335453582887
10.0166970837528	0.00313418663880090
10.1028192675098	0.00306033661153437
10.1889414512669	0.00299165072850000
10.2750636350240	0.00292795651447362
10.3632012635051	0.00286774194763897
10.4513388919862	0.00281233421980086
10.5394765204673	0.00276149762814921
10.6276141489484	0.00271498670892690
10.7197494921261	0.00267071449982972
10.8118848353039	0.00263058848627566
10.9040201784817	0.00259430168724237
10.9961555216594	0.00256154704614023
11.0865603570731	0.00253254409412969
11.1769651924869	0.00250635310726003
11.2673700279006	0.00248268631280200
11.3577748633143	0.00246126414540530
11.4470969932176	0.00244203670572826
11.5364191231210	0.00242447633106488
11.6257412530243	0.00240833544967022
11.7150633829276	0.00239337950146073
11.8051167656774	0.00237927453030842
11.8951701484272	0.00236592820724355
11.9852235311770	0.00235313583285804
12.0752769139267	0.00234070898286571
12.1675783486168	0.00232816959778119
12.2598797833068	0.00231565740670166
12.3521812179968	0.00230301550283197
12.4444826526868	0.00229010558782738
12.5406946243167	0.00227623243250815
12.6369065959466	0.00226181409847139
12.7331185675765	0.00224674819536857
12.8293305392064	0.00223095254839435
12.9317611576690	0.00221326220700661
13.0341917761316	0.00219461293948176
13.1366223945942	0.00217496669843211
13.2390530130568	0.00215430653425484
13.3436694630454	0.00213216042761313
13.4482859130340	0.00210897550024663
13.5529023630227	0.00208478583228249
13.6575188130113	0.00205964115897952
13.7639378760502	0.00203314846824758
13.8703569390891	0.00200581026227905
13.9767760021280	0.00197771412254268
14.0831950651669	0.00194895615379466
14.1948918891323	0.00191817261235700
14.3065887130976	0.00188689820551532
14.4182855370630	0.00185526105539976
14.5299823610283	0.00182339054567986
14.6523445390369	0.00178836218055046
14.7747067170456	0.00175337786300566
14.8970688950542	0.00171860037450741
15.0194310730629	0.00168418387431623
15.1511465632349	0.00164770602020323
15.2828620534069	0.00161198347502042
15.4145775435789	0.00157716757271374
15.5462930337509	0.00154338974964756
15.6816426907559	0.00150987973254800
15.8169923477609	0.00147768728162422
15.9523420047659	0.00144689157703550
16.0876916617709	0.00141754833106347
16.2195694981085	0.00139038781528192
16.3514473344461	0.00136465224202659
16.4833251707836	0.00134033668646711
16.6152030071212	0.00131741982360762
16.7409056818706	0.00129684510024694
16.8666083566200	0.00127746460318373
16.9923110313695	0.00125922485782425
17.1180137061189	0.00124206494777484
17.2460071843381	0.00122563191931612
17.3740006625573	0.00121016845918371
17.5019941407765	0.00119559087177442
17.6299876189957	0.00118181422206799
17.7565892512773	0.00116889081971332
17.8831908835589	0.00115658006343251
18.0097925158406	0.00114479722053440
18.1363941481222	0.00113346167473528
18.2599448561665	0.00112275667198115
18.3834955642107	0.00111233315513207
18.5070462722549	0.00110212536939103
18.6305969802992	0.00109207418889236
18.7553803779988	0.00108202721400442
18.8801637756984	0.00107203363504586
19.0049471733980	0.00106204861202595
19.1297305710976	0.00105203524331366
19.2592552219338	0.00104157914719604
19.3887798727700	0.00103103111568283
19.5183045236062	0.00102037008480707
19.6478291744424	0.00100958340604006
19.7861929856835	0.000997915457405533
19.9245567969247	0.000986096236758126
20.0629206081659	0.000974132087880943
20.2012844194070	0.000962037237657742
20.3511564871112	0.000948812568161169
20.5010285548154	0.000935488646603779
20.6509006225196	0.000922101239445910
20.8007726902238	0.000908691083066037
20.9588361116552	0.000894571575453118
21.1168995330866	0.000880527111168840
21.2749629545180	0.000866609533778640
21.4330263759494	0.000852869714468595
21.6190635682705	0.000836991601196404
21.8051007605917	0.000821498907175972
21.9911379529128	0.000806454075651978
22.1771751452340	0.000791908595449925
22.3458199885345	0.000779188569790446
22.5144648318351	0.000766933168217402
22.6831096751357	0.000755154748760185
22.8517545184363	0.000743857628596231
23.0203993617369	0.000733038763625739
23.1890442050374	0.000722686617367218
23.3576890483380	0.000712783267335374
23.5263338916386	0.000703306064977376
23.6920944741673	0.000694380164459560
23.8578550566961	0.000685808801843010
24.0236156392249	0.000677558739715562
24.1893762217536	0.000669596700116219
24.3482102075099	0.000662206514645281
24.5070441932662	0.000655018209593394
24.6658781790225	0.000648001467749084
24.8247121647788	0.000641128884205731
24.9797169326094	0.000634536839322821
25.1347217004401	0.000628034568464206
25.2897264682707	0.000621601558386181
25.4447312361014	0.000615221236078219
25.6022628713019	0.000608776967052045
25.7597945065025	0.000602359988225461
25.9173261417030	0.000595960653600374
26.0748577769036	0.000589573490746571
26.2399748574646	0.000582889323350141
26.4050919380255	0.000576214552828770
26.5702090185865	0.000569551040644484
26.7353260991475	0.000562904307189175
26.9135866885254	0.000555756574200366
27.0918472779033	0.000548648275563132
27.2701078672812	0.000541591954493199
27.4483684566591	0.000534602278167898
27.6461875512081	0.000526942551861039
27.8440066457571	0.000519403257003956
28.0418257403061	0.000512002787404768
28.2396448348551	0.000504758698164476
28.4582261869192	0.000496954933621816
28.6768075389832	0.000489376134565072
28.8953888910472	0.000482032601257737
29.1139702431113	0.000474930538774752
29.3320751105215	0.000468086555561179
29.5501799779317	0.000461479728646944
29.7682848453419	0.000455100842984758
29.9863897127521	0.000448938360096962
30.1847014566922	0.000443511282195221
30.3830132006322	0.000438237474559702
30.5813249445722	0.000433102209274378
30.7796366885122	0.000428091698551478
30.9653208272272	0.000423501450554257
31.1510049659422	0.000418996344571394
31.3366891046572	0.000414564997891114
31.5223732433722	0.000410198116878077
31.7057580297484	0.000405940881679752
31.8891428161245	0.000401730745180310
32.0725276025007	0.000397561305696550
32.2559123888769	0.000393428544261209
32.4435767931044	0.000389234816799492
32.6312411973319	0.000385074226004737
32.8189056015594	0.000380945668417679
33.0065700057869	0.000376850197571003
33.2035317736837	0.000372590030702007
33.4004935415806	0.000368371171445198
33.5974553094774	0.000364196916241677
33.7944170773742	0.000360071984321251
34.0042348370502	0.000355738040654536
34.2140525967261	0.000351471013830063
34.4238703564021	0.000347275772893273
34.6336881160780	0.000343157482701758
34.8550217447865	0.000338901813163765
35.0763553734949	0.000334739935298688
35.2976890022033	0.000330673605191865
35.5190226309117	0.000326704044516037
35.7420476120856	0.000322802299625405
35.9650725932595	0.000318996344292892
36.1880975744334	0.000315282447533848
36.4111225556072	0.000311656790806567
36.6266455989052	0.000308232945247465
36.8421686422032	0.000304881588812206
37.0576916855012	0.000301596742111486
37.2732147287991	0.000298373330392824
37.4822671682508	0.000295301004584193
37.6913196077025	0.000292276640249340
37.9003720471542	0.000289295445614509
38.1094244866059	0.000286354051585624
38.3178434323715	0.000283458697322469
38.5262623781370	0.000280597131262811
38.7346813239026	0.000277766993559718
38.9431002696682	0.000274967406858238
39.1562974204122	0.000272135243243924
39.3694945711562	0.000269334281167380
39.5826917219003	0.000266564523263487
39.7958888726443	0.000263827181352055
40.0176196036804	0.000261016599247134
40.2393503347166	0.000258243977899836
40.4610810657527	0.000255510580414186
40.6828117967889	0.000252818384452530
40.9137026787675	0.000250061053207010
41.1445935607461	0.000247351532048267
41.3754844427247	0.000244690453600470
41.6063753247033	0.000242078725099297
41.8420837151137	0.000239464183033314
42.0777921055241	0.000236900799896634
42.3135004959345	0.000234387192227939
42.5492088863449	0.000231922258094818
42.7832701060807	0.000229521560349918
43.0173313258165	0.000227164959012158
43.2513925455524	0.000224849692091567
43.4854537652882	0.000222573670371430
43.7158897201435	0.000220369491674047
43.9463256749988	0.000218198714424702
44.1767616298541	0.000216058802425064
44.4071975847094	0.000213948197635388
44.6370374295381	0.000211871226444052
44.8668772743667	0.000209820463128766
45.0967171191954	0.000207794490214043
45.3265569640240	0.000205792912463081
45.5600731725287	0.000203784456013014
45.7935893810333	0.000201800610308670
46.0271055895379	0.000199841074173508
46.2606217980426	0.000197906401741065
46.5007803538022	0.000195943618948877
46.7409389095619	0.000194008100489908
46.9810974653215	0.000192100004130579
47.2212560210812	0.000190220078064080
47.4680943172735	0.000188318184617745
47.7149326134659	0.000186446759662484
47.9617709096582	0.000184605507102157
48.2086092058506	0.000182794545140678
48.4587788964316	0.000180990238785690
48.7089485870126	0.000179216125982097
48.9591182775936	0.000177471047076022
49.2092879681746	0.000175754316536961
49.4069659761309	0.000174417444605723
49.6046439840873	0.000173097065833524
49.8023219920436	0.000171792477550956
50	0.000170503192743148

==> matlab/fig2b3.tex <==
0.0100000000000000	500.500000000000
0.0117160547237387	394.726789511777
0.0134321094474774	321.600771888221
0.0151481641712160	268.570488133953
0.0168642188949547	228.672519866279
0.0185802736186934	197.765421517909
0.0202963283424321	173.247764200022
0.0220123830661707	153.411788856764
0.0237284377899094	137.094861706957
0.0271767298921404	111.882220336383
0.0306250219943713	93.5565914395464
0.0340733140966023	79.7442791779936
0.0375216061988333	69.0288846019398
0.0427139279135350	56.8586592235442
0.0479062496282368	47.8915957390141
0.0530985713429385	41.0599490784515
0.0582908930576403	35.7136927343729
0.0666867029016913	29.2068379360460
0.0750825127457423	24.4644893075339
0.0834783225897933	20.8822498553968
0.0918741324338443	18.0981174764043
0.103221374695157	15.2104092688645
0.114568616956470	13.0182420423185
0.125915859217783	11.3075445788166
0.137263101479095	9.94210513830443
0.152303542411290	8.51412134807373
0.167343983343484	7.39864572591351
0.182384424275678	6.50750385282107
0.197424865207872	5.78212665050403
0.216556218911177	5.03684602649550
0.235687572614481	4.43892159080566
0.254818926317785	3.95044565167167
0.273950280021090	3.54519611706545
0.295702700579699	3.16206903931381
0.317455121138309	2.84291489243064
0.339207541696919	2.57364760023046
0.360959962255528	2.34393684575615
0.384856456254013	2.12803490984078
0.408752950252498	1.94285783273496
0.432649444250983	1.78257212701169
0.456545938249468	1.64269755508734
0.482428909122220	1.51019210104960
0.508311879994973	1.39407173830139
0.534194850867725	1.29160718794301
0.560077821740478	1.20062877690249
0.587789573063889	1.11398217620106
0.615501324387300	1.03677927578347
0.643213075710712	0.967622493609396
0.670924827034123	0.905370522238535
0.700315973473582	0.845845655058413
0.729707119913042	0.792104727573507
0.759098266352501	0.743379849320145
0.788489412791960	0.699030235724164
0.819413129909566	0.656501231064054
0.850336847027172	0.617691703918156
0.881260564144777	0.582155367526817
0.912184281262383	0.549513113146727
0.944496310546559	0.518146617809302
0.976808339830736	0.489270084305724
1.00912036911491	0.462611956549264
1.04143239839909	0.437938071804836
1.07499283168995	0.414194312138072
1.10855326498080	0.392174962141828
1.14211369827166	0.371708317939662
1.17567413156251	0.352644408750998
1.21035017643711	0.334280689482755
1.24502622131171	0.317146697952991
1.27970226618631	0.301130235782443
1.31437831106091	0.286132209387128
1.35004735827022	0.271674858212865
1.38571640547953	0.258117356138394
1.42138545268884	0.245384241281476
1.45705449989815	0.233408210948932
1.49360694715890	0.221858082145190
1.53015939441965	0.210981751591759
1.56671184168041	0.200727132575821
1.60326428894116	0.191047364949820
1.64060574378950	0.181708314993402
1.67794719863784	0.172884399680846
1.71528865348618	0.164538800822273
1.75263010833452	0.156638135516063
1.79068279737963	0.149013321313110
1.82873548642474	0.141789849699481
1.86678817546984	0.134941108897578
1.90484086451495	0.128442799152272
1.94354426897741	0.122169910083603
1.98224767343986	0.116215125327094
2.02095107790232	0.110558798094824
2.05965448236477	0.105182872404339
2.09896535948022	0.0999925073946368
2.13827623659567	0.0950582273896903
2.17758711371112	0.0903652283478241
2.21689799082656	0.0858998239050274
2.25679001376257	0.0815880587408723
2.29668203669857	0.0774853579511580
2.33657405963457	0.0735803427669015
2.37646608257057	0.0698624355591042
2.41692934917714	0.0662723327108927
2.45739261578371	0.0628550467863610
2.49785588239028	0.0596016602220459
2.53831914899685	0.0565038409741858
2.57935979595430	0.0535127353014854
2.62040044291174	0.0506660521251177
2.66144108986919	0.0479566683600047
2.70248173682663	0.0453778971348736
2.74412187579687	0.0428884955698076
2.78576201476712	0.0405209254889687
2.82740215373736	0.0382693899604098
2.86904229270760	0.0361284233449017
2.91132048022032	0.0340624736366070
2.95359866773304	0.0321001087112838
2.99587685524576	0.0302365239489649
3.03815504275849	0.0284671713384469
3.08112752419896	0.0267608926150180
3.12410000563943	0.0251432439044092
3.16707248707990	0.0236101715187852
3.21004496852037	0.0221578246560318
3.25378802052889	0.0207585660386368
3.29753107253741	0.0194355063029238
3.34127412454594	0.0181851656776947
3.38501717655446	0.0170042283461699
3.42963104837956	0.0158679964726913
3.47424492020467	0.0147974887090508
3.51885879202977	0.0137896674357685
3.56347266385488	0.0128416306993715
3.60908796232704	0.0119312408381439
3.65470326079919	0.0110776333661981
3.70031855927135	0.0102781130338620
3.74593385774351	0.00953009980681723
3.79272190093334	0.00881378104127426
3.83950994412316	0.00814651703486354
3.88629798731299	0.00752587763037415
3.93308603050281	0.00694953339127829
3.98127611499785	0.00639987030453927
4.02946619949289	0.00589250607631378
4.07765628398793	0.00542521373779880
4.12584636848297	0.00499585729405643
4.17453782062043	0.00459847893692844
4.22322927275788	0.00423572715398745
4.27192072489534	0.00390567083971542
4.32061217703279	0.00360645647877302
4.36915150529233	0.00333710850124808
4.41769083355186	0.00309496461059209
4.46623016181140	0.00287841259049515
4.51476949007093	0.00268590425430304
4.56328105147248	0.00251604664297757
4.61179261287403	0.00236730779411395
4.66030417427557	0.00223833018237245
4.70881573567712	0.00212781064886686
4.75743034626171	0.00203431995007880
4.80604495684629	0.00195691266153594
4.85465956743088	0.00189443930760344
4.90327417801546	0.00184579775922898
4.95214759150491	0.00180977502329283
5.00102100499435	0.00178564504056162
5.04989441848379	0.00177243106677827
5.09876783197324	0.00176919856940002
5.14804659394740	0.00177513974095298
5.19732535592155	0.00178945275136376
5.24660411789571	0.00181130860974940
5.29588287986987	0.00183991666758344
5.34571691623879	0.00187494631260719
5.39555095260772	0.00191537589881665
5.44538498897664	0.00196050601194799
5.49521902534556	0.00200967258516591
5.54578533292858	0.00206304208885901
5.59635164051159	0.00211930245742036
5.64691794809460	0.00217786997761906
5.69748425567761	0.00223819393893320
5.74900092501619	0.00230092255932847
5.80051759435478	0.00236442626266523
5.85203426369337	0.00242822654630807
5.90355093303196	0.00249187606948407
5.95629904554016	0.00255645654373820
6.00904715804837	0.00262003106483991
6.06179527055658	0.00268221876357652
6.11454338306479	0.00274266850818842
6.16890437576226	0.00280280878376606
6.22326536845974	0.00286044421251817
6.27762636115721	0.00291528687328972
6.33198735385468	0.00296707753995215
6.38842448996247	0.00301737047353977
6.44486162607025	0.00306390109634435
6.50129876217804	0.00310647414383926
6.55773589828582	0.00314492224428785
6.61342964774346	0.00317868403414728
6.66912339720110	0.00320818622077786
6.72481714665874	0.00323334468946263
6.78051089611637	0.00325409689414486
6.83589971047198	0.00327032489799911
6.89128852482759	0.00328213583452852
6.94667733918320	0.00328952893618396
7.00206615353882	0.00329252011769647
7.05758976165192	0.00329113352163990
7.11311336976503	0.00328540695276325
7.16863697787814	0.00327540459529885
7.22416058599125	0.00326120335159563
7.28021693986213	0.00324269781932205
7.33627329373302	0.00322011045633073
7.39232964760390	0.00319355792081316
7.44838600147478	0.00316316613385352
7.50538574262213	0.00312846592096529
7.56238548376949	0.00309008957360315
7.61938522491684	0.00304819742933259
7.67638496606419	0.00300295587187072
7.73480587272738	0.00295329148402646
7.79322677939057	0.00290048422660389
7.85164768605376	0.00284473199591995
7.91006859271695	0.00278623552770502
7.97053387043690	0.00272301957053029
8.03099914815685	0.00265731397600303
8.09146442587680	0.00258935051663366
8.15192970359676	0.00251936033895006
8.21535952756943	0.00244401299623591
8.27878935154210	0.00236695858575249
8.34221917551477	0.00228846222034633
8.40564899948744	0.00220878421493496
8.46793784799597	0.00212963788248422
8.53022669650450	0.00204984084830760
8.59251554501303	0.00196962776652146
8.65480439352156	0.00188922592419646
8.71642204054983	0.00180972154566120
8.77803968757810	0.00173045848922929
8.83965733460636	0.00165163797386404
8.90127498163463	0.00157345220445875
8.96300495617631	0.00149594537970533
9.02473493071799	0.00141943978201054
9.08646490525967	0.00134410464295597
9.14819487980135	0.00127009887686400
9.21071927424122	0.00119664919644020
9.27324366868109	0.00112486485770146
9.33576806312096	0.00105488254299274
9.39829245756083	0.000986827474501441
9.46233592838314	0.000919237179541030
9.52637939920544	0.000853903992996803
9.59042287002774	0.000790929882124860
9.65446634085004	0.000730404242161105
9.72096019267431	0.000670237309585468
9.78745404449858	0.000612870915482837
9.85394789632285	0.000558368050198807
9.92044174814712	0.000506777897846736
9.98759919027086	0.000457667031793959
10.0547566323946	0.000411592550000062
10.1219140745184	0.000368568804540975
10.1890715166421	0.000328597336813745
10.2546642923364	0.000292494421229438
10.3202570680308	0.000259276294652122
10.3858498437251	0.000228914933659708
10.4514426194195	0.000201372528041414
10.5165140917340	0.000176788843331036
10.5815855640486	0.000154881661733815
10.6466570363632	0.000135590743436558
10.7117285086778	0.000118848406770581
10.7771443606203	0.000104511541145121
10.8425602125627	9.25947467124406e-05
10.9079760645052	8.30112860650872e-05
10.9733919164476	7.56690199156130e-05
11.0399477645340	7.03991804032052e-05
11.1065036126204	6.72436232796153e-05
11.1730594607068	6.60925370344350e-05
11.2396153087932	6.68327000947779e-05
11.3082257087532	6.94529490017034e-05
11.3768361087133	7.38308244516194e-05
11.4454465086734	7.98351249259500e-05
11.5140569086335	8.73334015445340e-05
11.5852093098832	9.65453487832684e-05
11.6563617111329	0.000107072576210234
11.7275141123826	0.000118766979430665
11.7986665136323	0.000131481793250244
11.8677850418193	0.000144672886654719
11.9369035700062	0.000158559329565378
12.0060220981931	0.000173012714053848
12.0751406263801	0.000187907859958646
12.1433601380698	0.000202923704386643
12.2115796497596	0.000218137786571113
12.2797991614493	0.000233440397527891
12.3480186731391	0.000248726332174544
12.4163461472746	0.000263918919849513
12.4846736214100	0.000278897375667257
12.5530010955455	0.000293570177055417
12.6213285696809	0.000307851306472923
12.6907216414633	0.000321871509815004
12.7601147132457	0.000335325967861718
12.8295077850280	0.000348141911686579
12.8989008568104	0.000360252972002453
12.9703478268833	0.000371922721114178
13.0417947969561	0.000382722693474613
13.1132417670290	0.000392600899667874
13.1846887371018	0.000401512617786782
13.2595560962437	0.000409773057659555
13.3344234553855	0.000416895525302760
13.4092908145273	0.000422852541526347
13.4841581736692	0.000427624863238367
13.5575412493262	0.000431141965289926
13.6309243249833	0.000433506202303470
13.7043074006403	0.000434720346834440
13.7776904762973	0.000434793733809481
13.8500672006557	0.000433763961456320
13.9224439250142	0.000431660297575821
13.9948206493726	0.000428508384716524
14.0671973737310	0.000424338786028729
14.1398455416426	0.000419165666068136
14.2124937095543	0.000413042912340281
14.2851418774659	0.000406014400325066
14.3577900453776	0.000398127511199886
14.4318616952425	0.000389254901742439
14.5059333451073	0.000379599847161170
14.5800049949722	0.000369221884876112
14.6540766448371	0.000358182641763449
14.7309274464065	0.000346098329664187
14.8077782479759	0.000333443873726571
14.8846290495453	0.000320293320272394
14.9614798511146	0.000306721179234653
15.0406722118752	0.000292373649774883
15.1198645726358	0.000277740548323570
15.1990569333964	0.000262903289084954
15.2782492941569	0.000247941769706289
15.3552187760152	0.000233355670798224
15.4321882578735	0.000218797261352829
15.5091577397318	0.000204334924328508
15.5861272215900	0.000190034216912837
15.6625824441176	0.000176051239800899
15.7390376666451	0.000162349192042264
15.8154928891726	0.000148983883252882
15.8919481117002	0.000136007371301178
15.9693961674172	0.000123308472423677
16.0468442231342	0.000111105542408343
16.1242922788512	9.94413189812581e-05
16.2017403345682	8.83539886076145e-05
16.2817277574867	7.75447086661461e-05
16.3617151804052	6.74201062550796e-05
16.4417026033237	5.80079522661961e-05
16.5216900262422	4.93306706329225e-05
16.6043553465212	4.11536281780700e-05
16.6870206668002	3.37944459951745e-05
16.7696859870792	2.72615175622759e-05
16.8523513073581	2.15575267142560e-05
16.9322086407103	1.68321739266503e-05
17.0120659740625	1.28716076419798e-05
17.0919233074148	9.66484594700130e-06
17.1717806407670	7.19670585373666e-06
17.2507845102887	5.46317889863192e-06
17.3297883798104	4.41224900256514e-06
17.4087922493321	4.01877589971570e-06
17.4877961188537	4.25459375013698e-06
17.5676116379811	5.10041795619610e-06
17.6474271571085	6.52261182090365e-06
17.7272426762358	8.48436908639701e-06
17.8070581953632	1.09469363922267e-05
17.8893023304811	1.39656246636507e-05
17.9715464655990	1.74271609057983e-05
18.0537906007169	2.12842562294580e-05
18.1360347358348	2.54888646413987e-05
18.2213159234312	3.01638244210203e-05
18.3065971110275	3.51054131642005e-05
18.3918782986238	4.02589105540086e-05
18.4771594862202	4.55703371565284e-05
18.5595094175750	5.07992647103347e-05
18.6418593489297	5.60787141956657e-05
18.7242092802845	6.13627965168324e-05
18.8065592116393	6.66074201999155e-05
18.8880422520689	7.17165406954825e-05
18.9695252924985	7.67062019660157e-05
19.0510083329281	8.15391110270152e-05
19.1324913733577	8.61804978249796e-05
19.2148776329082	9.06456719061390e-05
19.2972638924588	9.48509221354555e-05
19.3796501520093	9.87679534584045e-05
19.4620364115598	0.000102371608584761
19.5470683095882	0.000105738925628151
19.6321002076166	0.000108727510736563
19.7171321056450	0.000111319498628099
19.8021640036734	0.000113500761220913
19.8908893408643	0.000115327497074465
19.9796146780552	0.000116687174038039
20.0683400152462	0.000117575394475534
20.1570653524371	0.000117991923718481
20.2428390648805	0.000117949588120032
20.3286127773240	0.000117476118076836
20.4143864897674	0.000116580841433459
20.5001602022109	0.000115276085304873
20.5852635054960	0.000113591728012570
20.6703668087812	0.000111536286072391
20.7554701120663	0.000109129084453426
20.8405734153514	0.000106391526281296
20.9270705233463	0.000103294634693986
21.0135676313412	9.99068046224423e-05
21.1000647393361	9.62556491945858e-05
21.1865618473310	9.23699847694755e-05
21.2766604059527	8.81053875424937e-05
21.3667589645743	8.36535868402887e-05
21.4568575231959	7.90498025288859e-05
21.5469560818176	7.43294274790508e-05
21.6381292498009	6.94703118625464e-05
21.7293024177842	6.45648621062862e-05
21.8204755857675	5.96490224286142e-05
21.9116487537508	5.47577065213711e-05
22.0004127698935	5.00514707181187e-05
22.0891767860362	4.54309170783459e-05
22.1779408021788	4.09247582861973e-05
22.2667048183215	3.65599348502620e-05
22.3556370337612	3.23539008761442e-05
22.4445692492010	2.83388224254709e-05
22.5335014646408	2.45362258757245e-05
22.6224336800805	2.09653138039077e-05
22.7139161549811	1.75516365826265e-05
22.8053986298817	1.44173267516055e-05
22.8968811047823	1.15757870019118e-05
22.9883635796829	9.03758194332528e-06
23.0838924299717	6.71940186177434e-06
23.1794212802604	4.74670255661738e-06
23.2749501305492	3.12227741660028e-06
23.3704789808380	1.84571581076059e-06
23.4621509718643	9.44694920667846e-07
23.5538229628905	3.55568170082765e-07
23.6454949539168	7.05272991193689e-08
23.7371669449431	7.95324408013874e-08
23.8279328445987	3.66304211620055e-07
23.9186987442544	9.15911797800991e-07
24.0094646439101	1.71303395715498e-06
24.1002305435658	2.74087919938781e-06
24.1926550919484	4.00587914091558e-06
24.2850796403311	5.47085444317882e-06
24.3775041887138	7.11426512505084e-06
24.4699287370964	8.91384529317392e-06
24.5667881185871	1.09424404891924e-05
24.6636475000779	1.30903515028071e-05
24.7605068815686	1.53302532000029e-05
24.8573662630593	1.76350302123194e-05
24.9520922059339	1.99260270181405e-05
25.0468181488086	2.22284047055917e-05
25.1415440916832	2.45178653352522e-05
25.2362700345578	2.67711679963137e-05
25.3292146875769	2.89255150699521e-05
25.4221593405961	3.10034887871110e-05
25.5151039936153	3.29861918402091e-05
25.6080486466344	3.48562886677358e-05
25.7019756638980	3.66156167449720e-05
25.7959026811617	3.82287400700097e-05
25.8898296984253	3.96823824650382e-05
25.9837567156889	4.09652460779256e-05
26.0813748678075	4.21074449844478e-05
26.1789930199261	4.30462448908217e-05
26.2766111720447	4.37751026500471e-05
26.3742293241633	4.42898708248313e-05
26.4732872431096	4.45914075966216e-05
26.5723451620558	4.46704752611162e-05
26.6714030810021	4.45292430551208e-05
26.7704609999484	4.41721484506471e-05
26.8668464553430	4.36236534977370e-05
26.9632319107376	4.28844996474191e-05
27.0596173661322	4.19638293784075e-05
27.1560028215268	4.08723097307961e-05
27.2528815695420	3.96151871388294e-05
27.3497603175572	3.82110145968880e-05
27.4466390655724	3.66741853925196e-05
27.5435178135875	3.50199883055469e-05
27.6439608492560	3.31981667946002e-05
27.7444038849244	3.12860431239206e-05
27.8448469205929	2.93025703682473e-05
27.9452899562613	2.72668997653361e-05
28.0482405279971	2.51463751314307e-05
28.1511910997329	2.30119616662822e-05
28.2541416714688	2.08839013579510e-05
28.3570922432046	1.87817703536990e-05
28.4567501555253	1.67893663632203e-05
28.5564080678461	1.48554202291560e-05
28.6560659801668	1.29953351410400e-05
28.7557238924876	1.12233283556248e-05
28.8557411898054	9.54663307874895e-06
28.9557584871233	7.98388451273656e-06
29.0557757844411	6.54566485850296e-06
29.1557930817590	5.24099777886389e-06
29.2596833575662	4.03529053113085e-06
29.3635736333734	2.98865246172458e-06
29.4674639091807	2.10600735474790e-06
29.5713541849879	1.39036534794981e-06
29.6759318863875	8.39894136004647e-07
29.7805095877872	4.59409148925445e-07
29.8850872891868	2.46585226198931e-07
29.9896649905864	1.97360696430743e-07
30.0911544966620	3.00676626990015e-07
30.1926440027376	5.46220520197498e-07
30.2941335088132	9.26179195896154e-07
30.3956230148889	1.43162967627854e-06
30.4978092358551	2.05729265446815e-06
30.5999954568214	2.78898546647386e-06
30.7021816777877	3.61479253653824e-06
30.8043678987539	4.52223598069417e-06
30.9109059456037	5.54126344756344e-06
31.0174439924534	6.61966543726990e-06
31.1239820393031	7.74194533233437e-06
31.2305200861528	8.89269573578537e-06
31.3364021990683	1.00494705553073e-05
31.4422843119837	1.12042964283844e-05
31.5481664248991	1.23426657204317e-05
31.6540485378145	1.34508215208159e-05
31.7574284840790	1.44911667107001e-05
31.8608084303435	1.54786722555133e-05
31.9641883766080	1.64026377874354e-05
32.0675683228725	1.72534736386667e-05
32.1722735824859	1.80319391291029e-05
32.2769788420993	1.87186566127396e-05
32.3816841017127	1.93068998295256e-05
32.4863893613262	1.97913451221114e-05
32.5963585110375	2.01840055380005e-05
32.7063276607488	2.04543714869440e-05
32.8162968104602	2.06006553998618e-05
32.9262659601715	2.06227761926684e-05
33.0345223500676	2.05246853308753e-05
33.1427787399638	2.03102634838468e-05
33.2510351298599	1.99834098478094e-05
33.3592915197560	1.95493361612110e-05
33.4657809711845	1.90239169150108e-05
33.5722704226130	1.84078761788042e-05
33.6787598740416	1.77090261665853e-05
33.7852493254701	1.69359630544484e-05
33.8941979357818	1.60779047338010e-05
34.0031465460936	1.51623620125499e-05
34.1120951564054	1.42002214385990e-05
34.2210437667172	1.32026514351523e-05
34.3366404896276	1.21181318475920e-05
34.4522372125380	1.10201984547294e-05
34.5678339354484	9.92230718135049e-06
34.6834306583588	8.83752592336933e-06
34.7936642990230	7.82686920415266e-06
34.9038979396873	6.85014447837958e-06
35.0141315803515	5.91716386022788e-06
35.1243652210157	5.03692074431285e-06
35.2343050512079	4.21969706390039e-06
35.3442448814002	3.47041903156087e-06
35.4541847115924	2.79539782308409e-06
35.5641245417846	2.19985596635892e-06
35.6786017627846	1.66869923716807e-06
35.7930789837846	1.23184302765692e-06
35.9075562047846	8.91534265891646e-07
36.0220334257847	6.48680255084522e-07
36.1362198980123	5.03197005580516e-07
36.2504063702399	4.52847946930673e-07
36.3645928424676	4.94930137874119e-07
36.4787793146952	6.25625334385488e-07
36.5900126053583	8.33548967852402e-07
36.7012458960214	1.11563259168572e-06
36.8124791866845	1.46575176225100e-06
36.9237124773476	1.87714533774615e-06
37.0369057108861	2.35113205598603e-06
37.1500989444246	2.87267386314938e-06
37.2632921779630	3.43307756724117e-06
37.3764854115015	4.02346054511276e-06
37.4962218645145	4.67060170371151e-06
37.6159583175275	5.33028581953224e-06
37.7356947705405	5.99173934822165e-06
37.8554312235534	6.64459905247891e-06
37.9694000931710	7.24892564877807e-06
38.0833689627887	7.82808697073698e-06
38.1973378324063	8.37430402015691e-06
38.3113067020239	8.88054467995461e-06
38.4249000672874	9.33904925657567e-06
38.5384934325510	9.74583664349273e-06
38.6520867978146	1.00960287858807e-05
38.7656801630782	1.03857130723253e-05
38.8839805724880	1.06198351961417e-05
39.0022809818979	1.07824827828408e-05
39.1205813913078	1.08721608841216e-05
39.2388818007176	1.08885528946785e-05
39.3577858169091	1.08319250044509e-05
39.4766898331005	1.07036204773709e-05
39.5955938492920	1.05062389566700e-05
39.7144978654834	1.02433748376560e-05
39.8306400259012	9.92766211795497e-06
39.9467821863190	9.55850722504440e-06
40.0629243467368	9.14130152112030e-06
40.1790665071546	8.68198738321455e-06
40.2979626814797	8.17484041760180e-06
40.4168588558048	7.63750628668878e-06
40.5357550301298	7.07745458877131e-06
40.6546512044549	6.50229470013761e-06
40.7793663330114	5.89112328802962e-06
40.9040814615679	5.28062382128155e-06
41.0287965901244	4.67938419962692e-06
41.1535117186809	4.09560116085195e-06
41.2728913030736	3.56032585977630e-06
41.3922708874662	3.05459528913372e-06
41.5116504718589	2.58423388399492e-06
41.6310300562516	2.15438626385401e-06
41.7513824171239	1.76659341616782e-06
41.8717347779962	1.42847348140358e-06
41.9920871388686	1.14313182475100e-06
42.1124394997409	9.12805582386086e-07
42.2403780838680	7.29863311367275e-07
42.3683166679951	6.11445888221836e-07
42.4962552521223	5.57224495897016e-07
42.6241938362494	5.65817500570300e-07
42.7459262128924	6.30189246000877e-07
42.8676585895354	7.46557190547559e-07
42.9893909661784	9.11450887866623e-07
43.1111233428215	1.12078990494019e-06
43.2323192820888	1.36877889808508e-06
43.3535152213561	1.65117064490466e-06
43.4747111606234	1.96251897920522e-06
43.5959070998906	2.29713791197951e-06
43.7230100636943	2.66665349456990e-06
43.8501130274980	3.04826294951027e-06
43.9772159913017	3.43492941413925e-06
44.1043189551053	3.81981041601252e-06
44.2286927690341	4.18832196621518e-06
44.3530665829628	4.54266277622268e-06
44.4774403968915	4.87712270260699e-06
44.6018142108202	5.18654130852586e-06
44.7243832234717	5.46244918213529e-06
44.8469522361232	5.70545892174493e-06
44.9695212487747	5.91212042622730e-06
45.0920902614261	6.07970441054021e-06
45.2192704569313	6.21007579231388e-06
45.3464506524364	6.29443993978280e-06
45.4736308479415	6.33188686138746e-06
45.6008110434466	6.32238256225974e-06
45.7293487437304	6.26582656315171e-06
45.8578864440142	6.16346781289238e-06
45.9864241442980	6.01743912552115e-06
46.1149618445818	5.83061005002522e-06
46.2403633884128	5.61235542779169e-06
46.3657649322439	5.36227485172338e-06
46.4911664760749	5.08446978340164e-06
46.6165680199060	4.78340488854534e-06
46.7458183814916	4.45377567924242e-06
46.8750687430772	4.10990374475129e-06
47.0043191046628	3.75730574034831e-06
47.1335694662484	3.40150725417423e-06
47.2659682689327	3.03944204236338e-06
47.3983670716170	2.68554575819952e-06
47.5307658743013	2.34529675316848e-06
47.6631646769855	2.02377116291682e-06
47.7913492952116	1.73471443512675e-06
47.9195339134376	1.47143643338338e-06
48.0477185316636	1.23726155433752e-06
48.1759031498897	1.03492715602020e-06
48.3075614879101	8.62536702814330e-07
48.4392198259305	7.27808930995255e-07
48.5708781639510	6.31813998521279e-07
48.7025365019714	5.74901556505026e-07
48.8366959423393	5.56786170135792e-07
48.9708553827072	5.77942552119338e-07
49.1050148230751	6.36696139023984e-07
49.2391742634430	7.30737688834983e-07
49.3688501639382	8.52482643189400e-07
49.4985260644335	1.00145987657145e-06
49.6282019649287	1.17422728406013e-06
49.7578778654240	1.36705323620854e-06
49.8184083990680	1.46281195605287e-06
49.8789389327120	1.56164991588424e-06
49.9394694663560	1.66313824773572e-06
50	1.76684406626454e-06

==> matlab/fig2c1.tex <==
0.0100000000000000	0.500000000000000
0.0179621434110699	0.478723637984091
0.0259242868221399	0.461894740314788
0.0338864302332098	0.447424761051175
0.0418485736442798	0.434508338231034
0.0489549209391593	0.423954749836263
0.0560612682340389	0.414130495763721
0.0631676155289185	0.404912313698334
0.0702739628237981	0.396210661660905
0.0834365541784869	0.381238650199266
0.0965991455331757	0.367504320230324
0.109761736887865	0.354794170844977
0.122924328242553	0.342953469362047
0.141422220690948	0.327563510663602
0.159920113139343	0.313418615739078
0.178418005587737	0.300336410958073
0.196915898036132	0.288176168265727
0.219013608897574	0.274703641887707
0.241111319759016	0.262236135904664
0.263209030620457	0.250651506852373
0.285306741481899	0.239849892762295
0.309342274650222	0.228893422337741
0.333377807818544	0.218675709631015
0.357413340986866	0.209121199227655
0.381448874155189	0.200165491856962
0.406933021704955	0.191262402464892
0.432417169254721	0.182912965428487
0.457901316804488	0.175067447476533
0.483385464354254	0.167682350833785
0.510146684095585	0.160380917499955
0.536907903836916	0.153505780308364
0.563669123578246	0.147022217973469
0.590430343319577	0.140899351976212
0.618396556862693	0.134856309834060
0.646362770405808	0.129148814141957
0.674328983948924	0.123751546585368
0.702295197492039	0.118641732402522
0.731440138666079	0.113600254889934
0.760585079840118	0.108827565987128
0.789730021014158	0.104304598740638
0.818874962188198	0.100014060264267
0.849202310632316	0.0957792988994329
0.879529659076434	0.0917630065520468
0.909857007520552	0.0879504598931537
0.940184355964671	0.0843282231571790
0.971722764316052	0.0807499927573395
1.00326117266743	0.0773516004234474
1.03479958101881	0.0741214407044956
1.06633798937020	0.0710488725973520
1.09914059673297	0.0680098249683145
1.13194320409574	0.0651205413250052
1.16474581145851	0.0623717087107959
1.19754841882128	0.0597547558377132
1.23169524674606	0.0571621488677891
1.26584207467084	0.0546956423184557
1.29998890259562	0.0523476386192253
1.33413573052039	0.0501111238588089
1.36973897643827	0.0478909356738819
1.40534222235615	0.0457780803057340
1.44094546827402	0.0437662590714104
1.47654871419190	0.0418496425432215
1.51333148231955	0.0399637778234500
1.55011425044721	0.0381682211380434
1.58689701857486	0.0364578387502075
1.62367978670251	0.0348278655144446
1.66101214689026	0.0332512034183161
1.69834450707800	0.0317484863052393
1.73567686726574	0.0303156954259071
1.77300922745348	0.0289490860272911
1.81093729414381	0.0276248444481982
1.84886536083414	0.0263618754550398
1.88679342752446	0.0251569771657690
1.92472149421479	0.0240071556420223
1.96329948808217	0.0228912381089017
2.00187748194955	0.0218266306587185
2.04045547581692	0.0208107396905662
2.07903346968430	0.0198411324905358
2.11832628074299	0.0188987734043542
2.15761909180168	0.0179997858158495
2.19691190286036	0.0171420353414882
2.23620471391905	0.0163235144152836
2.27628788215811	0.0155269887480871
2.31637105039716	0.0147674249134561
2.35645421863622	0.0140430396439267
2.39653738687527	0.0133521514783943
2.43749810706159	0.0126790904903524
2.47845882724791	0.0120377496210960
2.51941954743422	0.0114266172313111
2.56038026762054	0.0108442649151627
2.60231930174224	0.0102764114882172
2.64425833586394	0.00973593834275091
2.68619736998564	0.00922154625536131
2.72813640410734	0.00873200532291525
2.77117099359047	0.00825428742937993
2.81420558307360	0.00780031369975001
2.85724017255673	0.00736895267086606
2.90027476203986	0.00695913172004737
2.94454280820470	0.00655896720666053
2.98881085436955	0.00617946546425929
3.03307890053439	0.00581962870374940
3.07734694669924	0.00547851007461941
3.12301296380697	0.00514528078598571
3.16867898091470	0.00483007459939608
3.21434499802243	0.00453200105490714
3.26001101513015	0.00425021470661839
3.30727473639622	0.00397486555041952
3.35453845766229	0.00371525521688469
3.40180217892835	0.00347057992351877
3.44906590019442	0.00324007653523277
3.49817508767041	0.00301480748579515
3.54728427514641	0.00280328204989996
3.59639346262241	0.00260476663681279
3.64550265009840	0.00241856521026683
3.69677296104368	0.00223659299863129
3.74804327198896	0.00206660722242968
3.79931358293424	0.00190793096521444
3.85058389387952	0.00175992287217137
3.90443140626832	0.00161529530439905
3.95827891865712	0.00148109598560297
4.01212643104593	0.00135669308773431
4.06597394343473	0.00124148938472256
4.12210104024892	0.00113059048134554
4.17822813706310	0.00102846637567941
4.23435523387729	0.000934545810867574
4.29048233069147	0.000848290251092559
4.34732453072746	0.000768227634573614
4.40416673076345	0.000695006304816543
4.46100893079944	0.000628156481520997
4.51785113083543	0.000567236042658762
4.57582743647441	0.000510776263722936
4.63380374211339	0.000459634530403070
4.69178004775237	0.000413419218257685
4.74975635339135	0.000371762806861435
4.80927575174908	0.000333377945848600
4.86879515010681	0.000299082635318438
4.92831454846454	0.000268548054386423
4.98783394682227	0.000241466889606462
5.04934227097890	0.000216803919697981
5.11085059513554	0.000195224855489083
5.17235891929218	0.000176453040806791
5.23386724344882	0.000160231380586469
5.29789405007311	0.000145797124746816
5.36192085669741	0.000133615979375667
5.42594766332170	0.000123455832551858
5.48997446994599	0.000115102656784123
5.55719875822752	0.000108061054320853
5.62442304650904	0.000102582787655179
5.69164733479056	9.84747314442586e-05
5.75887162307208	9.55607346506392e-05
5.83023614825156	9.35946877945902e-05
5.90160067343103	9.26179914576048e-05
5.97296519861051	9.24724698833872e-05
6.04432972378998	9.30161357067788e-05
6.12127947749308	9.42284454422638e-05
6.19822923119618	9.59512755822698e-05
6.27517898489927	9.80586362943450e-05
6.35212873860237	0.000100440298321024
6.43723247735917	0.000103278296576522
6.52233621611597	0.000106221985725583
6.60743995487277	0.000109176197730006
6.69254369362957	0.000112061668161630
6.78171540330365	0.000114940367724434
6.87088711297772	0.000117611264790778
6.96005882265180	0.000120026800077338
7.04923053232588	0.000122151181900054
7.14466391282726	0.000124073463612996
7.24009729332864	0.000125613254710404
7.33553067383002	0.000126760407878200
7.43096405433140	0.000127513002957597
7.53934576535893	0.000127895979730635
7.64772747638647	0.000127794361129303
7.75610918741400	0.000127232767572156
7.86449089844153	0.000126240849667541
7.96911887225926	0.000124906963678762
8.07374684607698	0.000123238069814232
8.17837481989470	0.000121269505507788
8.28300279371242	0.000119036546322199
8.38717830981286	0.000116585619894685
8.49135382591330	0.000113943017747530
8.59552934201374	0.000111142649778691
8.69970485811419	0.000108216324001711
8.80416336793757	0.000105185850004830
8.90862187776095	0.000102088376650644
9.01308038758434	9.89507682258081e-05
9.11753889740773	9.57971108205929e-05
9.21807327203068	9.27671478180710e-05
9.31860764665363	8.97606212524111e-05
9.41914202127658	8.67933866356470e-05
9.51967639589953	8.38790726903399e-05
9.61962880891270	8.10457465432229e-05
9.71958122192588	7.82865678124838e-05
9.81953363493905	7.56099296483134e-05
9.91948604795222	7.30224784737707e-05
10.0207435189413	7.04974952466333e-05
10.1220009899305	6.80735656113869e-05
10.2232584609196	6.57534985163602e-05
10.3245159319087	6.35388089478376e-05
10.4283846120172	6.13769580344389e-05
10.5322532921256	5.93260084682492e-05
10.6361219722340	5.73845415599584e-05
10.7399906523424	5.55502866825424e-05
10.8475748287719	5.37602958575070e-05
10.9551590052014	5.20782579764684e-05
11.0627431816309	5.04997261814471e-05
11.1703273580604	4.90198284218639e-05
11.2826122346865	4.75748540313604e-05
11.3948971113127	4.62255177047463e-05
11.5071819879388	4.49655128727404e-05
11.6194668645650	4.37885028856771e-05
11.7372536318931	4.26361356274375e-05
11.8550403992212	4.15609722238905e-05
11.9728271665493	4.05560324271968e-05
12.0906139338774	3.96146374347149e-05
12.2143018181317	3.86875307766578e-05
12.3379897023860	3.78165303980204e-05
12.4616775866403	3.69951535541994e-05
12.5853654708946	3.62174370578939e-05
12.7146136383583	3.54455061188362e-05
12.8438618058221	3.47097091494502e-05
12.9731099732858	3.40050467962393e-05
13.1023581407496	3.33270915587505e-05
13.2358862805105	3.26506393602153e-05
13.3694144202714	3.19950203547971e-05
13.5029425600323	3.13572140650664e-05
13.6364706997933	3.07346503951155e-05
13.7724345754501	3.01142270118337e-05
13.9083984511069	2.95058629933995e-05
14.0443623267637	2.89083293294999e-05
14.1803262024205	2.83206271422830e-05
14.3171940356473	2.77382364196435e-05
14.4540618688741	2.71648767297794e-05
14.5909297021008	2.66004595785652e-05
14.7277975353276	2.60449173535782e-05
14.8649284638827	2.54972619580069e-05
15.0020593924377	2.49589713954674e-05
15.1391903209927	2.44304223176920e-05
15.2763212495477	2.39118747113971e-05
15.4138654423835	2.34020741577379e-05
15.5514096352193	2.29030979238909e-05
15.6889538280551	2.24153358200059e-05
15.8264980208909	2.19389967590740e-05
15.9650100243167	2.14710022743985e-05
16.1035220277425	2.10150687793473e-05
16.2420340311683	2.05713824526166e-05
16.3805460345941	2.01399360314363e-05
16.5206781669815	1.97158154755972e-05
16.6608102993689	1.93042006118196e-05
16.8009424317563	1.89050217288406e-05
16.9410745641437	1.85180326735851e-05
17.0834062487309	1.81371294952225e-05
17.2257379333181	1.77683070344173e-05
17.3680696179053	1.74112838734389e-05
17.5104013024924	1.70656314963535e-05
17.6553488510412	1.67248283712045e-05
17.8002963995899	1.63950044027176e-05
17.9452439481386	1.60757561633650e-05
18.0901914966873	1.57665623882941e-05
18.2379619557187	1.54611409503217e-05
18.3857324147501	1.51652339880725e-05
18.5335028737815	1.48784131925724e-05
18.6812733328129	1.46001535366606e-05
18.8318594722471	1.43248585659846e-05
18.9824456116813	1.40575713355962e-05
19.1330317511155	1.37979154151462e-05
19.2836178905498	1.35454271119081e-05
19.4368432212972	1.32954040467010e-05
19.5900685520447	1.30520825946879e-05
19.7432938827921	1.28151789773320e-05
19.8965192135396	1.25843208787024e-05
20.0521273153262	1.23556884925939e-05
20.2077354171128	1.21327685887774e-05
20.3633435188993	1.19153738355739e-05
20.5189516206859	1.17032204824811e-05
20.6767074948662	1.14932031421678e-05
20.8344633690465	1.12882193211383e-05
20.9922192432268	1.10881564260913e-05
21.1499751174070	1.08927959561056e-05
21.3097363309718	1.06995171384564e-05
21.4694975445366	1.05108183368371e-05
21.6292587581014	1.03266309182916e-05
21.7890199716662	1.01467729754493e-05
21.9507550228406	9.96890570751539e-06
22.1124900740149	9.79528565475202e-06
22.2742251251893	9.62586165094048e-06
22.4359601763636	9.46046556895749e-06
22.5997219235879	9.29691317395890e-06
22.7634836708122	9.13731326745529e-06
22.9272454180365	8.98161636855274e-06
23.0910071652607	8.82965574333308e-06
23.2568857402592	8.67935184143685e-06
23.4227643152578	8.53269990008868e-06
23.5886428902563	8.38964719399268e-06
23.7545214652548	8.25002558337015e-06
23.9225997668194	8.11186282749829e-06
24.0906780683841	7.97703701663408e-06
24.2587563699487	7.84549461938596e-06
24.4268346715134	7.71706923810964e-06
24.5971602465273	7.58992014553971e-06
24.7674858215413	7.46579138277732e-06
24.9378113965552	7.34463395873029e-06
25.1081369715692	7.22628822786626e-06
25.2807146345169	7.10906688968408e-06
25.4532922974645	6.99456704030131e-06
25.6258699604122	6.88274888226427e-06
25.7984476233598	6.77346337803784e-06
25.9732496005806	6.66518392126895e-06
26.1480515778014	6.55935962559859e-06
26.3228535550222	6.45596199074748e-06
26.4976555322430	6.35485395607469e-06
26.6746407580550	6.25466060509790e-06
26.8516259838669	6.15669384939733e-06
27.0286112096789	6.06093593286512e-06
27.2055964354908	5.96726084165397e-06
27.3847291106506	5.87442556329846e-06
27.5638617858103	5.78362268547124e-06
27.7429944609701	5.69484300131256e-06
27.9221271361299	5.60796936314761e-06
28.1033873526667	5.52186798200070e-06
28.2846475692035	5.43763120210931e-06
28.4659077857403	5.35525582254573e-06
28.6471680022771	5.27463128098651e-06
28.8305524749318	5.19471370513156e-06
29.0139369475864	5.11651111989890e-06
29.1973214202411	5.04002436975832e-06
29.3807058928957	4.96514783588830e-06
29.5662216026754	4.89091435006236e-06
29.7517373124551	4.81825871788224e-06
29.9372530222348	4.74718478001056e-06
30.1227687320145	4.67759104650369e-06
30.3104244405387	4.60857939703744e-06
30.4980801490630	4.54101833255182e-06
30.6857358575872	4.47491438618877e-06
30.8733915661115	4.41016999401563e-06
31.0631915046256	4.34595173191392e-06
31.2529914431398	4.28306627743650e-06
31.4427913816539	4.22152290955619e-06
31.6325913201681	4.16122803695728e-06
31.8245330634793	4.10140954185308e-06
32.0164748067905	4.04281602942003e-06
32.2084165501018	3.98545957999498e-06
32.4003582934130	3.92925057649525e-06
32.5944343723426	3.87347433377766e-06
32.7885104512723	3.81882540572495e-06
32.9825865302019	3.76531854919021e-06
33.1766626091316	3.71286794975318e-06
33.3728638888244	3.66081165491144e-06
33.5690651685172	3.60979466532790e-06
33.7652664482099	3.55983410623753e-06
33.9614677279027	3.51084764446598e-06
34.1597863981921	3.46222094725525e-06
34.3581050684815	3.41455412827976e-06
34.5564237387709	3.36786628994627e-06
34.7547424090604	3.32207820677316e-06
34.9551733102377	3.27661827469115e-06
35.1556042114151	3.23204611236752e-06
35.3560351125925	3.18838243561282e-06
35.5564660137699	3.14555079340607e-06
35.7590062381233	3.10301808560576e-06
35.9615464624766	3.06130725766355e-06
36.1640866868299	3.02044036417723e-06
36.3666269111833	2.98034347919421e-06
36.5712744813487	2.94051855352853e-06
36.7759220515142	2.90145505466910e-06
36.9805696216796	2.86317619277849e-06
37.1852171918451	2.82561039459352e-06
37.3919698016115	2.78829182495216e-06
37.5987224113779	2.75167916448904e-06
37.8054750211443	2.71579665310677e-06
38.0122276309107	2.68057494183739e-06
38.2210820628669	2.64557794476654e-06
38.4299364948231	2.61123592185244e-06
38.6387909267793	2.57757403575184e-06
38.8476453587355	2.54452504526270e-06
39.0585976322966	2.51168033322855e-06
39.2695499058576	2.47944391760258e-06
39.4805021794187	2.44784177322645e-06
39.6914544529798	2.41680864593348e-06
39.9045003567214	2.38596121510143e-06
40.1175462604631	2.35567930661692e-06
40.3305921642047	2.32598959069525e-06
40.5436380679464	2.29682867567451e-06
40.7587736492092	2.26783648583939e-06
40.9739092304720	2.23937057335707e-06
41.1890448117348	2.21145818966176e-06
41.4041803929976	2.18403768577521e-06
41.6214021542161	2.15677034303386e-06
41.8386239154346	2.12999320178383e-06
42.0558456766532	2.10373399287249e-06
42.2730674378717	2.07793270255234e-06
42.4923722413425	2.05227027186567e-06
42.7116770448134	2.02706482037063e-06
42.9309818482842	2.00234447294529e-06
43.1502866517551	1.97805075831983e-06
43.3716714967573	1.95388276428128e-06
43.5930563417596	1.93014111727638e-06
43.8144411867618	1.90685426531472e-06
44.0358260317640	1.88396519910202e-06
44.2592878797955	1.86118979542460e-06
44.4827497278270	1.83881247503992e-06
44.7062115758585	1.81686194796281e-06
44.9296734238900	1.79528259447646e-06
45.1552091541436	1.77380584481892e-06
45.3807448843971	1.75270108701639e-06
45.6062806146507	1.73199723772803e-06
45.8318163449043	1.71163999940403e-06
46.0594228148368	1.69137521911454e-06
46.2870292847694	1.67145832978050e-06
46.5146357547020	1.65191840338128e-06
46.7422422246345	1.63270240098992e-06
46.9719163573238	1.61356953794758e-06
47.2015904900131	1.59476228477005e-06
47.4312646227023	1.57630982159404e-06
47.6609387553916	1.55816030869585e-06
47.8926775894859	1.54008536559945e-06
48.1244164235803	1.52231541315845e-06
48.3561552576747	1.50487969734584e-06
48.5878940917691	1.48772752285934e-06
48.8216947775496	1.47064203102824e-06
49.0554954633302	1.45384242974049e-06
49.2892961491107	1.43735799354488e-06
49.5230968348912	1.42113912145784e-06
49.6423226261684	1.41295066444715e-06
49.7615484174456	1.40482868410183e-06
49.8807742087228	1.39677320707882e-06
50	1.38878279217464e-06

==> matlab/fig2c2.tex <==
0.0100000000000000	0.500000000000000
0.0148893961920471	0.461525762716727
0.0197787923840941	0.435300510830277
0.0246681885761412	0.415297698074918
0.0295575847681883	0.399056111960143
0.0344469809602354	0.385354736918460
0.0393363771522824	0.373480201248020
0.0442257733443295	0.362986578686943
0.0491151695363766	0.353575521379368
0.0566647429666537	0.340703756475454
0.0642143163969308	0.329400384799639
0.0717638898272080	0.319316739233307
0.0793134632574851	0.310210938914458
0.0908118553010885	0.297840676666230
0.102310247344692	0.286907910496589
0.113808639388295	0.277114659441000
0.125307031431899	0.268248496909845
0.141369341375589	0.257125583709661
0.157431651319280	0.247199002985915
0.173493961262971	0.238244879765867
0.189556271206662	0.230097436960830
0.209054765188173	0.221111769830521
0.228553259169684	0.212957900723800
0.248051753151195	0.205504026189621
0.267550247132706	0.198647354779973
0.290054092995263	0.191370335545095
0.312557938857820	0.184680250686168
0.335061784720377	0.178496926507045
0.357565630582934	0.172755375132141
0.382022894637376	0.166954352911318
0.406480158691819	0.161555499772225
0.430937422746262	0.156511736765939
0.455394686800704	0.151783616942690
0.481569771421338	0.147035349165217
0.507744856041972	0.142575646454314
0.533919940662606	0.138374846979369
0.560095025283240	0.134407507229455
0.587815541450838	0.130436072039196
0.615536057618436	0.126679165582548
0.643256573786034	0.123117090934407
0.670977089953632	0.119732655380805
0.700118255075150	0.116349766470605
0.729259420196668	0.113131053472154
0.758400585318186	0.110062888178674
0.787541750439704	0.107133214366724
0.818002822213866	0.104207268437741
0.848463893988028	0.101410013340258
0.878924965762190	0.0987317127494821
0.909386037536352	0.0961636608127512
0.941083529314273	0.0936000171135861
0.972781021092195	0.0911393571943603
1.00447851287012	0.0887745442892992
1.03617600464804	0.0864991406395947
1.06904120797423	0.0842280968917209
1.10190641130043	0.0820410113563508
1.13477161462662	0.0799325404095839
1.16763681795282	0.0778978278325483
1.20161504757622	0.0758670495596812
1.23559327719962	0.0739059126096284
1.26957150682302	0.0720103423848389
1.30354973644643	0.0701766119044317
1.33860026934466	0.0683461918674640
1.37365080224289	0.0665744980307962
1.40870133514113	0.0648583725932801
1.44375186803936	0.0631949103645091
1.47984820246859	0.0615340329798743
1.51594453689782	0.0599234741547455
1.55204087132705	0.0583607494744865
1.58813720575629	0.0568435609998492
1.62526753796055	0.0553281821436171
1.66239787016482	0.0538565932504135
1.69952820236909	0.0524268110467500
1.73665853457335	0.0510369917405989
1.77482648733532	0.0496481830966351
1.81299444009729	0.0482980635846278
1.85116239285926	0.0469850266360304
1.88933034562123	0.0457075711686178
1.92855606837490	0.0444303128221594
1.96778179112857	0.0431877408316386
2.00700751388225	0.0419785337364277
2.04623323663592	0.0408014505804052
2.08655507259207	0.0396237338417132
2.12687690854821	0.0384775546524257
2.16719874450436	0.0373618080245285
2.20752058046051	0.0362754508590612
2.24899759325488	0.0351876002875796
2.29047460604925	0.0341288101525828
2.33195161884362	0.0330981395709354
2.37342863163800	0.0320946955057878
2.41614443981355	0.0310888480456890
2.45886024798911	0.0301101191265338
2.50157605616466	0.0291576912081410
2.54429186434021	0.0282307838899382
2.58836050906038	0.0273004810578551
2.63242915378054	0.0263957886974015
2.67649779850070	0.0255159801014156
2.72056644322086	0.0246603574668529
2.76614153781910	0.0238002173914985
2.81171663241733	0.0229645404424552
2.85729172701556	0.0221526639562278
2.90286682161380	0.0213639477974881
2.94925709579494	0.0205842750172842
2.99564736997608	0.0198273520822170
3.04203764415721	0.0190925911954840
3.08842791833835	0.0183794210850471
3.13504806192754	0.0176839124974172
3.18166820551672	0.0170091235878769
3.22828834910590	0.0163545414397832
3.27490849269509	0.0157196648162583
3.32184817451336	0.0150998530855130
3.36878785633164	0.0144990534932958
3.41572753814992	0.0139168064342110
3.46266721996820	0.0133526607468866
3.51002497981212	0.0128013876716630
3.55738273965604	0.0122676613974778
3.60474049949997	0.0117510601172796
3.65209825934389	0.0112511683327107
3.69997786202684	0.0107623404784658
3.74785746470979	0.0102897744849884
3.79573706739275	0.00983307509466309
3.84361667007570	0.00939185199417279
3.89212998835124	0.00896018204994396
3.94064330662678	0.00854362468093427
3.98915662490232	0.00814180286648265
4.03766994317786	0.00775434372325709
4.08694045495193	0.00737516109705055
4.13621096672600	0.00701004461475270
4.18548147850007	0.00665862922369857
4.23475199027414	0.00632055361984952
4.28491921268052	0.00598966414208025
4.33508643508690	0.00567187294357266
4.38525365749328	0.00536682209351273
4.43542087989966	0.00507415734981101
4.48664627573137	0.00478773818302016
4.53787167156309	0.00451350990172634
4.58909706739480	0.00425111782220502
4.64032246322651	0.00400021116414594
4.69279768899344	0.00375473136525272
4.74527291476036	0.00352058204459895
4.79774814052728	0.00329740851003611
4.85022336629421	0.00308486043541892
4.90418235407362	0.00287702053969346
4.95814134185303	0.00267968777087110
5.01210032963244	0.00249250448406393
5.06605931741185	0.00231511810918258
5.12179691896912	0.00214180414003183
5.17753452052639	0.00197820398148020
5.23327212208366	0.00182395408191381
5.28900972364093	0.00167869694581848
5.34691229243864	0.00153694578068812
5.40481486123634	0.00140414080676884
5.46271743003406	0.00127990918517583
5.52061999883177	0.00116388545264749
5.58121953325118	0.00105085984791814
5.64181906767059	0.000946037251826246
5.70241860209001	0.000849031052373173
5.76301813650942	0.000759463804941825
5.82511460237858	0.000675016928256835
5.88721106824774	0.000597613450061610
5.94930753411689	0.000526882135152738
6.01140399998605	0.000462462118148517
6.07380159490291	0.000403734126906091
6.13619918981976	0.000350683180423612
6.19859678473662	0.000302977744137512
6.26099437965347	0.000260296939960966
6.32419436949673	0.000221872078313080
6.38739435933999	0.000187974103718613
6.45059434918325	0.000158304317158687
6.51379433902651	0.000132575075243578
6.57830719489551	0.000110088446372431
6.64282005076451	9.11376204714340e-05
6.70733290663351	7.54522396018934e-05
6.77184576250251	6.27735265784270e-05
6.83824117080171	5.26037045576107e-05
6.90463657910091	4.50993586961912e-05
6.97103198740010	4.00155787039592e-05
7.03742739569930	3.71197149360014e-05
7.10642156558373	3.61917825352429e-05
7.17541573546816	3.71534492886171e-05
7.24440990535259	3.97833479664111e-05
7.31340407523702	4.38732775933534e-05
7.38600948734619	4.95392657835910e-05
7.45861489945535	5.63919108940115e-05
7.53122031156452	6.42321104843600e-05
7.60382572367369	7.28752159807363e-05
7.68169060479945	8.28424273749795e-05
7.75955548592521	9.33420072351182e-05
7.83742036705097	0.000104196139395455
7.91528524817673	0.000115243517081503
7.99490567291899	0.000126587957127501
8.07452609766125	0.000137841372307232
8.15414652240351	0.000148878517902060
8.23376694714577	0.000159589035752438
8.31391886159019	0.000169943483463282
8.39407077603461	0.000179783661042442
8.47422269047904	0.000189036722734005
8.55437460492346	0.000197641827561078
8.63687721049298	0.000205770232200532
8.71937981606250	0.000213116717197476
8.80188242163202	0.000219649191539779
8.88438502720155	0.000225345499703512
8.97139686058978	0.000230433002646876
9.05840869397802	0.000234571377269402
9.14542052736626	0.000237765070397580
9.23243236075449	0.000240026696401804
9.32093858739016	0.000241391807293710
9.40944481402583	0.000241842574210375
9.49795104066150	0.000241413990930293
9.58645726729716	0.000240145868444507
9.67248667547180	0.000238150739754107
9.75851608364644	0.000235449479938430
9.84454549182108	0.000232089570323688
9.93057489999572	0.000228120002828751
10.0166970837528	0.000223586169543640
10.1028192675098	0.000218544888893525
10.1889414512669	0.000213049163483460
10.2750636350240	0.000207151429193684
10.3632012635051	0.000200753812149385
10.4513388919862	0.000194046068229812
10.5394765204673	0.000187082967429066
10.6276141489484	0.000179917053754397
10.7197494921261	0.000172264309390589
10.8118848353039	0.000164502331987198
10.9040201784817	0.000156684888166059
10.9961555216594	0.000148861907318848
11.0865603570731	0.000141225668575591
11.1769651924869	0.000133671434916495
11.2673700279006	0.000126237874859155
11.3577748633143	0.000118959716344097
11.4470969932176	0.000111952085323504
11.5364191231210	0.000105154886325764
11.6257412530243	9.85926839693244e-05
11.7150633829276	9.22864062952601e-05
11.8051167656774	8.62056816527605e-05
11.8951701484272	8.04191464908596e-05
11.9852235311770	7.49394693172350e-05
12.0752769139267	6.97760203086953e-05
12.1675783486168	6.48187034695801e-05
12.2598797833068	6.02052614242787e-05
12.3521812179968	5.59375173980859e-05
12.4444826526868	5.20144044874605e-05
12.5406946243167	4.82881339102790e-05
12.6369065959466	4.49264255733099e-05
12.7331185675765	4.19206819071415e-05
12.8293305392064	3.92599381156314e-05
12.9317611576690	3.67918908962106e-05
13.0341917761316	3.46829135071735e-05
13.1366223945942	3.29137622426402e-05
13.2390530130568	3.14635509244419e-05
13.3436694630454	3.02886334162663e-05
13.4482859130340	2.93989044343998e-05
13.5529023630227	2.87692131688847e-05
13.6575188130113	2.83740219056425e-05
13.7639378760502	2.81861408876538e-05
13.8703569390891	2.81874075311761e-05
13.9767760021280	2.83513220956151e-05
14.0831950651669	2.86521260665030e-05
14.1948918891323	2.90878705306614e-05
14.3065887130976	2.96191972660175e-05
14.4182855370630	3.02198647370674e-05
14.5299823610283	3.08654351269209e-05
14.6523445390369	3.15974104248616e-05
14.7747067170456	3.23286052504754e-05
14.8970688950542	3.30344627165984e-05
15.0194310730629	3.36935847762556e-05
15.1511465632349	3.43297722568605e-05
15.2828620534069	3.48709414028206e-05
15.4145775435789	3.53015536753476e-05
15.5462930337509	3.56100279002982e-05
15.6816426907559	3.57913487609327e-05
15.8169923477609	3.58301549031525e-05
15.9523420047659	3.57248817144729e-05
16.0876916617709	3.54771239421481e-05
16.2195694981085	3.51028417878052e-05
16.3514473344461	3.46040186794725e-05
16.4833251707836	3.39890743039028e-05
16.6152030071212	3.32678118441312e-05
16.7409056818706	3.24914829908198e-05
16.8666083566200	3.16394145617297e-05
16.9923110313695	3.07228529789355e-05
17.1180137061189	2.97531129206500e-05
17.2460071843381	2.87228569237327e-05
17.3740006625573	2.76618155769826e-05
17.5019941407765	2.65820784795027e-05
17.6299876189957	2.54949572174985e-05
17.7565892512773	2.44228832945181e-05
17.8831908835589	2.33642415085340e-05
18.0097925158406	2.23282586522495e-05
18.1363941481222	2.13229739560806e-05
18.2599448561665	2.03782918522805e-05
18.3834955642107	1.94756882207455e-05
18.5070462722549	1.86202070967493e-05
18.6305969802992	1.78157408097125e-05
18.7553803779988	1.70580358250669e-05
18.8801637756984	1.63578146992505e-05
19.0049471733980	1.57165136850205e-05
19.1297305710976	1.51345336414984e-05
19.2592552219338	1.45927202956951e-05
19.3887798727700	1.41132780598418e-05
19.5183045236062	1.36942799486021e-05
19.6478291744424	1.33329667529804e-05
19.7861929856835	1.30068848309794e-05
19.9245567969247	1.27381765127869e-05
20.0629206081659	1.25216933578859e-05
20.2012844194070	1.23517910822810e-05
20.3511564871112	1.22134234088865e-05
20.5010285548154	1.21151203369340e-05
20.6509006225196	1.20492301338010e-05
20.8007726902238	1.20081872214353e-05
20.9588361116552	1.19837538680167e-05
21.1168995330866	1.19707676177907e-05
21.2749629545180	1.19618245893458e-05
21.4330263759494	1.19502748850902e-05
21.6190635682705	1.19254550902789e-05
21.8051007605917	1.18810371035539e-05
21.9911379529128	1.18109111001592e-05
22.1771751452340	1.17107561676180e-05
22.3458199885345	1.15917524896314e-05
22.5144648318351	1.14451672162551e-05
22.6831096751357	1.12713047553653e-05
22.8517545184363	1.10712838737703e-05
23.0203993617369	1.08469577580116e-05
23.1890442050374	1.06011089331508e-05
23.3576890483380	1.03369794712785e-05
23.5263338916386	1.00580020550697e-05
23.6920944741673	9.77284844620509e-06
23.8578550566961	9.48077952260139e-06
24.0236156392249	9.18561766566925e-06
24.1893762217536	8.89084735081233e-06
24.3482102075099	8.61177935426059e-06
24.5070441932662	8.33902392084834e-06
24.6658781790225	8.07516563193928e-06
24.8247121647788	7.82227480055645e-06
24.9797169326094	7.58767678982683e-06
25.1347217004401	7.36663209459190e-06
25.2897264682707	7.16021836057990e-06
25.4447312361014	6.96902636600830e-06
25.6022628713019	6.79055312631247e-06
25.7597945065025	6.62816316585946e-06
25.9173261417030	6.48161042332647e-06
26.0748577769036	6.35024663000591e-06
26.2399748574646	6.22785127647220e-06
26.4050919380255	6.11999259600488e-06
26.5702090185865	6.02529272049114e-06
26.7353260991475	5.94211921722138e-06
26.9135866885254	5.86323061855930e-06
27.0918472779033	5.79359771609886e-06
27.2701078672812	5.73107041028095e-06
27.4483684566591	5.67347011632513e-06
27.6461875512081	5.61277817705967e-06
27.8440066457571	5.55313440465449e-06
28.0418257403061	5.49239541155218e-06
28.2396448348551	5.42868398138547e-06
28.4582261869192	5.35298471821854e-06
28.6768075389832	5.27055516065741e-06
28.8953888910472	5.18073151036571e-06
29.1139702431113	5.08326059321662e-06
29.3320751105215	4.97855589382012e-06
29.5501799779317	4.86737708207716e-06
29.7682848453419	4.75097343664851e-06
29.9863897127521	4.63063353197549e-06
30.1847014566922	4.51897616301059e-06
30.3830132006322	4.40662699874375e-06
30.5813249445722	4.29491457854647e-06
30.7796366885122	4.18493772781899e-06
30.9653208272272	4.08440103918543e-06
31.1510049659422	3.98716206495646e-06
31.3366891046572	3.89396370449309e-06
31.5223732433722	3.80528596221101e-06
31.7057580297484	3.72244827210748e-06
31.8891428161245	3.64466848726142e-06
32.0725276025007	3.57210892146909e-06
32.2559123888769	3.50469676896136e-06
32.4435767931044	3.44081226519712e-06
32.6312411973319	3.38189884316434e-06
32.8189056015594	3.32762984041765e-06
33.0065700057869	3.27750635180378e-06
33.2035317736837	3.22871805308969e-06
33.4004935415806	3.18327845740961e-06
33.5974553094774	3.14056436113753e-06
33.7944170773742	3.09987149062864e-06
34.0042348370502	3.05795176734716e-06
34.2140525967261	3.01688357842492e-06
34.4238703564021	2.97608301222873e-06
34.6336881160780	2.93497853571964e-06
34.8550217447865	2.89074237820210e-06
35.0763553734949	2.84535616258445e-06
35.2976890022033	2.79867548763616e-06
35.5190226309117	2.75059312126615e-06
35.7420476120856	2.70070487923731e-06
35.9650725932595	2.64966317613936e-06
36.1880975744334	2.59781487394363e-06
36.4111225556072	2.54545827466874e-06
36.6266455989052	2.49466787942667e-06
36.8421686422032	2.44416915737817e-06
37.0576916855012	2.39439989852163e-06
37.2732147287991	2.34566640137059e-06
37.4822671682508	2.29961474404820e-06
37.6913196077025	2.25510427471610e-06
37.9003720471542	2.21238607283895e-06
38.1094244866059	2.17156076949551e-06
38.3178434323715	2.13276125213095e-06
38.5262623781370	2.09596241406410e-06
38.7346813239026	2.06117952830047e-06
38.9431002696682	2.02829609258590e-06
39.1562974204122	1.99643291454003e-06
39.3694945711562	1.96626050347344e-06
39.5826917219003	1.93761782119399e-06
39.7958888726443	1.91025036382338e-06
40.0176196036804	1.88283156344541e-06
40.2393503347166	1.85628640298994e-06
40.4610810657527	1.83040820395141e-06
40.6828117967889	1.80493992273617e-06
40.9137026787675	1.77858189100817e-06
41.1445935607461	1.75227883469840e-06
41.3754844427247	1.72593871550932e-06
41.6063753247033	1.69944159650689e-06
41.8420837151137	1.67212362550546e-06
42.0777921055241	1.64461183710758e-06
42.3135004959345	1.61699937564782e-06
42.5492088863449	1.58933262295303e-06
42.7832701060807	1.56184868815409e-06
43.0173313258165	1.53455007734214e-06
43.2513925455524	1.50761398933870e-06
43.4854537652882	1.48113529640451e-06
43.7158897201435	1.45557287870509e-06
43.9463256749988	1.43068324542839e-06
44.1767616298541	1.40659200697845e-06
44.4071975847094	1.38332753415105e-06
44.6370374295381	1.36092850299484e-06
44.8668772743667	1.33940603035444e-06
45.0967171191954	1.31878503265876e-06
45.3265569640240	1.29900114994143e-06
45.5600731725287	1.27965057185811e-06
45.7935893810333	1.26103827957472e-06
46.0271055895379	1.24311337631730e-06
46.2606217980426	1.22575571428885e-06
46.5007803538022	1.20834488082511e-06
46.7409389095619	1.19133351881776e-06
46.9810974653215	1.17466088957690e-06
47.2212560210812	1.15821721869774e-06
47.4680943172735	1.14143092141585e-06
47.7149326134659	1.12475759971615e-06
47.9617709096582	1.10819331602160e-06
48.2086092058506	1.09169201393664e-06
48.4587788964316	1.07497956280669e-06
48.7089485870126	1.05834837071419e-06
48.9591182775936	1.04186279801387e-06
49.2092879681746	1.02553448195778e-06
49.4069659761309	1.01274575245911e-06
49.6046439840873	1.00010725396614e-06
49.8023219920436	9.87653492340754e-07
50	9.75398476275691e-07

==> matlab/fig2c3.tex <==
0.0100000000000000	0.500000000000000
0.0117160547237387	0.454095860774370
0.0134321094474774	0.420391926597804
0.0151481641712160	0.394500265385458
0.0168642188949547	0.373911452497757
0.0185802736186934	0.357100148434965
0.0202963283424321	0.343072246983724
0.0220123830661707	0.331156271993677
0.0237284377899094	0.320882201466450
0.0271767298921404	0.303924249678135
0.0306250219943713	0.290497035952064
0.0340733140966023	0.279525959984736
0.0375216061988333	0.270338100984411
0.0427139279135350	0.258935191312670
0.0479062496282368	0.249635739572755
0.0530985713429385	0.241844736254697
0.0582908930576403	0.235177764773884
0.0666867029016913	0.226146650137962
0.0750825127457423	0.218689283470022
0.0834783225897933	0.212368104562108
0.0918741324338443	0.206900031589918
0.103221374695157	0.200535790084879
0.114568616956470	0.195068310784611
0.125915859217783	0.190285474095049
0.137263101479095	0.186040674828647
0.152303542411290	0.181068891383740
0.167343983343484	0.176687616849911
0.182384424275678	0.172774665998804
0.197424865207872	0.169241514847808
0.216556218911177	0.165194281171658
0.235687572614481	0.161555513766214
0.254818926317785	0.158250844959280
0.273950280021090	0.155224163806589
0.295702700579699	0.152066102838300
0.317455121138309	0.149162325595912
0.339207541696919	0.146474152726331
0.360959962255528	0.143970918649711
0.384856456254013	0.141404901607610
0.408752950252498	0.139005781475967
0.432649444250983	0.136751884755859
0.456545938249468	0.134625384306022
0.482428909122220	0.132448702096788
0.508311879994973	0.130388301622056
0.534194850867725	0.128430918869300
0.560077821740478	0.126565354098339
0.587789573063889	0.124658955529914
0.615501324387300	0.122836827620904
0.643213075710712	0.121090352292866
0.670924827034123	0.119412108744493
0.700315973473582	0.117699555178102
0.729707119913042	0.116049809641254
0.759098266352501	0.114457029093782
0.788489412791960	0.112916105392516
0.819413129909566	0.111345885894555
0.850336847027172	0.109823471551910
0.881260564144777	0.108344779955331
0.912184281262383	0.106906198822151
0.944496310546559	0.105442404761945
0.976808339830736	0.104015627855114
1.00912036911491	0.102622956349558
1.04143239839909	0.101261788392441
1.07499283168995	0.0998788826853853
1.10855326498080	0.0985251002390588
1.14211369827166	0.0971983368486306
1.17567413156251	0.0958966969480986
1.21035017643711	0.0945763619204516
1.24502622131171	0.0932793258652950
1.27970226618631	0.0920040579591758
1.31437831106091	0.0907491697904586
1.35004735827022	0.0894782838177417
1.38571640547953	0.0882263996460262
1.42138545268884	0.0869924028058386
1.45705449989815	0.0857752767243088
1.49360694715890	0.0845445425766646
1.53015939441965	0.0833296661803075
1.56671184168041	0.0821298405987041
1.60326428894116	0.0809443261998264
1.64060574378950	0.0797472995337200
1.67794719863784	0.0785638713126769
1.71528865348618	0.0773934645986502
1.75263010833452	0.0762355483419195
1.79068279737963	0.0750679272451242
1.82873548642474	0.0739123311257842
1.86678817546984	0.0727683564920469
1.90484086451495	0.0716356305041015
1.94354426897741	0.0704947248727626
1.98224767343986	0.0693648056030188
2.02095107790232	0.0682456005689566
2.05965448236477	0.0671368572943681
2.09896535948022	0.0660211874202807
2.13827623659567	0.0649158836706851
2.17758711371112	0.0638207734240516
2.21689799082656	0.0627356956463737
2.25679001376257	0.0616446862209925
2.29668203669857	0.0605637503595253
2.33657405963457	0.0594927904369796
2.37646608257057	0.0584317144171425
2.41692934917714	0.0573654600154923
2.45739261578371	0.0563092433733800
2.49785588239028	0.0552630227247147
2.53831914899685	0.0542267573532658
2.57935979595430	0.0531858417185997
2.62040044291174	0.0521551293800292
2.66144108986919	0.0511346192553220
2.70248173682663	0.0501243078114906
2.74412187579687	0.0491096635387077
2.78576201476712	0.0481055463936024
2.82740215373736	0.0471119837429392
2.86904229270760	0.0461289977418641
2.91132048022032	0.0451417960052204
2.95359866773304	0.0441655705383987
2.99587685524576	0.0432003671017332
3.03815504275849	0.0422462240079067
3.08112752419896	0.0412877861341065
3.12410000563943	0.0403408744128693
3.16707248707990	0.0394055445393345
3.21004496852037	0.0384818428916392
3.25378802052889	0.0375535669679186
3.29753107253741	0.0366374506092220
3.34127412454594	0.0357335521182521
3.38501717655446	0.0348419188577492
3.42963104837956	0.0339452151494682
3.47424492020467	0.0330613776537263
3.51885879202977	0.0321904606895202
3.56347266385488	0.0313325061627751
3.60908796232704	0.0304687346271971
3.65470326079919	0.0296186061245876
3.70031855927135	0.0287821647637716
3.74593385774351	0.0279594408327569
3.79272190093334	0.0271298416898432
3.83950994412316	0.0263147381981201
3.88629798731299	0.0255141579936840
3.93308603050281	0.0247281134652796
3.98127611499785	0.0239337156091582
4.02946619949289	0.0231547596118796
4.07765628398793	0.0223912498233022
4.12584636848297	0.0216431738014715
4.17453782062043	0.0209029693438372
4.22322927275788	0.0201784880566922
4.27192072489534	0.0194697048796110
4.32061217703279	0.0187765781406218
4.36915150529233	0.0181011503194427
4.41769083355186	0.0174411885441481
4.46623016181140	0.0167966377077508
4.51476949007093	0.0161674274871047
4.56328105147248	0.0155538263890351
4.61179261287403	0.0149553966088310
4.66030417427557	0.0143720533590181
4.70881573567712	0.0138036979507639
4.75743034626171	0.0132490641578757
4.80604495684629	0.0127092716906143
4.85465956743088	0.0121842065439661
4.90327417801546	0.0116737420556813
4.95214759150491	0.0111751424811629
5.00102100499435	0.0106910309519949
5.04989441848379	0.0102212644864540
5.09876783197324	0.00976568861800654
5.14804659394740	0.00932053848653108
5.19732535592155	0.00888948872045891
5.24660411789571	0.00847236753087372
5.29588287986987	0.00806899279035602
5.34571691623879	0.00767486062525716
5.39555095260772	0.00729440162966521
5.44538498897664	0.00692741525301826
5.49521902534556	0.00657369175918080
5.54578533292858	0.00622810659950294
5.59635164051159	0.00589573313677096
5.64691794809460	0.00557634170960794
5.69748425567761	0.00526969465039676
5.74900092501619	0.00497013996572512
5.80051759435478	0.00468330833420719
5.85203426369337	0.00440893997879598
5.90355093303196	0.00414676834914215
5.95629904554016	0.00389068560413048
6.00904715804837	0.00364681966808055
6.06179527055658	0.00341487856550952
6.11454338306479	0.00319456487574429
6.16890437576226	0.00297936421522858
6.22326536845974	0.00277587020858709
6.27762636115721	0.00258375476148769
6.33198735385468	0.00240268582764549
6.38842448996247	0.00222603240851991
6.44486162607025	0.00206055885991721
6.50129876217804	0.00190589542128365
6.55773589828582	0.00176167018503577
6.61342964774346	0.00162921573018858
6.66912339720110	0.00150621405300668
6.72481714665874	0.00139231403125338
6.78051089611637	0.00128716474616950
6.83589971047198	0.00119092545106319
6.89128852482759	0.00110265990672545
6.94667733918320	0.00102203301993275
7.00206615353882	0.000948711780377262
7.05758976165192	0.000882213981957867
7.11311336976503	0.000822401619609501
7.16863697787814	0.000768952973812481
7.22416058599125	0.000721550038649328
7.28021693986213	0.000679506994205066
7.33627329373302	0.000642992633754385
7.39232964760390	0.000611697121337164
7.44838600147478	0.000585315860968875
7.50538574262213	0.000563222243955422
7.56238548376949	0.000545596098136423
7.61938522491684	0.000532138546192640
7.67638496606419	0.000522557483564588
7.73480587272738	0.000516462752105100
7.79322677939057	0.000513844809773380
7.85164768605376	0.000514414999576931
7.91006859271695	0.000517893094264901
7.97053387043690	0.000524266606453133
8.03099914815685	0.000533175506769323
8.09146442587680	0.000544340449321675
8.15192970359676	0.000557492470575175
8.21535952756943	0.000573143338119542
8.27878935154210	0.000590412887937590
8.34221917551477	0.000609029395390140
8.40564899948744	0.000628734093178971
8.46793784799597	0.000648906056680944
8.53022669650450	0.000669671305344826
8.59251554501303	0.000690821976369698
8.65480439352156	0.000712162133354997
8.71642204054983	0.000733278656936119
8.77803968757810	0.000754234699536830
8.83965733460636	0.000774874954138603
8.90127498163463	0.000795055034502473
8.96300495617631	0.000814676739914706
9.02473493071799	0.000833579851225912
9.08646490525967	0.000851651583837140
9.14819487980135	0.000868789339105115
9.21071927424122	0.000885101086291909
9.27324366868109	0.000900274712704023
9.33576806312096	0.000914234631773570
9.39829245756083	0.000926914850283399
9.46233592838314	0.000938517602096952
9.52637939920544	0.000948668543917329
9.59042287002774	0.000957326833665699
9.65446634085004	0.000964460706818448
9.72096019267431	0.000970230328649374
9.78745404449858	0.000974317401218796
9.85394789632285	0.000976715914902515
9.92044174814712	0.000977428462478290
9.98759919027086	0.000976448340975413
10.0547566323946	0.000973780652422476
10.1219140745184	0.000969453260346688
10.1890715166421	0.000963500812462384
10.2546642923364	0.000956158162466678
10.3202570680308	0.000947350278769485
10.3858498437251	0.000937127100712026
10.4514426194195	0.000925542799065177
10.5165140917340	0.000912763389103025
10.5815855640486	0.000898763963922343
10.6466570363632	0.000883609131165582
10.7117285086778	0.000867365848795575
10.7771443606203	0.000850009752231650
10.8425602125627	0.000831697770678248
10.9079760645052	0.000812504864956372
10.9733919164476	0.000792506776187035
11.0399477645340	0.000771413158267202
11.1065036126204	0.000749648297568879
11.1730594607068	0.000727294573081518
11.2396153087932	0.000704433672218682
11.3082257087532	0.000680422236125248
11.3768361087133	0.000656047922820665
11.4454465086734	0.000631398457389550
11.5140569086335	0.000606559328727706
11.5852093098832	0.000580689130525897
11.6563617111329	0.000554797425032464
11.7275141123826	0.000528973021766367
11.7986665136323	0.000503300821733162
11.8677850418193	0.000478585731063633
11.9369035700062	0.000454164168198977
12.0060220981931	0.000430104816266921
12.0751406263801	0.000406472103946442
12.1433601380698	0.000383624529734156
12.2115796497596	0.000361307564942060
12.2797991614493	0.000339572612047822
12.3480186731391	0.000318466661746561
12.4163461472746	0.000298001111932196
12.4846736214100	0.000278250105725080
12.5530010955455	0.000259249367085095
12.6213285696809	0.000241030116863612
12.6907216414633	0.000223354665829907
12.7601147132457	0.000206538540681984
12.8295077850280	0.000190602206122358
12.8989008568104	0.000175561560600920
12.9703478268833	0.000161024134785803
13.0417947969561	0.000147458087502255
13.1132417670290	0.000134867891964706
13.1846887371018	0.000123253429436367
13.2595560962437	0.000112125348660985
13.3344234553855	0.000102055413696413
13.4092908145273	9.30299599598578e-05
13.4841581736692	8.50307375395600e-05
13.5575412493262	7.81647105000365e-05
13.6309243249833	7.22393710283750e-05
13.7043074006403	6.72271413637404e-05
13.7776904762973	6.30972700752484e-05
13.8500672006557	5.98557873820444e-05
13.9224439250142	5.74059200205524e-05
13.9948206493726	5.57110813565219e-05
14.0671973737310	5.47327299659362e-05
14.1398455416426	5.44308719667461e-05
14.2124937095543	5.47685859098511e-05
14.2851418774659	5.57026154243576e-05
14.3577900453776	5.71887664673827e-05
14.4318616952425	5.92260580895266e-05
14.5059333451073	6.17426833446532e-05
14.5800049949722	6.46901949888052e-05
14.6540766448371	6.80201923469352e-05
14.7309274464065	7.18279460480389e-05
14.8077782479759	7.59422802796729e-05
14.8846290495453	8.03104647943595e-05
14.9614798511146	8.48809149617977e-05
15.0406722118752	8.97491439965406e-05
15.1198645726358	9.47251847352024e-05
15.1990569333964	9.97571842272830e-05
15.2782492941569	0.000104795572905283
15.3552187760152	0.000109653858106767
15.4321882578735	0.000114432216002222
15.5091577397318	0.000119091544302625
15.5861272215900	0.000123595348068539
15.6625824441176	0.000127881638174619
15.7390376666451	0.000131950208964869
15.8154928891726	0.000135772784679258
15.8919481117002	0.000139323903506508
15.9693961674172	0.000142621161959856
16.0468442231342	0.000145595715261162
16.1242922788512	0.000148229479113648
16.2017403345682	0.000150507355588643
16.2817277574867	0.000152473441067047
16.3617151804052	0.000154036546849821
16.4417026033237	0.000155189289864233
16.5216900262422	0.000155927435195451
16.6043553465212	0.000156253405133208
16.6870206668002	0.000156137125787319
16.7696859870792	0.000155583382015884
16.8523513073581	0.000154599978870196
16.9322086407103	0.000153252002974754
17.0120659740625	0.000151525020303705
17.0919233074148	0.000149432999074720
17.1717806407670	0.000146991847365558
17.2507845102887	0.000144250664132456
17.3297883798104	0.000141204055714104
17.4087922493321	0.000137872129056370
17.4877961188537	0.000134276135797809
17.5676116379811	0.000130397839148960
17.6474271571085	0.000126296997786931
17.7272426762358	0.000121998304827115
17.8070581953632	0.000117526900502399
17.8893023304811	0.000112765804098614
17.9715464655990	0.000107876979090299
18.0537906007169	0.000102888731236263
18.1360347358348	9.78290811150000e-05
18.2213159234312	9.25368714456939e-05
18.3065971110275	8.72284846973943e-05
18.3918782986238	8.19336330900159e-05
18.4771594862202	7.66809107565043e-05
18.5595094175750	7.16746135118014e-05
18.6418593489297	6.67573243639649e-05
18.7242092802845	6.19516068475021e-05
18.8065592116393	5.72785458117604e-05
18.8880422520689	5.28046135025410e-05
18.9695252924985	4.84978038581904e-05
19.0510083329281	4.43743414414624e-05
19.1324913733577	4.04487572397971e-05
19.2148776329082	3.66940860698328e-05
19.2972638924588	3.31669034796196e-05
19.3796501520093	2.98772332442325e-05
19.4620364115598	2.68332449223303e-05
19.5470683095882	2.39560034045750e-05
19.6321002076166	2.13527329078525e-05
19.7171321056450	1.90266929977510e-05
19.8021640036734	1.69791616010336e-05
19.8908893408643	1.51390373619100e-05
19.9796146780552	1.35990274946769e-05
20.0683400152462	1.23543980608364e-05
20.1570653524371	1.13984488189033e-05
20.2428390648805	1.07408139407039e-05
20.3286127773240	1.03359490772839e-05
20.4143864897674	1.01732485541359e-05
20.5001602022109	1.02408627554209e-05
20.5852635054960	1.05228249710427e-05
20.6703668087812	1.10051032825497e-05
20.7554701120663	1.16730996924718e-05
20.8405734153514	1.25115353425417e-05
20.9270705233463	1.35220319530878e-05
21.0135676313412	1.46749702532924e-05
21.1000647393361	1.59526734078446e-05
21.1865618473310	1.73373156586377e-05
21.2766604059527	1.88740402259639e-05
21.3667589645743	2.04870036992270e-05
21.4568575231959	2.21559700263370e-05
21.5469560818176	2.38611752794549e-05
21.6381292498009	2.56039448282709e-05
21.7293024177842	2.73445476079605e-05
21.8204755857675	2.90641629134259e-05
21.9116487537508	3.07450191450739e-05
22.0004127698935	3.23282868310439e-05
22.0891767860362	3.38442664536817e-05
22.1779408021788	3.52793356499734e-05
22.2667048183215	3.66211336653063e-05
22.3556370337612	3.78607618994691e-05
22.4445692492010	3.89854165798082e-05
22.5335014646408	3.99861961708062e-05
22.6224336800805	4.08556189750259e-05
22.7139161549811	4.16064692653562e-05
22.8053986298817	4.22064559644382e-05
22.8968811047823	4.26516344261754e-05
22.9883635796829	4.29396293949857e-05
23.0838924299717	4.30716371561795e-05
23.1794212802604	4.30317158933537e-05
23.2749501305492	4.28218384048027e-05
23.3704789808380	4.24456048135469e-05
23.4621509718643	4.19328629620692e-05
23.5538229628905	4.12771916255787e-05
23.6454949539168	4.04851875253703e-05
23.7371669449431	3.95644587662260e-05
23.8279328445987	3.85343878336968e-05
23.9186987442544	3.73955220019854e-05
24.0094646439101	3.61574868041186e-05
24.1002305435658	3.48304707888656e-05
24.1926550919484	3.33988254205097e-05
24.2850796403311	3.18977275767974e-05
24.3775041887138	3.03390941580195e-05
24.4699287370964	2.87349930697105e-05
24.5667881185871	2.70184044932482e-05
24.6636475000779	2.52793277879559e-05
24.7605068815686	2.35315491931455e-05
24.8573662630593	2.17885220924785e-05
24.9520922059339	2.01010745533769e-05
25.0468181488086	1.84426003529707e-05
25.1415440916832	1.68243310060650e-05
25.2362700345578	1.52568089209329e-05
25.3292146875769	1.37776372005507e-05
25.4221593405961	1.23655374389389e-05
25.5151039936153	1.10283522926278e-05
25.6080486466344	9.77306432023856e-06
25.7019756638980	8.59399828994152e-06
25.7959026811617	7.51040795150959e-06
25.8898296984253	6.52681512981301e-06
25.9837567156889	5.64676007687304e-06
26.0813748678075	4.84464932720448e-06
26.1789930199261	4.15911896020050e-06
26.2766111720447	3.59091835706484e-06
26.3742293241633	3.13971940326275e-06
26.4732872431096	2.80011149885503e-06
26.5723451620558	2.57720354747547e-06
26.6714030810021	2.46752216059391e-06
26.7704609999484	2.46668028091847e-06
26.8668464553430	2.56538275936881e-06
26.9632319107376	2.75662273890331e-06
27.0596173661322	3.03415676628050e-06
27.1560028215268	3.39121930713050e-06
27.2528815695420	3.82295648591389e-06
27.3497603175572	4.31989077421497e-06
27.4466390655724	4.87382365300883e-06
27.5435178135875	5.47637158869742e-06
27.6439608492560	6.14330713765174e-06
27.7444038849244	6.84359092599763e-06
27.8448469205929	7.56746617783220e-06
27.9452899562613	8.30537031811235e-06
28.0482405279971	9.06647225978917e-06
28.1511910997329	9.82251576537057e-06
28.2541416714688	1.05639167800316e-05
28.3570922432046	1.12816944668058e-05
28.4567501555253	1.19460905546062e-05
28.5564080678461	1.25732165741339e-05
28.6560659801668	1.31564304919101e-05
28.7557238924876	1.36898392438741e-05
28.8557411898054	1.41698761161638e-05
28.9557584871233	1.45898432494654e-05
29.0557757844411	1.49458118474308e-05
29.1557930817590	1.52347110750649e-05
29.2596833575662	1.54613513951763e-05
29.3635736333734	1.56113669075507e-05
29.4674639091807	1.56838230358065e-05
29.5713541849879	1.56787542543904e-05
29.6759318863875	1.55962810877472e-05
29.7805095877872	1.54378257913991e-05
29.8850872891868	1.52058092773954e-05
29.9896649905864	1.49034644250153e-05
30.0911544966620	1.45465426235843e-05
30.1926440027376	1.41312194769149e-05
30.2941335088132	1.36620852028676e-05
30.3956230148889	1.31441956785123e-05
30.4978092358551	1.25790193466484e-05
30.5999954568214	1.19758271917135e-05
30.7021816777877	1.13407062578335e-05
30.8043678987539	1.06799299850532e-05
30.9109059456037	9.97061828293003e-06
31.0174439924534	9.24773116414274e-06
31.1239820393031	8.51851877830593e-06
31.2305200861528	7.79011102339321e-06
31.3364021990683	7.07388440276520e-06
31.4422843119837	6.37197969489371e-06
31.5481664248991	5.69065672787981e-06
31.6540485378145	5.03577652343836e-06
31.7574284840790	4.42711591049317e-06
31.8608084303435	3.85355324020586e-06
31.9641883766080	3.31924955170349e-06
32.0675683228725	2.82784187302548e-06
32.1722735824859	2.37706382442159e-06
32.2769788420993	1.97621766163837e-06
32.3816841017127	1.62738575281308e-06
32.4863893613262	1.33204269179336e-06
32.5963585110375	1.08042031116754e-06
32.7063276607488	8.89146444182093e-07
32.8162968104602	7.57832342138005e-07
32.9262659601715	6.85418457588945e-07
33.0345223500676	6.70034667871325e-07
33.1427787399638	7.07895602336674e-07
33.2510351298599	7.96236529769054e-07
33.3592915197560	9.31834615413730e-07
33.4657809711845	1.10779751372080e-06
33.5722704226130	1.32208149361938e-06
33.6787598740416	1.57048512466932e-06
33.7852493254701	1.84859917158378e-06
33.8941979357818	2.15909775651419e-06
34.0031465460936	2.49073006855835e-06
34.1120951564054	2.83824251293870e-06
34.2210437667172	3.19642115862922e-06
34.3366404896276	3.58236444323497e-06
34.4522372125380	3.96830851391388e-06
34.5678339354484	4.34824951641296e-06
34.6834306583588	4.71655841793893e-06
34.7936642990230	5.05209952965749e-06
34.9038979396873	5.36786242478094e-06
35.0141315803515	5.65983558734181e-06
35.1243652210157	5.92449491177444e-06
35.2343050512079	6.15818527569157e-06
35.3442448814002	6.35893109831978e-06
35.4541847115924	6.52449748913377e-06
35.5641245417846	6.65321168821057e-06
35.6786017627846	6.74682827108409e-06
35.7930789837846	6.79837793338217e-06
35.9075562047846	6.80757882107397e-06
36.0220334257847	6.77479043013962e-06
36.1362198980123	6.70117624233068e-06
36.2504063702399	6.58804638433955e-06
36.3645928424676	6.43721690839583e-06
36.4787793146952	6.25100097602984e-06
36.5900126053583	6.03818392804540e-06
36.7012458960214	5.79719584506501e-06
36.8124791866845	5.53111591342424e-06
36.9237124773476	5.24328081721498e-06
37.0369057108861	4.93169992243648e-06
37.1500989444246	4.60513572934230e-06
37.2632921779630	4.26753508417442e-06
37.3764854115015	3.92289801397265e-06
37.4962218645145	3.55513090279906e-06
37.6159583175275	3.18868205597574e-06
37.7356947705405	2.82807618622079e-06
37.8554312235534	2.47764158466124e-06
37.9694000931710	2.15729328792441e-06
38.0833689627887	1.85319125378269e-06
38.1973378324063	1.56833191980959e-06
38.3113067020239	1.30538808324127e-06
38.4249000672874	1.06745624774583e-06
38.5384934325510	8.55626626712743e-07
38.6520867978146	6.71493269612230e-07
38.7656801630782	5.16260374881637e-07
38.8839805724880	3.86208296055160e-07
39.0022809818979	2.88900507176526e-07
39.1205813913078	2.24357573927008e-07
39.2388818007176	1.92163483401206e-07
39.3577858169091	1.91571357311055e-07
39.4766898331005	2.21562962888773e-07
39.5955938492920	2.80475229212055e-07
39.7144978654834	3.66317863492956e-07
39.8306400259012	4.73975458380011e-07
39.9467821863190	6.02712873493618e-07
40.0629243467368	7.49884563643906e-07
40.1790665071546	9.12709514261412e-07
40.2979626814797	1.09258416409411e-06
40.4168588558048	1.28254715394003e-06
40.5357550301298	1.47927313064383e-06
40.6546512044549	1.67948909486197e-06
40.7793663330114	1.88974507259767e-06
40.9040814615679	2.09658463961558e-06
41.0287965901244	2.29645309208144e-06
41.1535117186809	2.48608597805118e-06
41.2728913030736	2.65524561895401e-06
41.3922708874662	2.80978564338590e-06
41.5116504718589	2.94750454558197e-06
41.6310300562516	3.06656146279583e-06
41.7513824171239	3.16616184938317e-06
41.8717347779962	3.24394879924347e-06
41.9920871388686	3.29897134433878e-06
42.1124394997409	3.33069093911529e-06
42.2403780838680	3.33867090681410e-06
42.3683166679951	3.32025695675776e-06
42.4962552521223	3.27600171621525e-06
42.6241938362494	3.20693139204184e-06
42.7459262128924	3.11947022755326e-06
42.8676585895354	3.01228604400534e-06
42.9893909661784	2.88709251808225e-06
43.1111233428215	2.74585763230759e-06
43.2323192820888	2.59146458391975e-06
43.3535152213561	2.42559887608218e-06
43.4747111606234	2.25063769163592e-06
43.5959070998906	2.06904814257013e-06
43.7230100636943	1.87423810150820e-06
43.8501130274980	1.67782368007410e-06
43.9772159913017	1.48265148647662e-06
44.1043189551053	1.29148404721026e-06
44.2286927690341	1.11084749408364e-06
44.3530665829628	9.38926462949186e-07
44.4774403968915	7.77856415701812e-07
44.6018142108202	6.29553930159278e-07
44.7243832234717	4.97544648875896e-07
44.8469522361232	3.80972441102945e-07
44.9695212487747	2.80953435625455e-07
45.0920902614261	1.98331654962482e-07
45.2192704569313	1.31612953226938e-07
45.3464506524364	8.45937208074900e-08
45.4736308479415	5.72835664114048e-08
45.6008110434466	4.93867104112459e-08
45.7293487437304	6.05385622046815e-08
45.8578864440142	9.00218911630350e-08
45.9864241442980	1.36650728828204e-07
46.1149618445818	1.99012692415778e-07
46.2403633884128	2.73470134150994e-07
46.3657649322439	3.59654600188287e-07
46.4911664760749	4.55720289789184e-07
46.6165680199060	5.59745610323184e-07
46.7458183814916	6.73195200277140e-07
46.8750687430772	7.90712007580243e-07
47.0043191046628	9.10013121966740e-07
47.1335694662484	1.02889272212185e-06
47.2659682689327	1.14800608065591e-06
47.3983670716170	1.26217586623096e-06
47.5307658743013	1.36928904121688e-06
47.6631646769855	1.46747118891582e-06
47.7913492952116	1.55245281175639e-06
47.9195339134376	1.62612234160683e-06
48.0477185316636	1.68732734760857e-06
48.1759031498897	1.73519649325441e-06
48.3075614879101	1.76982902607364e-06
48.4392198259305	1.78926109118716e-06
48.5708781639510	1.79329368681587e-06
48.7025365019714	1.78204653513415e-06
48.8366959423393	1.75527493405903e-06
48.9708553827072	1.71366581035514e-06
49.1050148230751	1.65808981120317e-06
49.2391742634430	1.58968477153505e-06
49.3688501639382	1.51264279580212e-06
49.4985260644335	1.42622121101323e-06
49.6282019649287	1.33188730979374e-06
49.7578778654240	1.23122318147026e-06
49.8184083990680	1.18253744377266e-06
49.8789389327120	1.13300495829920e-06
49.9394694663560	1.08279881456360e-06
50	1.03209245877871e-06

==> matlab/fig2d1.tex <==
0.0100000000000000	0.500000000000000
0.0179621434110699	0.499999792809844
0.0259242868221399	0.499998322254717
0.0338864302332098	0.499994720970776
0.0418485736442798	0.499988315144213
0.0489549209391593	0.499979663878497
0.0560612682340389	0.499967854634410
0.0631676155289185	0.499952542114077
0.0702739628237981	0.499933414398371
0.0834365541784869	0.499886950497509
0.0965991455331757	0.499824780855124
0.109761736887865	0.499745525468714
0.122924328242553	0.499647997112988
0.141422220690948	0.499478048690892
0.159920113139343	0.499267426850824
0.178418005587737	0.499014112944478
0.196915898036132	0.498716467330314
0.219013608897574	0.498300879615762
0.241111319759016	0.497818214497711
0.263209030620457	0.497267131830820
0.285306741481899	0.496646702673129
0.309342274650222	0.495892396969103
0.333377807818544	0.495054882816158
0.357413340986866	0.494134133599780
0.381448874155189	0.493130441656833
0.406933021704955	0.491976256876464
0.432417169254721	0.490730336667215
0.457901316804488	0.489393871682093
0.483385464354254	0.487968277531135
0.510146684095585	0.486377034985848
0.536907903836916	0.484691272798613
0.563669123578246	0.482913199214998
0.590430343319577	0.481045168287741
0.618396556862693	0.478999565772613
0.646362770405808	0.476861326203468
0.674328983948924	0.474633481195526
0.702295197492039	0.472319142278731
0.731440138666079	0.469818628949842
0.760585079840118	0.467231239704686
0.789730021014158	0.464560654448298
0.818874962188198	0.461810577362548
0.849202310632316	0.458868521835913
0.879529659076434	0.455848581172928
0.909857007520552	0.452754927376477
0.940184355964671	0.449591708893134
0.971722764316052	0.446232800987334
1.00326117266743	0.442807677536034
1.03479958101881	0.439320862882534
1.06633798937020	0.435776815916497
1.09914059673297	0.432034696916075
1.13194320409574	0.428240244934194
1.16474581145851	0.424398210574330
1.19754841882128	0.420513241570856
1.23169524674606	0.416428342671295
1.26584207467084	0.412306821787995
1.29998890259562	0.408153540611825
1.33413573052039	0.403973223846289
1.36973897643827	0.399590765474423
1.40534222235615	0.395188923506653
1.44094546827402	0.390772563622591
1.47654871419190	0.386346382659299
1.51333148231955	0.381768050440000
1.55011425044721	0.377188857303637
1.58689701857486	0.372613410529766
1.62367978670251	0.368046127076731
1.66101214689026	0.363423287180060
1.69834450707800	0.358817418226876
1.73567686726574	0.354232539140179
1.77300922745348	0.349672476304034
1.81093729414381	0.345068800168222
1.84886536083414	0.340498087223702
1.88679342752446	0.335963745101542
1.92472149421479	0.331468991192489
1.96329948808217	0.326940947818021
2.00187748194955	0.322459966852297
2.04045547581692	0.318028835266129
2.07903346968430	0.313650155553440
2.11832628074299	0.309246759443185
2.15761909180168	0.304902632687035
2.19691190286036	0.300619942064245
2.23620471391905	0.296400678365783
2.27628788215811	0.292163778988533
2.31637105039716	0.287996496981599
2.35645421863622	0.283900385846104
2.39653738687527	0.279876833840097
2.43749810706159	0.275841421836768
2.47845882724791	0.271884168835787
2.51941954743422	0.268006026184463
2.56038026762054	0.264207792712406
2.60231930174224	0.260402307561098
2.64425833586394	0.256681780595931
2.68619736998564	0.253046574819716
2.72813640410734	0.249496915291189
2.77117099359047	0.245943544084049
2.81420558307360	0.242480258610185
2.85724017255673	0.239106848917679
2.90027476203986	0.235822983519577
2.94454280820470	0.232537944769921
2.98881085436955	0.229346522831971
3.03307890053439	0.226247950885593
3.07734694669924	0.223241358918662
3.12301296380697	0.220235166432029
3.16867898091470	0.217324603650714
3.21434499802243	0.214508362844984
3.26001101513015	0.211785053589954
3.30727473639622	0.209062754194430
3.35453845766229	0.206436660299336
3.40180217892835	0.203904938165064
3.44906590019442	0.201465694379865
3.49817508767041	0.199027069281281
3.54728427514641	0.196683872816204
3.59639346262241	0.194433757814694
3.64550265009840	0.192274343573864
3.69677296104368	0.190114054239839
3.74804327198896	0.188047153484065
3.79931358293424	0.186070788991768
3.85058389387952	0.184182105104600
3.90443140626832	0.182289745273250
3.95827891865712	0.180487569047833
4.01212643104593	0.178772219504837
4.06597394343473	0.177140372147951
4.12210104024892	0.175524755532266
4.17822813706310	0.173992518799580
4.23435523387729	0.172539960823295
4.29048233069147	0.171163451708702
4.34732453072746	0.169843256203654
4.40416673076345	0.168593709580851
4.46100893079944	0.167411208911980
4.51785113083543	0.166292249414580
4.57582743647441	0.165212873413219
4.63380374211339	0.164192470003158
4.69178004775237	0.163227576134113
4.74975635339135	0.162314849853874
4.80927575174908	0.161428705256746
4.86879515010681	0.160590720383189
4.92831454846454	0.159797612888859
4.98783394682227	0.159046241725289
5.04934227097890	0.158310413549201
5.11085059513554	0.157612726788211
5.17235891929218	0.156950119688470
5.23386724344882	0.156319690011370
5.29789405007311	0.155694660901078
5.36192085669741	0.155098539748303
5.42594766332170	0.154528525210567
5.48997446994599	0.153981992288560
5.55719875822752	0.153430742634666
5.62442304650904	0.152899975004020
5.69164733479056	0.152387189811938
5.75887162307208	0.151890079818080
5.83023614825156	0.151377130453380
5.90160067343103	0.150877086246661
5.97296519861051	0.150387795169661
6.04432972378998	0.149907313462805
6.12127947749308	0.149397087628058
6.19822923119618	0.148893090038643
6.27517898489927	0.148393572813120
6.35212873860237	0.147897013589553
6.43723247735917	0.147349700814545
6.52233621611597	0.146802880188908
6.60743995487277	0.146255292934492
6.69254369362957	0.145705928040973
6.78171540330365	0.145127542643552
6.87088711297772	0.144545675742204
6.96005882265180	0.143959873097400
7.04923053232588	0.143369873804437
7.14466391282726	0.142733701850126
7.24009729332864	0.142092724183084
7.33553067383002	0.141447199413513
7.43096405433140	0.140797520728755
7.53934576535893	0.140055311753345
7.64772747638647	0.139309340803040
7.75610918741400	0.138560643025230
7.86449089844153	0.137810316511689
7.96911887225926	0.137085517812475
8.07374684607698	0.136361370136197
8.17837481989470	0.135638950793249
8.28300279371242	0.134919304942303
8.38717830981286	0.134206536204663
8.49135382591330	0.133498503301468
8.59552934201374	0.132796119992181
8.69970485811419	0.132100228274801
8.80416336793757	0.131409744851604
8.90862187776095	0.130727286086533
9.01308038758434	0.130053485978558
9.11753889740773	0.129388896783857
9.21807327203068	0.128758417023823
9.31860764665363	0.128137265608466
9.41914202127658	0.127525729837104
9.51967639589953	0.126924035862251
9.61962880891270	0.126335747253867
9.71958122192588	0.125757452952098
9.81953363493905	0.125189201132240
9.91948604795222	0.124630996062706
10.0207435189413	0.124075706834168
10.1220009899305	0.123530592382818
10.2232584609196	0.122995519807503
10.3245159319087	0.122470328928615
10.4283846120172	0.121941663927036
10.5322532921256	0.121422950731298
10.6361219722340	0.120913920561355
10.7399906523424	0.120414294101795
10.8475748287719	0.119906397396893
10.9551590052014	0.119407918722433
11.0627431816309	0.118918496617042
11.1703273580604	0.118437775692501
11.2826122346865	0.117944947372114
11.3948971113127	0.117460791795863
11.5071819879388	0.116984899732704
11.6194668645650	0.116516883614756
11.7372536318931	0.116033992799858
11.8550403992212	0.115558925066573
11.9728271665493	0.115091270848053
12.0906139338774	0.114630655121526
12.2143018181317	0.114154157652718
12.3379897023860	0.113684640650291
12.4616775866403	0.113221741188948
12.5853654708946	0.112765138494064
12.7146136383583	0.112294425491973
12.8438618058221	0.111829958910560
12.9731099732858	0.111371459702502
13.1023581407496	0.110918690710952
13.2358862805105	0.110456729640862
13.3694144202714	0.110000454428651
13.5029425600323	0.109549683088658
13.6364706997933	0.109104267196237
13.7724345754501	0.108656102530340
13.9083984511069	0.108213241935287
14.0443623267637	0.107775582835407
14.1803262024205	0.107343043820892
14.3171940356473	0.106912733849982
14.4540618688741	0.106487479116810
14.5909297021008	0.106067220963326
14.7277975353276	0.105651910981314
14.8649284638827	0.105240723377728
15.0020593924377	0.104834413484321
15.1391903209927	0.104432934161742
15.2763212495477	0.104036241915043
15.4138654423835	0.103643120609384
15.5514096352193	0.103254720787726
15.6889538280551	0.102870987597645
15.8264980208909	0.102491867320876
15.9650100243167	0.102114686125420
16.1035220277425	0.101742061404824
16.2420340311683	0.101373923602540
16.3805460345941	0.101010204534448
16.5206781669815	0.100646657790317
16.6608102993689	0.100287482180832
16.8009424317563	0.0999325945108416
16.9410745641437	0.0995819146218370
17.0834062487309	0.0992299565390026
17.2257379333181	0.0988821661891003
17.3680696179053	0.0985384521207450
17.5104013024924	0.0981987279759669
17.6553488510412	0.0978567746907189
17.8002963995899	0.0975187779508055
17.9452439481386	0.0971846449123346
18.0901914966873	0.0968542895272800
18.2379619557187	0.0965213048019519
18.3857324147501	0.0961920702483390
18.5335028737815	0.0958664978171474
18.6812733328129	0.0955445071458405
18.8318594722471	0.0952199885437138
18.9824456116813	0.0948990288009012
19.1330317511155	0.0945815486749219
19.2836178905498	0.0942674765548313
19.4368432212972	0.0939513301110387
19.5900685520447	0.0936385713644764
19.7432938827921	0.0933291310932221
19.8965192135396	0.0930229468871754
20.0521273153262	0.0927152749128031
20.2077354171128	0.0924108392220147
20.3633435188993	0.0921095794100219
20.5189516206859	0.0918114406876590
20.6767074948662	0.0915123213198654
20.8344633690465	0.0912163024833661
20.9922192432268	0.0909233300874192
21.1499751174070	0.0906333544902657
21.3097363309718	0.0903426999555380
21.4694975445366	0.0900550207182695
21.6292587581014	0.0897702664446044
21.7890199716662	0.0894883903759289
21.9507550228406	0.0892059188673962
22.1124900740149	0.0889263038096986
22.2742251251893	0.0886494968471846
22.4359601763636	0.0883754526873888
22.5997219235879	0.0881007459930932
22.7634836708122	0.0878287810658493
22.9272454180365	0.0875595107723796
23.0910071652607	0.0872928908128751
23.2568857402592	0.0870254838791171
23.4227643152578	0.0867607077490694
23.5886428902563	0.0864985165754173
23.7545214652548	0.0862388672531556
23.9225997668194	0.0859783260815282
24.0906780683841	0.0857203091191062
24.2587563699487	0.0854647722838194
24.4268346715134	0.0852116741480342
24.5971602465273	0.0849576403342055
24.7674858215413	0.0847060294275061
24.9378113965552	0.0844567996137464
25.1081369715692	0.0842099115650971
25.2807146345169	0.0839621101963881
25.4532922974645	0.0837166363079946
25.6258699604122	0.0834734506273191
25.7984476233598	0.0832325160998006
25.9732496005806	0.0829907360367966
26.1480515778014	0.0827511938911311
26.3228535550222	0.0825138529054056
26.4976555322430	0.0822786782009098
26.6746407580550	0.0820427403040042
26.8516259838669	0.0818089561113864
27.0286112096789	0.0815772911294816
27.2055964354908	0.0813477123831405
27.3847291106506	0.0811174412806769
27.5638617858103	0.0808892442851461
27.7429944609701	0.0806630888317282
27.9221271361299	0.0804389435360639
28.1033873526667	0.0802141525745407
28.2846475692035	0.0799913600661864
28.4659077857403	0.0797705350820713
28.6471680022771	0.0795516475786902
28.8305524749318	0.0793321381655812
29.0139369475864	0.0791145550426496
29.1973214202411	0.0788988687293699
29.3807058928957	0.0786850503759654
29.5662216026754	0.0784706205262982
29.7517373124551	0.0782580480693709
29.9372530222348	0.0780473048879105
30.1227687320145	0.0778383632648922
30.3104244405387	0.0776288181489048
30.4980801490630	0.0774210647074466
30.6857358575872	0.0772150761607142
30.8733915661115	0.0770108259050212
31.0631915046256	0.0768059849667162
31.2529914431398	0.0766028731064162
31.4427913816539	0.0764014648662067
31.6325913201681	0.0762017347354268
31.8245330634793	0.0760014333877221
32.0164748067905	0.0758028015404333
32.2084165501018	0.0756058150206432
32.4003582934130	0.0754104493670078
32.5944343723426	0.0752145363393953
32.7885104512723	0.0750202360881082
32.9825865302019	0.0748275256603358
33.1766626091316	0.0746363815766619
33.3728638888244	0.0744447145337449
33.5690651685172	0.0742546061941680
33.7652664482099	0.0740660347437304
33.9614677279027	0.0738789776070414
34.1597863981921	0.0736914195044819
34.3581050684815	0.0735053684836316
34.5564237387709	0.0733208037876345
34.7547424090604	0.0731377036715821
34.9551733102377	0.0729541210857291
35.1556042114151	0.0727719962421913
35.3560351125925	0.0725913093722812
35.5564660137699	0.0724120395009041
35.7590062381233	0.0722323027890640
35.9615464624766	0.0720539766301405
36.1640866868299	0.0718770421894132
36.3666269111833	0.0717014792141688
36.5712744813487	0.0715254635466300
36.7759220515142	0.0713508132865677
36.9805696216796	0.0711775104899387
37.1852171918451	0.0710055355874086
37.3919698016115	0.0708331218423715
37.5987224113779	0.0706620303077142
37.8054750211443	0.0704922438914188
38.0122276309107	0.0703237436714201
38.2210820628669	0.0701548186510310
38.4299364948231	0.0699871744961986
38.6387909267793	0.0698207949284405
38.8476453587355	0.0696556616365324
39.0585976322966	0.0694901176260566
39.2695499058576	0.0693258148896851
39.4805021794187	0.0691627379229572
39.6914544529798	0.0690008689884739
39.9045003567214	0.0688386030197208
40.1175462604631	0.0686775403890074
40.3305921642047	0.0685176663266181
40.5436380679464	0.0683589636328607
40.7587736492092	0.0681998768345832
40.9739092304720	0.0680419570016781
41.1890448117348	0.0678851900620387
41.4041803929976	0.0677295593200419
41.6214021542161	0.0675735565478175
41.8386239154346	0.0674186858484425
42.0558456766532	0.0672649338135454
42.2730674378717	0.0671122842210857
42.4923722413425	0.0669592739379364
42.7116770448134	0.0668073622402896
42.9309818482842	0.0666565363528510
43.1502866517551	0.0665067804995031
43.3716714967573	0.0663566747589517
43.5930563417596	0.0662076354527466
43.8144411867618	0.0660596504104477
44.0358260317640	0.0659127042762433
44.2592878797955	0.0657654186690940
44.4827497278270	0.0656191686160816
44.7062115758585	0.0654739425250083
44.9296734238900	0.0653297254361310
45.1552091541436	0.0651851789463340
45.3807448843971	0.0650416383388578
45.6062806146507	0.0648990925743081
45.8318163449043	0.0647575270658818
46.0594228148368	0.0646156418621280
46.2870292847694	0.0644747340175142
46.5146357547020	0.0643347930211574
46.7422422246345	0.0641958046372237
46.9719163573238	0.0640565058595491
47.2015904900131	0.0639181570100527
47.4312646227023	0.0637807480833779
47.6609387553916	0.0636442651739816
47.8926775894859	0.0635074807581585
48.1244164235803	0.0633716198790042
48.3561552576747	0.0632366730151149
48.5878940917691	0.0631026265718972
48.8216947775496	0.0629682871186740
49.0554954633302	0.0628348458007749
49.2892961491107	0.0627022935605395
49.5230968348912	0.0625706170962282
49.6423226261684	0.0625038022006233
49.7615484174456	0.0624372114643348
49.8807742087228	0.0623708435784017
50	0.0623046972974247

==> matlab/fig2d2.tex <==
0.0100000000000000	0.500000000000000
0.0148893961920471	0.499999867658798
0.0197787923840941	0.499998905716276
0.0246681885761412	0.499996692161776
0.0295575847681883	0.499992985522694
0.0344469809602354	0.499987495925542
0.0393363771522824	0.499980067713750
0.0442257733443295	0.499970569223646
0.0491151695363766	0.499958894067777
0.0566647429666537	0.499936369911932
0.0642143163969308	0.499908124265310
0.0717638898272080	0.499873933488969
0.0793134632574851	0.499833619939293
0.0908118553010885	0.499760099541780
0.102310247344692	0.499671526601337
0.113808639388295	0.499567570354359
0.125307031431899	0.499447989440526
0.141369341375589	0.499254388653453
0.157431651319280	0.499029423147894
0.173493961262971	0.498772842031240
0.189556271206662	0.498484526170165
0.209054765188173	0.498091763085818
0.228553259169684	0.497652060392903
0.248051753151195	0.497165551187059
0.267550247132706	0.496632485993618
0.290054092995263	0.495959748815752
0.312557938857820	0.495225869483782
0.335061784720377	0.494431487641689
0.357565630582934	0.493577333167279
0.382022894637376	0.492582123670339
0.406480158691819	0.491518196566860
0.430937422746262	0.490386640776901
0.455394686800704	0.489188599743799
0.481569771421338	0.487834058578642
0.507744856041972	0.486406111219625
0.533919940662606	0.484906241387815
0.560095025283240	0.483335961213669
0.587815541450838	0.481597875148993
0.615536057618436	0.479784311634240
0.643256573786034	0.477897100192202
0.670977089953632	0.475938079161083
0.700118255075150	0.473803237808245
0.729259420196668	0.471593179842295
0.758400585318186	0.469310038699580
0.787541750439704	0.466955941311035
0.818002822213866	0.464421654961080
0.848463893988028	0.461814545557060
0.878924965762190	0.459137011683047
0.909386037536352	0.456391432800910
0.941083529314273	0.453464698375264
0.972781021092195	0.450469474641449
1.00447851287012	0.447408387538813
1.03617600464804	0.444284032937089
1.06904120797423	0.440980512516143
1.10190641130043	0.437614576615924
1.13477161462662	0.434189040567336
1.16763681795282	0.430706679672180
1.20161504757622	0.427049548466477
1.23559327719962	0.423337607489096
1.26957150682302	0.419573822840340
1.30354973644643	0.415761111172123
1.33860026934466	0.411779847675458
1.37365080224289	0.407752700588287
1.40870133514113	0.403682747386938
1.44375186803936	0.399573006929581
1.47984820246859	0.395302188758392
1.51594453689782	0.390995525310550
1.55204087132705	0.386656165341928
1.58813720575629	0.382287189885365
1.62526753796055	0.377765343604044
1.66239787016482	0.373218603103085
1.69952820236909	0.368650147735359
1.73665853457335	0.364063079976654
1.77482648733532	0.359331615991833
1.81299444009729	0.354586936006192
1.85116239285926	0.349832208777498
1.88933034562123	0.345070516914158
1.92855606837490	0.340172764496587
1.96778179112857	0.335274033474713
2.00700751388225	0.330377440282968
2.04623323663592	0.325486005772835
2.08655507259207	0.320466349951762
2.12687690854821	0.315458364770981
2.16719874450436	0.310465071896853
2.20752058046051	0.305489387785928
2.24899759325488	0.300392499339485
2.29047460604925	0.295320218875166
2.33195161884362	0.290275429741016
2.37342863163800	0.285260900221752
2.41614443981355	0.280131041195598
2.45886024798911	0.275038919086602
2.50157605616466	0.269987233592016
2.54429186434021	0.264978559218412
2.58836050906038	0.259858937128283
2.63242915378054	0.254790308977801
2.67649779850070	0.249775142599604
2.72056644322086	0.244815770158774
2.76614153781910	0.239747900203602
2.81171663241733	0.234744388928743
2.85729172701556	0.229807419437201
2.90286682161380	0.224939028212187
2.94925709579494	0.220055950968133
2.99564736997608	0.215247778811164
3.04203764415721	0.210516250567172
3.08842791833835	0.205862958744022
3.13504806192754	0.201266897821604
3.18166820551672	0.196752679091196
3.22828834910590	0.192321524402865
3.27490849269509	0.187974519035358
3.32184817451336	0.183683704639777
3.36878785633164	0.179480027479181
3.41572753814992	0.175364220456474
3.46266721996820	0.171336889951534
3.51002497981212	0.167363846097465
3.55738273965604	0.163481745096768
3.60474049949997	0.159690856620275
3.65209825934389	0.155991334227411
3.69997786202684	0.152343971995149
3.74785746470979	0.148789982565349
3.79573706739275	0.145329195671140
3.84361667007570	0.141961335846786
3.89212998835124	0.138643295136181
3.94064330662678	0.135419780358165
3.98915662490232	0.132290202624944
4.03766994317786	0.129253879406579
4.08694045495193	0.126264819527048
4.13621096672600	0.123370249371202
4.18548147850007	0.120569181047203
4.23475199027414	0.117860545382741
4.28491921268052	0.115196397925808
4.33508643508690	0.112625593221436
4.38525365749328	0.110146762410430
4.43542087989966	0.107758468713182
4.48664627573137	0.105411658758258
4.53787167156309	0.103156005231133
4.58909706739480	0.100989774708525
4.64032246322651	0.0989111804524935
4.69279768899344	0.0968708182018717
4.74527291476036	0.0949184520970914
4.79774814052728	0.0930519986428221
4.85022336629421	0.0912693372141952
4.90418235407362	0.0895213779893635
4.95814134185303	0.0878573407003197
5.01210032963244	0.0862748037413417
5.06605931741185	0.0847713266157817
5.12179691896912	0.0832986912208279
5.17753452052639	0.0819050443976982
5.23327212208366	0.0805876346533480
5.28900972364093	0.0793437126074120
5.34691229243864	0.0781263493542293
5.40481486123634	0.0769822311177728
5.46271743003406	0.0759082786614598
5.52061999883177	0.0749014397673952
5.58121953325118	0.0739162863660052
5.64181906767059	0.0729978658478573
5.70241860209001	0.0721427625312442
5.76301813650942	0.0713476185297139
5.82511460237858	0.0705915749154284
5.88721106824774	0.0698914995324263
5.94930753411689	0.0692439475289600
6.01140399998605	0.0686455599227400
6.07380159490291	0.0680904833483658
6.13619918981976	0.0675784691679267
6.19859678473662	0.0671063437525908
6.26099437965347	0.0666710368913038
6.32419436949673	0.0662646190386809
6.38739435933999	0.0658899116160134
6.45059434918325	0.0655440160935648
6.51379433902651	0.0652241529342654
6.57830719489551	0.0649217232505074
6.64282005076451	0.0646408997905399
6.70733290663351	0.0643790714777323
6.77184576250251	0.0641337608212971
6.83824117080171	0.0638960597303390
6.90463657910091	0.0636709172231772
6.97103198740010	0.0634560309965805
7.03742739569930	0.0632492466635838
7.10642156558373	0.0630407900491041
7.17541573546816	0.0628367829296167
7.24440990535259	0.0626352625756283
7.31340407523702	0.0624344290939206
7.38600948734619	0.0622220173903029
7.45861489945535	0.0620067854025222
7.53122031156452	0.0617871552080254
7.60382572367369	0.0615617286372961
7.68169060479945	0.0613121339785762
7.75955548592521	0.0610531355399760
7.83742036705097	0.0607836149231430
7.91528524817673	0.0605026555324473
7.99490567291899	0.0602027743470568
8.07452609766125	0.0598895755489580
8.15414652240351	0.0595626462477412
8.23376694714577	0.0592217467128447
8.31391886159019	0.0588643815336451
8.39407077603461	0.0584928512527967
8.47422269047904	0.0581073669116328
8.55437460492346	0.0577082664657080
8.63687721049298	0.0572837218980680
8.71937981606250	0.0568458561562210
8.80188242163202	0.0563953927275159
8.88438502720155	0.0559331421353676
8.97139686058978	0.0554338398093585
9.05840869397802	0.0549235607545606
9.14542052736626	0.0544035100739222
9.23243236075449	0.0538749367747876
9.32093858739016	0.0533298728387351
9.40944481402583	0.0527787312851890
9.49795104066150	0.0522229253284525
9.58645726729716	0.0516638576006449
9.67248667547180	0.0511186325391207
9.75851608364644	0.0505729221852109
9.84454549182108	0.0500279714774222
9.93057489999572	0.0494849789125751
10.0166970837528	0.0489445201754220
10.1028192675098	0.0484083083364161
10.1889414512669	0.0478774081017134
10.2750636350240	0.0473528140381382
10.3632012635051	0.0468234422073252
10.4513388919862	0.0463025853094087
10.5394765204673	0.0457910966437030
10.6276141489484	0.0452897401388121
10.7197494921261	0.0447772134759019
10.8118848353039	0.0442771962570637
10.9040201784817	0.0437902777271253
10.9961555216594	0.0433169399714963
11.0865603570731	0.0428660642732240
11.1769651924869	0.0424289139052687
11.2673700279006	0.0420056791296147
11.3577748633143	0.0415964626090451
11.4470969932176	0.0412059361002367
11.5364191231210	0.0408290655011094
11.6257412530243	0.0404657304265533
11.7150633829276	0.0401157448828962
11.8051167656774	0.0397761576871247
11.8951701484272	0.0394495769900747
11.9852235311770	0.0391356388712763
12.0752769139267	0.0388339336213248
12.1675783486168	0.0385369185571988
12.2598797833068	0.0382517481253504
12.3521812179968	0.0379778574607084
12.4444826526868	0.0377146565521519
12.5406946243167	0.0374510217895287
12.6369065959466	0.0371976134133265
12.7331185675765	0.0369536980596093
12.8293305392064	0.0367185410408878
12.9317611576690	0.0364769854872082
13.0341917761316	0.0362436306128712
13.1366223945942	0.0360176007698378
13.2390530130568	0.0357980496004829
13.3436694630454	0.0355796499268035
13.4482859130340	0.0353663033323865
13.5529023630227	0.0351572043988348
13.6575188130113	0.0349516026803267
13.7639378760502	0.0347453247411298
13.8703569390891	0.0345412491417454
13.9767760021280	0.0343387474864895
14.0831950651669	0.0341372614437525
14.1948918891323	0.0339263360237205
14.3065887130976	0.0337154792959360
14.4182855370630	0.0335042654842920
14.5299823610283	0.0332923521103419
14.6523445390369	0.0330590871279886
14.7747067170456	0.0328244034205496
14.8970688950542	0.0325881411480107
15.0194310730629	0.0323502381130182
15.1511465632349	0.0320923452346281
15.2828620534069	0.0318327098382941
15.4145775435789	0.0315715539034204
15.5462930337509	0.0313091789570798
15.6816426907559	0.0310386838225697
15.8169923477609	0.0307677637370535
15.9523420047659	0.0304969332372991
16.0876916617709	0.0302267303214503
16.2195694981085	0.0299645934048945
16.3514473344461	0.0297041184531168
16.4833251707836	0.0294458313572971
16.6152030071212	0.0291902315532315
16.7409056818706	0.0289495382537724
16.8666083566200	0.0287121195203650
16.9923110313695	0.0284783389862351
17.1180137061189	0.0282485159852769
17.2460071843381	0.0280188603135682
17.3740006625573	0.0277938614559892
17.5019941407765	0.0275737318432872
17.6299876189957	0.0273586283221022
17.7565892512773	0.0271509147833578
17.8831908835589	0.0269482921751560
18.0097925158406	0.0267507803698062
18.1363941481222	0.0265583523962983
18.2599448561665	0.0263753990264984
18.3834955642107	0.0261971296550673
18.5070462722549	0.0260234181927516
18.6305969802992	0.0258541097386069
18.7553803779988	0.0256873984964501
18.8801637756984	0.0255247884103805
19.0049471733980	0.0253660546074768
19.1297305710976	0.0252109593979123
19.2592552219338	0.0250535545591668
19.3887798727700	0.0248995153605796
19.5183045236062	0.0247485521806727
19.6478291744424	0.0246003796842734
19.7861929856835	0.0244448625629452
19.9245567969247	0.0242918746797333
20.0629206081659	0.0241410976559802
20.2012844194070	0.0239922379184695
20.3511564871112	0.0238328481416023
20.5010285548154	0.0236750750789262
20.6509006225196	0.0235186429155155
20.8007726902238	0.0233633228086976
20.9588361116552	0.0232005134506992
21.1168995330866	0.0230385588079330
21.2749629545180	0.0228773360983235
21.4330263759494	0.0227167754750816
21.6190635682705	0.0225286163333691
21.8051007605917	0.0223413757848374
21.9911379529128	0.0221551552677366
22.1771751452340	0.0219701120363780
22.3458199885345	0.0218035548891824
22.5144648318351	0.0216383130964245
22.6831096751357	0.0214745793599736
22.8517545184363	0.0213125449491571
23.0203993617369	0.0211523995343441
23.1890442050374	0.0209943390865808
23.3576890483380	0.0208385416659290
23.5263338916386	0.0206851568965140
23.6920944741673	0.0205368694179729
23.8578550566961	0.0203911451242561
24.0236156392249	0.0202480634602405
24.1893762217536	0.0201076686023320
24.3482102075099	0.0199756767788553
24.5070441932662	0.0198461675565277
24.6658781790225	0.0197191162393243
24.8247121647788	0.0195944736576909
24.9797169326094	0.0194750935677505
25.1347217004401	0.0193578687881366
25.2897264682707	0.0192427110331234
25.4447312361014	0.0191295203212725
25.6022628713019	0.0190163886084785
25.7597945065025	0.0189050587901983
25.9173261417030	0.0187954090148821
26.0748577769036	0.0186873170556712
26.2399748574646	0.0185755612448300
26.4050919380255	0.0184652497994455
26.5702090185865	0.0183562553511019
26.7353260991475	0.0182484613173554
26.9135866885254	0.0181333134892477
27.0918472779033	0.0180193251607048
27.2701078672812	0.0179063978529429
27.4483684566591	0.0177944538456721
27.6461875512081	0.0176713083305308
27.8440066457571	0.0175492507813625
28.0418257403061	0.0174282561200522
28.2396448348551	0.0173083228290959
28.4582261869192	0.0171770588936649
28.6768075389832	0.0170471742709142
28.8953888910472	0.0169187458150410
29.1139702431113	0.0167918534577623
29.3320751105215	0.0166668524133211
29.5501799779317	0.0165435664996738
29.7682848453419	0.0164220855665293
29.9863897127521	0.0163024732979709
30.1847014566922	0.0161953782919295
30.3830132006322	0.0160899060410204
30.5813249445722	0.0159860754851931
30.7796366885122	0.0158838831906910
30.9653208272272	0.0157896674414473
31.1510049659422	0.0156968555645052
31.3366891046572	0.0156054180444730
31.5223732433722	0.0155153130645180
31.7057580297484	0.0154275836832777
31.8891428161245	0.0153410577094904
32.0725276025007	0.0152556812686023
32.2559123888769	0.0151713961433861
32.4435767931044	0.0150862120399438
32.6312411973319	0.0150020483114881
32.8189056015594	0.0149188457056847
33.0065700057869	0.0148365473281074
33.2035317736837	0.0147510868827908
33.4004935415806	0.0146665126601408
33.5974553094774	0.0145827792827423
33.7944170773742	0.0144998482695499
34.0042348370502	0.0144123525635211
34.2140525967261	0.0143257096798893
34.4238703564021	0.0142399051964544
34.6336881160780	0.0141549310358161
34.8550217447865	0.0140661918963702
35.0763553734949	0.0139783899268201
35.2976890022033	0.0138915430451383
35.5190226309117	0.0138056670631467
35.7420476120856	0.0137201335765757
35.9650725932595	0.0136356302528553
36.1880975744334	0.0135521792038424
36.4111225556072	0.0134697909668388
36.6266455989052	0.0133911882337143
36.8421686422032	0.0133135917987833
37.0576916855012	0.0132370019321756
37.2732147287991	0.0131614069176233
37.4822671682508	0.0130890150110700
37.6913196077025	0.0130175288314108
37.9003720471542	0.0129469281838328
38.1094244866059	0.0128771853856993
38.3178434323715	0.0128084772936480
38.5262623781370	0.0127405644999740
38.7346813239026	0.0126734174647636
38.9431002696682	0.0126070038316918
39.1562974204122	0.0125397931279795
39.3694945711562	0.0124732883801324
39.5826917219003	0.0124074624240832
39.7958888726443	0.0123422886149263
40.0176196036804	0.0122751724384117
40.2393503347166	0.0122087183023972
40.4610810657527	0.0121429112415152
40.6828117967889	0.0120777374652252
40.9137026787675	0.0120105329363686
41.1445935607461	0.0119440024280665
41.3754844427247	0.0118781461034727
41.6063753247033	0.0118129622109370
41.8420837151137	0.0117471109698629
42.0777921055241	0.0116819684288061
42.3135004959345	0.0116175409130750
42.5492088863449	0.0115538280693372
42.7832701060807	0.0114912649859532
43.0173313258165	0.0114294086228755
43.2513925455524	0.0113682584235476
43.4854537652882	0.0113078055023665
43.7158897201435	0.0112489581733342
43.9463256749988	0.0111907688752183
44.1767616298541	0.0111332268924866
44.4071975847094	0.0110763151039790
44.6370374295381	0.0110201592543296
44.8668772743667	0.0109645980882889
45.0967171191954	0.0109096157668056
45.3265569640240	0.0108551928253785
45.5600731725287	0.0108004521436573
45.7935893810333	0.0107462551841234
46.0271055895379	0.0106925878438629
46.2606217980426	0.0106394342405551
46.5007803538022	0.0105852890857016
46.7409389095619	0.0105316641904293
46.9810974653215	0.0104785521707840
47.2212560210812	0.0104259437818556
47.4680943172735	0.0103723883341346
47.7149326134659	0.0103193564294675
47.9617709096582	0.0102668473898120
48.2086092058506	0.0102148566127517
48.4587788964316	0.0101626877813861
48.7089485870126	0.0101110494629758
48.9591182775936	0.0100599421644007
49.2092879681746	0.0100093602541161
49.4069659761309	0.00996975876940716
49.6046439840873	0.00993048109405348
49.8023219920436	0.00989152501848400
50	0.00985288666455278

==> matlab/fig2d3.tex <==
0.0100000000000000	0.500000000000000
0.0117160547237387	0.499999979488237
0.0134321094474774	0.499999837257519
0.0151481641712160	0.499999503536896
0.0168642188949547	0.499998938459117
0.0185802736186934	0.499998107211115
0.0202963283424321	0.499996990452119
0.0220123830661707	0.499995575546765
0.0237284377899094	0.499993854242857
0.0271767298921404	0.499989445141227
0.0306250219943713	0.499983730059953
0.0340733140966023	0.499976696873617
0.0375216061988333	0.499968345462058
0.0427139279135350	0.499953269212497
0.0479062496282368	0.499935174707478
0.0530985713429385	0.499914075495826
0.0582908930576403	0.499889994016472
0.0666867029016913	0.499844770400853
0.0750825127457423	0.499791792234740
0.0834783225897933	0.499731120417034
0.0918741324338443	0.499662830289267
0.103221374695157	0.499558497496685
0.114568616956470	0.499440392954568
0.125915859217783	0.499308622796517
0.137263101479095	0.499163308928541
0.152303542411290	0.498949976814886
0.167343983343484	0.498713160096279
0.182384424275678	0.498453049146518
0.197424865207872	0.498169855752454
0.216556218911177	0.497776559372998
0.235687572614481	0.497346499048152
0.254818926317785	0.496880009169615
0.273950280021090	0.496377450126598
0.295702700579699	0.495762627682904
0.317455121138309	0.495102018212687
0.339207541696919	0.494396075231999
0.360959962255528	0.493645270938376
0.384856456254013	0.492769281637823
0.408752950252498	0.491840252920593
0.432649444250983	0.490858767447967
0.456545938249468	0.489825420098383
0.482428909122220	0.488648335459119
0.508311879994973	0.487411809529081
0.534194850867725	0.486116580545907
0.560077821740478	0.484763394463563
0.587789573063889	0.483251189213067
0.615501324387300	0.481674296761938
0.643213075710712	0.480033635792937
0.670924827034123	0.478330129363607
0.700315973473582	0.476455736554325
0.729707119913042	0.474512792852689
0.759098266352501	0.472502419862654
0.788489412791960	0.470425740844823
0.819413129909566	0.468170425630168
0.850336847027172	0.465844282780043
0.881260564144777	0.463448654442879
0.912184281262383	0.460984881899205
0.944496310546559	0.458339152860175
0.976808339830736	0.455622053777342
1.00912036911491	0.452835158068795
1.04143239839909	0.449980035605539
1.07499283168995	0.446944057403975
1.10855326498080	0.443837975080659
1.14211369827166	0.440663595690631
1.17567413156251	0.437422719636967
1.21035017643711	0.434006176458787
1.24502622131171	0.430522597303279
1.27970226618631	0.426974016237558
1.31437831106091	0.423362456956074
1.35004735827022	0.419583898586321
1.38571640547953	0.415743091918069
1.42138545268884	0.411842282659146
1.45705449989815	0.407883701700172
1.49360694715890	0.403769476486950
1.53015939441965	0.399599363264921
1.56671184168041	0.395375796263943
1.60326428894116	0.391101189696273
1.64060574378950	0.386684114035967
1.67794719863784	0.382218890103295
1.71528865348618	0.377708111282707
1.75263010833452	0.373154345015371
1.79068279737963	0.368472267652402
1.82873548642474	0.363750941556428
1.86678817546984	0.358993085351509
1.90484086451495	0.354201385142591
1.94354426897741	0.349295781609054
1.98224767343986	0.344360760713123
2.02095107790232	0.339399129498318
2.05965448236477	0.334413655363857
2.09896535948022	0.329328347233104
2.13827623659567	0.324224163078783
2.17758711371112	0.319103960040931
2.21689799082656	0.313970548050528
2.25679001376257	0.308750598209997
2.29668203669857	0.303522817902091
2.33657405963457	0.298290075607391
2.37646608257057	0.293055184698928
2.41692934917714	0.287745983778018
2.45739261578371	0.282440318435461
2.49785588239028	0.277141030018712
2.53831914899685	0.271850896628511
2.57935979595430	0.266497431174793
2.62040044291174	0.261159028866353
2.66144108986919	0.255838466108293
2.70248173682663	0.250538447754097
2.74412187579687	0.245184727257211
2.78576201476712	0.239857625441943
2.82740215373736	0.234559816712781
2.86904229270760	0.229293895505751
2.91132048022032	0.223982510169790
2.95359866773304	0.218709218502443
2.99587685524576	0.213476556424163
3.03815504275849	0.208286971388959
3.08112752419896	0.203058752453487
3.12410000563943	0.197879937629306
3.16707248707990	0.192752888018122
3.21004496852037	0.187679867681979
3.25378802052889	0.182573624356449
3.29753107253741	0.177527871788557
3.34127412454594	0.172544759376860
3.38501717655446	0.167626330809449
3.42963104837956	0.162678640410249
3.47424492020467	0.157802271032821
3.51885879202977	0.152999121890320
3.56347266385488	0.148270977660001
3.60908796232704	0.143516006484563
3.65470326079919	0.138842929375146
3.70031855927135	0.134253353710538
3.74593385774351	0.129748763249278
3.79272190093334	0.125218092597480
3.83950994412316	0.120779673666807
3.88629798731299	0.116434774749383
3.93308603050281	0.112184530998125
3.98127611499785	0.107906950249117
4.02946619949289	0.103731870403129
4.07765628398793	0.0996601637890887
4.12584636848297	0.0956925593480640
4.17453782062043	0.0917900208493719
4.22322927275788	0.0879948900659781
4.27192072489534	0.0843075453589692
4.32061217703279	0.0807282251159111
4.36915150529233	0.0772677186410264
4.41769083355186	0.0739146850672565
4.46623016181140	0.0706690093590262
4.51476949007093	0.0675304497362613
4.56328105147248	0.0645003538474511
4.61179261287403	0.0615764439168497
4.66030417427557	0.0587581548138952
4.70881573567712	0.0560448078846189
4.75743034626171	0.0534301891469387
4.80604495684629	0.0509192977183509
4.85465956743088	0.0485111562405048
4.90327417801546	0.0462046871296483
4.95214759150491	0.0439872445779103
5.00102100499435	0.0418701090370127
5.04989441848379	0.0398519222634114
5.09876783197324	0.0379312391848793
5.14804659394740	0.0360917985288716
5.19732535592155	0.0343483004736852
5.24660411789571	0.0326990335993170
5.29588287986987	0.0311422135339944
5.34571691623879	0.0296599768031099
5.39555095260772	0.0282684120814156
5.44538498897664	0.0269654800707356
5.49521902534556	0.0257490831793035
5.54578533292858	0.0246010549778786
5.59635164051159	0.0235376112059389
5.64691794809460	0.0225564061305434
5.69748425567761	0.0216550514239421
5.74900092501619	0.0208163606945316
5.80051759435478	0.0200554266932172
5.85203426369337	0.0193696135285781
5.90355093303196	0.0187562598560043
5.95629904554016	0.0182005203568394
6.00904715804837	0.0177150282924265
6.06179527055658	0.0172968663548762
6.11454338306479	0.0169431110304922
6.16890437576226	0.0166428356013676
6.22326536845974	0.0164046463341303
6.27762636115721	0.0162253412547213
6.33198735385468	0.0161017347004401
6.38842448996247	0.0160289432660826
6.44486162607025	0.0160092422467937
6.50129876217804	0.0160391370151840
6.55773589828582	0.0161151769613243
6.61342964774346	0.0162321275005891
6.66912339720110	0.0163874597680139
6.72481714665874	0.0165779901573931
6.78051089611637	0.0168005971231801
6.83589971047198	0.0170507685479498
6.89128852482759	0.0173266804354493
6.94667733918320	0.0176254446771737
7.00206615353882	0.0179442498792818
7.05758976165192	0.0182811959817240
7.11311336976503	0.0186328409723957
7.16863697787814	0.0189965795088982
7.22416058599125	0.0193698959848454
7.28021693986213	0.0197540390778771
7.33627329373302	0.0201430514108079
7.39232964760390	0.0205346123751553
7.44838600147478	0.0209265033129900
7.50538574262213	0.0213231419419704
7.56238548376949	0.0217157961703490
7.61938522491684	0.0221024426554853
7.67638496606419	0.0224811720703587
7.73480587272738	0.0228592464408756
7.79322677939057	0.0232252869617947
7.85164768605376	0.0235775904265114
7.91006859271695	0.0239145802829146
7.97053387043690	0.0242456870171722
8.03099914815685	0.0245573462206568
8.09146442587680	0.0248482117066891
8.15192970359676	0.0251170782269251
8.21535952756943	0.0253743164570290
8.27878935154210	0.0256050824800954
8.34221917551477	0.0258084488930571
8.40564899948744	0.0259836472171920
8.46793784799597	0.0261276839899065
8.53022669650450	0.0262435104175795
8.59251554501303	0.0263308094141156
8.65480439352156	0.0263893950481565
8.71642204054983	0.0264190385814682
8.77803968757810	0.0264205798466747
8.83965733460636	0.0263941846539277
8.90127498163463	0.0263401252115104
8.96300495617631	0.0262586023662560
9.02473493071799	0.0261501632494023
9.08646490525967	0.0260153724186411
9.14819487980135	0.0258548800159657
9.21071927424122	0.0256668717575824
9.27324366868109	0.0254540902828554
9.33576806312096	0.0252174510555259
9.39829245756083	0.0249579353874585
9.46233592838314	0.0246694890974070
9.52637939920544	0.0243593260715425
9.59042287002774	0.0240286884062329
9.65446634085004	0.0236788632895002
9.72096019267431	0.0232967760601718
9.78745404449858	0.0228969769962920
9.85394789632285	0.0224810346204612
9.92044174814712	0.0220505382389624
9.98759919027086	0.0216026113448519
10.0547566323946	0.0211431600841588
10.1219140745184	0.0206738654544399
10.1890715166421	0.0201963994303009
10.2546642923364	0.0197237628573641
10.3202570680308	0.0192464637741786
10.3858498437251	0.0187660234977602
10.4514426194195	0.0182839314880497
10.5165140917340	0.0178054767606137
10.5815855640486	0.0173282322982185
10.6466570363632	0.0168535550410493
10.7117285086778	0.0163827528996387
10.7771443606203	0.0159146383138483
10.8425602125627	0.0154529535910668
10.9079760645052	0.0149988792125901
10.9733919164476	0.0145535319328381
11.0399477645340	0.0141104698710302
11.1065036126204	0.0136785885308648
11.1730594607068	0.0132588682146755
11.2396153087932	0.0128522116798912
11.3082257087532	0.0124475527076131
11.3768361087133	0.0120584901109843
11.4454465086734	0.0116857678578099
11.5140569086335	0.0113300380527117
11.5852093098832	0.0109796802165862
11.6563617111329	0.0106487433632513
11.7275141123826	0.0103376634887215
11.7986665136323	0.0100467726410198
11.8677850418193	0.00978375116671554
11.9369035700062	0.00954013486260028
12.0060220981931	0.00931597034363478
12.0751406263801	0.00911121998807420
12.1433601380698	0.00892805581131035
12.2115796497596	0.00876350644400114
12.2797991614493	0.00861731725901541
12.3480186731391	0.00848916564263377
12.4163461472746	0.00837850390578594
12.4846736214100	0.00828509957986596
12.5530010955455	0.00820844578303503
12.6213285696809	0.00814798221716118
12.6907216414633	0.00810251859850942
12.7601147132457	0.00807243458483453
12.8295077850280	0.00805699630958383
12.8989008568104	0.00805543116974804
12.9703478268833	0.00806746169542706
13.0417947969561	0.00809242052941184
13.1132417670290	0.00812935808922482
13.1846887371018	0.00817730287229138
13.2595560962437	0.00823827290627811
13.3344234553855	0.00830907721774694
13.4092908145273	0.00838854329563888
13.4841581736692	0.00847549845824039
13.5575412493262	0.00856686824852590
13.6309243249833	0.00866320388018273
13.7043074006403	0.00876341623792597
13.7776904762973	0.00886643781867183
13.8500672006557	0.00896977853334298
13.9224439250142	0.00907384897813361
13.9948206493726	0.00917769503638079
14.0671973737310	0.00928039965239192
14.1398455416426	0.00938145476603988
14.2124937095543	0.00947961468490260
14.2851418774659	0.00957406708147565
14.3577900453776	0.00966404962854052
14.4318616952425	0.00975045367767508
14.5059333451073	0.00983075963866844
14.5800049949722	0.00990431683880701
14.6540766448371	0.00997053686403148
14.7309274464065	0.0100309211563645
14.8077782479759	0.0100823112919100
14.8846290495453	0.0101242527300708
14.9614798511146	0.0101563663165053
15.0406722118752	0.0101788526453788
15.1198645726358	0.0101903150228344
15.1990569333964	0.0101905721270498
15.2782492941569	0.0101795238390185
15.3552187760152	0.0101579291884600
15.4321882578735	0.0101256759537116
15.5091577397318	0.0100828724830897
15.5861272215900	0.0100296900958424
15.6625824441176	0.00996681575433416
15.7390376666451	0.00989420936102999
15.8154928891726	0.00981220330426958
15.8919481117002	0.00972117811521222
15.9693961674172	0.00962021134697720
16.0468442231342	0.00951091437851779
16.1242922788512	0.00939381345786627
16.2017403345682	0.00926946881424473
16.2817277574867	0.00913407132769712
16.3617151804052	0.00899226479988131
16.4417026033237	0.00884475926099331
16.5216900262422	0.00869228250077520
16.6043553465212	0.00853026730559543
16.6870206668002	0.00836457568090493
16.7696859870792	0.00819605019385367
16.8523513073581	0.00802552958173385
16.9322086407103	0.00785968982940307
17.0120659740625	0.00769351611726068
17.0919233074148	0.00752774172391802
17.1717806407670	0.00736307824945713
17.2507845102887	0.00720194464793870
17.3297883798104	0.00704322442690578
17.4087922493321	0.00688753803068750
17.4877961188537	0.00673547152460664
17.5676116379811	0.00658608179608729
17.6474271571085	0.00644148982991274
17.7272426762358	0.00630219256376884
17.8070581953632	0.00616864148526194
17.8893023304811	0.00603746850564275
17.9715464655990	0.00591323163125309
18.0537906007169	0.00579627875665054
18.1360347358348	0.00568690122835990
18.2213159234312	0.00558173829082246
18.3065971110275	0.00548518436258710
18.3918782986238	0.00539738428028847
18.4771594862202	0.00531841828166765
18.5595094175750	0.00525056915061020
18.6418593489297	0.00519094360861540
18.7242092802845	0.00513945833839445
18.8065592116393	0.00509598043933780
18.8880422520689	0.00506066581248154
18.9695252924985	0.00503279949888157
19.0510083329281	0.00501212560562507
19.1324913733577	0.00499835086829594
19.2148776329082	0.00499110295945308
19.2972638924588	0.00499019919246174
19.3796501520093	0.00499523666547028
19.4620364115598	0.00500578683913245
19.5470683095882	0.00502197780436601
19.6321002076166	0.00504303743864338
19.7171321056450	0.00506842628337285
19.8021640036734	0.00509759289554858
19.8908893408643	0.00513144655666991
19.9796146780552	0.00516815156526352
20.0683400152462	0.00520705744329633
20.1570653524371	0.00524752023901728
20.2428390648805	0.00528751850264525
20.3286127773240	0.00532780672076479
20.4143864897674	0.00536783123501247
20.5001602022109	0.00540705977091322
20.5852635054960	0.00544469114474719
20.6703668087812	0.00548055461208205
20.7554701120663	0.00551419724154744
20.8405734153514	0.00554519817522693
20.9270705233463	0.00557359844153343
21.0135676313412	0.00559848765006115
21.1000647393361	0.00561952498202038
21.1865618473310	0.00563641134630414
21.2766604059527	0.00564930808804491
21.3667589645743	0.00565716933284420
21.4568575231959	0.00565979434515210
21.5469560818176	0.00565703438843500
21.6381292498009	0.00564865812150949
21.7293024177842	0.00563460946328756
21.8204755857675	0.00561488313005822
21.9116487537508	0.00558952457102742
22.0004127698935	0.00555951326457903
22.0891767860362	0.00552437689310692
22.1779408021788	0.00548428009352746
22.2667048183215	0.00543942449213879
22.3556370337612	0.00538994832943520
22.4445692492010	0.00533620192670781
22.5335014646408	0.00527848347532318
22.6224336800805	0.00521711641411678
22.7139161549811	0.00515054753913380
22.8053986298817	0.00508088590162857
22.8968811047823	0.00500854993629050
22.9883635796829	0.00493397054337858
23.0838924299717	0.00485417608844908
23.1794212802604	0.00477293203190142
23.2749501305492	0.00469075480308273
23.3704789808380	0.00460815596546741
23.4621509718643	0.00452896486533183
23.5538229628905	0.00445029455101964
23.6454949539168	0.00437257387899018
23.7371669449431	0.00429621305714434
23.8279328445987	0.00422233155646596
23.9186987442544	0.00415053193132434
24.0094646439101	0.00408115400827494
24.1002305435658	0.00401450947533793
24.1926550919484	0.00394974989363294
24.2850796403311	0.00388839381976947
24.3775041887138	0.00383068137427509
24.4699287370964	0.00377681599420622
24.5667881185871	0.00372467762872501
24.6636475000779	0.00367710565056325
24.7605068815686	0.00363421195767498
24.8573662630593	0.00359606252181901
24.9520922059339	0.00356336439427617
25.0468181488086	0.00353521120238896
25.1415440916832	0.00351154966966758
25.2362700345578	0.00349228900237512
25.3292146875769	0.00347754688819738
25.4221593405961	0.00346677203551061
25.5151039936153	0.00345978691047192
25.6080486466344	0.00345638747164092
25.7019756638980	0.00345636202490916
25.7959026811617	0.00345950583121958
25.8898296984253	0.00346553996379407
25.9837567156889	0.00347416924903396
26.0813748678075	0.00348555541235976
26.1789930199261	0.00349904683643510
26.2766111720447	0.00351427154120016
26.3742293241633	0.00353085367498424
26.4732872431096	0.00354867940956917
26.5723451620558	0.00356711479341635
26.6714030810021	0.00358576778296736
26.7704609999484	0.00360425787572103
26.8668464553430	0.00362174196259872
26.9632319107376	0.00363839228126567
27.0596173661322	0.00365389631930467
27.1560028215268	0.00366796310652110
27.2528815695420	0.00368038106718369
27.3497603175572	0.00369081906578000
27.4466390655724	0.00369904854545713
27.5435178135875	0.00370487032376298
27.6439608492560	0.00370818149070484
27.7444038849244	0.00370855878512983
27.8448469205929	0.00370587563348070
27.9452899562613	0.00370004267708609
28.0482405279971	0.00369073860922756
28.1511910997329	0.00367804436036148
28.2541416714688	0.00366197412389903
28.3570922432046	0.00364258032017333
28.4567501555253	0.00362072333407075
28.5564080678461	0.00359594217079068
28.6560659801668	0.00356837290613596
28.7557238924876	0.00353817763219209
28.8557411898054	0.00350542026936897
28.9557584871233	0.00347041519521670
29.0557757844411	0.00343339109160552
29.1557930817590	0.00339459227320870
29.2596833575662	0.00335268870148198
29.3635736333734	0.00330945292892566
29.4674639091807	0.00326519708330626
29.5713541849879	0.00322023695065082
29.6759318863875	0.00317458990189350
29.7805095877872	0.00312887857281111
29.8850872891868	0.00308342372685384
29.9896649905864	0.00303853526046833
30.0911544966620	0.00299579687154821
30.1926440027376	0.00295413779805531
30.2941335088132	0.00291380586474273
30.3956230148889	0.00287502910668768
30.4978092358551	0.00283776883646245
30.5999954568214	0.00280249259636843
30.7021816777877	0.00276937167989366
30.8043678987539	0.00273855064358961
30.9109059456037	0.00270899428041732
31.0174439924534	0.00268217578259045
31.1239820393031	0.00265817130884814
31.2305200861528	0.00263702324416466
31.3364021990683	0.00261884641963560
31.4422843119837	0.00260348490227069
31.5481664248991	0.00259089178051060
31.6540485378145	0.00258099085709984
31.7574284840790	0.00257382298143100
31.8608084303435	0.00256900508645957
31.9641883766080	0.00256639761234537
32.0675683228725	0.00256584180242998
32.1722735824859	0.00256718997317235
32.2769788420993	0.00257026253459540
32.3816841017127	0.00257484700534699
32.4863893613262	0.00258072107498264
32.5963585110375	0.00258802658856823
32.7063276607488	0.00259622372760360
32.8162968104602	0.00260503359495363
32.9262659601715	0.00261417941904505
33.0345223500676	0.00262324502856490
33.1427787399638	0.00263211212222333
33.2510351298599	0.00264053198657841
33.3592915197560	0.00264826990044284
33.4657809711845	0.00265500179384095
33.5722704226130	0.00266066124784044
33.6787598740416	0.00266506775029248
33.7852493254701	0.00266806178128003
33.8941979357818	0.00266951791718459
34.0031465460936	0.00266921978239460
34.1120951564054	0.00266706271790253
34.2210437667172	0.00266296920415368
34.3366404896276	0.00265645094103796
34.4522372125380	0.00264766016179217
34.5678339354484	0.00263659533354119
34.6834306583588	0.00262328816756916
34.7936642990230	0.00260856620765973
34.9038979396873	0.00259193789119478
35.0141315803515	0.00257350248963753
35.1243652210157	0.00255338037036260
35.2343050512079	0.00253177048161796
35.3442448814002	0.00250877666565758
35.4541847115924	0.00248456825697360
35.5641245417846	0.00245932607890118
35.6786017627846	0.00243214880527224
35.7930789837846	0.00240428310802239
35.9075562047846	0.00237595923850776
36.0220334257847	0.00234740806079951
36.1362198980123	0.00231893215348918
36.2504063702399	0.00229068761927758
36.3645928424676	0.00226289514354880
36.4787793146952	0.00223576389446454
36.5900126053583	0.00221015861068248
36.7012458960214	0.00218554190832703
36.8124791866845	0.00216207161476352
36.9237124773476	0.00213988729903445
37.0369057108861	0.00211875823364569
37.1500989444246	0.00209919944525544
37.2632921779630	0.00208130109830566
37.3764854115015	0.00206512959374922
37.4962218645145	0.00204995139063767
37.6159583175275	0.00203678284132937
37.7356947705405	0.00202562368185229
37.8554312235534	0.00201644466372161
37.9694000931710	0.00200949670989497
38.0833689627887	0.00200422517296870
38.1973378324063	0.00200054302701709
38.3113067020239	0.00199834515927419
38.4249000672874	0.00199751103202163
38.5384934325510	0.00199789653631872
38.6520867978146	0.00199935542119107
38.7656801630782	0.00200173204840271
38.8839805724880	0.00200500657362006
39.0022809818979	0.00200890602583032
39.1205813913078	0.00201323425093730
39.2388818007176	0.00201779565538052
39.3577858169091	0.00202241952851445
39.4766898331005	0.00202688712964450
39.5955938492920	0.00203101066965087
39.7144978654834	0.00203461404506351
39.8306400259012	0.00203747389708464
39.9467821863190	0.00203953648262018
40.0629243467368	0.00204067306076289
40.1790665071546	0.00204077253782685
40.2979626814797	0.00203970176375776
40.4168588558048	0.00203736023862380
40.5357550301298	0.00203368392364084
40.6546512044549	0.00202863140142281
40.7793663330114	0.00202183063110294
40.9040814615679	0.00201349156565824
41.0287965901244	0.00200363761642897
41.1535117186809	0.00199231745610856
41.2728913030736	0.00198017373361545
41.3922708874662	0.00196683128893846
41.5116504718589	0.00195238599628056
41.6310300562516	0.00193694834648179
41.7513824171239	0.00192050543058561
41.8717347779962	0.00190331719639615
41.9920871388686	0.00188553008669878
42.1124394997409	0.00186729628537920
42.2403780838680	0.00184759841153455
42.3683166679951	0.00182776558901162
42.4962552521223	0.00180798918455658
42.6241938362494	0.00178845472121365
42.7459262128924	0.00177025612608559
42.8676585895354	0.00175258823679723
42.9893909661784	0.00173558968659360
43.1111233428215	0.00171938546715826
43.2323192820888	0.00170415265963072
43.3535152213561	0.00168991706050194
43.4747111606234	0.00167676121448574
43.5959070998906	0.00166474938183223
43.7230100636943	0.00165343233919353
43.8501130274980	0.00164346189430136
43.9772159913017	0.00163485272965450
44.1043189551053	0.00162759670947307
44.2286927690341	0.00162177887169081
44.3530665829628	0.00161718564895758
44.4774403968915	0.00161375596294248
44.6018142108202	0.00161141231589895
44.7243832234717	0.00161007576164200
44.8469522361232	0.00160960461192737
44.9695212487747	0.00160988861326164
45.0920902614261	0.00161080943199297
45.2192704569313	0.00161230440274873
45.3464506524364	0.00161420407878936
45.4736308479415	0.00161635975815672
45.6008110434466	0.00161862359195008
45.7293487437304	0.00162087263911628
45.8578864440142	0.00162293373858584
45.9864241442980	0.00162466518614990
46.1149618445818	0.00162593612600611
46.2403633884128	0.00162661736153035
46.3657649322439	0.00162664283113431
46.4911664760749	0.00162592313259908
46.6165680199060	0.00162438456828436
46.7458183814916	0.00162187969603011
46.8750687430772	0.00161839224282160
47.0043191046628	0.00161389058518083
47.1335694662484	0.00160836283191459
47.2659682689327	0.00160164294823619
47.3983670716170	0.00159387626487932
47.5307658743013	0.00158510507591323
47.6631646769855	0.00157539000084255
47.7913492952116	0.00156515698464730
47.9195339134376	0.00155419293390418
48.0477185316636	0.00154259081002327
48.1759031498897	0.00153045270447991
48.3075614879101	0.00151754280938024
48.4392198259305	0.00150430924209439
48.5708781639510	0.00149088147849197
48.7025365019714	0.00147738947113568
48.8366959423393	0.00146370889269778
48.9708553827072	0.00145023231922251
49.1050148230751	0.00143708987093288
49.2391742634430	0.00142440207779511
49.3688501639382	0.00141267480502250
49.4985260644335	0.00140156894247128
49.6282019649287	0.00139116512768115
49.7578778654240	0.00138152975608097
49.8184083990680	0.00137731066684407
49.8789389327120	0.00137327548396136
49.9394694663560	0.00136942800857543
50	0.00136577133414702

==> matlab/fig2e1.tex <==
0.0100000000000000	0.0454545454545455
0.0179621434110699	0.0565772871227907
0.0259242868221399	0.0640560844176202
0.0338864302332098	0.0695586107171022
0.0418485736442798	0.0737915574304092
0.0489549209391593	0.0768086985367820
0.0560612682340389	0.0792827696351535
0.0631676155289185	0.0813271933171466
0.0702739628237981	0.0830235204491041
0.0834365541784869	0.0854420039390436
0.0965991455331757	0.0871387494753888
0.109761736887865	0.0882927454870038
0.122924328242553	0.0890277827388946
0.141422220690948	0.0895192659086339
0.159920113139343	0.0895322046615059
0.178418005587737	0.0891881057441134
0.196915898036132	0.0885739134104099
0.219013608897574	0.0875744052751419
0.241111319759016	0.0863604110078043
0.263209030620457	0.0849905394783953
0.285306741481899	0.0835084135827379
0.309342274650222	0.0818072124571030
0.333377807818544	0.0800442499315571
0.357413340986866	0.0782438114411248
0.381448874155189	0.0764244081253461
0.406933021704955	0.0744903882780843
0.432417169254721	0.0725638503991537
0.457901316804488	0.0706545460405296
0.483385464354254	0.0687698405414573
0.510146684095585	0.0668231894868496
0.536907903836916	0.0649144275746300
0.563669123578246	0.0630469035349073
0.590430343319577	0.0612229337580735
0.618396556862693	0.0593650015355427
0.646362770405808	0.0575572486846341
0.674328983948924	0.0558000748030705
0.702295197492039	0.0540934404253440
0.731440138666079	0.0523682378373134
0.760585079840118	0.0506967625359930
0.789730021014158	0.0490780457478505
0.818874962188198	0.0475109565128931
0.849202310632316	0.0459337535247745
0.879529659076434	0.0444095794314055
0.909857007520552	0.0429368618957640
0.940184355964671	0.0415139998862685
0.971722764316052	0.0400854648026351
1.00326117266743	0.0387072810160811
1.03479958101881	0.0373776537423678
1.06633798937020	0.0360948239192565
1.09914059673297	0.0348083721000396
1.13194320409574	0.0335687937966446
1.16474581145851	0.0323742617168997
1.19754841882128	0.0312230140964777
1.23169524674606	0.0300687417690451
1.26584207467084	0.0289576850065685
1.29998890259562	0.0278880746793450
1.33413573052039	0.0268582193357410
1.36973897643827	0.0258250253320619
1.40534222235615	0.0248315320093454
1.44094546827402	0.0238760660201430
1.47654871419190	0.0229570349184302
1.51333148231955	0.0220442105733752
1.55011425044721	0.0211670577684607
1.58689701857486	0.0203240600149415
1.62367978670251	0.0195137771460949
1.66101214689026	0.0187234309536049
1.69834450707800	0.0179640078183327
1.73567686726574	0.0172342120344368
1.77300922745348	0.0165328129724556
1.81093729414381	0.0158480961809339
1.84886536083414	0.0151903105993109
1.88679342752446	0.0145583448626895
1.92472149421479	0.0139511425764768
1.96329948808217	0.0133579010851086
2.00187748194955	0.0127882287524513
2.04045547581692	0.0122411659026781
2.07903346968430	0.0117157992562551
2.11832628074299	0.0112021004229313
2.15761909180168	0.0107091279398191
2.19691190286036	0.0102360459597864
2.23620471391905	0.00978205798100422
2.27628788215811	0.00933782359201318
2.31637105039716	0.00891189668613894
2.35645421863622	0.00850354218725402
2.39653738687527	0.00811205867139990
2.43749810706159	0.00772873579301964
2.47845882724791	0.00736164633661499
2.51941954743422	0.00701013720338829
2.56038026762054	0.00667358440883337
2.60231930174224	0.00634386625395710
2.64425833586394	0.00602858781444514
2.68619736998564	0.00572716275865356
2.72813640410734	0.00543903029441844
2.77117099359047	0.00515662589482375
2.81420558307360	0.00488709591537205
2.85724017255673	0.00462990850596042
2.90027476203986	0.00438455457940521
2.94454280820470	0.00414400150116868
2.98881085436955	0.00391494434078801
3.03307890053439	0.00369689578745461
3.07734694669924	0.00348938918153930
3.12301296380697	0.00328590243331880
3.16867898091470	0.00309268666729230
3.21434499802243	0.00290929101871985
3.26001101513015	0.00273528372430987
3.30727473639622	0.00256463435173889
3.35453845766229	0.00240315814979907
3.40180217892835	0.00225043403674207
3.44906590019442	0.00210605897069838
3.49817508767041	0.00196447667517167
3.54728427514641	0.00183107592075366
3.59639346262241	0.00170545981069766
3.64550265009840	0.00158724886951202
3.69677296104368	0.00147134392684752
3.74804327198896	0.00136271866389531
3.79931358293424	0.00126099549345442
3.85058389387952	0.00116581406035720
3.90443140626832	0.00107251467148241
3.95827891865712	0.000985670334197422
4.01212643104593	0.000904918247708316
4.06597394343473	0.000829913111523913
4.12210104024892	0.000757494732439117
4.17822813706310	0.000690607560961540
4.23435523387729	0.000628914443727485
4.29048233069147	0.000572095477705062
4.34732453072746	0.000519209258247093
4.40416673076345	0.000470710199382748
4.46100893079944	0.000426313851214191
4.51785113083543	0.000385750924807429
4.57582743647441	0.000348062978601146
4.63380374211339	0.000313840402106193
4.69178004775237	0.000282840423279121
4.74975635339135	0.000254833965518502
4.80927575174908	0.000228969142521431
4.86879515010681	0.000205809782158275
4.92831454846454	0.000185147539011743
4.98783394682227	0.000166786698732087
5.04934227097890	0.000150034911921446
5.11085059513554	0.000135353136133658
5.17235891929218	0.000122562436024492
5.23386724344882	0.000111495720936258
5.29789405007311	0.000101639132758446
5.36192085669741	9.33165773672821e-05
5.42594766332170	8.63749531862518e-05
5.48997446994599	8.06724248248749e-05
5.55719875822752	7.58748439316366e-05
5.62442304650904	7.21571158467852e-05
5.69164733479056	6.93893941599007e-05
5.75887162307208	6.74526927178857e-05
5.83023614825156	6.61844460706539e-05
5.90160067343103	6.56103154160458e-05
5.97296519861051	6.56218868026530e-05
6.04432972378998	6.61213698098528e-05
6.12127947749308	6.71054927934209e-05
6.19822923119618	6.84551135563655e-05
6.27517898489927	7.00820952311790e-05
6.35212873860237	7.19089026923450e-05
6.43723247735917	7.40802960338941e-05
6.52233621611597	7.63330216429010e-05
6.60743995487277	7.85988618056877e-05
6.69254369362957	8.08205694819469e-05
6.78171540330365	8.30494519480942e-05
6.87088711297772	8.51330696737154e-05
6.96005882265180	8.70360209041617e-05
7.04923053232588	8.87312398110275e-05
7.14466391282726	9.02931372687465e-05
7.24009729332864	9.15785742959316e-05
7.33553067383002	9.25786108420054e-05
7.43096405433140	9.32903229648485e-05
7.53934576535893	9.37520247380055e-05
7.64772747638647	9.38557145903301e-05
7.75610918741400	9.36175848750467e-05
7.86449089844153	9.30577337136026e-05
7.96911887225926	9.22341466046725e-05
8.07374684607698	9.11568023295517e-05
8.17837481989470	8.98507916717242e-05
8.28300279371242	8.83413650870426e-05
8.38717830981286	8.66616599186130e-05
8.49135382591330	8.48313089040199e-05
8.59552934201374	8.28751200819767e-05
8.69970485811419	8.08164997512423e-05
8.80416336793757	7.86718470519604e-05
8.90862187776095	7.64684879026240e-05
9.01308038758434	7.42265463770002e-05
9.11753889740773	7.19641752015505e-05
9.21807327203068	6.97829541383845e-05
9.31860764665363	6.76119395764252e-05
9.41914202127658	6.54633147340242e-05
9.51967639589953	6.33476367311334e-05
9.61962880891270	6.12859741934639e-05
9.71958122192588	5.92740105043252e-05
9.81953363493905	5.73184446192600e-05
9.91948604795222	5.54246717283633e-05
10.0207435189413	5.35735843348526e-05
10.1220009899305	5.17939015372141e-05
10.2232584609196	5.00881428634416e-05
10.3245159319087	4.84578411515245e-05
10.4283846120172	4.68646405638374e-05
10.5322532921256	4.53516360942536e-05
10.6361219722340	4.39181228295446e-05
10.7399906523424	4.25627284322603e-05
10.8475748287719	4.12391654084224e-05
10.9551590052014	3.99947369518435e-05
11.0627431816309	3.88263775105400e-05
11.1703273580604	3.77306700145972e-05
11.2826122346865	3.66605868420358e-05
11.3948971113127	3.56612132187094e-05
11.5071819879388	3.47279850496720e-05
11.6194668645650	3.38562856581681e-05
11.7372536318931	3.30029570791607e-05
11.8550403992212	3.22069552991628e-05
11.9728271665493	3.14631131525988e-05
12.0906139338774	3.07664674522803e-05
12.2143018181317	3.00805405064241e-05
12.3379897023860	2.94362240009839e-05
12.4616775866403	2.88286515427786e-05
12.5853654708946	2.82533351956008e-05
12.7146136383583	2.76821677958742e-05
12.8438618058221	2.71375078594878e-05
12.9731099732858	2.66155695748989e-05
13.1023581407496	2.61129949804272e-05
13.2358862805105	2.56110049370375e-05
13.3694144202714	2.51238589075857e-05
13.5029425600323	2.46492649088890e-05
13.6364706997933	2.41852731702869e-05
13.7724345754501	2.37220724346086e-05
13.9083984511069	2.32670410150120e-05
14.0443623267637	2.28192641482964e-05
14.1803262024205	2.23780034967578e-05
14.3171940356473	2.19398759349563e-05
14.4540618688741	2.15077075375558e-05
14.5909297021008	2.10814716698469e-05
14.7277975353276	2.06611568500846e-05
14.8649284638827	2.02460562893244e-05
15.0020593924377	1.98373430212144e-05
15.1391903209927	1.94353567581274e-05
15.2763212495477	1.90403444078932e-05
15.4138654423835	1.86513964200635e-05
15.5514096352193	1.82701515844792e-05
15.6889538280551	1.78969606307454e-05
15.8264980208909	1.75320298660772e-05
15.9650100243167	1.71730401220238e-05
16.1035220277425	1.68228871091650e-05
16.2420340311683	1.64817587830133e-05
16.3805460345941	1.61496875785954e-05
16.5206781669815	1.58229203324667e-05
16.6608102993689	1.55054813901275e-05
16.8009424317563	1.51973515907068e-05
16.9410745641437	1.48983687966590e-05
17.0834062487309	1.46038360065405e-05
17.2257379333181	1.43184116459643e-05
17.3680696179053	1.40419024569838e-05
17.5104013024924	1.37739949855144e-05
17.6553488510412	1.35096447706044e-05
17.8002963995899	1.32536210845759e-05
17.9452439481386	1.30056272058238e-05
18.0901914966873	1.27652693500008e-05
18.2379619557187	1.25276680282495e-05
18.3857324147501	1.22972991987639e-05
18.5335028737815	1.20738406131794e-05
18.6812733328129	1.18568898846452e-05
18.8318594722471	1.16420842722727e-05
18.9824456116813	1.14333649685467e-05
19.1330317511155	1.12304468225736e-05
19.2836178905498	1.10329722540362e-05
19.4368432212972	1.08372632382502e-05
19.5900685520447	1.06466418324456e-05
19.7432938827921	1.04608941550644e-05
19.8965192135396	1.02797329629442e-05
20.0521273153262	1.01001612340358e-05
20.2077354171128	9.92492455551157e-06
20.3633435188993	9.75388463177663e-06
20.5189516206859	9.58682344258687e-06
20.6767074948662	9.42129729342056e-06
20.8344633690465	9.25959804850183e-06
20.9922192432268	9.10164632101005e-06
21.1499751174070	8.94727521224299e-06
21.3097363309718	8.79441625071408e-06
21.4694975445366	8.64505406167638e-06
21.6292587581014	8.49914367952507e-06
21.7890199716662	8.35654646568782e-06
21.9507550228406	8.21541065296251e-06
22.1124900740149	8.07753532532655e-06
22.2742251251893	7.94288857631422e-06
22.4359601763636	7.81134161154041e-06
22.5997219235879	7.68115924321204e-06
22.7634836708122	7.55402782973171e-06
22.9272454180365	7.42991570255727e-06
23.0910071652607	7.30869385267810e-06
23.2568857402592	7.18870466394139e-06
23.4227643152578	7.07154785440739e-06
23.5886428902563	6.95718799403983e-06
23.7545214652548	6.84549361995611e-06
23.9225997668194	6.73488750070180e-06
24.0906780683841	6.62687918217881e-06
24.2587563699487	6.52143154665465e-06
24.4268346715134	6.41841335729680e-06
24.5971602465273	6.31634797005917e-06
24.7674858215413	6.21664075703622e-06
24.9378113965552	6.11925743387028e-06
25.1081369715692	6.02407125361332e-06
25.2807146345169	5.92972464935585e-06
25.4532922974645	5.83750803016930e-06
25.6258699604122	5.74739393577283e-06
25.7984476233598	5.65926345281132e-06
25.9732496005806	5.57188483130031e-06
26.1480515778014	5.48643219266585e-06
26.3228535550222	5.40288679353424e-06
26.4976555322430	5.32113884254555e-06
26.6746407580550	5.24007594516299e-06
26.8516259838669	5.16076408501087e-06
27.0286112096789	5.08319290890682e-06
27.2055964354908	5.00726110733735e-06
27.3847291106506	4.93196030878040e-06
27.5638617858103	4.85826225773313e-06
27.7429944609701	4.78616326814261e-06
27.9221271361299	4.71556880034209e-06
28.1033873526667	4.64555665349160e-06
28.2846475692035	4.57701928355990e-06
28.4659077857403	4.50995762609447e-06
28.6471680022771	4.44428208587137e-06
28.8305524749318	4.37914137405453e-06
29.0139369475864	4.31536115738517e-06
29.1973214202411	4.25294541024031e-06
29.3807058928957	4.19180816935290e-06
29.5662216026754	4.13115866073835e-06
29.7517373124551	4.07176444474789e-06
29.9372530222348	4.01363170108196e-06
30.1227687320145	3.95667746734313e-06
30.3104244405387	3.90016556189820e-06
30.4980801490630	3.84481079335341e-06
30.6857358575872	3.79062133285153e-06
30.8733915661115	3.73751709639474e-06
31.0631915046256	3.68481323840265e-06
31.2529914431398	3.63317523798185e-06
31.4427913816539	3.58261334181988e-06
31.6325913201681	3.53305042939098e-06
31.8245330634793	3.48385049361624e-06
32.0164748067905	3.43563254264434e-06
32.2084165501018	3.38840898259316e-06
32.4003582934130	3.34210570093905e-06
32.5944343723426	3.29613260220116e-06
32.7885104512723	3.25106532690005e-06
32.9825865302019	3.20691836872488e-06
33.1766626091316	3.16362051739576e-06
33.3728638888244	3.12062394619337e-06
33.5690651685172	3.07846444439640e-06
33.7652664482099	3.03715836160330e-06
33.9614677279027	2.99663715216246e-06
34.1597863981921	2.95639123820040e-06
34.3581050684815	2.91692023547425e-06
34.5564237387709	2.87824204230570e-06
34.7547424090604	2.84029049070839e-06
34.9551733102377	2.80259038176101e-06
35.1556042114151	2.76560863370896e-06
35.3560351125925	2.72936440517109e-06
35.5564660137699	2.69379364867505e-06
35.7590062381233	2.65845219825362e-06
35.9615464624766	2.62377730335773e-06
36.1640866868299	2.58978916679498e-06
36.3666269111833	2.55642567236505e-06
36.5712744813487	2.52327095901315e-06
36.7759220515142	2.49073513859236e-06
36.9805696216796	2.45883931730746e-06
37.1852171918451	2.42752318406177e-06
37.3919698016115	2.39639694841891e-06
37.5987224113779	2.36584571528011e-06
37.8054750211443	2.33589140050437e-06
38.0122276309107	2.30647540742934e-06
38.2210820628669	2.27723207592991e-06
38.4299364948231	2.24852337895978e-06
38.6387909267793	2.22037196272309e-06
38.8476453587355	2.19272086262948e-06
39.0585976322966	2.16522674770128e-06
39.2695499058576	2.13823018993417e-06
39.4805021794187	2.11175448190936e-06
39.6914544529798	2.08574420338610e-06
39.9045003567214	2.05987662825105e-06
40.1175462604631	2.03447256190400e-06
40.3305921642047	2.00955585244994e-06
40.5436380679464	1.98507253133139e-06
40.7587736492092	1.96071884151059e-06
40.9739092304720	1.93679735613185e-06
41.1890448117348	1.91333238884277e-06
41.4041803929976	1.89027133260659e-06
41.6214021542161	1.86732788987785e-06
41.8386239154346	1.84478781417610e-06
42.0558456766532	1.82267580410284e-06
42.2730674378717	1.80094053326610e-06
42.4923722413425	1.77931180429938e-06
42.7116770448134	1.75805982890478e-06
42.9309818482842	1.73720962316105e-06
43.1502866517551	1.71671107194811e-06
43.3716714967573	1.69630886536018e-06
43.5930563417596	1.67625882142622e-06
43.8144411867618	1.65658621784929e-06
44.0358260317640	1.63724209097088e-06
44.2592878797955	1.61798492886911e-06
44.4827497278270	1.59905719269170e-06
44.7062115758585	1.58048437360383e-06
44.9296734238900	1.56221860570296e-06
45.1552091541436	1.54403118192603e-06
45.3807448843971	1.52615215273501e-06
45.6062806146507	1.50860717891289e-06
45.8318163449043	1.49134944211225e-06
46.0594228148368	1.47416212448401e-06
46.2870292847694	1.45726373677008e-06
46.5146357547020	1.44068006842269e-06
46.7422422246345	1.42436530105543e-06
46.9719163573238	1.40811365938064e-06
47.2015904900131	1.39213291832461e-06
47.4312646227023	1.37644895813231e-06
47.6609387553916	1.36101691568916e-06
47.8926775894859	1.34564127823245e-06
48.1244164235803	1.33051982538527e-06
48.3561552576747	1.31567849403937e-06
48.5878940917691	1.30107333508621e-06
48.8216947775496	1.28651838314279e-06
49.0554954633302	1.27220210246600e-06
49.2892961491107	1.25815045643731e-06
49.5230968348912	1.24432037221401e-06
49.6423226261684	1.23733570813381e-06
49.7615484174456	1.23040651635539e-06
49.8807742087228	1.22353286014586e-06
50	1.21671351651654e-06

==> matlab/fig2e2.tex <==
0.0100000000000000	0.00495049504950495
0.0148893961920471	0.00677102348266696
0.0197787923840941	0.00844273139694727
0.0246681885761412	0.00999800915610076
0.0295575847681883	0.0114565081458570
0.0344469809602354	0.0128322741811714
0.0393363771522824	0.0141353255578871
0.0442257733443295	0.0153734590409777
0.0491151695363766	0.0165529221011404
0.0566647429666537	0.0182705923680698
0.0642143163969308	0.0198759030064631
0.0717638898272080	0.0213810257201489
0.0793134632574851	0.0227958834418730
0.0908118553010885	0.0247957191707696
0.102310247344692	0.0266291811754118
0.113808639388295	0.0283154944487158
0.125307031431899	0.0298704459271618
0.141369341375589	0.0318474249326162
0.157431651319280	0.0336235381157872
0.173493961262971	0.0352230597733240
0.189556271206662	0.0366661193087245
0.209054765188173	0.0382319068194291
0.228553259169684	0.0396175110139332
0.248051753151195	0.0408441667961739
0.267550247132706	0.0419298161819345
0.290054092995263	0.0430274586190824
0.312557938857820	0.0439776994167927
0.335061784720377	0.0447975512796800
0.357565630582934	0.0455015825785092
0.382022894637376	0.0461500206827087
0.406480158691819	0.0466903886123994
0.430937422746262	0.0471346708803036
0.455394686800704	0.0474932699191305
0.481569771421338	0.0477924029324795
0.507744856041972	0.0480134624860039
0.533919940662606	0.0481648931798277
0.560095025283240	0.0482540966671383
0.587815541450838	0.0482879454879138
0.615536057618436	0.0482660809688293
0.643256573786034	0.0481944690514787
0.670977089953632	0.0480783783110173
0.700118255075150	0.0479134879215801
0.729259420196668	0.0477093751797855
0.758400585318186	0.0474702746993297
0.787541750439704	0.0471999488413893
0.818002822213866	0.0468876278054768
0.848463893988028	0.0465482366671589
0.878924965762190	0.0461847965348523
0.909386037536352	0.0458000052070836
0.941083529314273	0.0453795177378316
0.972781021092195	0.0449409417493949
1.00447851287012	0.0444864445569717
1.03617600464804	0.0440179698360195
1.06904120797423	0.0435193393439738
1.10190641130043	0.0430092966637861
1.13477161462662	0.0424894060424613
1.16763681795282	0.0419610753344442
1.20161504757622	0.0414073243487711
1.23559327719962	0.0408471655810967
1.26957150682302	0.0402817353908077
1.30354973644643	0.0397120593948385
1.33860026934466	0.0391209357331113
1.37365080224289	0.0385271972366402
1.40870133514113	0.0379316749379728
1.44375186803936	0.0373351202642929
1.47984820246859	0.0367204040978243
1.51594453689782	0.0361059880075224
1.55204087132705	0.0354924834799301
1.58813720575629	0.0348804437147906
1.62526753796055	0.0342529273958290
1.66239787016482	0.0336279888581333
1.69952820236909	0.0330060800461475
1.73665853457335	0.0323876092561467
1.77482648733532	0.0317558271878112
1.81299444009729	0.0311284371907137
1.85116239285926	0.0305057735588628
1.88933034562123	0.0298881370087657
1.92855606837490	0.0292589069194497
1.96778179112857	0.0286355453296858
2.00700751388225	0.0280182980061782
2.04623323663592	0.0274073840691147
2.08655507259207	0.0267862069193643
2.12687690854821	0.0261721279350399
2.16719874450436	0.0255653244317771
2.20752058046051	0.0249659518397741
2.24899759325488	0.0243573059344440
2.29047460604925	0.0237568078615334
2.33195161884362	0.0231645800967368
2.37342863163800	0.0225807264818740
2.41614443981355	0.0219882820147674
2.45886024798911	0.0214049049901606
2.50157605616466	0.0208306719629620
2.54429186434021	0.0202656430464390
2.58836050906038	0.0196924157620402
2.63242915378054	0.0191290843571587
2.67649779850070	0.0185756848802894
2.72056644322086	0.0180322383771412
2.76614153781910	0.0174806945715248
2.81171663241733	0.0169398165038629
2.85729172701556	0.0164096023669070
2.90286682161380	0.0158900362411992
2.94925709579494	0.0153720858591760
2.99564736997608	0.0148651143654448
3.04203764415721	0.0143690846682545
3.08842791833835	0.0138839471639814
3.13504806192754	0.0134073207305071
3.18166820551672	0.0129415785910171
3.22828834910590	0.0124866544629545
3.27490849269509	0.0120424715282336
3.32184817451336	0.0116060114520750
3.36878785633164	0.0111802717235922
3.41572753814992	0.0107651612491365
3.46266721996820	0.0103605799824639
3.51002497981212	0.00996295823303134
3.55738273965604	0.00957583977566607
3.60474049949997	0.00919911172441019
3.65209825934389	0.00883265356679572
3.69997786202684	0.00847247001643249
3.74785746470979	0.00812252861430444
3.79573706739275	0.00778269681985726
3.84361667007570	0.00745283562811796
3.89212998835124	0.00712863176994747
3.94064330662678	0.00681437119091307
3.98915662490232	0.00650990323321707
4.03766994317786	0.00621507183551498
4.08694045495193	0.00592533852445268
4.13621096672600	0.00564521660045072
4.18548147850007	0.00537453839215160
4.23475199027414	0.00511313182955406
4.28491921268052	0.00485631396187148
4.33508643508690	0.00460874622339980
4.38525365749328	0.00437024469254944
4.43542087989966	0.00414062203360847
4.48664627573137	0.00391512166239674
4.53787167156309	0.00369848381058321
4.58909706739480	0.00349050877016247
4.64032246322651	0.00329099441453165
4.69279768899344	0.00309517317077969
4.74527291476036	0.00290780313977894
4.79774814052728	0.00272866898736064
4.85022336629421	0.00255755399901989
4.90418235407362	0.00238973536332887
4.95814134185303	0.00222993547109808
5.01210032963244	0.00207792316515632
5.06605931741185	0.00193346702599299
5.12179691896912	0.00179193886871007
5.17753452052639	0.00165797849752586
5.23327212208366	0.00153133825411258
5.28900972364093	0.00141177146476729
5.34691229243864	0.00129478932572668
5.40481486123634	0.00118490873883397
5.46271743003406	0.00108186413693842
5.52061999883177	0.000985392387132854
5.58121953325118	0.000891184298028228
5.64181906767059	0.000803600783414882
5.70241860209001	0.000722355727721200
5.76301813650942	0.000647167225276904
5.82511460237858	0.000576115009742297
5.88721106824774	0.000510841976944313
5.94930753411689	0.000451064201845560
6.01140399998605	0.000396503557188481
6.07380159490291	0.000346659565018886
6.13619918981976	0.000301541729758407
6.19859678473662	0.000260889299236706
6.26099437965347	0.000224448277043616
6.32419436949673	0.000191579043049418
6.38739435933999	0.000162528852717364
6.45059434918325	0.000137057110595086
6.51379433902651	0.000114930850599980
6.57830719489551	9.55616604371000e-05
6.64282005076451	7.92130141263822e-05
6.70733290663351	6.56625703977833e-05
6.77184576250251	5.46964843291716e-05
6.83824117080171	4.58925427789240e-05
6.90463657910091	3.93939276817619e-05
6.97103198740010	3.49954534846384e-05
7.03742739569930	3.25013572067781e-05
7.10642156558373	3.17272006920163e-05
7.17541573546816	3.26089159595740e-05
7.24440990535259	3.49578542775804e-05
7.31340407523702	3.85958632879385e-05
7.38600948734619	4.36318951970993e-05
7.45861489945535	4.97251088744940e-05
7.53122031156452	5.67030456919186e-05
7.60382572367369	6.44051215923508e-05
7.68169060479945	7.33002274572372e-05
7.75955548592521	8.26859862321007e-05
7.83742036705097	9.24058052178554e-05
7.91528524817673	0.000102317007847817
7.99490567291899	0.000112514662561597
8.07452609766125	0.000122651447144886
8.15414652240351	0.000132615011791720
8.23376694714577	0.000142305836310007
8.31391886159019	0.000151697298802590
8.39407077603461	0.000160645668011657
8.47422269047904	0.000169083980550314
8.55437460492346	0.000176955823951880
8.63687721049298	0.000184417855522278
8.71937981606250	0.000191189729958509
8.80188242163202	0.000197240313113016
8.88438502720155	0.000202547369209469
8.97139686058978	0.000207323602242042
9.05840869397802	0.000211250454009460
9.14542052736626	0.000214329366598389
9.23243236075449	0.000216569253641430
9.32093858739016	0.000218003255443529
9.40944481402583	0.000218609579700954
9.49795104066150	0.000218417694796387
9.58645726729716	0.000217461616066108
9.67248667547180	0.000215836283245911
9.75851608364644	0.000213564539849310
9.84454549182108	0.000210688067559120
9.93057489999572	0.000207250103037036
10.0166970837528	0.000203290960567314
10.1028192675098	0.000198861159596674
10.1889414512669	0.000194008116176939
10.2750636350240	0.000188778900585491
10.3632012635051	0.000183086800231348
10.4513388919862	0.000177100794837754
10.5394765204673	0.000170870536380115
10.6276141489484	0.000164443797465559
10.7197494921261	0.000157565675302349
10.8118848353039	0.000150575483369820
10.9040201784817	0.000143522537479752
10.9961555216594	0.000136452772821544
11.0865603570731	0.000129541147553617
11.1769651924869	0.000122694033502965
11.2673700279006	0.000115947333808218
11.3577748633143	0.000109333410827135
11.4470969932176	0.000102957852741842
11.5364191231210	9.67669339692716e-05
11.6257412530243	9.07838209494433e-05
11.7150633829276	8.50283688387439e-05
11.8051167656774	7.94735539236459e-05
11.8951701484272	7.41827691832936e-05
11.9852235311770	6.91683349861771e-05
12.0752769139267	6.44395352179380e-05
12.1675783486168	5.98961048144991e-05
12.2598797833068	5.56648536371678e-05
12.3521812179968	5.17481256811218e-05
12.4444826526868	4.81455754792231e-05
12.5406946243167	4.47219849607592e-05
12.6369065959466	4.16319522074324e-05
12.7331185675765	3.88681573329990e-05
12.8293305392064	3.64210488429854e-05
12.9317611576690	3.41510265805059e-05
13.0341917761316	3.22115981610229e-05
13.1366223945942	3.05855001356160e-05
13.2390530130568	2.92538849518807e-05
13.3436694630454	2.81769957008060e-05
13.4482859130340	2.73641368078900e-05
13.5529023630227	2.67923419956136e-05
13.6575188130113	2.64382221111745e-05
13.7639378760502	2.62770200877502e-05
13.8703569390891	2.62918640921964e-05
13.9767760021280	2.64583030579005e-05
14.0831950651669	2.67525201844132e-05
14.1948918891323	2.71735515119478e-05
14.3065887130976	2.76841353249676e-05
14.4182855370630	2.82598631101403e-05
14.5299823610283	2.88779611936358e-05
14.6523445390369	2.95787089871280e-05
14.7747067170456	3.02792102391853e-05
14.8970688950542	3.09564404764814e-05
15.0194310730629	3.15902900573246e-05
15.1511465632349	3.22042406654995e-05
15.2828620534069	3.27293681776438e-05
15.4145775435789	3.31509315480574e-05
15.5462930337509	3.34578825328941e-05
15.6816426907559	3.36457957464943e-05
15.8169923477609	3.36995625735484e-05
15.9523420047659	3.36175102548578e-05
16.0876916617709	3.34009439264754e-05
16.2195694981085	3.30642982695325e-05
16.3514473344461	3.26097171083999e-05
16.4833251707836	3.20449890700082e-05
16.6152030071212	3.13792266356220e-05
16.7409056818706	3.06600385553748e-05
16.8666083566200	2.98685460269637e-05
16.9923110313695	2.90152984060201e-05
17.1180137061189	2.81109288819768e-05
17.2460071843381	2.71486573394869e-05
17.3740006625573	2.61563287706522e-05
17.5019941407765	2.51453642379325e-05
17.6299876189957	2.41264669243811e-05
17.7565892512773	2.31207871102207e-05
17.8831908835589	2.21269378318087e-05
18.0097925158406	2.11536925104234e-05
18.1363941481222	2.02087110604151e-05
18.2599448561665	1.93202259022237e-05
18.3834955642107	1.84709319756074e-05
18.5070462722549	1.76656696010735e-05
18.6305969802992	1.69081911907379e-05
18.7553803779988	1.61945730367694e-05
18.8801637756984	1.55349937766561e-05
19.0049471733980	1.49308823334958e-05
19.1297305710976	1.43826838545357e-05
19.2592552219338	1.38724213441374e-05
19.3887798727700	1.34210699852092e-05
19.5183045236062	1.30268622322482e-05
19.6478291744424	1.26872346210292e-05
19.7861929856835	1.23811384598213e-05
19.9245567969247	1.21294096635575e-05
20.0629206081659	1.19272034677692e-05
20.2012844194070	1.17691947245352e-05
20.3511564871112	1.16413970918926e-05
20.5010285548154	1.15516533239001e-05
20.6509006225196	1.14927068582164e-05
20.8007726902238	1.14573724685791e-05
20.9588361116552	1.14380166619514e-05
21.1168995330866	1.14295178101544e-05
21.2749629545180	1.14248169806792e-05
21.4330263759494	1.14175658923393e-05
21.6190635682705	1.13982248159447e-05
21.8051007605917	1.13600555377067e-05
21.9911379529128	1.12971952882515e-05
22.1771751452340	1.12054850940623e-05
22.3458199885345	1.10952288080761e-05
22.5144648318351	1.09584384177002e-05
22.6831096751357	1.07953831002291e-05
22.8517545184363	1.06071132457682e-05
23.0203993617369	1.03953850095882e-05
23.1890442050374	1.01628481716553e-05
23.3576890483380	9.91259686869388e-06
23.5263338916386	9.64791214519915e-06
23.6920944741673	9.37705988900380e-06
23.8578550566961	9.09937977990542e-06
24.0236156392249	8.81853971026506e-06
24.1893762217536	8.53788714756873e-06
24.3482102075099	8.27204020566758e-06
24.5070441932662	8.01209368707967e-06
24.6658781790225	7.76053912371650e-06
24.8247121647788	7.51937598214385e-06
24.9797169326094	7.29561522466396e-06
25.1347217004401	7.08476063718650e-06
25.2897264682707	6.88786032105361e-06
25.4447312361014	6.70549461354729e-06
25.6022628713019	6.53529088944316e-06
25.7597945065025	6.38047205731031e-06
25.9173261417030	6.24081345897700e-06
26.0748577769036	6.11570258614322e-06
26.2399748574646	5.99922216396158e-06
26.4050919380255	5.89667670238028e-06
26.5702090185865	5.80674912089681e-06
26.7353260991475	5.72787550521368e-06
26.9135866885254	5.65318127291317e-06
27.0918472779033	5.58736002518513e-06
27.2701078672812	5.52834495775767e-06
27.4483684566591	5.47403969468368e-06
27.6461875512081	5.41684361623807e-06
27.8440066457571	5.36061141459788e-06
28.0418257403061	5.30327522810815e-06
28.2396448348551	5.24302221934812e-06
28.4582261869192	5.17127029032814e-06
28.6768075389832	5.09295670591347e-06
28.8953888910472	5.00743617277208e-06
29.1139702431113	4.91445984883848e-06
29.3320751105215	4.81442086924043e-06
29.5501799779317	4.70805307529236e-06
29.7682848453419	4.59656205296126e-06
29.9863897127521	4.48119264599605e-06
30.1847014566922	4.37406612854114e-06
30.3830132006322	4.26621259778824e-06
30.5813249445722	4.15891918930653e-06
30.7796366885122	4.05325158650649e-06
30.9653208272272	3.95662503276694e-06
31.1510049659422	3.86314845887537e-06
31.3366891046572	3.77354433527770e-06
31.5223732433722	3.68828078753522e-06
31.7057580297484	3.60863197502850e-06
31.8891428161245	3.53385171992769e-06
32.0725276025007	3.46410057797617e-06
32.2559123888769	3.39931109413822e-06
32.4435767931044	3.33792816621190e-06
32.6312411973319	3.28134059069547e-06
32.8189056015594	3.22923428972705e-06
33.0065700057869	3.18112772993031e-06
33.2035317736837	3.13432084070664e-06
33.4004935415806	3.09074262057459e-06
33.5974553094774	3.04978992894173e-06
33.7944170773742	3.01078043088385e-06
34.0042348370502	2.97059228694200e-06
34.2140525967261	2.93121086097385e-06
34.4238703564021	2.89206952126100e-06
34.6336881160780	2.85261326030491e-06
34.8550217447865	2.81011929564535e-06
35.0763553734949	2.76648577412299e-06
35.2976890022033	2.72157208065440e-06
35.5190226309117	2.67527365970597e-06
35.7420476120856	2.62720040535081e-06
35.9650725932595	2.57798299292165e-06
36.1880975744334	2.52795878978263e-06
36.4111225556072	2.47741812776087e-06
36.6266455989052	2.42836731397039e-06
36.8421686422032	2.37958065082374e-06
37.0576916855012	2.33148489257998e-06
37.2732147287991	2.28437898619027e-06
37.4822671682508	2.23985696694020e-06
37.6913196077025	2.19681977324182e-06
37.9003720471542	2.15551293881969e-06
38.1094244866059	2.11603551444497e-06
38.3178434323715	2.07851714650502e-06
38.5262623781370	2.04293533060214e-06
38.7346813239026	2.00930596446093e-06
38.9431002696682	1.97751645658140e-06
39.1562974204122	1.94671635592306e-06
39.3694945711562	1.91755391142023e-06
39.5826917219003	1.88987289006738e-06
39.7958888726443	1.86342578378321e-06
40.0176196036804	1.83692856903387e-06
40.2393503347166	1.81127389944848e-06
40.4610810657527	1.78626058027873e-06
40.6828117967889	1.76163814329931e-06
40.9137026787675	1.73614751329079e-06
41.1445935607461	1.71070105006097e-06
41.3754844427247	1.68520906396175e-06
41.6063753247033	1.65955457059693e-06
41.8420837151137	1.63309369324012e-06
42.0777921055241	1.60643411822455e-06
42.3135004959345	1.57966691908964e-06
42.5492088863449	1.55283752548521e-06
42.7832701060807	1.52617641688776e-06
43.0173313258165	1.49968767130523e-06
43.2513925455524	1.47354468885762e-06
43.4854537652882	1.44784047369186e-06
43.7158897201435	1.42302129832029e-06
43.9463256749988	1.39885231767309e-06
44.1767616298541	1.37545670740779e-06
44.4071975847094	1.35286259449982e-06
44.6370374295381	1.33110780078353e-06
44.8668772743667	1.31020399808301e-06
45.0967171191954	1.29017594474378e-06
45.3265569640240	1.27096105296316e-06
45.5600731725287	1.25216671101629e-06
45.7935893810333	1.23408932574880e-06
46.0271055895379	1.21667940040628e-06
46.2606217980426	1.19981962484160e-06
46.5007803538022	1.18290645914392e-06
46.7409389095619	1.16637939043171e-06
46.9810974653215	1.15017914673168e-06
47.2212560210812	1.13419840802658e-06
47.4680943172735	1.11788077079620e-06
47.7149326134659	1.10166904063633e-06
47.9617709096582	1.08555946729779e-06
48.2086092058506	1.06950703387817e-06
48.4587788964316	1.05324470426811e-06
48.7089485870126	1.03705746835562e-06
48.9591182775936	1.02100849085370e-06
49.2092879681746	1.00510928726853e-06
49.4069659761309	9.92654367610790e-07
49.6046439840873	9.80344102302003e-07
49.8023219920436	9.68212383084077e-07
50	9.56273015956607e-07

==> matlab/fig2e3.tex <==
0.0100000000000000	0.000499500499500499
0.0117160547237387	0.000575134244485415
0.0134321094474774	0.000653424089765141
0.0151481641712160	0.000734139105094429
0.0168642188949547	0.000817086503368084
0.0185802736186934	0.000902131101531800
0.0202963283424321	0.000989140189349071
0.0220123830661707	0.00107799695459018
0.0237284377899094	0.00116859718622699
0.0271767298921404	0.00135556322014514
0.0306250219943713	0.00154858477378427
0.0340733140966023	0.00174711196343557
0.0375216061988333	0.00195067222968663
0.0427139279135350	0.00226583503124703
0.0479062496282368	0.00259038874837375
0.0530985713429385	0.00292333979630785
0.0582908930576403	0.00326383280164956
0.0666867029016913	0.00382854452095189
0.0750825127457423	0.00440850575108592
0.0834783225897933	0.00500149003782376
0.0918741324338443	0.00560559413919545
0.103221374695157	0.00643691072712012
0.114568616956470	0.00728218984250268
0.125915859217783	0.00813846848534362
0.137263101479095	0.00900318066748862
0.152303542411290	0.0101585859026875
0.167343983343484	0.0113204682653433
0.182384424275678	0.0124849625858641
0.197424865207872	0.0136487296143042
0.216556218911177	0.0151234943866264
0.235687572614481	0.0165873724398017
0.254818926317785	0.0180360475290339
0.273950280021090	0.0194658768814476
0.295702700579699	0.0210648506029080
0.317455121138309	0.0226317876964425
0.339207541696919	0.0241636250937641
0.360959962255528	0.0256578988248820
0.384856456254013	0.0272538611596664
0.408752950252498	0.0288001704058426
0.432649444250983	0.0302953813055605
0.456545938249468	0.0317385191687165
0.482428909122220	0.0332422209863748
0.508311879994973	0.0346838634640514
0.534194850867725	0.0360635287208592
0.560077821740478	0.0373816258939224
0.587789573063889	0.0387253806703365
0.615501324387300	0.0400004319715420
0.643213075710712	0.0412081004587023
0.670924827034123	0.0423498910445965
0.700315973473582	0.0434907241377987
0.729707119913042	0.0445613800651383
0.759098266352501	0.0455640275608614
0.788489412791960	0.0465008975482052
0.819413129909566	0.0474180932828067
0.850336847027172	0.0482676172801331
0.881260564144777	0.0490520987403957
0.912184281262383	0.0497741391417242
0.944496310546559	0.0504646580496845
0.976808339830736	0.0510926429767178
1.00912036911491	0.0516608666010511
1.04143239839909	0.0521720175142916
1.07499283168995	0.0526452791211802
1.10855326498080	0.0530625796144362
1.14211369827166	0.0534266140219297
1.17567413156251	0.0537399650463466
1.21035017643711	0.0540131173291709
1.24502622131171	0.0542374061292274
1.27970226618631	0.0544153182393633
1.31437831106091	0.0545492199638228
1.35004735827022	0.0546434077117891
1.38571640547953	0.0546957463569507
1.42138545268884	0.0547084543334438
1.45705449989815	0.0546836337907148
1.49360694715890	0.0546213493426427
1.53015939441965	0.0545237927176681
1.56671184168041	0.0543929013198249
1.60326428894116	0.0542305068550019
1.64060574378950	0.0540338809347008
1.67794719863784	0.0538079532325059
1.71528865348618	0.0535543952386483
1.75263010833452	0.0532747856944810
1.79068279737963	0.0529645981700663
1.82873548642474	0.0526304244687440
1.86678817546984	0.0522736987950398
1.90484086451495	0.0518957755408343
1.94354426897741	0.0514909700771616
1.98224767343986	0.0510668616312527
2.02095107790232	0.0506246800952401
2.05965448236477	0.0501655872616797
2.09896535948022	0.0496831123520056
2.13827623659567	0.0491854434398124
2.17758711371112	0.0486736381924748
2.21689799082656	0.0481486961902921
2.25679001376257	0.0476035409794314
2.29668203669857	0.0470467985516732
2.33657405963457	0.0464793829857170
2.37646608257057	0.0459021585201589
2.41692934917714	0.0453074928393494
2.45739261578371	0.0447044177419497
2.49785588239028	0.0440937279652403
2.53831914899685	0.0434761750260255
2.57935979595430	0.0428435351095370
2.62040044291174	0.0422053025609506
2.66144108986919	0.0415621725950495
2.70248173682663	0.0409148024155884
2.74412187579687	0.0402542867962250
2.78576201476712	0.0395906944433335
2.82740215373736	0.0389246368315540
2.86904229270760	0.0382566914527537
2.91132048022032	0.0375771470201736
2.95359866773304	0.0368967927605632
2.99587685524576	0.0362161687030350
3.03815504275849	0.0355357839493294
3.08112752419896	0.0348449719162849
3.12410000563943	0.0341554124250074
3.16707248707990	0.0334675834231259
3.21004496852037	0.0327819341879989
3.25378802052889	0.0320866713455419
3.29753107253741	0.0313945573163489
3.34127412454594	0.0307060148917001
3.38501717655446	0.0300214397887134
3.42963104837956	0.0293277131093083
3.47424492020467	0.0286388996553330
3.51885879202977	0.0279553719403454
3.56347266385488	0.0272774764392463
3.60908796232704	0.0265905294308855
3.65470326079919	0.0259101604503783
3.70031855927135	0.0252366948417127
3.74593385774351	0.0245704324490349
3.79272190093334	0.0238948195586963
3.83950994412316	0.0232273830727030
3.88629798731299	0.0225684026445261
3.93308603050281	0.0219181324949120
3.98127611499785	0.0212577318308369
4.02946619949289	0.0206070780692060
4.07765628398793	0.0199664049902776
4.12584636848297	0.0193359205137098
4.17453782062043	0.0187094185712684
4.22322927275788	0.0180937065169063
4.27192072489534	0.0174889572741050
4.32061217703279	0.0168953196039575
4.36915150529233	0.0163147278349372
4.41769083355186	0.0157454386962416
4.46623016181140	0.0151875622167816
4.51476949007093	0.0146411871742398
4.56328105147248	0.0141066905080812
4.61179261287403	0.0135838280487002
4.66030417427557	0.0130726547539376
4.70881573567712	0.0125732067486698
4.75743034626171	0.0120844838361581
4.80604495684629	0.0116075803052807
4.85465956743088	0.0111425020187402
4.90327417801546	0.0106892380631451
4.95214759150491	0.0102454473504860
5.00102100499435	0.00981354921396765
5.04989441848379	0.00939350490008533
5.09876783197324	0.00898526065096142
5.14804659394740	0.00858551276850945
5.19732535592155	0.00819762847798711
5.24660411789571	0.00782152767166466
5.29588287986987	0.00745711683202261
5.34571691623879	0.00710038334048445
5.39555095260772	0.00675539161624060
5.44538498897664	0.00642202257773842
5.49521902534556	0.00610014522355752
5.54578533292858	0.00578514160094631
5.59635164051159	0.00548167990451388
5.64691794809460	0.00518960359986041
5.69748425567761	0.00490874566130882
5.74900092501619	0.00463396585723921
5.80051759435478	0.00437046458449048
5.85203426369337	0.00411804839531661
5.90355093303196	0.00387651476010953
5.95629904554016	0.00364026597107798
6.00904715804837	0.00341498399923999
6.06179527055658	0.00320043773268207
6.11454338306479	0.00299638841704833
6.16890437576226	0.00279682616139312
6.22326536845974	0.00260788866550624
6.27762636115721	0.00242930446262210
6.33198735385468	0.00226079598256681
6.38842448996247	0.00209621155452256
6.44486162607025	0.00194187262743469
6.50129876217804	0.00179746285459607
6.55773589828582	0.00166266157215206
6.61342964774346	0.00153874136947256
6.66912339720110	0.00142355847243422
6.72481714665874	0.00131680469605424
6.78051089611637	0.00121817026290997
6.83589971047198	0.00112782283563774
6.89128852482759	0.00104490030298838
6.94667733918320	0.000969102746943095
7.00206615353882	0.000900130796468798
7.05758976165192	0.000837543293108208
7.11311336976503	0.000781221771353028
7.16863697787814	0.000730873800459613
7.22416058599125	0.000686209308494379
7.28021693986213	0.000646590553078370
7.33627329373302	0.000612184251042022
7.39232964760390	0.000582705205835846
7.44838600147478	0.000557872235430438
7.50538574262213	0.000537100852083301
7.56238548376949	0.000520564623558263
7.61938522491684	0.000507985526182560
7.67638496606419	0.000499091175292555
7.73480587272738	0.000493520751286931
7.79322677939057	0.000491264027012433
7.85164768605376	0.000492050042565890
7.91006859271695	0.000495615194865109
7.97053387043690	0.000501959779294584
8.03099914815685	0.000510734574798764
8.09146442587680	0.000521675250173464
8.15192970359676	0.000534526814460557
8.21535952756943	0.000549794744680725
8.27878935154210	0.000566625546711334
8.34221917551477	0.000584760198178454
8.40564899948744	0.000603951585503725
8.46793784799597	0.000623599152337411
8.53022669650450	0.000643829090298319
8.59251554501303	0.000664441872354294
8.65480439352156	0.000685249103645423
8.71642204054983	0.000705849969531327
8.77803968757810	0.000726307696255112
8.83965733460636	0.000746472197554230
8.90127498163463	0.000766203699206181
8.96300495617631	0.000785407295673177
9.02473493071799	0.000803927100504444
9.08646490525967	0.000821653315759438
9.14819487980135	0.000838485850599994
9.21071927424122	0.000854531622588196
9.27324366868109	0.000869484387173280
9.33576806312096	0.000883269829182389
9.39829245756083	0.000895822847238344
9.46233592838314	0.000907344871544825
9.52637939920544	0.000917465432659954
9.59042287002774	0.000926143562105738
9.65446634085004	0.000933347071295687
9.72096019267431	0.000939240922123606
9.78745404449858	0.000943504034150381
9.85394789632285	0.000946129048631901
9.92044174814712	0.000947116984845593
9.98759919027086	0.000946462799841194
10.0547566323946	0.000944167033225105
10.1219140745184	0.000940255345230974
10.1890715166421	0.000934760053724640
10.2546642923364	0.000927901573130307
10.3202570680308	0.000919612660394850
10.3858498437251	0.000909940802252057
10.4514426194195	0.000898937678982232
10.5165140917340	0.000886761836460539
10.5815855640486	0.000873390353430373
10.6466570363632	0.000858885327436610
10.7117285086778	0.000843311226253483
10.7771443606203	0.000826644878991829
10.8425602125627	0.000809037205866102
10.9079760645052	0.000790560705043755
10.9733919164476	0.000771288717659393
11.0399477645340	0.000750941382770573
11.1065036126204	0.000729927977175097
11.1730594607068	0.000708328536936756
11.2396153087932	0.000686222504839261
11.3082257087532	0.000662987568096582
11.3768361087133	0.000639385784941829
11.4454465086734	0.000615502713319807
11.5140569086335	0.000591421807105933
11.5852093098832	0.000566327239594637
11.6563617111329	0.000541198271486398
11.7275141123826	0.000516121833524801
11.7986665136323	0.000491181110631163
11.8677850418193	0.000467159302876775
11.9369035700062	0.000443412631723133
12.0060220981931	0.000420008581144194
12.0751406263801	0.000397010522721502
12.1433601380698	0.000374768187200598
12.2115796497596	0.000353034631309400
12.2797991614493	0.000331860580930063
12.3480186731391	0.000311292474535633
12.4163461472746	0.000291342058986985
12.4846736214100	0.000272082247029182
12.5530010955455	0.000253548515663788
12.6213285696809	0.000235771948078750
12.6907216414633	0.000218521140695098
12.7601147132457	0.000202104555526980
12.8295077850280	0.000186542790880211
12.8989008568104	0.000171851974386193
12.9703478268833	0.000157649207975078
13.0417947969561	0.000144392328058646
13.1132417670290	0.000132086304708841
13.1846887371018	0.000120731597587191
13.2595560962437	0.000109850212342297
13.3344234553855	0.000100001671644336
13.4092908145273	9.11731885978089e-05
13.4841581736692	8.33474566441327e-05
13.5575412493262	7.66296501953519e-05
13.6309243249833	7.08318953370941e-05
13.7043074006403	6.59276248805504e-05
13.7776904762973	6.18871298258458e-05
13.8500672006557	5.87166311017000e-05
13.9224439250142	5.63217364544802e-05
13.9948206493726	5.46669058826841e-05
14.0671973737310	5.37146511792828e-05
14.1398455416426	5.34260569324126e-05
14.2124937095543	5.37651368569211e-05
14.2851418774659	5.46896873608312e-05
14.3577900453776	5.61565541120039e-05
14.4318616952425	5.81651462716255e-05
14.5059333451073	6.06450014660922e-05
14.5800049949722	6.35487099347316e-05
14.6540766448371	6.68288777043048e-05
14.7309274464065	7.05796026373861e-05
14.8077782479759	7.46325157403710e-05
14.8846290495453	7.89358927674920e-05
14.9614798511146	8.34391056947025e-05
15.0406722118752	8.82364634451296e-05
15.1198645726358	9.31409525818569e-05
15.1990569333964	9.81016005710425e-05
15.2782492941569	0.000103069653827772
15.3552187760152	0.000107861265915206
15.4321882578735	0.000112575259681175
15.5091577397318	0.000117173115623114
15.5861272215900	0.000121618862660207
15.6625824441176	0.000125851326359556
15.7390376666451	0.000129870308226147
15.8154928891726	0.000133647887106827
15.8919481117002	0.000137158901561625
15.9693961674172	0.000140420777191638
16.0468442231342	0.000143365432162868
16.1242922788512	0.000145974942359647
16.2017403345682	0.000148234319851494
16.2817277574867	0.000150187406543548
16.3617151804052	0.000151743739631675
16.4417026033237	0.000152895911611144
16.5216900262422	0.000153639616992635
16.6043553465212	0.000153977654505027
16.6870206668002	0.000153879701826805
16.7696859870792	0.000153350337705090
16.8523513073581	0.000152397123351813
16.9322086407103	0.000151083565970533
17.0120659740625	0.000149395886030702
17.0919233074148	0.000147347753937938
17.1717806407670	0.000144954760795457
17.2507845102887	0.000142265094683211
17.3297883798104	0.000139273516393086
17.4087922493321	0.000135999786694615
17.4877961188537	0.000132464804543545
17.5676116379811	0.000128650638180240
17.6474271571085	0.000124616058934548
17.7272426762358	0.000120385387930290
17.8070581953632	0.000115983397216802
17.8893023304811	0.000111294897326241
17.9715464655990	0.000106479364977900
18.0537906007169	0.000101564724202961
18.1360347358348	9.65786276862920e-05
18.2213159234312	9.13622519928139e-05
18.3065971110275	8.61288780556769e-05
18.3918782986238	8.09078593331539e-05
18.4771594862202	7.57274549886257e-05
18.5595094175750	7.07892581484211e-05
18.6418593489297	6.59381005057449e-05
18.7242092802845	6.11963059902450e-05
18.8065592116393	5.65847441463340e-05
18.8880422520689	5.21690882262209e-05
18.9695252924985	4.79178246831889e-05
19.0510083329281	4.38470347552721e-05
19.1324913733577	3.99711299461522e-05
19.2148776329082	3.62635457477932e-05
19.2972638924588	3.27802088749205e-05
19.3796501520093	2.95310862829840e-05
19.4620364115598	2.65243137479984e-05
19.5470683095882	2.36819750685383e-05
19.6321002076166	2.11100500394077e-05
19.7171321056450	1.88118281434640e-05
19.8021640036734	1.67886389959987e-05
19.8908893408643	1.49702854201975e-05
19.9796146780552	1.34484391978477e-05
20.0683400152462	1.22184884073518e-05
20.1570653524371	1.12738734449459e-05
20.2428390648805	1.06241631737019e-05
20.3286127773240	1.02243973996498e-05
20.4143864897674	1.00641366770577e-05
20.5001602022109	1.01317069751539e-05
20.5852635054960	1.04113512615953e-05
20.6703668087812	1.08892322213938e-05
20.7554701120663	1.15509426343685e-05
20.8405734153514	1.23813970350697e-05
20.9270705233463	1.33822451015945e-05
21.0135676313412	1.45241907680305e-05
21.1000647393361	1.57897625920408e-05
21.1865618473310	1.71613368440173e-05
21.2766604059527	1.86836665417431e-05
21.3667589645743	2.02816533810984e-05
21.4568575231959	2.19352743150317e-05
21.5469560818176	2.36249685053107e-05
21.6381292498009	2.53520705214129e-05
21.7293024177842	2.70772251292184e-05
21.8204755857675	2.87817909996626e-05
21.9116487537508	3.04481613305716e-05
22.0004127698935	3.20180108879602e-05
22.0891767860362	3.35213779619312e-05
22.1779408021788	3.49447554963346e-05
22.2667048183215	3.62758833618082e-05
22.3556370337612	3.75059326644847e-05
22.4445692492010	3.86221963283436e-05
22.5335014646408	3.96158347099375e-05
22.6224336800805	4.04794134019733e-05
22.7139161549811	4.12256408132067e-05
22.8053986298817	4.18224368584462e-05
22.8968811047823	4.22658672331564e-05
22.9883635796829	4.25535525664899e-05
23.0838924299717	4.26867534174635e-05
23.1794212802604	4.26495424605306e-05
23.2749501305492	4.24438472784879e-05
23.3704789808380	4.20732094865253e-05
23.4621509718643	4.15671014501813e-05
23.5538229628905	4.09192309221316e-05
23.6454949539168	4.01361173501586e-05
23.7371669449431	3.92252845915605e-05
23.8279328445987	3.82059138025206e-05
23.9186987442544	3.70785532449181e-05
24.0094646439101	3.58527334057620e-05
24.1002305435658	3.45385451465828e-05
24.1926550919484	3.31204881091917e-05
24.2850796403311	3.16334035609922e-05
24.3775041887138	3.00891025815000e-05
24.4699287370964	2.84995483684694e-05
24.5667881185871	2.67983222344883e-05
24.6636475000779	2.50746134367211e-05
24.7605068815686	2.33420965950759e-05
24.8573662630593	2.16141187253424e-05
24.9520922059339	1.99410862028066e-05
25.0468181488086	1.82966374678575e-05
25.1415440916832	1.66919217274810e-05
25.2362700345578	1.51374063383715e-05
25.3292146875769	1.36703992241605e-05
25.4221593405961	1.22698137743035e-05
25.5151039936153	1.09434424677953e-05
25.6080486466344	9.69822539464542e-06
25.7019756638980	8.52854594187846e-06
25.7959026811617	7.45351804598539e-06
25.8898296984253	6.47764252813173e-06
25.9837567156889	5.60444649256377e-06
26.0813748678075	4.80854840713853e-06
26.1789930199261	4.12829831920359e-06
26.2766111720447	3.56445535276962e-06
26.3742293241633	3.11670887597297e-06
26.4732872431096	2.77970414165058e-06
26.5723451620558	2.55852492584696e-06
26.6714030810021	2.44973728962358e-06
26.7704609999484	2.44899935939631e-06
26.8668464553430	2.54709250782166e-06
26.9632319107376	2.73707355876112e-06
27.0596173661322	3.01275344772636e-06
27.1560028215268	3.36742357995515e-06
27.2528815695420	3.79627323014853e-06
27.3497603175572	4.28989799719094e-06
27.4466390655724	4.84016271569073e-06
27.5435178135875	5.43874717332989e-06
27.6439608492560	6.10132891621486e-06
27.7444038849244	6.79707954278836e-06
27.8448469205929	7.51631124677052e-06
27.9452899562613	8.24952765102585e-06
28.0482405279971	9.00584526431681e-06
28.1511910997329	9.75719073320335e-06
28.2541416714688	1.04940421331990e-05
28.3570922432046	1.12074754405834e-05
28.4567501555253	1.18679104388831e-05
28.5564080678461	1.24913598518302e-05
28.6560659801668	1.30712203510490e-05
28.7557238924876	1.36016319372696e-05
28.8557411898054	1.40790470375287e-05
28.9557584871233	1.44968032229546e-05
29.0557757844411	1.48509903731815e-05
29.1557930817590	1.51385505103440e-05
29.2596833575662	1.53642763331779e-05
29.3635736333734	1.55138664431503e-05
29.4674639091807	1.55863843894245e-05
29.5713541849879	1.55818567952233e-05
29.6759318863875	1.55003992529086e-05
29.7805095877872	1.53434145233083e-05
29.8850872891868	1.51133016467910e-05
29.9896649905864	1.48132671465820e-05
30.0911544966620	1.44589478056518e-05
30.1926440027376	1.40465517299077e-05
30.2941335088132	1.35806368448457e-05
30.3956230148889	1.30662245993902e-05
30.4978092358551	1.25047733809765e-05
30.5999954568214	1.19054931867374e-05
30.7021816777877	1.12744326155397e-05
30.8043678987539	1.06178263293922e-05
30.9109059456037	9.91293702187768e-06
31.0174439924534	9.19450570986956e-06
31.1239820393031	8.46974039914531e-06
31.2305200861528	7.74573038440403e-06
31.3364021990683	7.03378706694898e-06
31.4422843119837	6.33604227198332e-06
31.5481664248991	5.65872244208091e-06
31.6540485378145	5.00765811243285e-06
31.7574284840790	4.40251603250524e-06
31.8608084303435	3.83224399995070e-06
31.9641883766080	3.30098336829646e-06
32.0675683228725	2.81235473899561e-06
32.1722735824859	2.36410860437559e-06
32.2769788420993	1.96549917306958e-06
32.3816841017127	1.61860178235114e-06
32.4863893613262	1.32488740896262e-06
32.5963585110375	1.07464584640074e-06
32.7063276607488	8.84418090630410e-07
32.8162968104602	7.53822431447982e-07
32.9262659601715	6.81809768252652e-07
33.0345223500676	6.66524209068659e-07
33.1427787399638	7.04204843810174e-07
33.2510351298599	7.92105339608094e-07
33.3592915197560	9.27023282439382e-07
33.4657809711845	1.10210477257388e-06
33.5722704226130	1.31531972564429e-06
33.6787598740416	1.56249077161966e-06
33.7852493254701	1.83923334441061e-06
33.8941979357818	2.14821123982796e-06
34.0031465460936	2.47823141594819e-06
34.1120951564054	2.82406785667575e-06
34.2210437667172	3.18053349283046e-06
34.3366404896276	3.56464786151104e-06
34.4522372125380	3.94878144968986e-06
34.5678339354484	4.32695956909545e-06
34.6834306583588	4.69357994589446e-06
34.7936642990230	5.02760265424490e-06
34.9038979396873	5.34195707273250e-06
35.0141315803515	5.63264943892143e-06
35.1243652210157	5.89617073316600e-06
35.2343050512079	6.12888089036947e-06
35.3442448814002	6.32881185039233e-06
35.4541847115924	6.49373698562340e-06
35.5641245417846	6.62198900149299e-06
35.6786017627846	6.71531780468130e-06
35.7930789837846	6.76677820470725e-06
35.9075562047846	6.77608682499017e-06
36.0220334257847	6.74359870599708e-06
36.1362198980123	6.67046889630176e-06
36.2504063702399	6.55799931991467e-06
36.3645928424676	6.40799530173253e-06
36.4787793146952	6.22275722257327e-06
36.5900126053583	6.01102549360586e-06
36.7012458960214	5.77123924134820e-06
36.8124791866845	5.50646232890941e-06
36.9237124773476	5.22001524541649e-06
37.0369057108861	4.90991670229810e-06
37.1500989444246	4.58488742246343e-06
37.2632921779630	4.24885623121121e-06
37.3764854115015	3.90580522660005e-06
37.4962218645145	3.53971436143413e-06
37.6159583175275	3.17492027541483e-06
37.7356947705405	2.81592851302584e-06
37.8554312235534	2.46704939986118e-06
37.9694000931710	2.14811194293150e-06
38.0833689627887	1.84533938180914e-06
38.1973378324063	1.56171657363079e-06
38.3113067020239	1.29990630323835e-06
38.4249000672874	1.06299340637242e-06
38.5384934325510	8.52065145146710e-07
38.6520867978146	6.68710490613114e-07
38.7656801630782	5.14130264753503e-07
38.8839805724880	3.84622022547708e-07
39.0022809818979	2.87719278579278e-07
39.1205813913078	2.23444383202828e-07
39.2388818007176	1.91384850728062e-07
39.3577858169091	1.90798624678544e-07
39.4766898331005	2.20673273025632e-07
39.5955938492920	2.79354025202374e-07
39.7144978654834	3.64860047546183e-07
39.8306400259012	4.72097414675602e-07
39.9467821863190	6.00335096987518e-07
40.0629243467368	7.46938981390226e-07
40.1790665071546	9.09139820856393e-07
40.2979626814797	1.08832978799041e-06
40.4168588558048	1.27757502278464e-06
40.5357550301298	1.47356345493784e-06
40.6546512044549	1.67303493600093e-06
40.7793663330114	1.88251607660172e-06
40.9040814615679	2.08860091594007e-06
41.0287965901244	2.28774796712079e-06
41.1535117186809	2.47670465976925e-06
41.2728913030736	2.64526924906790e-06
41.3922708874662	2.79927409859276e-06
41.5116504718589	2.93652514268199e-06
41.6310300562516	3.05518749138126e-06
41.7513824171239	3.15446901023320e-06
41.8717347779962	3.23202011279476e-06
41.9920871388686	3.28689225269441e-06
42.1124394997409	3.31854775801679e-06
42.2403780838680	3.32655369102178e-06
42.3683166679951	3.30826091579661e-06
42.4962552521223	3.26421878704327e-06
42.6241938362494	3.19544859817441e-06
42.7459262128924	3.10834810816896e-06
42.8676585895354	3.00159163077971e-06
42.9893909661784	2.87688592729143e-06
43.1111233428215	2.73619128386561e-06
43.2323192820888	2.58237995192527e-06
43.3535152213561	2.41713120947622e-06
43.4747111606234	2.24281352469224e-06
43.5959070998906	2.06188512711380e-06
43.7230100636943	1.86777769115279e-06
43.8501130274980	1.67206534186151e-06
43.9772159913017	1.47758495364647e-06
44.1043189551053	1.28708977294966e-06
44.2286927690341	1.10708371342138e-06
44.3530665829628	9.35758513024716e-07
44.4774403968915	7.75242881981398e-07
44.6018142108202	6.27447492543454e-07
44.7243832234717	4.95886719839779e-07
44.8469522361232	3.79708140030388e-07
44.9695212487747	2.80024855922845e-07
45.0920902614261	1.97678810735396e-07
45.2192704569313	1.31181545998389e-07
45.3464506524364	8.43175973687977e-08
45.4736308479415	5.70973677137076e-08
45.6008110434466	4.92268491671072e-08
45.7293487437304	6.03434261858177e-08
45.8578864440142	8.97329357564880e-08
45.9864241442980	1.36213934413509e-07
46.1149618445818	1.98379211727700e-07
46.2403633884128	2.72603174170062e-07
46.3657649322439	3.58519024561550e-07
46.4911664760749	4.54287195281897e-07
46.6165680199060	5.57992465114966e-07
46.7458183814916	6.71095437969933e-07
46.8750687430772	7.88255860714424e-07
47.0043191046628	9.07198011505427e-07
47.1335694662484	1.02572290244609e-06
47.2659682689327	1.14448410033485e-06
47.3983670716170	1.25831978693674e-06
47.5307658743013	1.36512313385651e-06
47.6631646769855	1.46302510692759e-06
47.7913492952116	1.54776810990781e-06
47.9195339134376	1.62123495066237e-06
48.0477185316636	1.68227622220940e-06
48.1759031498897	1.73002272454187e-06
48.3075614879101	1.76457348932526e-06
48.4392198259305	1.78396943402091e-06
48.5708781639510	1.78801158952680e-06
48.7025365019714	1.77681877366497e-06
48.8366959423393	1.75014685065667e-06
48.9708553827072	1.70867978884873e-06
49.1050148230751	1.65328519163105e-06
49.2391742634430	1.58509712724323e-06
49.3688501639382	1.50829462430618e-06
49.4985260644335	1.42213751700299e-06
49.6282019649287	1.32808861638884e-06
49.7578778654240	1.22772527315880e-06
49.8184083990680	1.17918395552637e-06
49.8789389327120	1.12979776672273e-06
49.9394694663560	1.07973929650368e-06
50	1.02918149392503e-06

==> matlab/fig2f1.tex <==
0.0100000000000000	51.6528925619835
0.0179621434110699	20.1882703816768
0.0259242868221399	11.1083029334618
0.0338864302332098	7.14623403711110
0.0418485736442798	5.03147697953507
0.0489549209391593	3.86875239919637
0.0560612682340389	3.07826442694318
0.0631676155289185	2.51416287921236
0.0702739628237981	2.09625388251990
0.0834365541784869	1.56112659461268
0.0965991455331757	1.21155895976667
0.109761736887865	0.969727432985382
0.122924328242553	0.794998156609491
0.141422220690948	0.620623014405764
0.159920113139343	0.498690709769246
0.178418005587737	0.409903119406304
0.196915898036132	0.343141786510630
0.219013608897574	0.282961808549427
0.241111319759016	0.237454467116772
0.263209030620457	0.202175527683994
0.285306741481899	0.174253432914720
0.309342274650222	0.150002464524458
0.333377807818544	0.130496087431495
0.357413340986866	0.114566327982982
0.381448874155189	0.101385284838793
0.406933021704955	0.0897457614590347
0.432417169254721	0.0799971197992759
0.457901316804488	0.0717496369026039
0.483385464354254	0.0647094006076575
0.510146684095585	0.0583702241820718
0.536907903836916	0.0529131382995442
0.563669123578246	0.0481815742238103
0.590430343319577	0.0440523040536047
0.618396556862693	0.0402745580854453
0.646362770405808	0.0369579938804016
0.674328983948924	0.0340305322697925
0.702295197492039	0.0314336649590890
0.731440138666079	0.0290275481225728
0.760585079840118	0.0268839534028509
0.789730021014158	0.0249661173136047
0.818874962188198	0.0232434969132646
0.849202310632316	0.0216308040620344
0.879529659076434	0.0201777086207835
0.909857007520552	0.0188639018292076
0.940184355964671	0.0176722044147780
0.971722764316052	0.0165467588767902
1.00326117266743	0.0155235744374271
1.03479958101881	0.0145906881593646
1.06633798937020	0.0137378346986150
1.09914059673297	0.0129262040353400
1.13194320409574	0.0121829902005638
1.16474581145851	0.0115007612168073
1.19754841882128	0.0108730656705431
1.23169524674606	0.0102715331284901
1.26584207467084	0.00971747486212813
1.29998890259562	0.00920605953690130
1.33413573052039	0.00873305358679026
1.36973897643827	0.00827675977627586
1.40534222235615	0.00785446587438109
1.44094546827402	0.00746290377843121
1.47654871419190	0.00709918758514181
1.51333148231955	0.00674995503933176
1.55011425044721	0.00642521842236093
1.58689701857486	0.00612276025907693
1.62367978670251	0.00584060749145267
1.66101214689026	0.00557319357357406
1.69834450707800	0.00532323896988935
1.73567686726574	0.00508927152714819
1.77300922745348	0.00486997037858942
1.81093729414381	0.00466096669624264
1.84886536083414	0.00446475367073224
1.88679342752446	0.00428031986849695
1.92472149421479	0.00410675140738080
1.96329948808217	0.00394050165964031
2.00187748194955	0.00378384793368682
2.04045547581692	0.00363607426441900
2.07903346968430	0.00349652988087216
2.11832628074299	0.00336224664750298
2.15761909180168	0.00323531533203669
2.19691190286036	0.00311521549806961
2.23620471391905	0.00300147169352055
2.27628788215811	0.00289153800524825
2.31637105039716	0.00278734316040033
2.35645421863622	0.00268849973623904
2.39653738687527	0.00259465225760217
2.43749810706159	0.00250357161612824
2.47845882724791	0.00241704665068642
2.51941954743422	0.00233478265249434
2.56038026762054	0.00225650820724555
2.60231930174224	0.00218023659327073
2.64425833586394	0.00210763724741424
2.68619736998564	0.00203848148478772
2.72813640410734	0.00197255802473257
2.77117099359047	0.00190806770487935
2.81420558307360	0.00184657968951206
2.85724017255673	0.00178791320309471
2.90027476203986	0.00173190077476629
2.94454280820470	0.00167688864933412
2.98881085436955	0.00162436380293683
3.03307890053439	0.00157418079508314
3.07734694669924	0.00152620458124187
3.12301296380697	0.00147889287995121
3.16867898091470	0.00143366795206125
3.21434499802243	0.00139041077626801
3.26001101513015	0.00134901062989205
3.30727473639622	0.00130800787136796
3.35453845766229	0.00126877752997628
3.40180217892835	0.00123122054822974
3.44906590019442	0.00119524463615895
3.49817508767041	0.00115944658087355
3.54728427514641	0.00112517259000286
3.59639346262241	0.00109233879131977
3.64550265009840	0.00106086695438685
3.69677296104368	0.00102938432255564
3.74804327198896	0.000999229044545852
3.79931358293424	0.000970328801814448
3.85058389387952	0.000942616091210757
3.90443140626832	0.000914719939497795
3.95827891865712	0.000887995972090398
4.01212643104593	0.000862380562209333
4.06597394343473	0.000837814303009680
4.12210104024892	0.000813264883147882
4.17822813706310	0.000789736310302891
4.23435523387729	0.000767173761683214
4.29048233069147	0.000745526011387193
4.34732453072746	0.000724485783584692
4.40416673076345	0.000704288125808377
4.46100893079944	0.000684889458425974
4.51785113083543	0.000666248956148795
4.57582743647441	0.000647977869001049
4.63380374211339	0.000630417607849621
4.69178004775237	0.000613532455208929
4.74975635339135	0.000597288886905783
4.80927575174908	0.000581247372051190
4.86879515010681	0.000565816867302136
4.92831454846454	0.000550967316724794
4.98783394682227	0.000536670471230060
5.04934227097890	0.000522448380195929
5.11085059513554	0.000508760609920502
5.17235891929218	0.000495581239754887
5.23386724344882	0.000482885885682826
5.29789405007311	0.000470160162772284
5.36192085669741	0.000457909678792261
5.42594766332170	0.000446111523035591
5.48997446994599	0.000434744134321013
5.55719875822752	0.000423250434755389
5.62442304650904	0.000412187111579450
5.69164733479056	0.000401533368499935
5.75887162307208	0.000391269636762512
5.83023614825156	0.000380780000167823
5.90160067343103	0.000370688404846077
5.97296519861051	0.000360975368253611
6.04432972378998	0.000351622572293788
6.12127947749308	0.000341921636697921
6.19822923119618	0.000332599213453246
6.27517898489927	0.000323636264488179
6.35212873860237	0.000315014920405727
6.43723247735917	0.000305857629875340
6.52233621611597	0.000297076390432260
6.60743995487277	0.000288651313652029
6.69254369362957	0.000280563793813532
6.78171540330365	0.000272432862272587
6.87088711297772	0.000264634663273526
6.96005882265180	0.000257151665809476
7.04923053232588	0.000249967465077111
7.14466391282726	0.000242592394127127
7.24009729332864	0.000235524359035269
7.33553067383002	0.000228746910685716
7.43096405433140	0.000222244673983117
7.53934576535893	0.000215175781976957
7.64772747638647	0.000208423683581862
7.75610918741400	0.000201970132191349
7.86449089844153	0.000195798160594901
7.96911887225926	0.000190092253662083
8.07374684607698	0.000184620782246717
8.17837481989470	0.000179371356853752
8.28300279371242	0.000174332385773285
8.38717830981286	0.000169513527359061
8.49135382591330	0.000164882503830647
8.59552934201374	0.000160429894303767
8.69970485811419	0.000156146853858001
8.80416336793757	0.000152014087675263
8.90862187776095	0.000148035580685537
9.01308038758434	0.000144203922425402
9.11753889740773	0.000140512136502812
9.21807327203068	0.000137084994980405
9.31860764665363	0.000133775795135990
9.41914202127658	0.000130579309892678
9.51967639589953	0.000127490594838509
9.61962880891270	0.000124521965002038
9.71958122192588	0.000121650879406538
9.81953363493905	0.000118873209399773
9.91948604795222	0.000116185039618650
10.0207435189413	0.000113549227715004
10.1220009899305	0.000110997790618442
10.2232584609196	0.000108527249041272
10.3245159319087	0.000106134298828319
10.4283846120172	0.000103756969316701
10.5322532921256	0.000101454762698146
10.6361219722340	9.92246212410394e-05
10.7399906523424	9.70636391344348e-05
10.8475748287719	9.48953245670320e-05
10.9551590052014	9.27953247979217e-05
11.0627431816309	9.07608679269540e-05
11.1703273580604	8.87893193263887e-05
11.2826122346865	8.67960093006969e-05
11.3948971113127	8.48657898679977e-05
11.5071819879388	8.29960899137922e-05
11.6194668645650	8.11844661863226e-05
11.7372536318931	7.93439528564018e-05
11.8550403992212	7.75622440990287e-05
11.9728271665493	7.58369215139685e-05
12.0906139338774	7.41656880440588e-05
12.2143018181317	7.24665601566867e-05
12.3379897023860	7.08222705210394e-05
12.4616775866403	6.92305416209484e-05
12.5853654708946	6.76892113148711e-05
12.7146136383583	6.61302139539412e-05
12.8438618058221	6.46217823959082e-05
12.9731099732858	6.31618066227466e-05
13.1023581407496	6.17482839928927e-05
13.2358862805105	6.03347210557635e-05
13.3694144202714	5.89667189607141e-05
13.5029425600323	5.76423887083582e-05
13.6364706997933	5.63599368063840e-05
13.7724345754501	5.50953616131654e-05
13.9083984511069	5.38707318103340e-05
14.0443623267637	5.26844242547575e-05
14.1803262024205	5.15348962370026e-05
14.3171940356473	5.04133879196300e-05
14.4540618688741	4.93262399667052e-05
14.5909297021008	4.82720980359497e-05
14.7277975353276	4.72496728967431e-05
14.8649284638827	4.62558585861566e-05
15.0020593924377	4.52914740772588e-05
15.1391903209927	4.43553980098482e-05
15.2763212495477	4.34465611483543e-05
15.4138654423835	4.25613222631423e-05
15.5514096352193	4.17014787847685e-05
15.6889538280551	4.08660932020069e-05
15.8264980208909	4.00542702323528e-05
15.9650100243167	3.92596805703323e-05
16.1035220277425	3.84872842922886e-05
16.2420340311683	3.77362836552422e-05
16.3805460345941	3.70059159077788e-05
16.5206781669815	3.62872563782509e-05
16.6608102993689	3.55882458731962e-05
16.8009424317563	3.49081929902393e-05
16.9410745641437	3.42464360171854e-05
17.0834062487309	3.35923690540238e-05
17.2257379333181	3.29558878040392e-05
17.3680696179053	3.23363837570731e-05
17.5104013024924	3.17332741000164e-05
17.6553488510412	3.11353519343229e-05
17.8002963995899	3.05532882543207e-05
17.9452439481386	2.99865417612299e-05
18.0901914966873	2.94345937051615e-05
18.2379619557187	2.88866146457749e-05
18.3857324147501	2.83529941291859e-05
18.5335028737815	2.78332479839445e-05
18.6812733328129	2.73269119637461e-05
18.8318594722471	2.68242629319867e-05
18.9824456116813	2.63346256213945e-05
19.1330317511155	2.58575665887368e-05
19.2836178905498	2.53926700123472e-05
19.4368432212972	2.49316977502483e-05
19.5900685520447	2.44825014759375e-05
19.7432938827921	2.40446940769270e-05
19.8965192135396	2.36179039716470e-05
20.0521273153262	2.31953855844462e-05
20.2077354171128	2.27835030699930e-05
20.3633435188993	2.23819119091506e-05
20.5189516206859	2.19902812030050e-05
20.6767074948662	2.16030866823002e-05
20.8344633690465	2.12254844809369e-05
20.9922192432268	2.08571688035513e-05
21.1499751174070	2.04978457530418e-05
21.3097363309718	2.01428307902944e-05
21.4694975445366	1.97964666460265e-05
21.6292587581014	1.94584820618293e-05
21.7890199716662	1.91286161610631e-05
21.9507550228406	1.88026878980055e-05
22.1124900740149	1.84845724886570e-05
22.2742251251893	1.81740289338047e-05
22.4359601763636	1.78708253082656e-05
22.5997219235879	1.75710723281857e-05
22.7634836708122	1.72783924205022e-05
22.9272454180365	1.69925708158339e-05
23.0910071652607	1.67134007051093e-05
23.2568857402592	1.64371990594043e-05
23.4227643152578	1.61674182072175e-05
23.5886428902563	1.59038660737845e-05
23.7545214652548	1.56463575982107e-05
23.9225997668194	1.53914159988956e-05
24.0906780683841	1.51423175027493e-05
24.2587563699487	1.48988897787555e-05
24.4268346715134	1.46609667002950e-05
24.5971602465273	1.44253139114255e-05
24.7674858215413	1.41949887288905e-05
24.9378113965552	1.39698361619581e-05
25.1081369715692	1.37497067242307e-05
25.2807146345169	1.35316421568440e-05
25.4532922974645	1.33184416732195e-05
25.6258699604122	1.31099656596792e-05
25.7984476233598	1.29060793945758e-05
25.9732496005806	1.27041110387701e-05
26.1480515778014	1.25065876889031e-05
26.3228535550222	1.23133834612150e-05
26.4976555322430	1.21243768241607e-05
26.6746407580550	1.19371660340634e-05
26.8516259838669	1.17540204193124e-05
27.0286112096789	1.15748263915017e-05
27.2055964354908	1.13994742369529e-05
27.3847291106506	1.12257981699161e-05
27.5638617858103	1.10558430206163e-05
27.7429944609701	1.08895062085258e-05
27.9221271361299	1.07266886056803e-05
28.1033873526667	1.05654214849347e-05
28.2846475692035	1.04075636205725e-05
28.4659077857403	1.02530222704947e-05
28.6471680022771	1.01017077727063e-05
28.8305524749318	9.95181519405575e-06
29.0139369475864	9.80504997874703e-06
29.1973214202411	9.66132816558771e-06
29.3807058928957	9.52056854545314e-06
29.5662216026754	9.38110685216619e-06
29.7517373124551	9.24451752231223e-06
29.9372530222348	9.11072443141351e-06
30.1227687320145	8.97965391818339e-06
30.3104244405387	8.84976851890789e-06
30.4980801490630	8.72252451425115e-06
30.6857358575872	8.59785278401549e-06
30.8733915661115	8.47568641638240e-06
31.0631915046256	8.35460644724414e-06
31.2529914431398	8.23595824592004e-06
31.4427913816539	8.11967896769331e-06
31.6325913201681	8.00570775083576e-06
31.8245330634793	7.89273752343575e-06
32.0164748067905	7.78200839610362e-06
32.2084165501018	7.67346316127220e-06
32.4003582934130	7.56704639440175e-06
32.5944343723426	7.46155560204778e-06
32.7885104512723	7.35813217278829e-06
32.9825865302019	7.25672397369443e-06
33.1766626091316	7.15728047703002e-06
33.3728638888244	7.05869516503338e-06
33.5690651685172	6.96201870389379e-06
33.7652664482099	6.86720353565440e-06
33.9614677279027	6.77420354913430e-06
34.1597863981921	6.68199898208342e-06
34.3581050684815	6.59155851923106e-06
34.5564237387709	6.50283873098565e-06
34.7547424090604	6.41579749326862e-06
34.9551733102377	6.32949300442589e-06
35.1556042114151	6.24482035019541e-06
35.3560351125925	6.16173982907595e-06
35.5564660137699	6.08021291901356e-06
35.7590062381233	5.99936814034306e-06
35.9615464624766	5.92003423465792e-06
36.1640866868299	5.84217486987623e-06
36.3666269111833	5.76575478075813e-06
36.5712744813487	5.68996649947594e-06
36.7759220515142	5.61557836590354e-06
36.9805696216796	5.54255709644041e-06
37.1852171918451	5.47087037362745e-06
37.3919698016115	5.39976950014948e-06
37.5987224113779	5.32996730861985e-06
37.8054750211443	5.26143327699440e-06
38.0122276309107	5.19413775918977e-06
38.2210820628669	5.12738624954881e-06
38.4299364948231	5.06184033609188e-06
38.6387909267793	4.99747200167375e-06
38.8476453587355	4.93425402423182e-06
39.0585976322966	4.87154185850554e-06
39.2695499058576	4.80994979939377e-06
39.4805021794187	4.74945210464782e-06
39.6914544529798	4.69002375446585e-06
39.9045003567214	4.63106615001873e-06
40.1175462604631	4.57315006250295e-06
40.3305921642047	4.51625181796844e-06
40.5436380679464	4.46034839959807e-06
40.7587736492092	4.40488337463191e-06
40.9739092304720	4.35038755574147e-06
41.1890448117348	4.29683915131886e-06
41.4041803929976	4.24421696809362e-06
41.6214021542161	4.19200326087512e-06
41.8386239154346	4.14069216967292e-06
42.0558456766532	4.09026361761125e-06
42.2730674378717	4.04069807316840e-06
42.4923722413425	3.99151334401220e-06
42.7116770448134	3.94316985711223e-06
42.9309818482842	3.89564909912628e-06
43.1502866517551	3.84893305426958e-06
43.3716714967573	3.80257228015736e-06
43.5930563417596	3.75699613359060e-06
43.8144411867618	3.71218752828024e-06
44.0358260317640	3.66812983233043e-06
44.2592878797955	3.62440383210777e-06
44.4827497278270	3.58141018961108e-06
44.7062115758585	3.53913312231517e-06
44.9296734238900	3.49755726306443e-06
45.1552091541436	3.45629133089337e-06
45.3807448843971	3.41570945703553e-06
45.6062806146507	3.37579705124230e-06
45.8318163449043	3.33653990331637e-06
46.0594228148368	3.29757255342006e-06
46.2870292847694	3.25924459448846e-06
46.5146357547020	3.22154252761396e-06
46.7422422246345	3.18445320194213e-06
46.9719163573238	3.14763503184212e-06
47.2015904900131	3.11141491146461e-06
47.4312646227023	3.07578034175086e-06
47.6609387553916	3.04071914267610e-06
47.8926775894859	3.00591181290396e-06
48.1244164235803	2.97166424048174e-06
48.3561552576747	2.93796484317772e-06
48.5878940917691	2.90480233145082e-06
48.8216947775496	2.87187764939546e-06
49.0554954633302	2.83947722943899e-06
49.2892961491107	2.80759033076930e-06
49.5230968348912	2.77620648132799e-06
49.6423226261684	2.76039277651145e-06
49.7615484174456	2.74470589922205e-06
49.8807742087228	2.72914453774484e-06
50	2.71370739697146e-06

==> matlab/fig2f2.tex <==
0.0100000000000000	24.5074012351730
0.0148893961920471	16.3014220877333
0.0197787923840941	12.1542533535015
0.0246681885761412	9.65242069153071
0.0295575847681883	7.97939161609705
0.0344469809602354	6.78222777006838
0.0393363771522824	5.88346796872704
0.0442257733443295	5.18412848281473
0.0491151695363766	4.62464102840510
0.0566647429666537	3.95141507003684
0.0642143163969308	3.43755733988396
0.0717638898272080	3.03274431093546
0.0793134632574851	2.70581379017925
0.0908118553010885	2.31365053432518
0.102310247344692	2.01100515829274
0.113808639388295	1.77069439659712
0.125307031431899	1.57551485395517
0.141369341375589	1.35747665202286
0.157431651319280	1.18537905404053
0.173493961262971	1.04639083567881
0.189556271206662	0.932034245608830
0.209054765188173	0.818065337210282
0.228553259169684	0.724710599362227
0.248051753151195	0.647042069288992
0.267550247132706	0.581573064034296
0.290054092995263	0.517899114474851
0.312557938857820	0.464272016869556
0.335061784720377	0.418612682545771
0.357565630582934	0.379369639876089
0.382022894637376	0.342625862995685
0.406480158691819	0.310909102702747
0.430937422746262	0.283324750601755
0.455394686800704	0.259173431656226
0.481569771421338	0.236502956217267
0.507744856041972	0.216590181620217
0.533919940662606	0.199002476555704
0.560095025283240	0.183390227531613
0.587815541450838	0.168693693609490
0.615536057618436	0.155615624098315
0.643256573786034	0.143927909943215
0.670977089953632	0.133441626204148
0.700118255075150	0.123540781896534
0.729259420196668	0.114640391486866
0.758400585318186	0.106611906532987
0.787541750439704	0.0993468345324663
0.818002822213866	0.0924689871136673
0.848463893988028	0.0862352246320973
0.878924965762190	0.0805692523999142
0.909386037536352	0.0754057114580834
0.941083529314273	0.0705055633736742
0.972781021092195	0.0660339318734585
1.00447851287012	0.0619436150447050
1.03617600464804	0.0581936834646620
1.06904120797423	0.0546269913444286
1.10190641130043	0.0513533227066194
1.13477161462662	0.0483424554791634
1.16763681795282	0.0455679183993233
1.20161504757622	0.0429231791188960
1.23559327719962	0.0404835773453680
1.26957150682302	0.0382291903925327
1.30354973644643	0.0361424189046247
1.33860026934466	0.0341489307512903
1.37365080224289	0.0323020442468494
1.40870133514113	0.0305882883624585
1.44375186803936	0.0289956758533168
1.47984820246859	0.0274708846003203
1.51594453689782	0.0260528098888457
1.55204087132705	0.0247321347552543
1.58813720575629	0.0235005159076017
1.62526753796055	0.0223186545737091
1.66239787016482	0.0212157857263802
1.69952820236909	0.0201853319102347
1.73665853457335	0.0192213704983270
1.77482648733532	0.0182941587885577
1.81299444009729	0.0174263241783007
1.85116239285926	0.0166131345270995
1.88933034562123	0.0158503081876177
1.92855606837490	0.0151147390200056
1.96778179112857	0.0144244459073122
2.00700751388225	0.0137759635064830
2.04623323663592	0.0131661430546459
2.08655507259207	0.0125765666276261
2.12687690854821	0.0120219822358897
2.16719874450436	0.0114998092075329
2.20752058046051	0.0110076938999733
2.24899759325488	0.0105305787134940
2.29047460604925	0.0100808566803082
2.33195161884362	0.00965657459102252
2.37342863163800	0.00925594527578057
2.41614443981355	0.00886634579725558
2.45886024798911	0.00849845800354919
2.50157605616466	0.00815077996868190
2.54429186434021	0.00782193357885716
2.58836050906038	0.00750106806986251
2.63242915378054	0.00719762161113630
2.67649779850070	0.00691042085986350
2.72056644322086	0.00663838662166282
2.76614153781910	0.00637194964940309
2.81171663241733	0.00611965930043672
2.85729172701556	0.00588058393745815
2.90286682161380	0.00565386498185492
2.94925709579494	0.00543496261909788
2.99564736997608	0.00522727096109880
3.04203764415721	0.00503007796967083
3.08842791833835	0.00484272545349638
3.13504806192754	0.00466374377095606
3.18166820551672	0.00449351275830484
3.22828834910590	0.00433150177801424
3.27490849269509	0.00417721850846119
3.32184817451336	0.00402922219201180
3.36878785633164	0.00388816273065564
3.41572753814992	0.00375363682137892
3.46266721996820	0.00362526908395523
3.51002497981212	0.00350164332290063
3.55738273965604	0.00338359526678550
3.60474049949997	0.00327081274786019
3.65209825934389	0.00316300440530899
3.69997786202684	0.00305878716004803
3.74785746470979	0.00295911332604037
3.79573706739275	0.00286373718684083
3.84361667007570	0.00277242885297153
3.89212998835124	0.00268384046228393
3.94064330662678	0.00259899761660794
3.98915662490232	0.00251770385282127
4.03766994317786	0.00243977498152321
4.08694045495193	0.00236389613367653
4.13621096672600	0.00229113995646280
4.18548147850007	0.00222134701946943
4.23475199027414	0.00215436758748460
4.28491921268052	0.00208891450070984
4.33508643508690	0.00202609277435728
4.38525365749328	0.00196577116589037
4.43542087989966	0.00190782622952551
4.48664627573137	0.00185099076959436
4.53787167156309	0.00179639576774407
4.58909706739480	0.00174393165322518
4.64032246322651	0.00169349523782558
4.69279768899344	0.00164382914692570
4.74527291476036	0.00159609040368601
4.79774814052728	0.00155018622109725
4.85022336629421	0.00150602913251883
4.90418235407362	0.00146235856602349
4.95814134185303	0.00142036349709730
5.01210032963244	0.00137996418120589
5.06605931741185	0.00134108539404538
5.12179691896912	0.00130244627262403
5.17753452052639	0.00126528000086308
5.23327212208366	0.00122951693976473
5.28900972364093	0.00119509137145074
5.34691229243864	0.00116067853978467
5.40481486123634	0.00112757652493995
5.46271743003406	0.00109572340153339
5.52061999883177	0.00106506072756720
5.58121953325118	0.00103418479209194
5.64181906767059	0.00100449267266596
5.70241860209001	0.000975928087205404
5.76301813650942	0.000948437939142840
5.82511460237858	0.000921330903010235
5.88721106824774	0.000895248530370929
5.94930753411689	0.000870142791561352
6.01140399998605	0.000845968337125145
6.07380159490291	0.000822571499875846
6.13619918981976	0.000800030661893174
6.19859678473662	0.000778306980951817
6.26099437965347	0.000757363713521260
6.32419436949673	0.000736911064375648
6.38739435933999	0.000717189150966004
6.45059434918325	0.000698165588807372
6.51379433902651	0.000679809702558310
6.57830719489551	0.000661730948298609
6.64282005076451	0.000644288310961267
6.70733290663351	0.000627454025894538
6.77184576250251	0.000611201771667656
6.83824117080171	0.000595056702650285
6.90463657910091	0.000579475886366504
6.97103198740010	0.000564434861193931
7.03742739569930	0.000549910428422084
7.10642156558373	0.000535341204363984
7.17541573546816	0.000521282621666803
7.24440990535259	0.000507712481486179
7.31340407523702	0.000494609734132084
7.38600948734619	0.000481303975286287
7.45861489945535	0.000468471654270990
7.53122031156452	0.000456091881330071
7.60382572367369	0.000444144864071621
7.68169060479945	0.000431791996793154
7.75955548592521	0.000419893382113861
7.83742036705097	0.000408428313061048
7.91528524817673	0.000397377206044105
7.99490567291899	0.000386485707258496
8.07452609766125	0.000375988929736391
8.15414652240351	0.000365869139183169
8.23376694714577	0.000356109549633924
8.31391886159019	0.000346632537520274
8.39407077603461	0.000337489080841080
8.47422269047904	0.000328664622520571
8.55437460492346	0.000320145361775527
8.63687721049298	0.000311681203783369
8.71937981606250	0.000303513005239869
8.80188242163202	0.000295627934181127
8.88438502720155	0.000288013820960970
8.97139686058978	0.000280264400750387
9.05840869397802	0.000272790688347857
9.14542052736626	0.000265580523161737
9.23243236075449	0.000258622382992077
9.32093858739016	0.000251792027178601
9.40944481402583	0.000245200230993316
9.49795104066150	0.000238836663781552
9.58645726729716	0.000232691527408998
9.67248667547180	0.000226918877213444
9.75851608364644	0.000221335705644903
9.84454549182108	0.000215934297754521
9.93057489999572	0.000210707312695984
10.0166970837528	0.000205642394370303
10.1028192675098	0.000200738596812246
10.1889414512669	0.000195989560669790
10.2750636350240	0.000191389225577691
10.3632012635051	0.000186829167316456
10.4513388919862	0.000182412898222957
10.5394765204673	0.000178134792545889
10.6276141489484	0.000173989486731527
10.7197494921261	0.000169792582756754
10.8118848353039	0.000165729641005309
10.9040201784817	0.000161795356550510
10.9961555216594	0.000157984674682255
11.0865603570731	0.000154361053057001
11.1769651924869	0.000150847452758685
11.2673700279006	0.000147439727960285
11.3577748633143	0.000144133918974652
11.4470969932176	0.000140964092063421
11.5364191231210	0.000137886572544214
11.6257412530243	0.000134898023377613
11.7150633829276	0.000131995251305386
11.8051167656774	0.000129152445978982
11.8951701484272	0.000126390722448969
11.9852235311770	0.000123707209415271
12.0752769139267	0.000121099156778189
12.1675783486168	0.000118501551101115
12.2598797833068	0.000115977735203776
12.3521812179968	0.000113525106521427
12.4444826526868	0.000111141171905186
12.5406946243167	0.000108726780535233
12.6369065959466	0.000106381840923303
12.7331185675765	0.000104103872829212
12.8293305392064	0.000101890501580423
12.9317611576690	9.96025123232990e-05
13.0341917761316	9.73825378599682e-05
13.1366223945942	9.52280687581973e-05
13.2390530130568	9.31367059080764e-05
13.3436694630454	9.10634701029097e-05
13.4482859130340	8.90513321461755e-05
13.5529023630227	8.70980572013245e-05
13.6575188130113	8.52015078412591e-05
13.7639378760502	8.33283700241447e-05
13.8703569390891	8.15097544770515e-05
13.9767760021280	7.97436912616034e-05
14.0831950651669	7.80282952594228e-05
14.1948918891323	7.62803523722687e-05
14.3065887130976	7.45842437736656e-05
14.4182855370630	7.29380617398098e-05
14.5299823610283	7.13399822064601e-05
14.6523445390369	6.96424575942581e-05
14.7747067170456	6.79983778976572e-05
14.8970688950542	6.64056557410881e-05
15.0194310730629	6.48623008435383e-05
15.1511465632349	6.32539706972075e-05
15.2828620534069	6.16983895717669e-05
15.4145775435789	6.01934120641553e-05
15.5462930337509	5.87369966573360e-05
15.6816426907559	5.72889450754580e-05
15.8169923477609	5.58881135967227e-05
15.9523420047659	5.45325926354856e-05
16.0876916617709	5.32205645491459e-05
16.2195694981085	5.19823736463125e-05
16.3514473344461	5.07823034140038e-05
16.4833251707836	4.96188977428628e-05
16.6152030071212	4.84907667731416e-05
16.7409056818706	4.74470794469306e-05
16.8666083566200	4.64331356513676e-05
16.9923110313695	4.54478831396210e-05
17.1180137061189	4.44903140295678e-05
17.2460071843381	4.35427408676238e-05
17.3740006625573	4.26218915339243e-05
17.5019941407765	4.17268303748805e-05
17.6299876189957	4.08566607808330e-05
17.7565892512773	4.00195982172174e-05
17.8831908835589	3.92052502106013e-05
18.0097925158406	3.84128513542569e-05
18.1363941481222	3.76416669891096e-05
18.2599448561665	3.69088461408788e-05
18.3834955642107	3.61949278808533e-05
18.5070462722549	3.54993065506381e-05
18.6305969802992	3.48213996340824e-05
18.7553803779988	3.41541388614021e-05
18.8801637756984	3.35038206903830e-05
19.0049471733980	3.28699106948078e-05
19.1297305710976	3.22518945535625e-05
19.2592552219338	3.16266774214113e-05
19.3887798727700	3.10175188343870e-05
19.5183045236062	3.04239064390552e-05
19.6478291744424	2.98453473763609e-05
19.7861929856835	2.92433995347674e-05
19.9245567969247	2.86575331217706e-05
20.0629206081659	2.80872146012378e-05
20.2012844194070	2.75319315411004e-05
20.3511564871112	2.69468563833309e-05
20.5010285548154	2.63782443050132e-05
20.6509006225196	2.58255202279036e-05
20.8007726902238	2.52881330152342e-05
20.9588361116552	2.47374091471270e-05
21.1168995330866	2.42025633009657e-05
21.2749629545180	2.36830272818087e-05
21.4330263759494	2.31782571233825e-05
21.6190635682705	2.26023652056228e-05
21.8051007605917	2.20453967859369e-05
21.9911379529128	2.15065808510284e-05
22.1771751452340	2.09851837832953e-05
22.3458199885345	2.05269983669506e-05
22.5144648318351	2.00820563947296e-05
22.6831096751357	1.96498827665383e-05
22.8517545184363	1.92300226911975e-05
23.0203993617369	1.88220406806868e-05
23.1890442050374	1.84255196009168e-05
23.3576890483380	1.80400597754811e-05
23.5263338916386	1.76652781390830e-05
23.6920944741673	1.73069561378816e-05
23.8578550566961	1.69582608069047e-05
24.0236156392249	1.66188709882134e-05
24.1893762217536	1.62884782968188e-05
24.3482102075099	1.59800585487427e-05
24.5070441932662	1.56793771059533e-05
24.6658781790225	1.53861927672635e-05
24.8247121647788	1.51002732981432e-05
24.9797169326094	1.48280371811768e-05
25.1347217004401	1.45623065164672e-05
25.2897264682707	1.43028881221254e-05
25.4447312361014	1.40495956600828e-05
25.6022628713019	1.37982654304435e-05
25.7597945065025	1.35528947699770e-05
25.9173261417030	1.33133080641858e-05
26.0748577769036	1.30793358725802e-05
26.2399748574646	1.28399457655261e-05
26.4050919380255	1.26063626948865e-05
26.5702090185865	1.23784116286070e-05
26.7353260991475	1.21559238279842e-05
26.9135866885254	1.19216712773310e-05
27.0918472779033	1.16933996378694e-05
27.2701078672812	1.14709192278218e-05
27.4483684566591	1.12540475391796e-05
27.6461875512081	1.10197336277012e-05
27.8440066457571	1.07918799616662e-05
28.0418257403061	1.05702654083213e-05
28.2396448348551	1.03546778568839e-05
28.4582261869192	1.01232275007240e-05
28.6768075389832	9.89862442811998e-06
28.8953888910472	9.68061726956819e-06
29.1139702431113	9.46896564903795e-06
29.3320751105215	9.26388115153618e-06
29.5501799779317	9.06467696961982e-06
29.7682848453419	8.87114383705584e-06
29.9863897127521	8.68308136164867e-06
30.1847014566922	8.51667240560630e-06
30.3830132006322	8.35448891968001e-06
30.5813249445722	8.19639762621515e-06
30.7796366885122	8.04227026071996e-06
30.9653208272272	7.90144077598138e-06
31.1510049659422	7.76388048938773e-06
31.3366891046572	7.62949508018852e-06
31.5223732433722	7.49819347459386e-06
31.7057580297484	7.37145857194980e-06
31.8891428161245	7.24756391110578e-06
32.0725276025007	7.12643036618585e-06
32.2559123888769	7.00798144200810e-06
32.4435767931044	6.88947046802019e-06
32.6312411973319	6.77361679891475e-06
32.8189056015594	6.66034636746679e-06
33.0065700057869	6.54958757020398e-06
33.2035317736837	6.43596720723442e-06
33.4004935415806	6.32495991754246e-06
33.5974553094774	6.21649100714934e-06
33.7944170773742	6.11048832974749e-06
34.0042348370502	6.00020134955902e-06
34.2140525967261	5.89255266641124e-06
34.4238703564021	5.78746385416685e-06
34.6336881160780	5.68485926782313e-06
34.8550217447865	5.57923520210114e-06
35.0763553734949	5.47621177269972e-06
35.2976890022033	5.37570942645677e-06
35.5190226309117	5.27765151278630e-06
35.7420476120856	5.18124189391280e-06
35.9650725932595	5.08716636570494e-06
36.1880975744334	4.99535471480431e-06
36.4111225556072	4.90573924734560e-06
36.6266455989052	4.82116346429011e-06
36.8421686422032	4.73852077357522e-06
37.0576916855012	4.65775625786786e-06
37.2732147287991	4.57881686150025e-06
37.4822671682508	4.50394269179895e-06
37.6913196077025	4.43069221193338e-06
37.9003720471542	4.35902164447037e-06
38.1094244866059	4.28888862080279e-06
38.3178434323715	4.22045789802212e-06
38.5262623781370	4.15347530124712e-06
38.7346813239026	4.08790272444735e-06
38.9431002696682	4.02370325859829e-06
39.1562974204122	3.95941537915044e-06
39.3694945711562	3.89648981393436e-06
39.5826917219003	3.83489066630762e-06
39.7958888726443	3.77458316875232e-06
40.0176196036804	3.71319580200736e-06
40.2393503347166	3.65313244792532e-06
40.4610810657527	3.59435760129091e-06
40.6828117967889	3.53683689337097e-06
40.9137026787675	3.47823697259873e-06
41.1445935607461	3.42092452301320e-06
41.3754844427247	3.36486437879591e-06
41.6063753247033	3.31002252051398e-06
41.8420837151137	3.25525889000560e-06
42.0777921055241	3.20169673471427e-06
42.3135004959345	3.14930328415237e-06
42.5492088863449	3.09804683462612e-06
42.7832701060807	3.04824339703832e-06
43.0173313258165	2.99950179938099e-06
43.2513925455524	2.95179389215579e-06
43.4854537652882	2.90509241665871e-06
43.7158897201435	2.86007178830358e-06
43.9463256749988	2.81597665582761e-06
44.1767616298541	2.77278335832380e-06
44.4071975847094	2.73046895709720e-06
44.6370374295381	2.68911736977304e-06
44.8668772743667	2.64859660610251e-06
45.0967171191954	2.60888590407717e-06
45.3265569640240	2.56996512120904e-06
45.5600731725287	2.53121064020555e-06
45.7935893810333	2.49323149033230e-06
46.0271055895379	2.45600837835008e-06
46.2606217980426	2.41952258428754e-06
46.5007803538022	2.38274890617645e-06
46.7409389095619	2.34671670466341e-06
46.9810974653215	2.31140738488378e-06
47.2212560210812	2.27680290878139e-06
47.4680943172735	2.24195206824139e-06
47.7149326134659	2.20780890949520e-06
47.9617709096582	2.17435556017465e-06
48.2086092058506	2.14157468683579e-06
48.4587788964316	2.10902031460561e-06
48.7089485870126	2.07712244613692e-06
48.9591182775936	2.04586461501210e-06
49.2092879681746	2.01523084796137e-06
49.4069659761309	1.99145596565762e-06
49.6046439840873	1.96805360768730e-06
49.8023219920436	1.94501650610797e-06
50	1.92233756247597e-06

==> matlab/fig2f3.tex <==
0.0100000000000000	5.61376685252809
0.0117160547237387	5.18359454388332
0.0134321094474774	4.83837248009412
0.0151481641712160	4.55328287851160
0.0168642188949547	4.31260079530955
0.0185802736186934	4.10581529539661
0.0202963283424321	3.92559840389803
0.0220123830661707	3.76666423330685
0.0237284377899094	3.62509113743311
0.0271767298921404	3.38174752716487
0.0306250219943713	3.18010641562286
0.0340733140966023	3.00932704469445
0.0375216061988333	2.86214504083249
0.0427139279135350	2.67426017883419
0.0479062496282368	2.51690188851832
0.0530985713429385	2.38241776468587
0.0582908930576403	2.26560051085759
0.0666867029016913	2.10509767780435
0.0750825127457423	1.97089983061694
0.0834783225897933	1.85624271814271
0.0918741324338443	1.75658162288000
0.103221374695157	1.64021196840554
0.114568616956470	1.54007980867219
0.125915859217783	1.45249654840058
0.137263101479095	1.37486582963221
0.152303542411290	1.28415172692531
0.167343983343484	1.20449146065754
0.182384424275678	1.13365205589515
0.197424865207872	1.07000720963534
0.216556218911177	0.997561084493906
0.235687572614481	0.932944388854833
0.254818926317785	0.874786976333440
0.273950280021090	0.822054654789003
0.295702700579699	0.767681267971630
0.317455121138309	0.718379242523290
0.339207541696919	0.673434664098094
0.360959962255528	0.632278679756116
0.384856456254013	0.590886352286411
0.408752950252498	0.553010991534881
0.432649444250983	0.518241521719085
0.456545938249468	0.486235029009624
0.482428909122220	0.454350009395604
0.508311879994973	0.425054184505194
0.534194850867725	0.398080444867756
0.560077821740478	0.373198516679821
0.587789573063889	0.348650568917237
0.615501324387300	0.326056779548648
0.643213075710712	0.305229571424504
0.670924827034123	0.286003841052458
0.700315973473582	0.267200365967293
0.729707119913042	0.249879646947094
0.759098266352501	0.233904621200781
0.788489412791960	0.219153234576275
0.819413129909566	0.204834042010477
0.850336847027172	0.191635258856387
0.881260564144777	0.179455409453817
0.912184281262383	0.168203574640525
0.944496310546559	0.157349606804180
0.976808339830736	0.147336150513999
1.00912036911491	0.138088163581802
1.04143239839909	0.129538185193158
1.07499283168995	0.121331775335395
1.10855326498080	0.113751595136646
1.14211369827166	0.106742524531997
1.17567413156251	0.100254902739532
1.21035017643711	0.0940518131738865
1.24502622131171	0.0883130347158363
1.27970226618631	0.0829983810570873
1.31437831106091	0.0780715767745262
1.35004735827022	0.0733738443387719
1.38571640547953	0.0690195723153912
1.42138545268884	0.0649796295917307
1.45705449989815	0.0612276676082043
1.49360694715890	0.0576566069689833
1.53015939441965	0.0543396708462639
1.56671184168041	0.0512558069761169
1.60326428894116	0.0483859321441116
1.64060574378950	0.0456570746353705
1.67794719863784	0.0431167188732383
1.71528865348618	0.0407496550132767
1.75263010833452	0.0385420627570475
1.79068279737963	0.0364434703550748
1.82873548642474	0.0344853270571333
1.86678817546984	0.0326566184232704
1.90484086451495	0.0309473107984409
1.94354426897741	0.0293218187302687
1.98224767343986	0.0278016011360919
2.02095107790232	0.0263786453450190
2.05965448236477	0.0250456330110493
2.09896535948022	0.0237768875278473
2.13827623659567	0.0225876177321033
2.17758711371112	0.0214719574284670
2.21689799082656	0.0204245345993698
2.25679001376257	0.0194263282083742
2.29668203669857	0.0184886031023053
2.33657405963457	0.0176070309658492
2.37646608257057	0.0167776378060813
2.41692934917714	0.0159859254221296
2.45739261578371	0.0152406365871365
2.49785588239028	0.0145385492070582
2.53831914899685	0.0138766975205817
2.57935979595430	0.0132436991827086
2.62040044291174	0.0126466553728999
2.66144108986919	0.0120831441034055
2.70248173682663	0.0115509307364335
2.74412187579687	0.0110408115308724
2.78576201476712	0.0105587964896364
2.82740215373736	0.0101030461483928
2.86904229270760	0.00967185952485331
2.91132048022032	0.00925757869860229
2.95359866773304	0.00886547232345535
2.99587685524576	0.00849412814913688
3.03815504275849	0.00814223753456709
3.08112752419896	0.00780325346402866
3.12410000563943	0.00748193158148290
3.16707248707990	0.00717717535348482
3.21004496852037	0.00688796677176682
3.25378802052889	0.00660856361467982
3.29753107253741	0.00634336386641527
3.34127412454594	0.00609150610403027
3.38501717655446	0.00585218924013665
3.42963104837956	0.00562025326277032
3.47424492020467	0.00539985104805564
3.51885879202977	0.00519029753168329
3.56347266385488	0.00499095469232166
3.60908796232704	0.00479707517787363
3.65470326079919	0.00461265609544764
3.70031855927135	0.00443714550598190
3.74593385774351	0.00427002873492065
3.79272190093334	0.00410683278263909
3.83950994412316	0.00395147916141204
3.88629798731299	0.00380351687016755
3.93308603050281	0.00366252494844192
3.98127611499785	0.00352417996539103
4.02946619949289	0.00339241126365070
4.07765628398793	0.00326684443729127
4.12584636848297	0.00314712978815216
4.17453782062043	0.00303178040598591
4.22322927275788	0.00292175676716070
4.27192072489534	0.00281676409658806
4.32061217703279	0.00271652654735234
4.36915150529233	0.00262107819258793
4.41769083355186	0.00252985882622281
4.46623016181140	0.00244264361028407
4.51476949007093	0.00235922158739096
4.56328105147248	0.00227943938178427
4.61179261287403	0.00220306248641958
4.66030417427557	0.00212991634085216
4.70881573567712	0.00205983678369968
4.75743034626171	0.00199252966571020
4.80604495684629	0.00192800071901979
4.85465956743088	0.00186611211849219
4.90327417801546	0.00180673399092144
4.95214759150491	0.00174944668417244
5.00102100499435	0.00169445557575494
5.04989441848379	0.00164164997079053
5.09876783197324	0.00159092538452900
5.14804659394740	0.00154178691000283
5.19732535592155	0.00149456826849766
5.24660411789571	0.00144917919149336
5.29588287986987	0.00140553435259737
5.34571691623879	0.00136308919595229
5.39555095260772	0.00132226636459754
5.44538498897664	0.00128299119396593
5.49521902534556	0.00124519302279685
5.54578533292858	0.00120828044619427
5.59635164051159	0.00117275354065066
5.64691794809460	0.00113854964163170
5.69748425567761	0.00110560938760316
5.74900092501619	0.00107329133391295
5.80051759435478	0.00104217011497881
5.85203426369337	0.00101219231349567
5.90355093303196	0.000983307292045478
5.95629904554016	0.000954813945160404
6.00904715804837	0.000927367033424948
6.06179527055658	0.000900920223255278
6.11454338306479	0.000875429573960087
6.16890437576226	0.000850115911801723
6.22326536845974	0.000825730235884514
6.27762636115721	0.000802231519277017
6.33198735385468	0.000779580851253535
6.38842448996247	0.000756922824872397
6.44486162607025	0.000735099905381178
6.50129876217804	0.000714074965037163
6.55773589828582	0.000693812802310605
6.61342964774346	0.000674532710253562
6.66912339720110	0.000655932456741863
6.72481714665874	0.000637983108685836
6.78051089611637	0.000620657170725605
6.83589971047198	0.000604018516181328
6.89128852482759	0.000587946152709321
6.94667733918320	0.000572416806586857
7.00206615353882	0.000557408321437246
7.05758976165192	0.000542864881742838
7.11311336976503	0.000528803391097847
7.16863697787814	0.000515204555881878
7.22416058599125	0.000502049985057977
7.28021693986213	0.000489202031030310
7.33627329373302	0.000476771824304112
7.39232964760390	0.000464742950882196
7.44838600147478	0.000453099750662494
7.50538574262213	0.000441640659499829
7.56238548376949	0.000430549885434958
7.61938522491684	0.000419813118836344
7.67638496606419	0.000409416700109457
7.73480587272738	0.000399100607761698
7.79322677939057	0.000389114940722968
7.85164768605376	0.000379446903664294
7.91006859271695	0.000370084280701452
7.97053387043690	0.000360703231910683
8.03099914815685	0.000351624505503242
8.09146442587680	0.000342836321022269
8.15192970359676	0.000334327434899586
8.21535952756943	0.000325689822998592
8.27878935154210	0.000317335937480043
8.34221917551477	0.000309254509246587
8.40564899948744	0.000301434792699173
8.46793784799597	0.000294000512480656
8.53022669650450	0.000286799461774887
8.59251554501303	0.000279822789098007
8.65480439352156	0.000273062036047056
8.71642204054983	0.000266578649089891
8.77803968757810	0.000260291155441277
8.83965733460636	0.000254192392107080
8.90127498163463	0.000248275502688329
8.96300495617631	0.000242523611825833
9.02473493071799	0.000236941348313486
9.08646490525967	0.000231522656475406
9.14819487980135	0.000226261733765669
9.21071927424122	0.000221088241668046
9.27324366868109	0.000216065361516940
9.33576806312096	0.000211187784409003
9.39829245756083	0.000206450420594119
9.46233592838314	0.000201738223608609
9.52637939920544	0.000197162986640684
9.59042287002774	0.000192719889231678
9.65446634085004	0.000188404309638093
9.72096019267431	0.000184053792385103
9.78745404449858	0.000179831205586797
9.85394789632285	0.000175731993627764
9.92044174814712	0.000171751790904558
9.98759919027086	0.000167848402342203
10.0547566323946	0.000164058009151672
10.1219140745184	0.000160376649381024
10.1890715166421	0.000156800523821822
10.2546642923364	0.000153405810373372
10.3202570680308	0.000150104748769473
10.3858498437251	0.000146894208382454
10.4514426194195	0.000143771181232180
10.5165140917340	0.000140756598178168
10.5815855640486	0.000137822584055142
10.6466570363632	0.000134966528917654
10.7117285086778	0.000132185921931884
10.7771443606203	0.000129464207794582
10.8425602125627	0.000126813938717626
10.9079760645052	0.000124232841132326
10.9733919164476	0.000121718726300536
11.0399477645340	0.000119227366939887
11.1065036126204	0.000116801026818535
11.1730594607068	0.000114437648607793
11.2396153087932	0.000112135251313470
11.3082257087532	0.000109823596479253
11.3768361087133	0.000107572706178461
11.4454465086734	0.000105380643765633
11.5140569086335	0.000103245544975450
11.5852093098832	0.000101089590943680
11.6563617111329	9.89910430205046e-05
11.7275141123826	9.69480478852510e-05
11.7986665136323	9.49588223807566e-05
11.8677850418193	9.30763165457968e-05
11.9369035700062	9.12414157032718e-05
12.0060220981931	8.94526596889989e-05
12.0751406263801	8.77086408768175e-05
12.1433601380698	8.60298491872962e-05
12.2115796497596	8.43920573870859e-05
12.2797991614493	8.27940506520894e-05
12.3480186731391	8.12346563934658e-05
12.4163461472746	7.97103631552219e-05
12.4846736214100	7.82225708343391e-05
12.5530010955455	7.67702188180242e-05
12.6213285696809	7.53522826603648e-05
12.6907216414633	7.39464401960030e-05
12.7601147132457	7.25740732397771e-05
12.8295077850280	7.12342144615560e-05
12.8989008568104	6.99259293377343e-05
12.9703478268833	6.86109582637834e-05
13.0417947969561	6.73275484494218e-05
13.1132417670290	6.60747805953591e-05
13.1846887371018	6.48517668293213e-05
13.2595560962437	6.36011938463283e-05
13.3344234553855	6.23813977932911e-05
13.4092908145273	6.11914595483970e-05
13.4841581736692	6.00304922027710e-05
13.5575412493262	5.89198313183982e-05
13.6309243249833	5.78354031220831e-05
13.7043074006403	5.67764555506418e-05
13.7776904762973	5.57422618508069e-05
13.8500672006557	5.47458127716282e-05
13.9224439250142	5.37721083346162e-05
13.9948206493726	5.28205182336345e-05
14.0671973737310	5.18904326715302e-05
14.1398455416426	5.09778904586242e-05
14.2124937095543	5.00858424572805e-05
14.2851418774659	4.92137297930863e-05
14.3577900453776	4.83610114882709e-05
14.4318616952425	4.75110102979844e-05
14.5059333451073	4.66800891789452e-05
14.5800049949722	4.58677280552563e-05
14.6540766448371	4.50734234984663e-05
14.7309274464065	4.42678808543923e-05
14.8077782479759	4.34807238375913e-05
14.8846290495453	4.27114429076588e-05
14.9614798511146	4.19595451069105e-05
15.0406722118752	4.12024195154680e-05
15.1198645726358	4.04627411908139e-05
15.1990569333964	3.97400219352633e-05
15.2782492941569	3.90337895923826e-05
15.3552187760152	3.83627463070525e-05
15.4321882578735	3.77064399934762e-05
15.5091577397318	3.70644775571703e-05
15.5861272215900	3.64364782199188e-05
15.6625824441176	3.58261338113103e-05
15.7390376666451	3.52288521620376e-05
15.8154928891726	3.46442936493618e-05
15.8919481117002	3.40721290239375e-05
15.9693961674172	3.35048438639683e-05
16.0468442231342	3.29496272744705e-05
16.1242922788512	3.24061673370076e-05
16.2017403345682	3.18741616045811e-05
16.2817277574867	3.13364249923150e-05
16.3617151804052	3.08102799802361e-05
16.4417026033237	3.02954230134239e-05
16.5216900262422	2.97915598761455e-05
16.6043553465212	2.92820770436077e-05
16.6870206668002	2.87837268468818e-05
16.7696859870792	2.82962137744791e-05
16.8523513073581	2.78192515303396e-05
16.9322086407103	2.73682496106208e-05
17.0120659740625	2.69265924889748e-05
17.0919233074148	2.64940448811816e-05
17.1717806407670	2.60703784644974e-05
17.2507845102887	2.56597619475349e-05
17.3297883798104	2.52574125964122e-05
17.4087922493321	2.48631281191833e-05
17.4877961188537	2.44767120416478e-05
17.5676116379811	2.40941217226732e-05
17.6474271571085	2.37191763730926e-05
17.7272426762358	2.33516903205192e-05
17.8070581953632	2.29914831928593e-05
17.8893023304811	2.26277451040662e-05
17.9715464655990	2.22713633701191e-05
18.0537906007169	2.19221571668714e-05
18.1360347358348	2.15799508943841e-05
18.2213159234312	2.12323180293591e-05
18.3065971110275	2.08918436665612e-05
18.3918782986238	2.05583486541654e-05
18.4771594862202	2.02316591098263e-05
18.5595094175750	1.99224986509700e-05
18.6418593489297	1.96193788364725e-05
18.7242092802845	1.93221561855592e-05
18.8065592116393	1.90306912239341e-05
18.8880422520689	1.87478285780453e-05
18.9695252924985	1.84703425346979e-05
19.0510083329281	1.81981088388649e-05
19.1324913733577	1.79310066118086e-05
19.2148776329082	1.76660407257237e-05
19.2972638924588	1.74060822087807e-05
19.3796501520093	1.71510160008946e-05
19.4620364115598	1.69007301506901e-05
19.5470683095882	1.66473046131476e-05
19.6321002076166	1.63987388361385e-05
19.7171321056450	1.61549195120366e-05
19.8021640036734	1.59157364394021e-05
19.8908893408643	1.56709910252170e-05
19.9796146780552	1.54310582891299e-05
20.0683400152462	1.51958231767947e-05
20.1570653524371	1.49651738676204e-05
20.2428390648805	1.47464548675921e-05
20.3286127773240	1.45318245307575e-05
20.4143864897674	1.43211899126324e-05
20.5001602022109	1.41144605533269e-05
20.5852635054960	1.39131197880804e-05
20.6703668087812	1.37154530582990e-05
20.7554701120663	1.35213788269249e-05
20.8405734153514	1.33308176850770e-05
20.9270705233463	1.31406557578976e-05
21.0135676313412	1.29539639551138e-05
21.1000647393361	1.27706652615961e-05
21.1865618473310	1.25906846724956e-05
21.2766604059527	1.24066597680874e-05
21.3667589645743	1.22260753954243e-05
21.4568575231959	1.20488533286130e-05
21.5469560818176	1.18749174334205e-05
21.6381292498009	1.17021764624193e-05
21.7293024177842	1.15326498962785e-05
21.8204755857675	1.13662649906180e-05
21.9116487537508	1.12029509371712e-05
22.0004127698935	1.10468368369538e-05
22.0891767860362	1.08935061488181e-05
22.1779408021788	1.07428985070921e-05
22.2667048183215	1.05949550860911e-05
22.3556370337612	1.04493455951708e-05
22.4445692492010	1.03062966870859e-05
22.5335014646408	1.01657535850063e-05
22.6224336800805	1.00276628905813e-05
22.7139161549811	9.88811632213273e-06
22.8053986298817	9.75105451589495e-06
22.8968811047823	9.61642365153109e-06
22.9883635796829	9.48417128002769e-06
23.0838924299717	9.34855251013401e-06
23.1794212802604	9.21541486200571e-06
23.2749501305492	9.08470312364205e-06
23.3704789808380	8.95636352818854e-06
23.4621509718643	8.83538731627870e-06
23.5538229628905	8.71650224170393e-06
23.6454949539168	8.59966432733268e-06
23.7371669449431	8.48483068412943e-06
23.8279328445987	8.37306563657650e-06
23.9186987442544	8.26318481327008e-06
24.0094646439101	8.15514956245615e-06
24.1002305435658	8.04892216531075e-06
24.1926550919484	7.94257323448099e-06
24.2850796403311	7.83802274009497e-06
24.3775041887138	7.73523367640389e-06
24.4699287370964	7.63416993361795e-06
24.5667881185871	7.53006989842677e-06
24.6636475000779	7.42778647443105e-06
24.7605068815686	7.32728109244647e-06
24.8573662630593	7.22851614671579e-06
24.9520922059339	7.13357475587091e-06
25.0468181488086	7.04022944124973e-06
25.1415440916832	6.94844755254639e-06
25.2362700345578	6.85819722539238e-06
25.3292146875769	6.77110261487289e-06
25.4221593405961	6.68542387986182e-06
25.5151039936153	6.60113300771299e-06
25.6080486466344	6.51820263802246e-06
25.7019756638980	6.43575065160510e-06
25.7959026811617	6.35463384537712e-06
25.8898296984253	6.27482590537867e-06
25.9837567156889	6.19630112798731e-06
26.0813748678075	6.11602333179450e-06
26.1789930199261	6.03707688729300e-06
26.2766111720447	5.95943492456558e-06
26.3742293241633	5.88307121187875e-06
26.4732872431096	5.80686157497829e-06
26.5723451620558	5.73191567600620e-06
26.6714030810021	5.65820801223755e-06
26.7704609999484	5.58571368660586e-06
26.8668464553430	5.51631672186668e-06
26.9632319107376	5.44802362105151e-06
27.0596173661322	5.38081301222945e-06
27.1560028215268	5.31466401049685e-06
27.2528815695420	5.24922563249982e-06
27.3497603175572	5.18481888071865e-06
27.4466390655724	5.12142395883045e-06
27.5435178135875	5.05902151765544e-06
27.6439608492560	4.99535092767536e-06
27.7444038849244	4.93270626522544e-06
27.8448469205929	4.87106740980240e-06
27.9452899562613	4.81041470534632e-06
28.0482405279971	4.74925111560371e-06
28.1511910997329	4.68908315799466e-06
28.2541416714688	4.62989110653101e-06
28.3570922432046	4.57165569520532e-06
28.4567501555253	4.51617631993104e-06
28.5564080678461	4.46155905423329e-06
28.6560659801668	4.40778759000699e-06
28.7557238924876	4.35484598229262e-06
28.8557411898054	4.30253211403728e-06
28.9557584871233	4.25102298356092e-06
29.0557757844411	4.20030352055754e-06
29.1557930817590	4.15035898695612e-06
29.2596833575662	4.09928551271102e-06
29.3635736333734	4.04901680120739e-06
29.4674639091807	3.99953741628001e-06
29.5713541849879	3.95083227028992e-06
29.6759318863875	3.90257186327691e-06
29.7805095877872	3.85506632706975e-06
29.8850872891868	3.80830128794446e-06
29.9896649905864	3.76226269436249e-06
30.0911544966620	3.71826520363422e-06
30.1926440027376	3.67492666744692e-06
30.2941335088132	3.63223506961861e-06
30.3956230148889	3.59017865194671e-06
30.4978092358551	3.54846360561674e-06
30.5999954568214	3.50736933159430e-06
30.7021816777877	3.46688458204102e-06
30.8043678987539	3.42699834907174e-06
30.9109059456037	3.38603913381385e-06
31.0174439924534	3.34570684414538e-06
31.1239820393031	3.30598979742475e-06
31.2305200861528	3.26687656731140e-06
31.3364021990683	3.22859135024819e-06
31.4422843119837	3.19088076500248e-06
31.5481664248991	3.15373431030614e-06
31.6540485378145	3.11714171083995e-06
31.7574284840790	3.08193860503803e-06
31.8608084303435	3.04724473954106e-06
31.9641883766080	3.01305114389514e-06
32.0675683228725	2.97934903371714e-06
32.1722735824859	2.94570703943475e-06
32.2769788420993	2.91255163607975e-06
32.3816841017127	2.87987425326798e-06
32.4863893613262	2.84766649836649e-06
32.5963585110375	2.81433619071417e-06
32.7063276607488	2.78150553177203e-06
32.8162968104602	2.74916540148375e-06
32.9262659601715	2.71730687579457e-06
33.0345223500676	2.68640646906556e-06
33.1427787399638	2.65595616376050e-06
33.2510351298599	2.62594797609914e-06
33.3592915197560	2.59637408905668e-06
33.4657809711845	2.56769919862076e-06
33.5722704226130	2.53943000494209e-06
33.6787598740416	2.51155951769858e-06
33.7852493254701	2.48408088841161e-06
33.8941979357818	2.45636623505660e-06
34.0031465460936	2.42904768500842e-06
34.1120951564054	2.40211834392043e-06
34.2210437667172	2.37557145875955e-06
34.3366404896276	2.34781546285749e-06
34.4522372125380	2.32047484128932e-06
34.5678339354484	2.29354202490589e-06
34.6834306583588	2.26700960696319e-06
34.7936642990230	2.24207447001464e-06
34.9038979396873	2.21749069351522e-06
35.0141315803515	2.19325224762024e-06
35.1243652210157	2.16935322435344e-06
35.2343050512079	2.14585020622915e-06
35.3442448814002	2.12267341804167e-06
35.4541847115924	2.09981734461071e-06
35.5641245417846	2.07727658056819e-06
35.6786017627846	2.05413491455824e-06
35.7930789837846	2.03132351730048e-06
35.9075562047846	2.00883664840027e-06
36.0220334257847	1.98666868496263e-06
36.1362198980123	1.96486923256604e-06
36.2504063702399	1.94337623226994e-06
36.3645928424676	1.92218443714960e-06
36.4787793146952	1.90128870608161e-06
36.5900126053583	1.88121327167982e-06
36.7012458960214	1.86140943952653e-06
36.8124791866845	1.84187273371600e-06
36.9237124773476	1.82259876522369e-06
37.0369057108861	1.80325046549062e-06
37.1500989444246	1.78416533936997e-06
37.2632921779630	1.76533902655500e-06
37.3764854115015	1.74676725183026e-06
37.4962218645145	1.72739430666534e-06
37.6159583175275	1.70829662500692e-06
37.7356947705405	1.68946944340658e-06
37.8554312235534	1.67090809549651e-06
37.9694000931710	1.65348358416094e-06
38.0833689627887	1.63629190674234e-06
38.1973378324063	1.61932927326837e-06
38.3113067020239	1.60259196643542e-06
38.4249000672874	1.58613039558667e-06
38.5384934325510	1.56988550511899e-06
38.6520867978146	1.55385382051856e-06
38.7656801630782	1.53803193290298e-06
38.8839805724880	1.52177383666602e-06
39.0022809818979	1.50573595197476e-06
39.1205813913078	1.48991464551771e-06
39.2388818007176	1.47430635459471e-06
39.3577858169091	1.45882954741173e-06
39.4766898331005	1.44356092699092e-06
39.5955938492920	1.42849708196332e-06
39.7144978654834	1.41363466680530e-06
39.8306400259012	1.39930879256284e-06
39.9467821863190	1.38516896891962e-06
40.0629243467368	1.37121225218504e-06
40.1790665071546	1.35743575353673e-06
40.2979626814797	1.34351629971595e-06
40.4168588558048	1.32977975656585e-06
40.5357550301298	1.31622319592641e-06
40.6546512044549	1.30284374485877e-06
40.7793663330114	1.28899672945775e-06
40.9040814615679	1.27533829182899e-06
41.0287965901244	1.26186530358652e-06
41.1535117186809	1.24857469747543e-06
41.2728913030736	1.23602075552190e-06
41.3922708874662	1.22362858056556e-06
41.5116504718589	1.21139563298936e-06
41.6310300562516	1.19931942014739e-06
41.7513824171239	1.18730097547393e-06
41.8717347779962	1.17543688294663e-06
41.9920871388686	1.16372472737119e-06
42.1124394997409	1.15216213807608e-06
42.2403780838680	1.14003211933147e-06
42.3683166679951	1.12806574464907e-06
42.4962552521223	1.11626032463697e-06
42.6241938362494	1.10461322196741e-06
42.7459262128924	1.09367573259339e-06
42.8676585895354	1.08287704532450e-06
42.9893909661784	1.07221501396733e-06
43.1111233428215	1.06168753142614e-06
43.2323192820888	1.05133804884707e-06
43.3535152213561	1.04111787653189e-06
43.4747111606234	1.03102504585633e-06
43.5959070998906	1.02105762350818e-06
43.7230100636943	1.01073704768381e-06
43.8501130274980	1.00055016464392e-06
43.9772159913017	9.90494864373915e-07
44.1043189551053	9.80569076092179e-07
44.2286927690341	9.70979830967303e-07
44.3530665829628	9.61510780190976e-07
44.4774403968915	9.52160088071808e-07
44.6018142108202	9.42925951951227e-07
44.7243832234717	9.33938120873972e-07
44.8469522361232	9.25060103999929e-07
44.9695212487747	9.16290266355991e-07
45.0920902614261	9.07627001652090e-07
45.2192704569313	8.98748788717303e-07
45.3464506524364	8.89981887610837e-07
45.4736308479415	8.81324597831878e-07
45.6008110434466	8.72775249488394e-07
45.7293487437304	8.64242650216912e-07
45.8578864440142	8.55816971397727e-07
45.9864241442980	8.47496580495196e-07
46.1149618445818	8.39279874343456e-07
46.2403633884128	8.31362061245099e-07
46.3657649322439	8.23540000338208e-07
46.4911664760749	8.15812280519806e-07
46.6165680199060	8.08177515191575e-07
46.7458183814916	8.00404261388185e-07
46.8750687430772	7.92726842393045e-07
47.0043191046628	7.85143818448296e-07
47.1335694662484	7.77653775282844e-07
47.2659682689327	7.70076234086668e-07
47.3983670716170	7.62593334299954e-07
47.5307658743013	7.55203635578591e-07
47.6631646769855	7.47905723406824e-07
47.7913492952116	7.40926240980352e-07
47.9195339134376	7.34030254135831e-07
48.0477185316636	7.27216545598887e-07
48.1759031498897	7.20483919007890e-07
48.3075614879101	7.13652015229305e-07
48.4392198259305	7.06903155109472e-07
48.5708781639510	7.00236108551833e-07
48.7025365019714	6.93649666930852e-07
48.8366959423393	6.87019790307886e-07
48.9708553827072	6.80471142592153e-07
49.1050148230751	6.74002511019786e-07
49.2391742634430	6.67612704163018e-07
49.3688501639382	6.61510258426007e-07
49.4985260644335	6.55479324325366e-07
49.6282019649287	6.49518880538254e-07
49.7578778654240	6.43627922931800e-07
49.8184083990680	6.40901631818420e-07
49.8789389327120	6.38190166289454e-07
49.9394694663560	6.35493427950378e-07
50	6.32811319177324e-07
